Low Language Transfer Speech-to-Text

A multilingual speech recogniser has heard much speech in its own languages. We ask how much of that it brings to a language it was never trained on, when it is fine-tuned on the little that language has. We score 28 open multilingual models untouched on Low-Language-TTS, 50 low-resource languages in 11 writing systems, and fine-tune 24 of them on at most 1,000 clips a language, 82 hours in all, with a dev set choosing every epoch. Fine-tuning lowers every model's macro character error rate (CER), by 16.6 to 53.1 points, to 9.5 at best, and a word language model takes three CTC models 1.2 to 1.4 points lower; WER is still 34.4 at best. On the 12 languages that no model lists, every model starts at 46 or worse and the best ends at 11.7. The same architectures from random weights stay 60 points or more behind, so the gain is transfer, and an encoder left untouched already gives a Whisper or Qwen decoder most of what it needs. It is the language, not the corpus: on FLEURS recordings that ours do not share, the median model keeps 79% of its gain. It costs the languages the models knew, 5.7 points of CER on English, Spanish, French and German in the median model. Low-rank adapters on 4% of the weights come within 1.1 points of tuning everything, and on 2 of 3 models forget less. Seq2seq and language-model decoders are done within three to five epochs, while a new CTC head is still improving at twenty or thirty. Data beats epochs: 25 clips a language take Qwen3-ASR 0.6B from 60.9 to 39.3, and at equal clips presented, ten times the data is worth 9.7 points. A model that first learned forty of the languages learns the other ten no faster. On a public Malay benchmark, untouched Whisper large-v3 scores 8.9 when it detects the language and 14.9 when told the clip is Malay, because it then translates the English that speakers mix in; trained on the Scicom telephony dataset it scores 6.0.

==> numbers.tex <==
% generated by make_tables.py from results/; do not edit
\makeatletter
\newcommand{\val}[1]{\ifcsname v@#1\endcsname\csname v@#1\endcsname\else\textbf{??}\PackageWarning{val}{undefined value #1}\fi}
\newcommand{\late}[3]{\ifcsname v@late/#1\endcsname #2\else #3\fi}
\newcommand{\ifval}[3]{\ifcsname v@#1\endcsname #2\else #3\fi}
\expandafter\def\csname v@ad/lora/cost-max\endcsname{1.1}
\expandafter\def\csname v@ad/lora/n\endcsname{3}
\expandafter\def\csname v@ad/lora/share-max\endcsname{4}
\expandafter\def\csname v@ad/mms-1b/cer\endcsname{11.0}
\expandafter\def\csname v@ad/mms-1b/lora/cer\endcsname{11.7}
\expandafter\def\csname v@ad/mms-1b/lora/cost\endcsname{0.7}
\expandafter\def\csname v@ad/mms-1b/lora/cost-ci\endcsname{0.5 to 0.9}
\expandafter\def\csname v@ad/mms-1b/lora/lr\endcsname{1e-4}
\expandafter\def\csname v@ad/mms-1b/lora/share\endcsname{3.6}
\expandafter\def\csname v@ad/mms-1b/lora/trainable\endcsname{36.4}
\expandafter\def\csname v@ad/mms-1b/lr\endcsname{1e-5}
\expandafter\def\csname v@ad/mms-1b/mmsad/cer\endcsname{14.0}
\expandafter\def\csname v@ad/mms-1b/mmsad/cost\endcsname{3.0}
\expandafter\def\csname v@ad/mms-1b/mmsad/cost-ci\endcsname{2.8 to 3.3}
\expandafter\def\csname v@ad/mms-1b/mmsad/lr\endcsname{3e-4}
\expandafter\def\csname v@ad/mms-1b/mmsad/share\endcsname{0.3}
\expandafter\def\csname v@ad/mms-1b/mmsad/trainable\endcsname{3.2}
\expandafter\def\csname v@ad/mms-1b/mmsadl/behind-shared\endcsname{2.8}
\expandafter\def\csname v@ad/mms-1b/mmsadl/behind-shared-ci\endcsname{2.4 to 3.1}
\expandafter\def\csname v@ad/mms-1b/mmsadl/cer\endcsname{16.8}
\expandafter\def\csname v@ad/mms-1b/mmsadl/cer-e10\endcsname{19.3}
\expandafter\def\csname v@ad/mms-1b/mmsadl/cost\endcsname{5.8}
\expandafter\def\csname v@ad/mms-1b/mmsadl/cost-ci\endcsname{5.5 to 6.1}
\expandafter\def\csname v@ad/mms-1b/mmsadl/e10-behind-shared\endcsname{5.3}
\expandafter\def\csname v@ad/mms-1b/mmsadl/longer-max\endcsname{210}
\expandafter\def\csname v@ad/mms-1b/mmsadl/lr\endcsname{3e-4}
\expandafter\def\csname v@ad/mms-1b/mmsadl/n-longer\endcsname{10}
\expandafter\def\csname v@ad/mms-1b/mmsadl/on-own\endcsname{16.5}
\expandafter\def\csname v@ad/mms-1b/mmsadl/own\endcsname{14.7}
\expandafter\def\csname v@ad/mms-1b/mmsadl/share\endcsname{0.2}
\expandafter\def\csname v@ad/mms-1b/mmsadl/trainable\endcsname{2.2}
\expandafter\def\csname v@ad/mms-1b/share\endcsname{100.0}
\expandafter\def\csname v@ad/mms-1b/trainable\endcsname{965.7}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/cer\endcsname{18.2}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/cer\endcsname{18.4}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/cost\endcsname{0.2}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/cost-ci\endcsname{-0.3 to 0.7}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/lr\endcsname{1e-4}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/share\endcsname{3.6}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lora/trainable\endcsname{29.5}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/lr\endcsname{1e-5}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/share\endcsname{100.0}
\expandafter\def\csname v@ad/qwen3-asr-0.6b/trainable\endcsname{782.4}
\expandafter\def\csname v@ad/whisper-large-v3/cer\endcsname{13.5}
\expandafter\def\csname v@ad/whisper-large-v3/lora/cer\endcsname{14.6}
\expandafter\def\csname v@ad/whisper-large-v3/lora/cost\endcsname{1.1}
\expandafter\def\csname v@ad/whisper-large-v3/lora/cost-ci\endcsname{0.7 to 1.5}
\expandafter\def\csname v@ad/whisper-large-v3/lora/lr\endcsname{3e-4}
\expandafter\def\csname v@ad/whisper-large-v3/lora/share\endcsname{3.6}
\expandafter\def\csname v@ad/whisper-large-v3/lora/trainable\endcsname{57.7}
\expandafter\def\csname v@ad/whisper-large-v3/lr\endcsname{1e-5}
\expandafter\def\csname v@ad/whisper-large-v3/share\endcsname{100.0}
\expandafter\def\csname v@ad/whisper-large-v3/trainable\endcsname{1543.5}
\expandafter\def\csname v@an/cohere-transcribe/disjoint\endcsname{16.1}
\expandafter\def\csname v@an/cohere-transcribe/shared\endcsname{11.3}
\expandafter\def\csname v@an/cohere-transcribe/spearman\endcsname{-0.46}
\expandafter\def\csname v@an/dev-fail\endcsname{5.0}
\expandafter\def\csname v@an/dev-gap\endcsname{7.2}
\expandafter\def\csname v@an/dev-gap-max\endcsname{8.3}
\expandafter\def\csname v@an/dev-gap-min\endcsname{5.5}
\expandafter\def\csname v@an/easy-names\endcsname{Haitian Creole (1), Khasi (2), Finnish (2), Southern Pastaza Quechua (2), Estonian (3)}
\expandafter\def\csname v@an/floor-mean\endcsname{10.4}
\expandafter\def\csname v@an/gemma4-12b/disjoint\endcsname{20.7}
\expandafter\def\csname v@an/gemma4-12b/shared\endcsname{11.9}
\expandafter\def\csname v@an/gemma4-12b/spearman\endcsname{-0.33}
\expandafter\def\csname v@an/gemma4-e2b/disjoint\endcsname{19.1}
\expandafter\def\csname v@an/gemma4-e2b/shared\endcsname{13.6}
\expandafter\def\csname v@an/gemma4-e2b/spearman\endcsname{-0.49}
\expandafter\def\csname v@an/gemma4-e4b/disjoint\endcsname{17.0}
\expandafter\def\csname v@an/gemma4-e4b/shared\endcsname{12.4}
\expandafter\def\csname v@an/gemma4-e4b/spearman\endcsname{-0.52}
\expandafter\def\csname v@an/granite-2b/disjoint\endcsname{23.4}
\expandafter\def\csname v@an/granite-2b/shared\endcsname{14.2}
\expandafter\def\csname v@an/granite-2b/spearman\endcsname{-0.30}
\expandafter\def\csname v@an/hard-names\endcsname{Tibetan (37), Nigerian Fulfulde (30), Breton (25), Kok Borok (22), Lule Sami (20)}
\expandafter\def\csname v@an/lfm3-audio/disjoint\endcsname{18.3}
\expandafter\def\csname v@an/lfm3-audio/shared\endcsname{12.7}
\expandafter\def\csname v@an/lfm3-audio/spearman\endcsname{-0.43}
\expandafter\def\csname v@an/mms-1b/disjoint\endcsname{11.5}
\expandafter\def\csname v@an/mms-1b/shared\endcsname{6.4}
\expandafter\def\csname v@an/mms-1b/spearman\endcsname{-0.46}
\expandafter\def\csname v@an/mms/beat-list\endcsname{MMS 1B at 10.0, omniASR CTC 1B at 11.1, w2v-BERT 2.0 at 12.5, Whisper large-v3 at 13.8 and Whisper large-v2 at 14.5}
\expandafter\def\csname v@an/mms/beat-n\endcsname{5}
\expandafter\def\csname v@an/mms/cohere-transcribe\endcsname{16.6}
\expandafter\def\csname v@an/mms/cohere-transcribe/before\endcsname{69.5}
\expandafter\def\csname v@an/mms/gemma4-12b\endcsname{20.6}
\expandafter\def\csname v@an/mms/gemma4-12b/before\endcsname{74.3}
\expandafter\def\csname v@an/mms/gemma4-e2b\endcsname{19.0}
\expandafter\def\csname v@an/mms/gemma4-e2b/before\endcsname{35.9}
\expandafter\def\csname v@an/mms/gemma4-e4b\endcsname{16.5}
\expandafter\def\csname v@an/mms/gemma4-e4b/before\endcsname{35.9}
\expandafter\def\csname v@an/mms/granite-2b\endcsname{23.7}
\expandafter\def\csname v@an/mms/granite-2b/before\endcsname{63.6}
\expandafter\def\csname v@an/mms/lfm3-audio\endcsname{18.2}
\expandafter\def\csname v@an/mms/lfm3-audio/before\endcsname{66.0}
\expandafter\def\csname v@an/mms/mms-1b\endcsname{10.0}
\expandafter\def\csname v@an/mms/n\endcsname{26}
\expandafter\def\csname v@an/mms/nemotron-30b\endcsname{16.3}
\expandafter\def\csname v@an/mms/nemotron-30b/before\endcsname{58.2}
\expandafter\def\csname v@an/mms/nemotron-stream\endcsname{38.6}
\expandafter\def\csname v@an/mms/nemotron-stream/before\endcsname{70.4}
\expandafter\def\csname v@an/mms/omni-ctc-1b\endcsname{11.1}
\expandafter\def\csname v@an/mms/omni-ctc-1b/before\endcsname{19.4}
\expandafter\def\csname v@an/mms/own\endcsname{14.7}
\expandafter\def\csname v@an/mms/parakeet-tdt-v3\endcsname{22.7}
\expandafter\def\csname v@an/mms/parakeet-tdt-v3/before\endcsname{55.9}
\expandafter\def\csname v@an/mms/qwen3-asr-0.6b\endcsname{18.4}
\expandafter\def\csname v@an/mms/qwen3-asr-0.6b/before\endcsname{62.4}
\expandafter\def\csname v@an/mms/qwen3-asr-1.7b\endcsname{16.8}
\expandafter\def\csname v@an/mms/qwen3-asr-1.7b/before\endcsname{61.1}
\expandafter\def\csname v@an/mms/voxtral-mini\endcsname{16.8}
\expandafter\def\csname v@an/mms/voxtral-mini/before\endcsname{60.9}
\expandafter\def\csname v@an/mms/w2v-bert\endcsname{12.5}
\expandafter\def\csname v@an/mms/whisper-large-v2\endcsname{14.5}
\expandafter\def\csname v@an/mms/whisper-large-v2/before\endcsname{55.6}
\expandafter\def\csname v@an/mms/whisper-large-v3\endcsname{13.8}
\expandafter\def\csname v@an/mms/whisper-large-v3-turbo\endcsname{15.0}
\expandafter\def\csname v@an/mms/whisper-large-v3-turbo/before\endcsname{51.2}
\expandafter\def\csname v@an/mms/whisper-large-v3/before\endcsname{45.3}
\expandafter\def\csname v@an/mms/whisper-medium\endcsname{14.9}
\expandafter\def\csname v@an/mms/whisper-medium/before\endcsname{61.9}
\expandafter\def\csname v@an/mms/whisper-small\endcsname{17.4}
\expandafter\def\csname v@an/mms/whisper-small/before\endcsname{63.2}
\expandafter\def\csname v@an/mms/whisper-tiny\endcsname{27.0}
\expandafter\def\csname v@an/mms/whisper-tiny/before\endcsname{64.6}
\expandafter\def\csname v@an/nemotron-30b/disjoint\endcsname{16.4}
\expandafter\def\csname v@an/nemotron-30b/listed-after\endcsname{4.0}
\expandafter\def\csname v@an/nemotron-30b/listed-before\endcsname{3.7}
\expandafter\def\csname v@an/nemotron-30b/listed-n\endcsname{4}
\expandafter\def\csname v@an/nemotron-30b/other-after\endcsname{16.8}
\expandafter\def\csname v@an/nemotron-30b/other-before\endcsname{62.8}
\expandafter\def\csname v@an/nemotron-30b/shared\endcsname{10.2}
\expandafter\def\csname v@an/nemotron-30b/spearman\endcsname{-0.47}
\expandafter\def\csname v@an/nemotron-stream/disjoint\endcsname{37.2}
\expandafter\def\csname v@an/nemotron-stream/listed-after\endcsname{20.8}
\expandafter\def\csname v@an/nemotron-stream/listed-before\endcsname{9.7}
\expandafter\def\csname v@an/nemotron-stream/listed-n\endcsname{4}
\expandafter\def\csname v@an/nemotron-stream/other-after\endcsname{37.2}
\expandafter\def\csname v@an/nemotron-stream/other-before\endcsname{73.8}
\expandafter\def\csname v@an/nemotron-stream/shared\endcsname{23.6}
\expandafter\def\csname v@an/nemotron-stream/spearman\endcsname{-0.38}
\expandafter\def\csname v@an/omni-ctc-1b/disjoint\endcsname{12.2}
\expandafter\def\csname v@an/omni-ctc-1b/shared\endcsname{10.4}
\expandafter\def\csname v@an/omni-ctc-1b/spearman\endcsname{-0.41}
\expandafter\def\csname v@an/parakeet-tdt-v3/disjoint\endcsname{21.7}
\expandafter\def\csname v@an/parakeet-tdt-v3/listed-after\endcsname{5.4}
\expandafter\def\csname v@an/parakeet-tdt-v3/listed-before\endcsname{5.3}
\expandafter\def\csname v@an/parakeet-tdt-v3/listed-n\endcsname{4}
\expandafter\def\csname v@an/parakeet-tdt-v3/other-after\endcsname{22.4}
\expandafter\def\csname v@an/parakeet-tdt-v3/other-before\endcsname{60.1}
\expandafter\def\csname v@an/parakeet-tdt-v3/shared\endcsname{15.1}
\expandafter\def\csname v@an/parakeet-tdt-v3/spearman\endcsname{-0.42}
\expandafter\def\csname v@an/qwen3-asr-0.6b/disjoint\endcsname{19.0}
\expandafter\def\csname v@an/qwen3-asr-0.6b/shared\endcsname{10.5}
\expandafter\def\csname v@an/qwen3-asr-0.6b/spearman\endcsname{-0.30}
\expandafter\def\csname v@an/qwen3-asr-1.7b/disjoint\endcsname{17.3}
\expandafter\def\csname v@an/qwen3-asr-1.7b/listed-after\endcsname{15.1}
\expandafter\def\csname v@an/qwen3-asr-1.7b/listed-before\endcsname{8.6}
\expandafter\def\csname v@an/qwen3-asr-1.7b/listed-n\endcsname{1}
\expandafter\def\csname v@an/qwen3-asr-1.7b/other-after\endcsname{16.6}
\expandafter\def\csname v@an/qwen3-asr-1.7b/other-before\endcsname{60.3}
\expandafter\def\csname v@an/qwen3-asr-1.7b/shared\endcsname{9.7}
\expandafter\def\csname v@an/qwen3-asr-1.7b/spearman\endcsname{-0.35}
\expandafter\def\csname v@an/script/CTC/latin\endcsname{11.3}
\expandafter\def\csname v@an/script/CTC/other\endcsname{13.5}
\expandafter\def\csname v@an/script/language model/latin\endcsname{17.0}
\expandafter\def\csname v@an/script/language model/other\endcsname{20.5}
\expandafter\def\csname v@an/script/seq2seq/latin\endcsname{15.1}
\expandafter\def\csname v@an/script/seq2seq/other\endcsname{20.0}
\expandafter\def\csname v@an/script/transducer/latin\endcsname{24.6}
\expandafter\def\csname v@an/script/transducer/other\endcsname{38.2}
\expandafter\def\csname v@an/shared-pct-max\endcsname{85}
\expandafter\def\csname v@an/shared-pct-median\endcsname{61}
\expandafter\def\csname v@an/shared-pct-min\endcsname{54}
\expandafter\def\csname v@an/test-fail\endcsname{1.0}
\expandafter\def\csname v@an/voxtral-mini/disjoint\endcsname{16.9}
\expandafter\def\csname v@an/voxtral-mini/shared\endcsname{10.4}
\expandafter\def\csname v@an/voxtral-mini/spearman\endcsname{-0.41}
\expandafter\def\csname v@an/w2v-bert/disjoint\endcsname{13.2}
\expandafter\def\csname v@an/w2v-bert/shared\endcsname{8.4}
\expandafter\def\csname v@an/w2v-bert/spearman\endcsname{-0.55}
\expandafter\def\csname v@an/whisper-large-v2/disjoint\endcsname{14.8}
\expandafter\def\csname v@an/whisper-large-v2/shared\endcsname{9.0}
\expandafter\def\csname v@an/whisper-large-v2/spearman\endcsname{-0.45}
\expandafter\def\csname v@an/whisper-large-v3-turbo/disjoint\endcsname{15.0}
\expandafter\def\csname v@an/whisper-large-v3-turbo/shared\endcsname{8.2}
\expandafter\def\csname v@an/whisper-large-v3-turbo/spearman\endcsname{-0.38}
\expandafter\def\csname v@an/whisper-large-v3/disjoint\endcsname{14.2}
\expandafter\def\csname v@an/whisper-large-v3/listed-after\endcsname{13.4}
\expandafter\def\csname v@an/whisper-large-v3/listed-before\endcsname{32.4}
\expandafter\def\csname v@an/whisper-large-v3/listed-n\endcsname{17}
\expandafter\def\csname v@an/whisper-large-v3/other-after\endcsname{13.6}
\expandafter\def\csname v@an/whisper-large-v3/other-before\endcsname{59.6}
\expandafter\def\csname v@an/whisper-large-v3/shared\endcsname{7.6}
\expandafter\def\csname v@an/whisper-large-v3/spearman\endcsname{-0.45}
\expandafter\def\csname v@an/whisper-medium/disjoint\endcsname{15.4}
\expandafter\def\csname v@an/whisper-medium/listed-after\endcsname{15.0}
\expandafter\def\csname v@an/whisper-medium/listed-before\endcsname{50.7}
\expandafter\def\csname v@an/whisper-medium/listed-n\endcsname{17}
\expandafter\def\csname v@an/whisper-medium/other-after\endcsname{14.7}
\expandafter\def\csname v@an/whisper-medium/other-before\endcsname{70.4}
\expandafter\def\csname v@an/whisper-medium/shared\endcsname{8.9}
\expandafter\def\csname v@an/whisper-medium/spearman\endcsname{-0.43}
\expandafter\def\csname v@an/whisper-small/disjoint\endcsname{17.7}
\expandafter\def\csname v@an/whisper-small/shared\endcsname{9.6}
\expandafter\def\csname v@an/whisper-small/spearman\endcsname{-0.39}
\expandafter\def\csname v@an/whisper-tiny/disjoint\endcsname{26.9}
\expandafter\def\csname v@an/whisper-tiny/shared\endcsname{14.9}
\expandafter\def\csname v@an/whisper-tiny/spearman\endcsname{-0.29}
\expandafter\def\csname v@an/worse/all-n\endcsname{0}
\expandafter\def\csname v@an/worse/all-names\endcsname{none}
\expandafter\def\csname v@an/worse/cohere-transcribe/n\endcsname{0}
\expandafter\def\csname v@an/worse/ever-n\endcsname{11}
\expandafter\def\csname v@an/worse/gemma4-12b/n\endcsname{0}
\expandafter\def\csname v@an/worse/gemma4-e2b/n\endcsname{6}
\expandafter\def\csname v@an/worse/gemma4-e4b/n\endcsname{3}
\expandafter\def\csname v@an/worse/granite-2b/n\endcsname{0}
\expandafter\def\csname v@an/worse/lfm3-audio/n\endcsname{4}
\expandafter\def\csname v@an/worse/models\endcsname{19}
\expandafter\def\csname v@an/worse/nemotron-30b/n\endcsname{3}
\expandafter\def\csname v@an/worse/nemotron-stream/n\endcsname{5}
\expandafter\def\csname v@an/worse/omni-ctc-1b/n\endcsname{9}
\expandafter\def\csname v@an/worse/parakeet-tdt-v3/n\endcsname{3}
\expandafter\def\csname v@an/worse/qwen3-asr-0.6b/n\endcsname{1}
\expandafter\def\csname v@an/worse/qwen3-asr-1.7b/n\endcsname{1}
\expandafter\def\csname v@an/worse/voxtral-mini/n\endcsname{0}
\expandafter\def\csname v@an/worse/whisper-large-v2/n\endcsname{2}
\expandafter\def\csname v@an/worse/whisper-large-v3-turbo/n\endcsname{4}
\expandafter\def\csname v@an/worse/whisper-large-v3/n\endcsname{3}
\expandafter\def\csname v@an/worse/whisper-medium/n\endcsname{0}
\expandafter\def\csname v@an/worse/whisper-small/n\endcsname{1}
\expandafter\def\csname v@an/worse/whisper-tiny/n\endcsname{2}
\expandafter\def\csname v@bl/canary-1b-v2/cer\endcsname{62.4}
\expandafter\def\csname v@bl/canary-1b-v2/empty\endcsname{3}
\expandafter\def\csname v@bl/canary-1b-v2/loop\endcsname{52}
\expandafter\def\csname v@bl/canary-1b-v2/median\endcsname{62.0}
\expandafter\def\csname v@bl/canary-1b-v2/n\endcsname{50}
\expandafter\def\csname v@bl/canary-1b-v2/raw\endcsname{84.3}
\expandafter\def\csname v@bl/canary-1b-v2/wer\endcsname{90.4}
\expandafter\def\csname v@bl/cohere-transcribe/cer\endcsname{68.0}
\expandafter\def\csname v@bl/cohere-transcribe/empty\endcsname{0}
\expandafter\def\csname v@bl/cohere-transcribe/loop\endcsname{40}
\expandafter\def\csname v@bl/cohere-transcribe/median\endcsname{65.6}
\expandafter\def\csname v@bl/cohere-transcribe/n\endcsname{50}
\expandafter\def\csname v@bl/cohere-transcribe/raw\endcsname{93.0}
\expandafter\def\csname v@bl/cohere-transcribe/wer\endcsname{95.8}
\expandafter\def\csname v@bl/fun-asr-nano/cer\endcsname{73.5}
\expandafter\def\csname v@bl/fun-asr-nano/empty\endcsname{1}
\expandafter\def\csname v@bl/fun-asr-nano/loop\endcsname{26}
\expandafter\def\csname v@bl/fun-asr-nano/median\endcsname{78.5}
\expandafter\def\csname v@bl/fun-asr-nano/n\endcsname{50}
\expandafter\def\csname v@bl/fun-asr-nano/raw\endcsname{81.4}
\expandafter\def\csname v@bl/fun-asr-nano/wer\endcsname{97.7}
\expandafter\def\csname v@bl/gemma/alone-span\endcsname{47.7 to 52.2}
\expandafter\def\csname v@bl/gemma/cer-span\endcsname{39.8 to 43.5}
\expandafter\def\csname v@bl/gemma/sizes\endcsname{two sizes}
\expandafter\def\csname v@bl/gemma/told-gain-span\endcsname{7.9 to 8.7}
\expandafter\def\csname v@bl/gemma4-12b/alone\endcsname{75.8}
\expandafter\def\csname v@bl/gemma4-12b/cer\endcsname{72.9}
\expandafter\def\csname v@bl/gemma4-12b/empty\endcsname{49}
\expandafter\def\csname v@bl/gemma4-12b/known\endcsname{2.2}
\expandafter\def\csname v@bl/gemma4-12b/loop\endcsname{67}
\expandafter\def\csname v@bl/gemma4-12b/median\endcsname{80.4}
\expandafter\def\csname v@bl/gemma4-12b/n\endcsname{50}
\expandafter\def\csname v@bl/gemma4-12b/raw\endcsname{97.7}
\expandafter\def\csname v@bl/gemma4-12b/told-gain\endcsname{2.9}
\expandafter\def\csname v@bl/gemma4-12b/told-gain-ci\endcsname{2.0 to 3.8}
\expandafter\def\csname v@bl/gemma4-12b/wer\endcsname{96.4}
\expandafter\def\csname v@bl/gemma4-e2b/alone\endcsname{52.2}
\expandafter\def\csname v@bl/gemma4-e2b/cer\endcsname{43.5}
\expandafter\def\csname v@bl/gemma4-e2b/empty\endcsname{0}
\expandafter\def\csname v@bl/gemma4-e2b/known\endcsname{2.8}
\expandafter\def\csname v@bl/gemma4-e2b/loop\endcsname{1}
\expandafter\def\csname v@bl/gemma4-e2b/median\endcsname{41.4}
\expandafter\def\csname v@bl/gemma4-e2b/n\endcsname{50}
\expandafter\def\csname v@bl/gemma4-e2b/raw\endcsname{43.7}
\expandafter\def\csname v@bl/gemma4-e2b/told-gain\endcsname{8.7}
\expandafter\def\csname v@bl/gemma4-e2b/told-gain-ci\endcsname{7.9 to 9.9}
\expandafter\def\csname v@bl/gemma4-e2b/wer\endcsname{80.2}
\expandafter\def\csname v@bl/gemma4-e4b/alone\endcsname{47.7}
\expandafter\def\csname v@bl/gemma4-e4b/cer\endcsname{39.8}
\expandafter\def\csname v@bl/gemma4-e4b/empty\endcsname{0}
\expandafter\def\csname v@bl/gemma4-e4b/known\endcsname{2.3}
\expandafter\def\csname v@bl/gemma4-e4b/loop\endcsname{5}
\expandafter\def\csname v@bl/gemma4-e4b/median\endcsname{35.2}
\expandafter\def\csname v@bl/gemma4-e4b/n\endcsname{50}
\expandafter\def\csname v@bl/gemma4-e4b/raw\endcsname{41.7}
\expandafter\def\csname v@bl/gemma4-e4b/told-gain\endcsname{7.9}
\expandafter\def\csname v@bl/gemma4-e4b/told-gain-ci\endcsname{6.9 to 9.1}
\expandafter\def\csname v@bl/gemma4-e4b/wer\endcsname{77.0}
\expandafter\def\csname v@bl/granite-2b/cer\endcsname{62.1}
\expandafter\def\csname v@bl/granite-2b/empty\endcsname{0}
\expandafter\def\csname v@bl/granite-2b/loop\endcsname{7}
\expandafter\def\csname v@bl/granite-2b/median\endcsname{56.1}
\expandafter\def\csname v@bl/granite-2b/n\endcsname{50}
\expandafter\def\csname v@bl/granite-2b/raw\endcsname{68.3}
\expandafter\def\csname v@bl/granite-2b/wer\endcsname{95.9}
\expandafter\def\csname v@bl/granite-ctc/cer\endcsname{69.7}
\expandafter\def\csname v@bl/granite-ctc/empty\endcsname{5}
\expandafter\def\csname v@bl/granite-ctc/loop\endcsname{0}
\expandafter\def\csname v@bl/granite-ctc/median\endcsname{71.0}
\expandafter\def\csname v@bl/granite-ctc/n\endcsname{50}
\expandafter\def\csname v@bl/granite-ctc/raw\endcsname{69.8}
\expandafter\def\csname v@bl/granite-ctc/wer\endcsname{95.8}
\expandafter\def\csname v@bl/lfm3-audio/cer\endcsname{64.3}
\expandafter\def\csname v@bl/lfm3-audio/empty\endcsname{0}
\expandafter\def\csname v@bl/lfm3-audio/loop\endcsname{15}
\expandafter\def\csname v@bl/lfm3-audio/median\endcsname{70.8}
\expandafter\def\csname v@bl/lfm3-audio/n\endcsname{50}
\expandafter\def\csname v@bl/lfm3-audio/raw\endcsname{78.1}
\expandafter\def\csname v@bl/lfm3-audio/wer\endcsname{89.5}
\expandafter\def\csname v@bl/mms-1b-all/cer\endcsname{14.7}
\expandafter\def\csname v@bl/mms-1b-all/empty\endcsname{0}
\expandafter\def\csname v@bl/mms-1b-all/loop\endcsname{0}
\expandafter\def\csname v@bl/mms-1b-all/median\endcsname{8.9}
\expandafter\def\csname v@bl/mms-1b-all/n\endcsname{26}
\expandafter\def\csname v@bl/mms-1b-all/raw\endcsname{14.9}
\expandafter\def\csname v@bl/mms-1b-all/wer\endcsname{42.7}
\expandafter\def\csname v@bl/mms-1b/cer\endcsname{30.6}
\expandafter\def\csname v@bl/mms-1b/empty\endcsname{0}
\expandafter\def\csname v@bl/mms-1b/loop\endcsname{2}
\expandafter\def\csname v@bl/mms-1b/median\endcsname{16.9}
\expandafter\def\csname v@bl/mms-1b/n\endcsname{50}
\expandafter\def\csname v@bl/mms-1b/raw\endcsname{31.1}
\expandafter\def\csname v@bl/mms-1b/wer\endcsname{62.9}
\expandafter\def\csname v@bl/nemotron-30b/cer\endcsname{58.1}
\expandafter\def\csname v@bl/nemotron-30b/empty\endcsname{1}
\expandafter\def\csname v@bl/nemotron-30b/loop\endcsname{3}
\expandafter\def\csname v@bl/nemotron-30b/median\endcsname{62.7}
\expandafter\def\csname v@bl/nemotron-30b/n\endcsname{50}
\expandafter\def\csname v@bl/nemotron-30b/raw\endcsname{59.4}
\expandafter\def\csname v@bl/nemotron-30b/wer\endcsname{86.3}
\expandafter\def\csname v@bl/nemotron-stream/cer\endcsname{68.7}
\expandafter\def\csname v@bl/nemotron-stream/empty\endcsname{120}
\expandafter\def\csname v@bl/nemotron-stream/loop\endcsname{8}
\expandafter\def\csname v@bl/nemotron-stream/median\endcsname{79.1}
\expandafter\def\csname v@bl/nemotron-stream/n\endcsname{50}
\expandafter\def\csname v@bl/nemotron-stream/raw\endcsname{69.7}
\expandafter\def\csname v@bl/nemotron-stream/wer\endcsname{92.2}
\expandafter\def\csname v@bl/omni-ctc-1b/cer\endcsname{28.5}
\expandafter\def\csname v@bl/omni-ctc-1b/empty\endcsname{2}
\expandafter\def\csname v@bl/omni-ctc-1b/loop\endcsname{0}
\expandafter\def\csname v@bl/omni-ctc-1b/median\endcsname{20.9}
\expandafter\def\csname v@bl/omni-ctc-1b/n\endcsname{50}
\expandafter\def\csname v@bl/omni-ctc-1b/raw\endcsname{28.8}
\expandafter\def\csname v@bl/omni-ctc-1b/wer\endcsname{63.1}
\expandafter\def\csname v@bl/omni-ctc-300m/cer\endcsname{31.5}
\expandafter\def\csname v@bl/omni-ctc-300m/empty\endcsname{0}
\expandafter\def\csname v@bl/omni-ctc-300m/loop\endcsname{1}
\expandafter\def\csname v@bl/omni-ctc-300m/median\endcsname{23.2}
\expandafter\def\csname v@bl/omni-ctc-300m/n\endcsname{50}
\expandafter\def\csname v@bl/omni-ctc-300m/raw\endcsname{31.7}
\expandafter\def\csname v@bl/omni-ctc-300m/wer\endcsname{69.5}
\expandafter\def\csname v@bl/omni-ctc-7b/cer\endcsname{29.7}
\expandafter\def\csname v@bl/omni-ctc-7b/empty\endcsname{1}
\expandafter\def\csname v@bl/omni-ctc-7b/loop\endcsname{0}
\expandafter\def\csname v@bl/omni-ctc-7b/median\endcsname{19.2}
\expandafter\def\csname v@bl/omni-ctc-7b/n\endcsname{50}
\expandafter\def\csname v@bl/omni-ctc-7b/raw\endcsname{29.9}
\expandafter\def\csname v@bl/omni-ctc-7b/wer\endcsname{59.2}
\expandafter\def\csname v@bl/omni-llm-1b/cer\endcsname{27.8}
\expandafter\def\csname v@bl/omni-llm-1b/empty\endcsname{0}
\expandafter\def\csname v@bl/omni-llm-1b/loop\endcsname{2}
\expandafter\def\csname v@bl/omni-llm-1b/median\endcsname{16.6}
\expandafter\def\csname v@bl/omni-llm-1b/n\endcsname{50}
\expandafter\def\csname v@bl/omni-llm-1b/raw\endcsname{28.3}
\expandafter\def\csname v@bl/omni-llm-1b/wer\endcsname{56.4}
\expandafter\def\csname v@bl/parakeet-tdt-v3/cer\endcsname{55.7}
\expandafter\def\csname v@bl/parakeet-tdt-v3/empty\endcsname{73}
\expandafter\def\csname v@bl/parakeet-tdt-v3/loop\endcsname{0}
\expandafter\def\csname v@bl/parakeet-tdt-v3/median\endcsname{53.5}
\expandafter\def\csname v@bl/parakeet-tdt-v3/n\endcsname{50}
\expandafter\def\csname v@bl/parakeet-tdt-v3/raw\endcsname{56.4}
\expandafter\def\csname v@bl/parakeet-tdt-v3/wer\endcsname{88.0}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/cer\endcsname{60.9}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/empty\endcsname{0}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/loop\endcsname{1}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/median\endcsname{60.1}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/n\endcsname{50}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/raw\endcsname{61.5}
\expandafter\def\csname v@bl/qwen3-asr-0.6b/wer\endcsname{94.2}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/cer\endcsname{59.3}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/empty\endcsname{0}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/loop\endcsname{0}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/median\endcsname{56.9}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/n\endcsname{50}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/raw\endcsname{59.8}
\expandafter\def\csname v@bl/qwen3-asr-1.7b/wer\endcsname{92.9}
\expandafter\def\csname v@bl/vibevoice/cer\endcsname{84.9}
\expandafter\def\csname v@bl/vibevoice/empty\endcsname{0}
\expandafter\def\csname v@bl/vibevoice/loop\endcsname{146}
\expandafter\def\csname v@bl/vibevoice/median\endcsname{87.8}
\expandafter\def\csname v@bl/vibevoice/n\endcsname{50}
\expandafter\def\csname v@bl/vibevoice/raw\endcsname{135.2}
\expandafter\def\csname v@bl/vibevoice/wer\endcsname{98.3}
\expandafter\def\csname v@bl/voxtral-mini/cer\endcsname{61.8}
\expandafter\def\csname v@bl/voxtral-mini/empty\endcsname{0}
\expandafter\def\csname v@bl/voxtral-mini/loop\endcsname{16}
\expandafter\def\csname v@bl/voxtral-mini/median\endcsname{63.0}
\expandafter\def\csname v@bl/voxtral-mini/n\endcsname{50}
\expandafter\def\csname v@bl/voxtral-mini/raw\endcsname{67.2}
\expandafter\def\csname v@bl/voxtral-mini/wer\endcsname{91.2}
\expandafter\def\csname v@bl/whisper-base/cer\endcsname{62.7}
\expandafter\def\csname v@bl/whisper-base/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-base/loop\endcsname{89}
\expandafter\def\csname v@bl/whisper-base/median\endcsname{64.2}
\expandafter\def\csname v@bl/whisper-base/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-base/raw\endcsname{94.3}
\expandafter\def\csname v@bl/whisper-base/wer\endcsname{94.5}
\expandafter\def\csname v@bl/whisper-large-v2/cer\endcsname{57.8}
\expandafter\def\csname v@bl/whisper-large-v2/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-large-v2/loop\endcsname{94}
\expandafter\def\csname v@bl/whisper-large-v2/median\endcsname{61.3}
\expandafter\def\csname v@bl/whisper-large-v2/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-large-v2/raw\endcsname{72.3}
\expandafter\def\csname v@bl/whisper-large-v2/wer\endcsname{86.8}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/cer\endcsname{54.6}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/loop\endcsname{154}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/median\endcsname{57.1}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/raw\endcsname{89.7}
\expandafter\def\csname v@bl/whisper-large-v3-turbo/wer\endcsname{84.8}
\expandafter\def\csname v@bl/whisper-large-v3/cer\endcsname{50.3}
\expandafter\def\csname v@bl/whisper-large-v3/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-large-v3/loop\endcsname{101}
\expandafter\def\csname v@bl/whisper-large-v3/median\endcsname{49.4}
\expandafter\def\csname v@bl/whisper-large-v3/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-large-v3/raw\endcsname{59.5}
\expandafter\def\csname v@bl/whisper-large-v3/wer\endcsname{83.7}
\expandafter\def\csname v@bl/whisper-medium/cer\endcsname{63.7}
\expandafter\def\csname v@bl/whisper-medium/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-medium/loop\endcsname{170}
\expandafter\def\csname v@bl/whisper-medium/median\endcsname{65.8}
\expandafter\def\csname v@bl/whisper-medium/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-medium/raw\endcsname{80.0}
\expandafter\def\csname v@bl/whisper-medium/wer\endcsname{89.3}
\expandafter\def\csname v@bl/whisper-small/cer\endcsname{65.7}
\expandafter\def\csname v@bl/whisper-small/empty\endcsname{0}
\expandafter\def\csname v@bl/whisper-small/loop\endcsname{303}
\expandafter\def\csname v@bl/whisper-small/median\endcsname{76.2}
\expandafter\def\csname v@bl/whisper-small/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-small/raw\endcsname{82.7}
\expandafter\def\csname v@bl/whisper-small/wer\endcsname{91.5}
\expandafter\def\csname v@bl/whisper-tiny/cer\endcsname{66.6}
\expandafter\def\csname v@bl/whisper-tiny/empty\endcsname{2}
\expandafter\def\csname v@bl/whisper-tiny/loop\endcsname{130}
\expandafter\def\csname v@bl/whisper-tiny/median\endcsname{70.2}
\expandafter\def\csname v@bl/whisper-tiny/n\endcsname{50}
\expandafter\def\csname v@bl/whisper-tiny/raw\endcsname{102.0}
\expandafter\def\csname v@bl/whisper-tiny/wer\endcsname{96.1}
\expandafter\def\csname v@cs/after-median\endcsname{36.2}
\expandafter\def\csname v@cs/before-median\endcsname{60.2}
\expandafter\def\csname v@cs/best/cer\endcsname{26.2}
\expandafter\def\csname v@cs/best/name\endcsname{w2v-BERT 2.0}
\expandafter\def\csname v@cs/better-n\endcsname{17}
\expandafter\def\csname v@cs/cohere-transcribe/after\endcsname{42.8}
\expandafter\def\csname v@cs/cohere-transcribe/after-wer\endcsname{79.1}
\expandafter\def\csname v@cs/cohere-transcribe/before\endcsname{65.8}
\expandafter\def\csname v@cs/cohere-transcribe/en-after\endcsname{0}
\expandafter\def\csname v@cs/cohere-transcribe/en-before\endcsname{34}
\expandafter\def\csname v@cs/cohere-transcribe/gain\endcsname{22.9}
\expandafter\def\csname v@cs/cohere-transcribe/gain-ci\endcsname{21.7 to 24.3}
\expandafter\def\csname v@cs/cohere-transcribe/mono-after\endcsname{20.4}
\expandafter\def\csname v@cs/en-after-median\endcsname{1}
\expandafter\def\csname v@cs/en-before-median\endcsname{12}
\expandafter\def\csname v@cs/en-chars-max\endcsname{27}
\expandafter\def\csname v@cs/en-chars-min\endcsname{22}
\expandafter\def\csname v@cs/en-lost-n\endcsname{17}
\expandafter\def\csname v@cs/en-n\endcsname{20}
\expandafter\def\csname v@cs/gain-median\endcsname{22.7}
\expandafter\def\csname v@cs/gap-max\endcsname{25.4}
\expandafter\def\csname v@cs/gap-median\endcsname{20.0}
\expandafter\def\csname v@cs/gap-min\endcsname{6.0}
\expandafter\def\csname v@cs/gemma4-12b/after\endcsname{41.9}
\expandafter\def\csname v@cs/gemma4-12b/after-wer\endcsname{72.5}
\expandafter\def\csname v@cs/gemma4-12b/before\endcsname{83.7}
\expandafter\def\csname v@cs/gemma4-12b/en-after\endcsname{1}
\expandafter\def\csname v@cs/gemma4-12b/en-before\endcsname{11}
\expandafter\def\csname v@cs/gemma4-12b/gain\endcsname{41.8}
\expandafter\def\csname v@cs/gemma4-12b/gain-ci\endcsname{40.2 to 43.3}
\expandafter\def\csname v@cs/gemma4-12b/mono-after\endcsname{21.9}
\expandafter\def\csname v@cs/gemma4-e2b/after\endcsname{36.8}
\expandafter\def\csname v@cs/gemma4-e2b/after-wer\endcsname{67.3}
\expandafter\def\csname v@cs/gemma4-e2b/before\endcsname{34.1}
\expandafter\def\csname v@cs/gemma4-e2b/en-after\endcsname{2}
\expandafter\def\csname v@cs/gemma4-e2b/en-before\endcsname{11}
\expandafter\def\csname v@cs/gemma4-e2b/gain\endcsname{-2.7}
\expandafter\def\csname v@cs/gemma4-e2b/gain-ci\endcsname{-3.8 to -1.6}
\expandafter\def\csname v@cs/gemma4-e2b/mono-after\endcsname{13.9}
\expandafter\def\csname v@cs/gemma4-e4b/after\endcsname{34.5}
\expandafter\def\csname v@cs/gemma4-e4b/after-wer\endcsname{59.9}
\expandafter\def\csname v@cs/gemma4-e4b/before\endcsname{32.7}
\expandafter\def\csname v@cs/gemma4-e4b/en-after\endcsname{3}
\expandafter\def\csname v@cs/gemma4-e4b/en-before\endcsname{13}
\expandafter\def\csname v@cs/gemma4-e4b/gain\endcsname{-1.8}
\expandafter\def\csname v@cs/gemma4-e4b/gain-ci\endcsname{-2.9 to -0.6}
\expandafter\def\csname v@cs/gemma4-e4b/mono-after\endcsname{9.1}
\expandafter\def\csname v@cs/granite-2b/after\endcsname{41.3}
\expandafter\def\csname v@cs/granite-2b/after-wer\endcsname{79.1}
\expandafter\def\csname v@cs/granite-2b/before\endcsname{64.3}
\expandafter\def\csname v@cs/granite-2b/en-after\endcsname{0}
\expandafter\def\csname v@cs/granite-2b/en-before\endcsname{28}
\expandafter\def\csname v@cs/granite-2b/gain\endcsname{23.0}
\expandafter\def\csname v@cs/granite-2b/gain-ci\endcsname{21.8 to 24.2}
\expandafter\def\csname v@cs/granite-2b/mono-after\endcsname{24.3}
\expandafter\def\csname v@cs/lfm3-audio/after\endcsname{36.2}
\expandafter\def\csname v@cs/lfm3-audio/after-wer\endcsname{68.1}
\expandafter\def\csname v@cs/lfm3-audio/before\endcsname{60.9}
\expandafter\def\csname v@cs/lfm3-audio/en-after\endcsname{1}
\expandafter\def\csname v@cs/lfm3-audio/en-before\endcsname{33}
\expandafter\def\csname v@cs/lfm3-audio/gain\endcsname{24.7}
\expandafter\def\csname v@cs/lfm3-audio/gain-ci\endcsname{23.5 to 25.7}
\expandafter\def\csname v@cs/lfm3-audio/mono-after\endcsname{14.4}
\expandafter\def\csname v@cs/mms-1b/after\endcsname{28.4}
\expandafter\def\csname v@cs/mms-1b/after-wer\endcsname{61.7}
\expandafter\def\csname v@cs/mms-1b/before\endcsname{27.9}
\expandafter\def\csname v@cs/mms-1b/en-after\endcsname{0}
\expandafter\def\csname v@cs/mms-1b/en-before\endcsname{0}
\expandafter\def\csname v@cs/mms-1b/gain\endcsname{-0.5}
\expandafter\def\csname v@cs/mms-1b/gain-ci\endcsname{-4.0 to -2.9}
\expandafter\def\csname v@cs/mms-1b/mono-after\endcsname{7.5}
\expandafter\def\csname v@cs/mono-after-median\endcsname{15.0}
\expandafter\def\csname v@cs/n\endcsname{21}
\expandafter\def\csname v@cs/nemotron-30b/after\endcsname{34.2}
\expandafter\def\csname v@cs/nemotron-30b/after-wer\endcsname{62.9}
\expandafter\def\csname v@cs/nemotron-30b/before\endcsname{56.6}
\expandafter\def\csname v@cs/nemotron-30b/en-after\endcsname{3}
\expandafter\def\csname v@cs/nemotron-30b/en-before\endcsname{35}
\expandafter\def\csname v@cs/nemotron-30b/gain\endcsname{22.4}
\expandafter\def\csname v@cs/nemotron-30b/gain-ci\endcsname{21.2 to 23.5}
\expandafter\def\csname v@cs/nemotron-30b/mono-after\endcsname{12.0}
\expandafter\def\csname v@cs/nemotron-stream/after\endcsname{57.9}
\expandafter\def\csname v@cs/nemotron-stream/after-wer\endcsname{91.8}
\expandafter\def\csname v@cs/nemotron-stream/before\endcsname{62.0}
\expandafter\def\csname v@cs/nemotron-stream/en-after\endcsname{0}
\expandafter\def\csname v@cs/nemotron-stream/en-before\endcsname{12}
\expandafter\def\csname v@cs/nemotron-stream/gain\endcsname{4.0}
\expandafter\def\csname v@cs/nemotron-stream/gain-ci\endcsname{3.2 to 4.8}
\expandafter\def\csname v@cs/nemotron-stream/mono-after\endcsname{52.0}
\expandafter\def\csname v@cs/omni-ctc-1b/after\endcsname{27.2}
\expandafter\def\csname v@cs/omni-ctc-1b/after-wer\endcsname{62.3}
\expandafter\def\csname v@cs/omni-ctc-1b/before\endcsname{27.8}
\expandafter\def\csname v@cs/omni-ctc-1b/en-after\endcsname{1}
\expandafter\def\csname v@cs/omni-ctc-1b/en-before\endcsname{0}
\expandafter\def\csname v@cs/omni-ctc-1b/gain\endcsname{0.7}
\expandafter\def\csname v@cs/omni-ctc-1b/gain-ci\endcsname{0.2 to 1.1}
\expandafter\def\csname v@cs/omni-ctc-1b/mono-after\endcsname{7.8}
\expandafter\def\csname v@cs/parakeet-tdt-v3/after\endcsname{52.2}
\expandafter\def\csname v@cs/parakeet-tdt-v3/after-wer\endcsname{74.5}
\expandafter\def\csname v@cs/parakeet-tdt-v3/before\endcsname{59.4}
\expandafter\def\csname v@cs/parakeet-tdt-v3/en-after\endcsname{1}
\expandafter\def\csname v@cs/parakeet-tdt-v3/en-before\endcsname{28}
\expandafter\def\csname v@cs/parakeet-tdt-v3/gain\endcsname{7.2}
\expandafter\def\csname v@cs/parakeet-tdt-v3/gain-ci\endcsname{5.9 to 8.7}
\expandafter\def\csname v@cs/parakeet-tdt-v3/mono-after\endcsname{27.8}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/after\endcsname{39.6}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/after-wer\endcsname{76.8}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/before\endcsname{64.1}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/en-after\endcsname{1}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/en-before\endcsname{15}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/gain\endcsname{24.5}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/gain-ci\endcsname{23.6 to 25.4}
\expandafter\def\csname v@cs/qwen3-asr-0.6b/mono-after\endcsname{20.2}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/after\endcsname{37.6}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/after-wer\endcsname{71.5}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/before\endcsname{65.6}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/en-after\endcsname{1}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/en-before\endcsname{11}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/gain\endcsname{28.0}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/gain-ci\endcsname{27.1 to 28.9}
\expandafter\def\csname v@cs/qwen3-asr-1.7b/mono-after\endcsname{16.7}
\expandafter\def\csname v@cs/voxtral-mini/after\endcsname{35.1}
\expandafter\def\csname v@cs/voxtral-mini/after-wer\endcsname{61.8}
\expandafter\def\csname v@cs/voxtral-mini/before\endcsname{69.7}
\expandafter\def\csname v@cs/voxtral-mini/en-after\endcsname{1}
\expandafter\def\csname v@cs/voxtral-mini/en-before\endcsname{16}
\expandafter\def\csname v@cs/voxtral-mini/gain\endcsname{34.6}
\expandafter\def\csname v@cs/voxtral-mini/gain-ci\endcsname{33.4 to 35.9}
\expandafter\def\csname v@cs/voxtral-mini/mono-after\endcsname{13.3}
\expandafter\def\csname v@cs/w2v-bert/after\endcsname{26.2}
\expandafter\def\csname v@cs/w2v-bert/after-wer\endcsname{59.0}
\expandafter\def\csname v@cs/w2v-bert/en-after\endcsname{1}
\expandafter\def\csname v@cs/w2v-bert/mono-after\endcsname{8.8}
\expandafter\def\csname v@cs/whisper-large-v2/after\endcsname{33.8}
\expandafter\def\csname v@cs/whisper-large-v2/after-wer\endcsname{60.7}
\expandafter\def\csname v@cs/whisper-large-v2/before\endcsname{56.4}
\expandafter\def\csname v@cs/whisper-large-v2/en-after\endcsname{0}
\expandafter\def\csname v@cs/whisper-large-v2/en-before\endcsname{2}
\expandafter\def\csname v@cs/whisper-large-v2/gain\endcsname{22.6}
\expandafter\def\csname v@cs/whisper-large-v2/gain-ci\endcsname{21.6 to 23.5}
\expandafter\def\csname v@cs/whisper-large-v2/mono-after\endcsname{14.8}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/after\endcsname{35.5}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/after-wer\endcsname{63.8}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/before\endcsname{59.0}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/en-after\endcsname{2}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/en-before\endcsname{12}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/gain\endcsname{23.4}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/gain-ci\endcsname{22.4 to 24.5}
\expandafter\def\csname v@cs/whisper-large-v3-turbo/mono-after\endcsname{15.7}
\expandafter\def\csname v@cs/whisper-large-v3/after\endcsname{33.6}
\expandafter\def\csname v@cs/whisper-large-v3/after-wer\endcsname{60.2}
\expandafter\def\csname v@cs/whisper-large-v3/before\endcsname{47.4}
\expandafter\def\csname v@cs/whisper-large-v3/en-after\endcsname{0}
\expandafter\def\csname v@cs/whisper-large-v3/en-before\endcsname{5}
\expandafter\def\csname v@cs/whisper-large-v3/gain\endcsname{13.7}
\expandafter\def\csname v@cs/whisper-large-v3/gain-ci\endcsname{12.8 to 14.8}
\expandafter\def\csname v@cs/whisper-large-v3/mono-after\endcsname{13.5}
\expandafter\def\csname v@cs/whisper-medium/after\endcsname{34.5}
\expandafter\def\csname v@cs/whisper-medium/after-wer\endcsname{64.9}
\expandafter\def\csname v@cs/whisper-medium/before\endcsname{57.2}
\expandafter\def\csname v@cs/whisper-medium/en-after\endcsname{1}
\expandafter\def\csname v@cs/whisper-medium/en-before\endcsname{7}
\expandafter\def\csname v@cs/whisper-medium/gain\endcsname{22.7}
\expandafter\def\csname v@cs/whisper-medium/gain-ci\endcsname{21.8 to 23.7}
\expandafter\def\csname v@cs/whisper-medium/mono-after\endcsname{15.0}
\expandafter\def\csname v@cs/whisper-small/after\endcsname{37.0}
\expandafter\def\csname v@cs/whisper-small/after-wer\endcsname{70.7}
\expandafter\def\csname v@cs/whisper-small/before\endcsname{61.8}
\expandafter\def\csname v@cs/whisper-small/en-after\endcsname{1}
\expandafter\def\csname v@cs/whisper-small/en-before\endcsname{0}
\expandafter\def\csname v@cs/whisper-small/gain\endcsname{24.8}
\expandafter\def\csname v@cs/whisper-small/gain-ci\endcsname{23.8 to 25.9}
\expandafter\def\csname v@cs/whisper-small/mono-after\endcsname{19.4}
\expandafter\def\csname v@cs/whisper-tiny/after\endcsname{43.3}
\expandafter\def\csname v@cs/whisper-tiny/after-wer\endcsname{83.8}
\expandafter\def\csname v@cs/whisper-tiny/before\endcsname{63.5}
\expandafter\def\csname v@cs/whisper-tiny/en-after\endcsname{0}
\expandafter\def\csname v@cs/whisper-tiny/en-before\endcsname{9}
\expandafter\def\csname v@cs/whisper-tiny/gain\endcsname{20.2}
\expandafter\def\csname v@cs/whisper-tiny/gain-ci\endcsname{18.9 to 21.6}
\expandafter\def\csname v@cs/whisper-tiny/mono-after\endcsname{33.0}
\expandafter\def\csname v@cs/with-before-n\endcsname{20}
\expandafter\def\csname v@csms/better-n\endcsname{11}
\expandafter\def\csname v@csms/cohere-transcribe/after\endcsname{19.9}
\expandafter\def\csname v@csms/cohere-transcribe/before\endcsname{28.4}
\expandafter\def\csname v@csms/cohere-transcribe/gain\endcsname{8.5}
\expandafter\def\csname v@csms/cohere-transcribe/gain-ci\endcsname{5.7 to 11.5}
\expandafter\def\csname v@csms/gain-median\endcsname{7.4}
\expandafter\def\csname v@csms/gemma4-12b/after\endcsname{35.9}
\expandafter\def\csname v@csms/gemma4-12b/before\endcsname{47.7}
\expandafter\def\csname v@csms/gemma4-12b/gain\endcsname{11.8}
\expandafter\def\csname v@csms/gemma4-12b/gain-ci\endcsname{6.5 to 17.3}
\expandafter\def\csname v@csms/gemma4-e2b/after\endcsname{21.7}
\expandafter\def\csname v@csms/gemma4-e2b/before\endcsname{17.0}
\expandafter\def\csname v@csms/gemma4-e2b/gain\endcsname{-4.7}
\expandafter\def\csname v@csms/gemma4-e2b/gain-ci\endcsname{-6.1 to -3.4}
\expandafter\def\csname v@csms/gemma4-e4b/after\endcsname{16.8}
\expandafter\def\csname v@csms/gemma4-e4b/before\endcsname{15.2}
\expandafter\def\csname v@csms/gemma4-e4b/gain\endcsname{-1.6}
\expandafter\def\csname v@csms/gemma4-e4b/gain-ci\endcsname{-2.4 to -0.9}
\expandafter\def\csname v@csms/granite-2b/after\endcsname{34.5}
\expandafter\def\csname v@csms/granite-2b/before\endcsname{26.7}
\expandafter\def\csname v@csms/granite-2b/gain\endcsname{-7.8}
\expandafter\def\csname v@csms/granite-2b/gain-ci\endcsname{-9.9 to -6.0}
\expandafter\def\csname v@csms/lfm3-audio/after\endcsname{27.5}
\expandafter\def\csname v@csms/lfm3-audio/before\endcsname{51.1}
\expandafter\def\csname v@csms/lfm3-audio/gain\endcsname{23.7}
\expandafter\def\csname v@csms/lfm3-audio/gain-ci\endcsname{19.7 to 27.4}
\expandafter\def\csname v@csms/mms-1b/after\endcsname{16.5}
\expandafter\def\csname v@csms/mms-1b/before\endcsname{14.4}
\expandafter\def\csname v@csms/mms-1b/gain\endcsname{-2.1}
\expandafter\def\csname v@csms/mms-1b/gain-ci\endcsname{-2.5 to -1.7}
\expandafter\def\csname v@csms/n\endcsname{19}
\expandafter\def\csname v@csms/nemotron-stream/after\endcsname{54.0}
\expandafter\def\csname v@csms/nemotron-stream/before\endcsname{79.5}
\expandafter\def\csname v@csms/nemotron-stream/gain\endcsname{25.5}
\expandafter\def\csname v@csms/nemotron-stream/gain-ci\endcsname{22.9 to 27.8}
\expandafter\def\csname v@csms/omni-ctc-1b/after\endcsname{17.4}
\expandafter\def\csname v@csms/omni-ctc-1b/before\endcsname{16.0}
\expandafter\def\csname v@csms/omni-ctc-1b/gain\endcsname{-1.4}
\expandafter\def\csname v@csms/omni-ctc-1b/gain-ci\endcsname{-2.3 to -0.5}
\expandafter\def\csname v@csms/parakeet-tdt-v3/after\endcsname{25.3}
\expandafter\def\csname v@csms/parakeet-tdt-v3/before\endcsname{30.9}
\expandafter\def\csname v@csms/parakeet-tdt-v3/gain\endcsname{5.7}
\expandafter\def\csname v@csms/parakeet-tdt-v3/gain-ci\endcsname{3.3 to 7.8}
\expandafter\def\csname v@csms/qwen3-asr-0.6b/after\endcsname{24.5}
\expandafter\def\csname v@csms/qwen3-asr-0.6b/before\endcsname{14.7}
\expandafter\def\csname v@csms/qwen3-asr-0.6b/gain\endcsname{-9.8}
\expandafter\def\csname v@csms/qwen3-asr-0.6b/gain-ci\endcsname{-11.4 to -8.5}
\expandafter\def\csname v@csms/qwen3-asr-1.7b/after\endcsname{18.3}
\expandafter\def\csname v@csms/qwen3-asr-1.7b/before\endcsname{17.5}
\expandafter\def\csname v@csms/qwen3-asr-1.7b/gain\endcsname{-0.8}
\expandafter\def\csname v@csms/qwen3-asr-1.7b/gain-ci\endcsname{-2.5 to 0.9}
\expandafter\def\csname v@csms/voxtral-mini/after\endcsname{18.0}
\expandafter\def\csname v@csms/voxtral-mini/before\endcsname{27.4}
\expandafter\def\csname v@csms/voxtral-mini/gain\endcsname{9.4}
\expandafter\def\csname v@csms/voxtral-mini/gain-ci\endcsname{7.7 to 11.2}
\expandafter\def\csname v@csms/whisper-large-v2/after\endcsname{15.9}
\expandafter\def\csname v@csms/whisper-large-v2/before\endcsname{25.3}
\expandafter\def\csname v@csms/whisper-large-v2/gain\endcsname{9.3}
\expandafter\def\csname v@csms/whisper-large-v2/gain-ci\endcsname{7.7 to 11.0}
\expandafter\def\csname v@csms/whisper-large-v3-turbo/after\endcsname{16.6}
\expandafter\def\csname v@csms/whisper-large-v3-turbo/before\endcsname{26.3}
\expandafter\def\csname v@csms/whisper-large-v3-turbo/gain\endcsname{9.7}
\expandafter\def\csname v@csms/whisper-large-v3-turbo/gain-ci\endcsname{8.2 to 11.4}
\expandafter\def\csname v@csms/whisper-large-v3/after\endcsname{14.6}
\expandafter\def\csname v@csms/whisper-large-v3/before\endcsname{25.3}
\expandafter\def\csname v@csms/whisper-large-v3/gain\endcsname{10.7}
\expandafter\def\csname v@csms/whisper-large-v3/gain-ci\endcsname{9.3 to 12.3}
\expandafter\def\csname v@csms/whisper-medium/after\endcsname{15.4}
\expandafter\def\csname v@csms/whisper-medium/before\endcsname{22.8}
\expandafter\def\csname v@csms/whisper-medium/gain\endcsname{7.4}
\expandafter\def\csname v@csms/whisper-medium/gain-ci\endcsname{5.7 to 9.5}
\expandafter\def\csname v@csms/whisper-small/after\endcsname{19.2}
\expandafter\def\csname v@csms/whisper-small/before\endcsname{28.9}
\expandafter\def\csname v@csms/whisper-small/gain\endcsname{9.7}
\expandafter\def\csname v@csms/whisper-small/gain-ci\endcsname{7.8 to 11.8}
\expandafter\def\csname v@csms/whisper-tiny/after\endcsname{38.8}
\expandafter\def\csname v@csms/whisper-tiny/before\endcsname{33.4}
\expandafter\def\csname v@csms/whisper-tiny/gain\endcsname{-5.4}
\expandafter\def\csname v@csms/whisper-tiny/gain-ci\endcsname{-8.7 to -1.9}
\expandafter\def\csname v@cv/absent\endcsname{37}
\expandafter\def\csname v@cv/big-n\endcsname{8}
\expandafter\def\csname v@cv/big-only-better\endcsname{6}
\expandafter\def\csname v@cv/both-better\endcsname{9}
\expandafter\def\csname v@cv/both-gain\endcsname{4.1}
\expandafter\def\csname v@cv/both-gain-ci\endcsname{3.2 to 4.9}
\expandafter\def\csname v@cv/both-vs-only\endcsname{7.6}
\expandafter\def\csname v@cv/both-worse-max\endcsname{1.0}
\expandafter\def\csname v@cv/both-worse-n\endcsname{2}
\expandafter\def\csname v@cv/both-worse-names\endcsname{Lao and Occitan}
\expandafter\def\csname v@cv/both-worse-small\endcsname{2}
\expandafter\def\csname v@cv/cap\endcsname{4,000}
\expandafter\def\csname v@cv/clips\endcsname{30,594}
\expandafter\def\csname v@cv/cv-clips\endcsname{30,535}
\expandafter\def\csname v@cv/cv-hours\endcsname{41.9}
\expandafter\def\csname v@cv/cv_both/bre_Latn\endcsname{20.4}
\expandafter\def\csname v@cv/cv_both/cer\endcsname{12.8}
\expandafter\def\csname v@cv/cv_both/chv_Cyrl\endcsname{10.3}
\expandafter\def\csname v@cv/cv_both/ekk_Latn\endcsname{6.4}
\expandafter\def\csname v@cv/cv_both/epoch\endcsname{6}
\expandafter\def\csname v@cv/cv_both/fin_Latn\endcsname{9.1}
\expandafter\def\csname v@cv/cv_both/fry_Latn\endcsname{8.0}
\expandafter\def\csname v@cv/cv_both/lao_Laoo\endcsname{16.9}
\expandafter\def\csname v@cv/cv_both/lvs_Latn\endcsname{6.5}
\expandafter\def\csname v@cv/cv_both/oci_Latn\endcsname{23.5}
\expandafter\def\csname v@cv/cv_both/slv_Latn\endcsname{15.4}
\expandafter\def\csname v@cv/cv_both/tgk_Cyrl\endcsname{8.5}
\expandafter\def\csname v@cv/cv_both/wer\endcsname{43.3}
\expandafter\def\csname v@cv/cv_both/zgh_Tfng\endcsname{15.8}
\expandafter\def\csname v@cv/cv_main/bre_Latn\endcsname{33.6}
\expandafter\def\csname v@cv/cv_main/cer\endcsname{16.9}
\expandafter\def\csname v@cv/cv_main/chv_Cyrl\endcsname{15.5}
\expandafter\def\csname v@cv/cv_main/ekk_Latn\endcsname{10.7}
\expandafter\def\csname v@cv/cv_main/epoch\endcsname{7}
\expandafter\def\csname v@cv/cv_main/fin_Latn\endcsname{16.0}
\expandafter\def\csname v@cv/cv_main/fry_Latn\endcsname{16.0}
\expandafter\def\csname v@cv/cv_main/lao_Laoo\endcsname{16.5}
\expandafter\def\csname v@cv/cv_main/lvs_Latn\endcsname{9.2}
\expandafter\def\csname v@cv/cv_main/oci_Latn\endcsname{22.4}
\expandafter\def\csname v@cv/cv_main/slv_Latn\endcsname{18.3}
\expandafter\def\csname v@cv/cv_main/tgk_Cyrl\endcsname{9.0}
\expandafter\def\csname v@cv/cv_main/wer\endcsname{53.3}
\expandafter\def\csname v@cv/cv_main/zgh_Tfng\endcsname{19.1}
\expandafter\def\csname v@cv/cv_only/bre_Latn\endcsname{16.4}
\expandafter\def\csname v@cv/cv_only/cer\endcsname{20.4}
\expandafter\def\csname v@cv/cv_only/chv_Cyrl\endcsname{14.3}
\expandafter\def\csname v@cv/cv_only/ekk_Latn\endcsname{10.2}
\expandafter\def\csname v@cv/cv_only/epoch\endcsname{7}
\expandafter\def\csname v@cv/cv_only/fin_Latn\endcsname{10.7}
\expandafter\def\csname v@cv/cv_only/fry_Latn\endcsname{9.6}
\expandafter\def\csname v@cv/cv_only/lao_Laoo\endcsname{49.6}
\expandafter\def\csname v@cv/cv_only/lvs_Latn\endcsname{11.1}
\expandafter\def\csname v@cv/cv_only/oci_Latn\endcsname{40.5}
\expandafter\def\csname v@cv/cv_only/slv_Latn\endcsname{22.7}
\expandafter\def\csname v@cv/cv_only/tgk_Cyrl\endcsname{22.0}
\expandafter\def\csname v@cv/cv_only/wer\endcsname{56.9}
\expandafter\def\csname v@cv/cv_only/zgh_Tfng\endcsname{17.6}
\expandafter\def\csname v@cv/enough\endcsname{11}
\expandafter\def\csname v@cv/ft50\endcsname{19.5}
\expandafter\def\csname v@cv/ft50-epoch\endcsname{4}
\expandafter\def\csname v@cv/ft50-gain\endcsname{2.6}
\expandafter\def\csname v@cv/ft50-gain-ci\endcsname{1.4 to 4.0}
\expandafter\def\csname v@cv/locales\endcsname{137}
\expandafter\def\csname v@cv/main-clips\endcsname{10,157}
\expandafter\def\csname v@cv/main-hours\endcsname{23.4}
\expandafter\def\csname v@cv/matched\endcsname{13}
\expandafter\def\csname v@cv/n\endcsname{11}
\expandafter\def\csname v@cv/only-better\endcsname{6}
\expandafter\def\csname v@cv/only-loss\endcsname{3.5}
\expandafter\def\csname v@cv/only-loss-ci\endcsname{2.1 to 4.8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/both\endcsname{12.0}
\expandafter\def\csname v@cv/parakeet-tdt-v3/both-better\endcsname{8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/both-epoch\endcsname{8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/both-gain\endcsname{4.8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/both-gain-ci\endcsname{3.6 to 5.8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/ft50\endcsname{16.8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/ft50-gain\endcsname{0.1}
\expandafter\def\csname v@cv/parakeet-tdt-v3/ft50-gain-ci\endcsname{-1.2 to 1.3}
\expandafter\def\csname v@cv/parakeet-tdt-v3/main\endcsname{16.7}
\expandafter\def\csname v@cv/parakeet-tdt-v3/main-epoch\endcsname{9}
\expandafter\def\csname v@cv/parakeet-tdt-v3/only\endcsname{19.3}
\expandafter\def\csname v@cv/parakeet-tdt-v3/only-better\endcsname{4}
\expandafter\def\csname v@cv/parakeet-tdt-v3/only-epoch\endcsname{8}
\expandafter\def\csname v@cv/parakeet-tdt-v3/only-loss\endcsname{2.6}
\expandafter\def\csname v@cv/parakeet-tdt-v3/only-loss-ci\endcsname{1.0 to 4.3}
\expandafter\def\csname v@cv/small-main\endcsname{16.0}
\expandafter\def\csname v@cv/small-n\endcsname{3}
\expandafter\def\csname v@cv/small-names\endcsname{Lao, Occitan and Tajik}
\expandafter\def\csname v@cv/small-only\endcsname{37.4}
\expandafter\def\csname v@cv/update-share\endcsname{24}
\expandafter\def\csname v@cv/whisper-small/both\endcsname{11.7}
\expandafter\def\csname v@cv/whisper-small/both-better\endcsname{9}
\expandafter\def\csname v@cv/whisper-small/both-epoch\endcsname{7}
\expandafter\def\csname v@cv/whisper-small/both-gain\endcsname{3.5}
\expandafter\def\csname v@cv/whisper-small/both-gain-ci\endcsname{2.7 to 4.3}
\expandafter\def\csname v@cv/whisper-small/ft50\endcsname{16.6}
\expandafter\def\csname v@cv/whisper-small/ft50-gain\endcsname{1.5}
\expandafter\def\csname v@cv/whisper-small/ft50-gain-ci\endcsname{0.7 to 2.3}
\expandafter\def\csname v@cv/whisper-small/main\endcsname{15.2}
\expandafter\def\csname v@cv/whisper-small/main-epoch\endcsname{9}
\expandafter\def\csname v@cv/whisper-small/only\endcsname{18.9}
\expandafter\def\csname v@cv/whisper-small/only-better\endcsname{3}
\expandafter\def\csname v@cv/whisper-small/only-epoch\endcsname{4}
\expandafter\def\csname v@cv/whisper-small/only-loss\endcsname{3.7}
\expandafter\def\csname v@cv/whisper-small/only-loss-ci\endcsname{2.7 to 4.6}
\expandafter\def\csname v@data/bad-test-clips\endcsname{2}
\expandafter\def\csname v@data/dev-clips\endcsname{1,250}
\expandafter\def\csname v@data/dev-hours\endcsname{2.58}
\expandafter\def\csname v@data/dev-rare\endcsname{72}
\expandafter\def\csname v@data/dev-spk-median\endcsname{2}
\expandafter\def\csname v@data/disjoint\endcsname{45}
\expandafter\def\csname v@data/families\endcsname{13}
\expandafter\def\csname v@data/fetch-n\endcsname{1,250}
\expandafter\def\csname v@data/fetch-same\endcsname{1,250}
\expandafter\def\csname v@data/fleurs-test-clips\endcsname{151}
\expandafter\def\csname v@data/fleurs-test-from-test\endcsname{55}
\expandafter\def\csname v@data/fleurs-test-from-train\endcsname{18}
\expandafter\def\csname v@data/fleurs-test-langs\endcsname{7}
\expandafter\def\csname v@data/fleurs-train-clips\endcsname{12,219}
\expandafter\def\csname v@data/fleurs-whole-n\endcsname{4}
\expandafter\def\csname v@data/fleurs-whole-names\endcsname{Estonian, Latvian, Occitan and Slovenian}
\expandafter\def\csname v@data/k100-clips\endcsname{4,820}
\expandafter\def\csname v@data/k100-full\endcsname{45}
\expandafter\def\csname v@data/k100-hours\endcsname{8}
\expandafter\def\csname v@data/k1000-clips\endcsname{42,816}
\expandafter\def\csname v@data/k1000-full\endcsname{36}
\expandafter\def\csname v@data/k1000-hours\endcsname{82}
\expandafter\def\csname v@data/k1000-minutes\endcsname{98}
\expandafter\def\csname v@data/k200-clips\endcsname{9,542}
\expandafter\def\csname v@data/k200-full\endcsname{44}
\expandafter\def\csname v@data/k200-hours\endcsname{17}
\expandafter\def\csname v@data/k2000-clips\endcsname{77,278}
\expandafter\def\csname v@data/k2000-full\endcsname{29}
\expandafter\def\csname v@data/k2000-hours\endcsname{159}
\expandafter\def\csname v@data/k25-clips\endcsname{1,209}
\expandafter\def\csname v@data/k25-full\endcsname{46}
\expandafter\def\csname v@data/k25-hours\endcsname{2}
\expandafter\def\csname v@data/k4000-clips\endcsname{129,236}
\expandafter\def\csname v@data/k4000-full\endcsname{21}
\expandafter\def\csname v@data/k4000-hours\endcsname{279}
\expandafter\def\csname v@data/k50-clips\endcsname{2,419}
\expandafter\def\csname v@data/k50-full\endcsname{46}
\expandafter\def\csname v@data/k50-hours\endcsname{4}
\expandafter\def\csname v@data/k500-clips\endcsname{22,896}
\expandafter\def\csname v@data/k500-full\endcsname{38}
\expandafter\def\csname v@data/k500-hours\endcsname{42}
\expandafter\def\csname v@data/latin\endcsname{36}
\expandafter\def\csname v@data/listed/nemotron_stream\endcsname{4}
\expandafter\def\csname v@data/listed/nemotron_transcribe\endcsname{4}
\expandafter\def\csname v@data/listed/parakeet\endcsname{4}
\expandafter\def\csname v@data/listed/qwen3\endcsname{1}
\expandafter\def\csname v@data/listed/whisper\endcsname{17}
\expandafter\def\csname v@data/max-hours\endcsname{19.9}
\expandafter\def\csname v@data/median-clips\endcsname{3,201}
\expandafter\def\csname v@data/median-hours\endcsname{4.6}
\expandafter\def\csname v@data/min-clips\endcsname{96}
\expandafter\def\csname v@data/min-hours\endcsname{0.1}
\expandafter\def\csname v@data/nonlatin\endcsname{14}
\expandafter\def\csname v@data/pairs-n\endcsname{125,984}
\expandafter\def\csname v@data/pairs-off\endcsname{1}
\expandafter\def\csname v@data/scripts\endcsname{11}
\expandafter\def\csname v@data/shared\endcsname{5}
\expandafter\def\csname v@data/shared-names\endcsname{Crimean Tatar, Goan Konkani, Gurani, Meitei and Wayuu}
\expandafter\def\csname v@data/test-clips\endcsname{1,250}
\expandafter\def\csname v@data/test-corpus-trains\endcsname{50}
\expandafter\def\csname v@data/test-hours\endcsname{2.56}
\expandafter\def\csname v@data/test-one-corpus\endcsname{41}
\expandafter\def\csname v@data/test-rare\endcsname{11}
\expandafter\def\csname v@data/test-speakers\endcsname{514}
\expandafter\def\csname v@data/test-spk-median\endcsname{118}
\expandafter\def\csname v@data/test-subsets\endcsname{59}
\expandafter\def\csname v@data/train-clips\endcsname{129,236}
\expandafter\def\csname v@data/train-hours\endcsname{279}
\expandafter\def\csname v@data/train-rare\endcsname{28}
\expandafter\def\csname v@data/train-speakers\endcsname{27,206}
\expandafter\def\csname v@data/train-spk-median\endcsname{36}
\expandafter\def\csname v@data/train-subsets\endcsname{90}
\expandafter\def\csname v@data/uncovered/nemotron-stream\endcsname{7}
\expandafter\def\csname v@data/uncovered/parakeet-tdt-v3\endcsname{10}
\expandafter\def\csname v@dec/CTC/best\endcsname{11.0}
\expandafter\def\csname v@dec/CTC/best-name\endcsname{MMS 1B}
\expandafter\def\csname v@dec/CTC/median\endcsname{12.0}
\expandafter\def\csname v@dec/CTC/n\endcsname{3}
\expandafter\def\csname v@dec/assist/max\endcsname{19.8}
\expandafter\def\csname v@dec/assist/min\endcsname{16.6}
\expandafter\def\csname v@dec/assist/n\endcsname{4}
\expandafter\def\csname v@dec/band-hi\endcsname{0.81}
\expandafter\def\csname v@dec/band-lo\endcsname{0.58}
\expandafter\def\csname v@dec/ctc-langs-max\endcsname{1,600+}
\expandafter\def\csname v@dec/ctc-langs-min\endcsname{143}
\expandafter\def\csname v@dec/gap\endcsname{0.8}
\expandafter\def\csname v@dec/gap-ci\endcsname{0.4 to 1.2}
\expandafter\def\csname v@dec/gap-ctc\endcsname{w2v-BERT 2.0}
\expandafter\def\csname v@dec/gap-other\endcsname{Whisper large-v3}
\expandafter\def\csname v@dec/language model/best\endcsname{15.8}
\expandafter\def\csname v@dec/language model/best-name\endcsname{Nemotron 3.5 Transcribe 30B}
\expandafter\def\csname v@dec/language model/median\endcsname{17.8}
\expandafter\def\csname v@dec/language model/n\endcsname{9}
\expandafter\def\csname v@dec/other-langs-max\endcsname{99}
\expandafter\def\csname v@dec/seq2seq/best\endcsname{13.5}
\expandafter\def\csname v@dec/seq2seq/best-name\endcsname{Whisper large-v3}
\expandafter\def\csname v@dec/seq2seq/median\endcsname{14.8}
\expandafter\def\csname v@dec/seq2seq/n\endcsname{7}
\expandafter\def\csname v@dec/speechlm/max\endcsname{22.5}
\expandafter\def\csname v@dec/speechlm/min\endcsname{15.8}
\expandafter\def\csname v@dec/transducer/best\endcsname{21.0}
\expandafter\def\csname v@dec/transducer/best-name\endcsname{Parakeet TDT 0.6B v3}
\expandafter\def\csname v@dec/transducer/median\endcsname{28.4}
\expandafter\def\csname v@dec/transducer/n\endcsname{2}
\expandafter\def\csname v@ep/cohere-transcribe/best\endcsname{10}
\expandafter\def\csname v@ep/cohere-transcribe/d3-last\endcsname{0.7}
\expandafter\def\csname v@ep/cohere-transcribe/d3-last-ci\endcsname{0.3 to 1.2}
\expandafter\def\csname v@ep/cohere-transcribe/t1\endcsname{22.0}
\expandafter\def\csname v@ep/cohere-transcribe/t10\endcsname{15.6}
\expandafter\def\csname v@ep/cohere-transcribe/t2\endcsname{17.1}
\expandafter\def\csname v@ep/cohere-transcribe/t3\endcsname{16.3}
\expandafter\def\csname v@ep/cohere-transcribe/t4\endcsname{16.1}
\expandafter\def\csname v@ep/cohere-transcribe/t5\endcsname{15.5}
\expandafter\def\csname v@ep/cohere-transcribe/t6\endcsname{15.9}
\expandafter\def\csname v@ep/cohere-transcribe/t7\endcsname{15.9}
\expandafter\def\csname v@ep/cohere-transcribe/t8\endcsname{15.3}
\expandafter\def\csname v@ep/cohere-transcribe/t9\endcsname{15.7}
\expandafter\def\csname v@ep/cohere-transcribe/within\endcsname{4}
\expandafter\def\csname v@ep/d3-flat-names\endcsname{Whisper large-v2, Whisper small, Qwen3-ASR 1.7B, Qwen3-ASR 0.6B, Nemotron 3.5 Transcribe 30B, Voxtral Mini 3B, Granite Speech 5.0 2B, LFM3-Audio 2B, Gemma 4 E2B, Gemma 4 E4B and Gemma 4 12B}
\expandafter\def\csname v@ep/d3-n\endcsname{21}
\expandafter\def\csname v@ep/d3-seq-sig-max\endcsname{1.6}
\expandafter\def\csname v@ep/d3-seq-sig-n\endcsname{5}
\expandafter\def\csname v@ep/d3-seq-sig-names\endcsname{Whisper large-v3, Whisper large-v3-turbo, Whisper medium, Whisper tiny and Cohere Transcribe 2B}
\expandafter\def\csname v@ep/d3-sig\endcsname{10}
\expandafter\def\csname v@ep/d3-sig-names\endcsname{Whisper large-v3, Whisper large-v3-turbo, Whisper medium, Whisper tiny, Parakeet TDT 0.6B v3, Nemotron 3.5 streaming 0.6B, w2v-BERT 2.0, MMS 1B, omniASR CTC 1B and Cohere Transcribe 2B}
\expandafter\def\csname v@ep/first-share\endcsname{90}
\expandafter\def\csname v@ep/gemma4-12b/best\endcsname{2}
\expandafter\def\csname v@ep/gemma4-12b/d3-last\endcsname{0.4}
\expandafter\def\csname v@ep/gemma4-12b/d3-last-ci\endcsname{-0.4 to 1.1}
\expandafter\def\csname v@ep/gemma4-12b/t1\endcsname{22.6}
\expandafter\def\csname v@ep/gemma4-12b/t2\endcsname{19.8}
\expandafter\def\csname v@ep/gemma4-12b/t3\endcsname{21.4}
\expandafter\def\csname v@ep/gemma4-12b/t4\endcsname{21.0}
\expandafter\def\csname v@ep/gemma4-12b/within\endcsname{2}
\expandafter\def\csname v@ep/gemma4-e2b/best\endcsname{5}
\expandafter\def\csname v@ep/gemma4-e2b/d3-last\endcsname{-0.1}
\expandafter\def\csname v@ep/gemma4-e2b/d3-last-ci\endcsname{-0.8 to 0.5}
\expandafter\def\csname v@ep/gemma4-e2b/t1\endcsname{18.9}
\expandafter\def\csname v@ep/gemma4-e2b/t2\endcsname{18.1}
\expandafter\def\csname v@ep/gemma4-e2b/t3\endcsname{18.4}
\expandafter\def\csname v@ep/gemma4-e2b/t4\endcsname{17.8}
\expandafter\def\csname v@ep/gemma4-e2b/t5\endcsname{18.5}
\expandafter\def\csname v@ep/gemma4-e2b/within\endcsname{3}
\expandafter\def\csname v@ep/gemma4-e4b/best\endcsname{2}
\expandafter\def\csname v@ep/gemma4-e4b/d3-last\endcsname{-0.9}
\expandafter\def\csname v@ep/gemma4-e4b/d3-last-ci\endcsname{-1.5 to -0.3}
\expandafter\def\csname v@ep/gemma4-e4b/t1\endcsname{17.4}
\expandafter\def\csname v@ep/gemma4-e4b/t2\endcsname{16.6}
\expandafter\def\csname v@ep/gemma4-e4b/t3\endcsname{17.4}
\expandafter\def\csname v@ep/gemma4-e4b/t4\endcsname{18.0}
\expandafter\def\csname v@ep/gemma4-e4b/t5\endcsname{18.3}
\expandafter\def\csname v@ep/gemma4-e4b/within\endcsname{2}
\expandafter\def\csname v@ep/granite-2b/best\endcsname{7}
\expandafter\def\csname v@ep/granite-2b/d3-last\endcsname{0.3}
\expandafter\def\csname v@ep/granite-2b/d3-last-ci\endcsname{-0.2 to 1.0}
\expandafter\def\csname v@ep/granite-2b/t1\endcsname{26.9}
\expandafter\def\csname v@ep/granite-2b/t10\endcsname{22.5}
\expandafter\def\csname v@ep/granite-2b/t2\endcsname{24.4}
\expandafter\def\csname v@ep/granite-2b/t3\endcsname{22.8}
\expandafter\def\csname v@ep/granite-2b/t4\endcsname{22.4}
\expandafter\def\csname v@ep/granite-2b/t5\endcsname{23.1}
\expandafter\def\csname v@ep/granite-2b/t6\endcsname{23.3}
\expandafter\def\csname v@ep/granite-2b/t7\endcsname{22.5}
\expandafter\def\csname v@ep/granite-2b/t8\endcsname{23.3}
\expandafter\def\csname v@ep/granite-2b/t9\endcsname{23.3}
\expandafter\def\csname v@ep/granite-2b/within\endcsname{4}
\expandafter\def\csname v@ep/lfm3-audio/best\endcsname{3}
\expandafter\def\csname v@ep/lfm3-audio/d3-last\endcsname{-0.4}
\expandafter\def\csname v@ep/lfm3-audio/d3-last-ci\endcsname{-0.9 to 0.1}
\expandafter\def\csname v@ep/lfm3-audio/t1\endcsname{21.2}
\expandafter\def\csname v@ep/lfm3-audio/t10\endcsname{18.2}
\expandafter\def\csname v@ep/lfm3-audio/t2\endcsname{18.2}
\expandafter\def\csname v@ep/lfm3-audio/t3\endcsname{17.8}
\expandafter\def\csname v@ep/lfm3-audio/t4\endcsname{18.3}
\expandafter\def\csname v@ep/lfm3-audio/t5\endcsname{18.1}
\expandafter\def\csname v@ep/lfm3-audio/t6\endcsname{18.2}
\expandafter\def\csname v@ep/lfm3-audio/t7\endcsname{18.2}
\expandafter\def\csname v@ep/lfm3-audio/t8\endcsname{18.4}
\expandafter\def\csname v@ep/lfm3-audio/t9\endcsname{17.9}
\expandafter\def\csname v@ep/lfm3-audio/within\endcsname{2}
\expandafter\def\csname v@ep/mms-1b/best\endcsname{10}
\expandafter\def\csname v@ep/mms-1b/d3-last\endcsname{3.5}
\expandafter\def\csname v@ep/mms-1b/d3-last-ci\endcsname{3.1 to 3.9}
\expandafter\def\csname v@ep/mms-1b/t1\endcsname{16.4}
\expandafter\def\csname v@ep/mms-1b/t10\endcsname{11.0}
\expandafter\def\csname v@ep/mms-1b/t2\endcsname{14.4}
\expandafter\def\csname v@ep/mms-1b/t3\endcsname{14.5}
\expandafter\def\csname v@ep/mms-1b/t4\endcsname{13.2}
\expandafter\def\csname v@ep/mms-1b/t5\endcsname{12.3}
\expandafter\def\csname v@ep/mms-1b/t6\endcsname{12.0}
\expandafter\def\csname v@ep/mms-1b/t7\endcsname{11.8}
\expandafter\def\csname v@ep/mms-1b/t8\endcsname{12.1}
\expandafter\def\csname v@ep/mms-1b/t9\endcsname{11.5}
\expandafter\def\csname v@ep/mms-1b/within\endcsname{6}
\expandafter\def\csname v@ep/nemotron-30b/best\endcsname{2}
\expandafter\def\csname v@ep/nemotron-30b/d3-last\endcsname{0.0}
\expandafter\def\csname v@ep/nemotron-30b/d3-last-ci\endcsname{-0.4 to 0.4}
\expandafter\def\csname v@ep/nemotron-30b/t1\endcsname{16.7}
\expandafter\def\csname v@ep/nemotron-30b/t2\endcsname{15.8}
\expandafter\def\csname v@ep/nemotron-30b/t3\endcsname{16.3}
\expandafter\def\csname v@ep/nemotron-30b/t4\endcsname{16.3}
\expandafter\def\csname v@ep/nemotron-30b/within\endcsname{1}
\expandafter\def\csname v@ep/nemotron-stream/best\endcsname{10}
\expandafter\def\csname v@ep/nemotron-stream/d3-last\endcsname{9.2}
\expandafter\def\csname v@ep/nemotron-stream/d3-last-ci\endcsname{8.6 to 9.9}
\expandafter\def\csname v@ep/nemotron-stream/t1\endcsname{45.7}
\expandafter\def\csname v@ep/nemotron-stream/t10\endcsname{35.9}
\expandafter\def\csname v@ep/nemotron-stream/t2\endcsname{45.7}
\expandafter\def\csname v@ep/nemotron-stream/t3\endcsname{45.1}
\expandafter\def\csname v@ep/nemotron-stream/t4\endcsname{44.9}
\expandafter\def\csname v@ep/nemotron-stream/t5\endcsname{41.1}
\expandafter\def\csname v@ep/nemotron-stream/t6\endcsname{37.6}
\expandafter\def\csname v@ep/nemotron-stream/t7\endcsname{48.6}
\expandafter\def\csname v@ep/nemotron-stream/t8\endcsname{37.1}
\expandafter\def\csname v@ep/nemotron-stream/t9\endcsname{37.6}
\expandafter\def\csname v@ep/nemotron-stream/within\endcsname{10}
\expandafter\def\csname v@ep/omni-ctc-1b/best\endcsname{7}
\expandafter\def\csname v@ep/omni-ctc-1b/d3-last\endcsname{3.2}
\expandafter\def\csname v@ep/omni-ctc-1b/d3-last-ci\endcsname{3.0 to 3.4}
\expandafter\def\csname v@ep/omni-ctc-1b/t1\endcsname{16.6}
\expandafter\def\csname v@ep/omni-ctc-1b/t10\endcsname{11.7}
\expandafter\def\csname v@ep/omni-ctc-1b/t2\endcsname{15.6}
\expandafter\def\csname v@ep/omni-ctc-1b/t3\endcsname{14.9}
\expandafter\def\csname v@ep/omni-ctc-1b/t4\endcsname{14.8}
\expandafter\def\csname v@ep/omni-ctc-1b/t5\endcsname{14.2}
\expandafter\def\csname v@ep/omni-ctc-1b/t6\endcsname{12.8}
\expandafter\def\csname v@ep/omni-ctc-1b/t7\endcsname{12.0}
\expandafter\def\csname v@ep/omni-ctc-1b/t8\endcsname{11.7}
\expandafter\def\csname v@ep/omni-ctc-1b/t9\endcsname{11.9}
\expandafter\def\csname v@ep/omni-ctc-1b/within\endcsname{7}
\expandafter\def\csname v@ep/parakeet-tdt-v3/best\endcsname{9}
\expandafter\def\csname v@ep/parakeet-tdt-v3/d3-last\endcsname{11.2}
\expandafter\def\csname v@ep/parakeet-tdt-v3/d3-last-ci\endcsname{10.2 to 12.3}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t1\endcsname{35.3}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t10\endcsname{20.6}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t2\endcsname{30.8}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t3\endcsname{31.8}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t4\endcsname{25.6}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t5\endcsname{24.5}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t6\endcsname{22.1}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t7\endcsname{21.4}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t8\endcsname{20.9}
\expandafter\def\csname v@ep/parakeet-tdt-v3/t9\endcsname{21.0}
\expandafter\def\csname v@ep/parakeet-tdt-v3/within\endcsname{8}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/best\endcsname{4}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/d3-last\endcsname{0.4}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/d3-last-ci\endcsname{-0.1 to 0.9}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t1\endcsname{22.3}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t10\endcsname{18.3}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t2\endcsname{19.4}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t3\endcsname{18.7}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t4\endcsname{18.2}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t5\endcsname{18.2}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t6\endcsname{18.1}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t7\endcsname{17.9}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t8\endcsname{18.2}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/t9\endcsname{19.1}
\expandafter\def\csname v@ep/qwen3-asr-0.6b/within\endcsname{3}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/best\endcsname{4}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/d3-last\endcsname{0.1}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/d3-last-ci\endcsname{-0.4 to 0.6}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t1\endcsname{19.4}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t10\endcsname{17.3}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t2\endcsname{18.0}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t3\endcsname{17.3}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t4\endcsname{16.6}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t5\endcsname{16.6}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t6\endcsname{16.8}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t7\endcsname{17.4}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t8\endcsname{16.7}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/t9\endcsname{16.4}
\expandafter\def\csname v@ep/qwen3-asr-1.7b/within\endcsname{3}
\expandafter\def\csname v@ep/three-share\endcsname{99}
\expandafter\def\csname v@ep/voxtral-mini/best\endcsname{3}
\expandafter\def\csname v@ep/voxtral-mini/d3-last\endcsname{0.2}
\expandafter\def\csname v@ep/voxtral-mini/d3-last-ci\endcsname{-0.4 to 0.7}
\expandafter\def\csname v@ep/voxtral-mini/t1\endcsname{18.1}
\expandafter\def\csname v@ep/voxtral-mini/t2\endcsname{16.7}
\expandafter\def\csname v@ep/voxtral-mini/t3\endcsname{16.3}
\expandafter\def\csname v@ep/voxtral-mini/t4\endcsname{16.1}
\expandafter\def\csname v@ep/voxtral-mini/within\endcsname{2}
\expandafter\def\csname v@ep/w2v-bert/best\endcsname{9}
\expandafter\def\csname v@ep/w2v-bert/d3-last\endcsname{3.8}
\expandafter\def\csname v@ep/w2v-bert/d3-last-ci\endcsname{3.4 to 4.1}
\expandafter\def\csname v@ep/w2v-bert/t1\endcsname{26.6}
\expandafter\def\csname v@ep/w2v-bert/t10\endcsname{12.7}
\expandafter\def\csname v@ep/w2v-bert/t2\endcsname{18.7}
\expandafter\def\csname v@ep/w2v-bert/t3\endcsname{16.5}
\expandafter\def\csname v@ep/w2v-bert/t4\endcsname{15.9}
\expandafter\def\csname v@ep/w2v-bert/t5\endcsname{14.6}
\expandafter\def\csname v@ep/w2v-bert/t6\endcsname{13.7}
\expandafter\def\csname v@ep/w2v-bert/t7\endcsname{13.4}
\expandafter\def\csname v@ep/w2v-bert/t8\endcsname{13.3}
\expandafter\def\csname v@ep/w2v-bert/t9\endcsname{12.7}
\expandafter\def\csname v@ep/w2v-bert/within\endcsname{8}
\expandafter\def\csname v@ep/whisper-large-v2/best\endcsname{4}
\expandafter\def\csname v@ep/whisper-large-v2/d3-last\endcsname{0.4}
\expandafter\def\csname v@ep/whisper-large-v2/d3-last-ci\endcsname{0.0 to 0.8}
\expandafter\def\csname v@ep/whisper-large-v2/t1\endcsname{18.5}
\expandafter\def\csname v@ep/whisper-large-v2/t2\endcsname{15.4}
\expandafter\def\csname v@ep/whisper-large-v2/t3\endcsname{14.7}
\expandafter\def\csname v@ep/whisper-large-v2/t4\endcsname{14.2}
\expandafter\def\csname v@ep/whisper-large-v2/t5\endcsname{14.3}
\expandafter\def\csname v@ep/whisper-large-v2/within\endcsname{3}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/best\endcsname{9}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/d3-last\endcsname{0.8}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/d3-last-ci\endcsname{0.4 to 1.2}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t1\endcsname{21.4}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t10\endcsname{14.3}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t2\endcsname{16.5}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t3\endcsname{15.1}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t4\endcsname{14.7}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t5\endcsname{14.2}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t6\endcsname{14.2}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t7\endcsname{14.2}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t8\endcsname{14.1}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/t9\endcsname{14.3}
\expandafter\def\csname v@ep/whisper-large-v3-turbo/within\endcsname{3}
\expandafter\def\csname v@ep/whisper-large-v3/best\endcsname{8}
\expandafter\def\csname v@ep/whisper-large-v3/d3-last\endcsname{0.5}
\expandafter\def\csname v@ep/whisper-large-v3/d3-last-ci\endcsname{0.2 to 0.7}
\expandafter\def\csname v@ep/whisper-large-v3/t1\endcsname{17.1}
\expandafter\def\csname v@ep/whisper-large-v3/t10\endcsname{13.4}
\expandafter\def\csname v@ep/whisper-large-v3/t2\endcsname{14.8}
\expandafter\def\csname v@ep/whisper-large-v3/t3\endcsname{13.8}
\expandafter\def\csname v@ep/whisper-large-v3/t4\endcsname{13.6}
\expandafter\def\csname v@ep/whisper-large-v3/t5\endcsname{13.6}
\expandafter\def\csname v@ep/whisper-large-v3/t6\endcsname{13.2}
\expandafter\def\csname v@ep/whisper-large-v3/t7\endcsname{13.4}
\expandafter\def\csname v@ep/whisper-large-v3/t8\endcsname{13.5}
\expandafter\def\csname v@ep/whisper-large-v3/t9\endcsname{13.5}
\expandafter\def\csname v@ep/whisper-large-v3/within\endcsname{3}
\expandafter\def\csname v@ep/whisper-medium/best\endcsname{10}
\expandafter\def\csname v@ep/whisper-medium/d3-last\endcsname{0.8}
\expandafter\def\csname v@ep/whisper-medium/d3-last-ci\endcsname{0.5 to 1.2}
\expandafter\def\csname v@ep/whisper-medium/t1\endcsname{19.2}
\expandafter\def\csname v@ep/whisper-medium/t10\endcsname{14.8}
\expandafter\def\csname v@ep/whisper-medium/t2\endcsname{16.2}
\expandafter\def\csname v@ep/whisper-medium/t3\endcsname{15.6}
\expandafter\def\csname v@ep/whisper-medium/t4\endcsname{15.3}
\expandafter\def\csname v@ep/whisper-medium/t5\endcsname{15.2}
\expandafter\def\csname v@ep/whisper-medium/t6\endcsname{15.2}
\expandafter\def\csname v@ep/whisper-medium/t7\endcsname{15.5}
\expandafter\def\csname v@ep/whisper-medium/t8\endcsname{15.2}
\expandafter\def\csname v@ep/whisper-medium/t9\endcsname{15.0}
\expandafter\def\csname v@ep/whisper-medium/within\endcsname{3}
\expandafter\def\csname v@ep/whisper-small/best\endcsname{9}
\expandafter\def\csname v@ep/whisper-small/d3-last\endcsname{0.2}
\expandafter\def\csname v@ep/whisper-small/d3-last-ci\endcsname{-0.3 to 0.6}
\expandafter\def\csname v@ep/whisper-small/t1\endcsname{22.2}
\expandafter\def\csname v@ep/whisper-small/t10\endcsname{17.4}
\expandafter\def\csname v@ep/whisper-small/t2\endcsname{18.9}
\expandafter\def\csname v@ep/whisper-small/t3\endcsname{17.6}
\expandafter\def\csname v@ep/whisper-small/t4\endcsname{17.1}
\expandafter\def\csname v@ep/whisper-small/t5\endcsname{16.9}
\expandafter\def\csname v@ep/whisper-small/t6\endcsname{17.3}
\expandafter\def\csname v@ep/whisper-small/t7\endcsname{17.2}
\expandafter\def\csname v@ep/whisper-small/t8\endcsname{16.9}
\expandafter\def\csname v@ep/whisper-small/t9\endcsname{16.9}
\expandafter\def\csname v@ep/whisper-small/within\endcsname{3}
\expandafter\def\csname v@ep/whisper-tiny/best\endcsname{5}
\expandafter\def\csname v@ep/whisper-tiny/d3-last\endcsname{1.6}
\expandafter\def\csname v@ep/whisper-tiny/d3-last-ci\endcsname{0.8 to 2.3}
\expandafter\def\csname v@ep/whisper-tiny/t1\endcsname{34.3}
\expandafter\def\csname v@ep/whisper-tiny/t10\endcsname{26.9}
\expandafter\def\csname v@ep/whisper-tiny/t2\endcsname{30.1}
\expandafter\def\csname v@ep/whisper-tiny/t3\endcsname{28.5}
\expandafter\def\csname v@ep/whisper-tiny/t4\endcsname{27.2}
\expandafter\def\csname v@ep/whisper-tiny/t5\endcsname{25.7}
\expandafter\def\csname v@ep/whisper-tiny/t6\endcsname{26.1}
\expandafter\def\csname v@ep/whisper-tiny/t7\endcsname{26.9}
\expandafter\def\csname v@ep/whisper-tiny/t8\endcsname{26.5}
\expandafter\def\csname v@ep/whisper-tiny/t9\endcsname{27.5}
\expandafter\def\csname v@ep/whisper-tiny/within\endcsname{5}
\expandafter\def\csname v@ep/within-max\endcsname{10}
\expandafter\def\csname v@ep/within-median\endcsname{3}
\expandafter\def\csname v@ep20/mms-1b/after10\endcsname{1.0}
\expandafter\def\csname v@ep20/mms-1b/after20\endcsname{0.0}
\expandafter\def\csname v@ep20/mms-1b/cer\endcsname{10.3}
\expandafter\def\csname v@ep20/mms-1b/d1\endcsname{23.2}
\expandafter\def\csname v@ep20/mms-1b/d10\endcsname{18.5}
\expandafter\def\csname v@ep20/mms-1b/d11\endcsname{18.4}
\expandafter\def\csname v@ep20/mms-1b/d12\endcsname{18.3}
\expandafter\def\csname v@ep20/mms-1b/d13\endcsname{18.0}
\expandafter\def\csname v@ep20/mms-1b/d14\endcsname{18.5}
\expandafter\def\csname v@ep20/mms-1b/d15\endcsname{18.0}
\expandafter\def\csname v@ep20/mms-1b/d16\endcsname{18.0}
\expandafter\def\csname v@ep20/mms-1b/d17\endcsname{17.8}
\expandafter\def\csname v@ep20/mms-1b/d18\endcsname{17.8}
\expandafter\def\csname v@ep20/mms-1b/d19\endcsname{17.9}
\expandafter\def\csname v@ep20/mms-1b/d2\endcsname{22.0}
\expandafter\def\csname v@ep20/mms-1b/d20\endcsname{17.7}
\expandafter\def\csname v@ep20/mms-1b/d3\endcsname{20.9}
\expandafter\def\csname v@ep20/mms-1b/d4\endcsname{20.6}
\expandafter\def\csname v@ep20/mms-1b/d5\endcsname{20.0}
\expandafter\def\csname v@ep20/mms-1b/d6\endcsname{19.1}
\expandafter\def\csname v@ep20/mms-1b/d7\endcsname{19.1}
\expandafter\def\csname v@ep20/mms-1b/d8\endcsname{19.7}
\expandafter\def\csname v@ep20/mms-1b/d9\endcsname{18.8}
\expandafter\def\csname v@ep20/mms-1b/dev\endcsname{17.7}
\expandafter\def\csname v@ep20/mms-1b/dev-after10\endcsname{0.8}
\expandafter\def\csname v@ep20/mms-1b/done\endcsname{1}
\expandafter\def\csname v@ep20/mms-1b/epoch\endcsname{20}
\expandafter\def\csname v@ep20/mms-1b/last\endcsname{10.3}
\expandafter\def\csname v@ep20/mms-1b/last-epoch\endcsname{20}
\expandafter\def\csname v@ep20/mms-1b/t1\endcsname{15.9}
\expandafter\def\csname v@ep20/mms-1b/t10\endcsname{11.3}
\expandafter\def\csname v@ep20/mms-1b/t11\endcsname{11.1}
\expandafter\def\csname v@ep20/mms-1b/t12\endcsname{10.9}
\expandafter\def\csname v@ep20/mms-1b/t13\endcsname{10.7}
\expandafter\def\csname v@ep20/mms-1b/t14\endcsname{11.0}
\expandafter\def\csname v@ep20/mms-1b/t15\endcsname{10.8}
\expandafter\def\csname v@ep20/mms-1b/t16\endcsname{10.7}
\expandafter\def\csname v@ep20/mms-1b/t17\endcsname{10.6}
\expandafter\def\csname v@ep20/mms-1b/t18\endcsname{10.3}
\expandafter\def\csname v@ep20/mms-1b/t19\endcsname{10.5}
\expandafter\def\csname v@ep20/mms-1b/t2\endcsname{14.7}
\expandafter\def\csname v@ep20/mms-1b/t20\endcsname{10.3}
\expandafter\def\csname v@ep20/mms-1b/t3\endcsname{13.6}
\expandafter\def\csname v@ep20/mms-1b/t4\endcsname{13.1}
\expandafter\def\csname v@ep20/mms-1b/t5\endcsname{12.4}
\expandafter\def\csname v@ep20/mms-1b/t6\endcsname{11.9}
\expandafter\def\csname v@ep20/mms-1b/t7\endcsname{11.8}
\expandafter\def\csname v@ep20/mms-1b/t8\endcsname{12.1}
\expandafter\def\csname v@ep20/mms-1b/t9\endcsname{11.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/after10\endcsname{0.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/after20\endcsname{0.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/cer\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/d1\endcsname{24.9}
\expandafter\def\csname v@ep20/omni-ctc-1b/d10\endcsname{19.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/d11\endcsname{19.2}
\expandafter\def\csname v@ep20/omni-ctc-1b/d12\endcsname{19.2}
\expandafter\def\csname v@ep20/omni-ctc-1b/d13\endcsname{19.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/d14\endcsname{18.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d15\endcsname{18.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d16\endcsname{18.9}
\expandafter\def\csname v@ep20/omni-ctc-1b/d17\endcsname{18.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d18\endcsname{18.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d19\endcsname{18.9}
\expandafter\def\csname v@ep20/omni-ctc-1b/d2\endcsname{23.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d20\endcsname{18.7}
\expandafter\def\csname v@ep20/omni-ctc-1b/d3\endcsname{22.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/d4\endcsname{22.4}
\expandafter\def\csname v@ep20/omni-ctc-1b/d5\endcsname{22.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/d6\endcsname{20.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/d7\endcsname{19.5}
\expandafter\def\csname v@ep20/omni-ctc-1b/d8\endcsname{19.4}
\expandafter\def\csname v@ep20/omni-ctc-1b/d9\endcsname{19.7}
\expandafter\def\csname v@ep20/omni-ctc-1b/dev\endcsname{18.7}
\expandafter\def\csname v@ep20/omni-ctc-1b/dev-after10\endcsname{0.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/done\endcsname{1}
\expandafter\def\csname v@ep20/omni-ctc-1b/epoch\endcsname{20}
\expandafter\def\csname v@ep20/omni-ctc-1b/last\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/last-epoch\endcsname{20}
\expandafter\def\csname v@ep20/omni-ctc-1b/t1\endcsname{17.1}
\expandafter\def\csname v@ep20/omni-ctc-1b/t10\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/t11\endcsname{11.8}
\expandafter\def\csname v@ep20/omni-ctc-1b/t12\endcsname{11.7}
\expandafter\def\csname v@ep20/omni-ctc-1b/t13\endcsname{11.5}
\expandafter\def\csname v@ep20/omni-ctc-1b/t14\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/t15\endcsname{11.4}
\expandafter\def\csname v@ep20/omni-ctc-1b/t16\endcsname{11.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/t17\endcsname{11.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/t18\endcsname{11.4}
\expandafter\def\csname v@ep20/omni-ctc-1b/t19\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/t2\endcsname{16.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/t20\endcsname{11.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/t3\endcsname{15.5}
\expandafter\def\csname v@ep20/omni-ctc-1b/t4\endcsname{14.6}
\expandafter\def\csname v@ep20/omni-ctc-1b/t5\endcsname{13.9}
\expandafter\def\csname v@ep20/omni-ctc-1b/t6\endcsname{12.3}
\expandafter\def\csname v@ep20/omni-ctc-1b/t7\endcsname{12.0}
\expandafter\def\csname v@ep20/omni-ctc-1b/t8\endcsname{11.9}
\expandafter\def\csname v@ep20/omni-ctc-1b/t9\endcsname{11.8}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/after10\endcsname{1.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/after20\endcsname{0.0}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/cer\endcsname{20.8}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d1\endcsname{43.9}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d10\endcsname{27.6}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d11\endcsname{27.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d12\endcsname{27.6}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d13\endcsname{27.0}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d14\endcsname{27.5}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d15\endcsname{27.1}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d16\endcsname{26.9}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d17\endcsname{27.1}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d18\endcsname{26.4}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d19\endcsname{27.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d2\endcsname{39.0}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d20\endcsname{26.4}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d3\endcsname{38.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d4\endcsname{32.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d5\endcsname{31.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d6\endcsname{30.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d7\endcsname{29.3}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d8\endcsname{28.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/d9\endcsname{28.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/dev\endcsname{26.4}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/dev-after10\endcsname{1.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/done\endcsname{1}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/epoch\endcsname{20}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/last\endcsname{20.8}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/last-epoch\endcsname{20}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t1\endcsname{39.5}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t10\endcsname{21.9}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t11\endcsname{21.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t12\endcsname{21.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t13\endcsname{21.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t14\endcsname{21.1}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t15\endcsname{20.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t16\endcsname{20.8}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t17\endcsname{20.9}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t18\endcsname{20.5}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t19\endcsname{20.9}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t2\endcsname{33.6}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t20\endcsname{20.8}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t3\endcsname{31.7}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t4\endcsname{26.6}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t5\endcsname{25.3}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t6\endcsname{24.2}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t7\endcsname{23.1}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t8\endcsname{22.5}
\expandafter\def\csname v@ep20/parakeet-tdt-v3/t9\endcsname{22.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/after10\endcsname{0.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/after20\endcsname{-0.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/cer\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d1\endcsname{31.1}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d10\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d11\endcsname{25.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d12\endcsname{25.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d13\endcsname{25.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d14\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d15\endcsname{25.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d16\endcsname{25.5}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d17\endcsname{25.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d18\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d19\endcsname{25.9}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d2\endcsname{27.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d20\endcsname{25.5}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d21\endcsname{26.9}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d22\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d23\endcsname{25.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d24\endcsname{25.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d25\endcsname{26.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d26\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d27\endcsname{25.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d28\endcsname{26.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d29\endcsname{25.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d3\endcsname{25.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d30\endcsname{26.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d4\endcsname{25.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d5\endcsname{26.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d6\endcsname{25.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d7\endcsname{25.1}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d8\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/d9\endcsname{25.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/dev\endcsname{25.1}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/dev-after10\endcsname{0.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/done\endcsname{1}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/epoch\endcsname{7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/last\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/last-epoch\endcsname{30}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t1\endcsname{23.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t10\endcsname{18.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t11\endcsname{18.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t12\endcsname{18.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t13\endcsname{17.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t14\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t15\endcsname{18.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t16\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t17\endcsname{17.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t18\endcsname{18.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t19\endcsname{17.7}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t2\endcsname{20.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t20\endcsname{17.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t21\endcsname{19.5}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t22\endcsname{18.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t23\endcsname{18.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t24\endcsname{18.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t25\endcsname{18.3}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t26\endcsname{17.8}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t27\endcsname{18.0}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t28\endcsname{18.6}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t29\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t3\endcsname{18.4}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t30\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t4\endcsname{18.5}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t5\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t6\endcsname{18.1}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t7\endcsname{18.2}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t8\endcsname{18.5}
\expandafter\def\csname v@ep30/qwen3-asr-0.6b/t9\endcsname{17.9}
\expandafter\def\csname v@ep30/w2v-bert/after10\endcsname{2.2}
\expandafter\def\csname v@ep30/w2v-bert/after20\endcsname{0.3}
\expandafter\def\csname v@ep30/w2v-bert/cer\endcsname{10.6}
\expandafter\def\csname v@ep30/w2v-bert/d1\endcsname{37.2}
\expandafter\def\csname v@ep30/w2v-bert/d10\endcsname{20.1}
\expandafter\def\csname v@ep30/w2v-bert/d11\endcsname{19.9}
\expandafter\def\csname v@ep30/w2v-bert/d12\endcsname{19.4}
\expandafter\def\csname v@ep30/w2v-bert/d13\endcsname{19.7}
\expandafter\def\csname v@ep30/w2v-bert/d14\endcsname{19.5}
\expandafter\def\csname v@ep30/w2v-bert/d15\endcsname{19.0}
\expandafter\def\csname v@ep30/w2v-bert/d16\endcsname{19.2}
\expandafter\def\csname v@ep30/w2v-bert/d17\endcsname{18.8}
\expandafter\def\csname v@ep30/w2v-bert/d18\endcsname{19.2}
\expandafter\def\csname v@ep30/w2v-bert/d19\endcsname{18.7}
\expandafter\def\csname v@ep30/w2v-bert/d2\endcsname{26.7}
\expandafter\def\csname v@ep30/w2v-bert/d20\endcsname{18.8}
\expandafter\def\csname v@ep30/w2v-bert/d21\endcsname{18.4}
\expandafter\def\csname v@ep30/w2v-bert/d22\endcsname{18.6}
\expandafter\def\csname v@ep30/w2v-bert/d23\endcsname{18.3}
\expandafter\def\csname v@ep30/w2v-bert/d24\endcsname{18.6}
\expandafter\def\csname v@ep30/w2v-bert/d25\endcsname{18.2}
\expandafter\def\csname v@ep30/w2v-bert/d26\endcsname{17.7}
\expandafter\def\csname v@ep30/w2v-bert/d27\endcsname{18.0}
\expandafter\def\csname v@ep30/w2v-bert/d28\endcsname{17.9}
\expandafter\def\csname v@ep30/w2v-bert/d29\endcsname{18.0}
\expandafter\def\csname v@ep30/w2v-bert/d3\endcsname{24.9}
\expandafter\def\csname v@ep30/w2v-bert/d30\endcsname{17.6}
\expandafter\def\csname v@ep30/w2v-bert/d4\endcsname{23.4}
\expandafter\def\csname v@ep30/w2v-bert/d5\endcsname{21.8}
\expandafter\def\csname v@ep30/w2v-bert/d6\endcsname{21.5}
\expandafter\def\csname v@ep30/w2v-bert/d7\endcsname{21.2}
\expandafter\def\csname v@ep30/w2v-bert/d8\endcsname{20.6}
\expandafter\def\csname v@ep30/w2v-bert/d9\endcsname{20.4}
\expandafter\def\csname v@ep30/w2v-bert/dev\endcsname{17.6}
\expandafter\def\csname v@ep30/w2v-bert/dev-after10\endcsname{2.5}
\expandafter\def\csname v@ep30/w2v-bert/done\endcsname{1}
\expandafter\def\csname v@ep30/w2v-bert/epoch\endcsname{30}
\expandafter\def\csname v@ep30/w2v-bert/last\endcsname{10.6}
\expandafter\def\csname v@ep30/w2v-bert/last-epoch\endcsname{30}
\expandafter\def\csname v@ep30/w2v-bert/t1\endcsname{31.2}
\expandafter\def\csname v@ep30/w2v-bert/t10\endcsname{12.8}
\expandafter\def\csname v@ep30/w2v-bert/t11\endcsname{12.5}
\expandafter\def\csname v@ep30/w2v-bert/t12\endcsname{11.8}
\expandafter\def\csname v@ep30/w2v-bert/t13\endcsname{11.9}
\expandafter\def\csname v@ep30/w2v-bert/t14\endcsname{11.7}
\expandafter\def\csname v@ep30/w2v-bert/t15\endcsname{11.5}
\expandafter\def\csname v@ep30/w2v-bert/t16\endcsname{11.7}
\expandafter\def\csname v@ep30/w2v-bert/t17\endcsname{11.3}
\expandafter\def\csname v@ep30/w2v-bert/t18\endcsname{11.2}
\expandafter\def\csname v@ep30/w2v-bert/t19\endcsname{11.2}
\expandafter\def\csname v@ep30/w2v-bert/t2\endcsname{19.7}
\expandafter\def\csname v@ep30/w2v-bert/t20\endcsname{11.0}
\expandafter\def\csname v@ep30/w2v-bert/t21\endcsname{10.9}
\expandafter\def\csname v@ep30/w2v-bert/t22\endcsname{11.1}
\expandafter\def\csname v@ep30/w2v-bert/t23\endcsname{11.1}
\expandafter\def\csname v@ep30/w2v-bert/t24\endcsname{11.0}
\expandafter\def\csname v@ep30/w2v-bert/t25\endcsname{11.0}
\expandafter\def\csname v@ep30/w2v-bert/t26\endcsname{10.6}
\expandafter\def\csname v@ep30/w2v-bert/t27\endcsname{10.7}
\expandafter\def\csname v@ep30/w2v-bert/t28\endcsname{10.8}
\expandafter\def\csname v@ep30/w2v-bert/t29\endcsname{10.7}
\expandafter\def\csname v@ep30/w2v-bert/t3\endcsname{17.7}
\expandafter\def\csname v@ep30/w2v-bert/t30\endcsname{10.6}
\expandafter\def\csname v@ep30/w2v-bert/t4\endcsname{16.2}
\expandafter\def\csname v@ep30/w2v-bert/t5\endcsname{14.5}
\expandafter\def\csname v@ep30/w2v-bert/t6\endcsname{14.2}
\expandafter\def\csname v@ep30/w2v-bert/t7\endcsname{13.6}
\expandafter\def\csname v@ep30/w2v-bert/t8\endcsname{13.5}
\expandafter\def\csname v@ep30/w2v-bert/t9\endcsname{12.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/after10\endcsname{0.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/after20\endcsname{0.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/cer\endcsname{13.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d1\endcsname{29.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d10\endcsname{21.9}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d11\endcsname{22.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d12\endcsname{21.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d13\endcsname{21.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d14\endcsname{21.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d15\endcsname{22.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d16\endcsname{21.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d17\endcsname{21.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d18\endcsname{21.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d19\endcsname{21.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d2\endcsname{23.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d20\endcsname{22.0}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d21\endcsname{21.9}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d22\endcsname{21.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d23\endcsname{21.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d24\endcsname{21.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d25\endcsname{21.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d26\endcsname{21.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d27\endcsname{21.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d28\endcsname{21.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d29\endcsname{21.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d3\endcsname{22.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d30\endcsname{21.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d4\endcsname{21.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d5\endcsname{21.9}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d6\endcsname{21.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d7\endcsname{21.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d8\endcsname{21.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/d9\endcsname{21.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/dev\endcsname{21.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/dev-after10\endcsname{0.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/done\endcsname{1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/epoch\endcsname{9}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/last\endcsname{13.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/last-epoch\endcsname{30}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t1\endcsname{21.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t10\endcsname{14.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t11\endcsname{14.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t12\endcsname{14.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t13\endcsname{14.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t14\endcsname{14.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t15\endcsname{14.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t16\endcsname{14.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t17\endcsname{13.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t18\endcsname{13.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t19\endcsname{13.6}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t2\endcsname{16.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t20\endcsname{14.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t21\endcsname{13.9}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t22\endcsname{14.0}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t23\endcsname{13.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t24\endcsname{14.0}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t25\endcsname{14.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t26\endcsname{14.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t27\endcsname{14.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t28\endcsname{14.2}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t29\endcsname{14.5}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t3\endcsname{15.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t30\endcsname{13.7}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t4\endcsname{14.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t5\endcsname{14.8}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t6\endcsname{14.3}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t7\endcsname{14.1}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t8\endcsname{14.4}
\expandafter\def\csname v@ep30/whisper-large-v3-turbo/t9\endcsname{13.8}
\expandafter\def\csname v@ep30/whisper-small/after10\endcsname{0.2}
\expandafter\def\csname v@ep30/whisper-small/after20\endcsname{0.6}
\expandafter\def\csname v@ep30/whisper-small/cer\endcsname{16.9}
\expandafter\def\csname v@ep30/whisper-small/d1\endcsname{29.4}
\expandafter\def\csname v@ep30/whisper-small/d10\endcsname{24.9}
\expandafter\def\csname v@ep30/whisper-small/d11\endcsname{24.6}
\expandafter\def\csname v@ep30/whisper-small/d12\endcsname{24.7}
\expandafter\def\csname v@ep30/whisper-small/d13\endcsname{24.3}
\expandafter\def\csname v@ep30/whisper-small/d14\endcsname{24.5}
\expandafter\def\csname v@ep30/whisper-small/d15\endcsname{24.7}
\expandafter\def\csname v@ep30/whisper-small/d16\endcsname{25.1}
\expandafter\def\csname v@ep30/whisper-small/d17\endcsname{24.8}
\expandafter\def\csname v@ep30/whisper-small/d18\endcsname{24.8}
\expandafter\def\csname v@ep30/whisper-small/d19\endcsname{24.8}
\expandafter\def\csname v@ep30/whisper-small/d2\endcsname{26.5}
\expandafter\def\csname v@ep30/whisper-small/d20\endcsname{25.4}
\expandafter\def\csname v@ep30/whisper-small/d21\endcsname{24.9}
\expandafter\def\csname v@ep30/whisper-small/d22\endcsname{24.5}
\expandafter\def\csname v@ep30/whisper-small/d23\endcsname{24.6}
\expandafter\def\csname v@ep30/whisper-small/d24\endcsname{24.8}
\expandafter\def\csname v@ep30/whisper-small/d25\endcsname{25.6}
\expandafter\def\csname v@ep30/whisper-small/d26\endcsname{25.2}
\expandafter\def\csname v@ep30/whisper-small/d27\endcsname{24.7}
\expandafter\def\csname v@ep30/whisper-small/d28\endcsname{25.2}
\expandafter\def\csname v@ep30/whisper-small/d29\endcsname{24.9}
\expandafter\def\csname v@ep30/whisper-small/d3\endcsname{25.1}
\expandafter\def\csname v@ep30/whisper-small/d30\endcsname{24.8}
\expandafter\def\csname v@ep30/whisper-small/d4\endcsname{24.5}
\expandafter\def\csname v@ep30/whisper-small/d5\endcsname{24.9}
\expandafter\def\csname v@ep30/whisper-small/d6\endcsname{25.0}
\expandafter\def\csname v@ep30/whisper-small/d7\endcsname{24.6}
\expandafter\def\csname v@ep30/whisper-small/d8\endcsname{24.9}
\expandafter\def\csname v@ep30/whisper-small/d9\endcsname{25.1}
\expandafter\def\csname v@ep30/whisper-small/dev\endcsname{24.3}
\expandafter\def\csname v@ep30/whisper-small/dev-after10\endcsname{0.5}
\expandafter\def\csname v@ep30/whisper-small/done\endcsname{1}
\expandafter\def\csname v@ep30/whisper-small/epoch\endcsname{13}
\expandafter\def\csname v@ep30/whisper-small/last\endcsname{17.7}
\expandafter\def\csname v@ep30/whisper-small/last-epoch\endcsname{30}
\expandafter\def\csname v@ep30/whisper-small/t1\endcsname{21.9}
\expandafter\def\csname v@ep30/whisper-small/t10\endcsname{17.1}
\expandafter\def\csname v@ep30/whisper-small/t11\endcsname{17.2}
\expandafter\def\csname v@ep30/whisper-small/t12\endcsname{17.3}
\expandafter\def\csname v@ep30/whisper-small/t13\endcsname{16.9}
\expandafter\def\csname v@ep30/whisper-small/t14\endcsname{16.9}
\expandafter\def\csname v@ep30/whisper-small/t15\endcsname{17.1}
\expandafter\def\csname v@ep30/whisper-small/t16\endcsname{17.0}
\expandafter\def\csname v@ep30/whisper-small/t17\endcsname{16.9}
\expandafter\def\csname v@ep30/whisper-small/t18\endcsname{17.1}
\expandafter\def\csname v@ep30/whisper-small/t19\endcsname{17.3}
\expandafter\def\csname v@ep30/whisper-small/t2\endcsname{18.9}
\expandafter\def\csname v@ep30/whisper-small/t20\endcsname{17.5}
\expandafter\def\csname v@ep30/whisper-small/t21\endcsname{16.7}
\expandafter\def\csname v@ep30/whisper-small/t22\endcsname{17.3}
\expandafter\def\csname v@ep30/whisper-small/t23\endcsname{16.9}
\expandafter\def\csname v@ep30/whisper-small/t24\endcsname{17.5}
\expandafter\def\csname v@ep30/whisper-small/t25\endcsname{17.5}
\expandafter\def\csname v@ep30/whisper-small/t26\endcsname{17.5}
\expandafter\def\csname v@ep30/whisper-small/t27\endcsname{17.2}
\expandafter\def\csname v@ep30/whisper-small/t28\endcsname{17.4}
\expandafter\def\csname v@ep30/whisper-small/t29\endcsname{17.2}
\expandafter\def\csname v@ep30/whisper-small/t3\endcsname{17.4}
\expandafter\def\csname v@ep30/whisper-small/t30\endcsname{17.7}
\expandafter\def\csname v@ep30/whisper-small/t4\endcsname{17.2}
\expandafter\def\csname v@ep30/whisper-small/t5\endcsname{17.0}
\expandafter\def\csname v@ep30/whisper-small/t6\endcsname{17.0}
\expandafter\def\csname v@ep30/whisper-small/t7\endcsname{17.2}
\expandafter\def\csname v@ep30/whisper-small/t8\endcsname{17.0}
\expandafter\def\csname v@ep30/whisper-small/t9\endcsname{17.2}
\expandafter\def\csname v@fk/all-worse-n\endcsname{20}
\expandafter\def\csname v@fk/better-n\endcsname{0}
\expandafter\def\csname v@fk/better-names\endcsname{none}
\expandafter\def\csname v@fk/cohere-transcribe/after\endcsname{6.5}
\expandafter\def\csname v@fk/cohere-transcribe/before\endcsname{2.1}
\expandafter\def\csname v@fk/cohere-transcribe/deu_Latn/after\endcsname{4.7}
\expandafter\def\csname v@fk/cohere-transcribe/deu_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/cohere-transcribe/eng_Latn/after\endcsname{3.3}
\expandafter\def\csname v@fk/cohere-transcribe/eng_Latn/before\endcsname{2.6}
\expandafter\def\csname v@fk/cohere-transcribe/fra_Latn/after\endcsname{11.9}
\expandafter\def\csname v@fk/cohere-transcribe/fra_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/cohere-transcribe/loss\endcsname{4.4}
\expandafter\def\csname v@fk/cohere-transcribe/loss-ci\endcsname{4.0 to 4.8}
\expandafter\def\csname v@fk/cohere-transcribe/spa_Latn/after\endcsname{5.9}
\expandafter\def\csname v@fk/cohere-transcribe/spa_Latn/before\endcsname{1.8}
\expandafter\def\csname v@fk/gemma4-12b/after\endcsname{8.9}
\expandafter\def\csname v@fk/gemma4-12b/before\endcsname{2.2}
\expandafter\def\csname v@fk/gemma4-12b/deu_Latn/after\endcsname{6.2}
\expandafter\def\csname v@fk/gemma4-12b/deu_Latn/before\endcsname{1.6}
\expandafter\def\csname v@fk/gemma4-12b/eng_Latn/after\endcsname{13.3}
\expandafter\def\csname v@fk/gemma4-12b/eng_Latn/before\endcsname{2.9}
\expandafter\def\csname v@fk/gemma4-12b/fra_Latn/after\endcsname{13.3}
\expandafter\def\csname v@fk/gemma4-12b/fra_Latn/before\endcsname{2.9}
\expandafter\def\csname v@fk/gemma4-12b/loss\endcsname{6.7}
\expandafter\def\csname v@fk/gemma4-12b/loss-ci\endcsname{6.0 to 7.4}
\expandafter\def\csname v@fk/gemma4-12b/spa_Latn/after\endcsname{2.7}
\expandafter\def\csname v@fk/gemma4-12b/spa_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/gemma4-e2b/after\endcsname{13.4}
\expandafter\def\csname v@fk/gemma4-e2b/before\endcsname{2.8}
\expandafter\def\csname v@fk/gemma4-e2b/deu_Latn/after\endcsname{13.8}
\expandafter\def\csname v@fk/gemma4-e2b/deu_Latn/before\endcsname{2.6}
\expandafter\def\csname v@fk/gemma4-e2b/eng_Latn/after\endcsname{17.3}
\expandafter\def\csname v@fk/gemma4-e2b/eng_Latn/before\endcsname{3.5}
\expandafter\def\csname v@fk/gemma4-e2b/fra_Latn/after\endcsname{15.9}
\expandafter\def\csname v@fk/gemma4-e2b/fra_Latn/before\endcsname{3.8}
\expandafter\def\csname v@fk/gemma4-e2b/loss\endcsname{10.6}
\expandafter\def\csname v@fk/gemma4-e2b/loss-ci\endcsname{9.7 to 11.4}
\expandafter\def\csname v@fk/gemma4-e2b/spa_Latn/after\endcsname{6.7}
\expandafter\def\csname v@fk/gemma4-e2b/spa_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/gemma4-e4b/after\endcsname{3.5}
\expandafter\def\csname v@fk/gemma4-e4b/before\endcsname{2.3}
\expandafter\def\csname v@fk/gemma4-e4b/deu_Latn/after\endcsname{3.0}
\expandafter\def\csname v@fk/gemma4-e4b/deu_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/gemma4-e4b/eng_Latn/after\endcsname{4.0}
\expandafter\def\csname v@fk/gemma4-e4b/eng_Latn/before\endcsname{2.9}
\expandafter\def\csname v@fk/gemma4-e4b/fra_Latn/after\endcsname{5.3}
\expandafter\def\csname v@fk/gemma4-e4b/fra_Latn/before\endcsname{2.9}
\expandafter\def\csname v@fk/gemma4-e4b/loss\endcsname{1.2}
\expandafter\def\csname v@fk/gemma4-e4b/loss-ci\endcsname{0.9 to 1.5}
\expandafter\def\csname v@fk/gemma4-e4b/spa_Latn/after\endcsname{1.7}
\expandafter\def\csname v@fk/gemma4-e4b/spa_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/granite-2b/after\endcsname{9.4}
\expandafter\def\csname v@fk/granite-2b/before\endcsname{6.8}
\expandafter\def\csname v@fk/granite-2b/deu_Latn/after\endcsname{9.6}
\expandafter\def\csname v@fk/granite-2b/deu_Latn/before\endcsname{8.7}
\expandafter\def\csname v@fk/granite-2b/eng_Latn/after\endcsname{5.2}
\expandafter\def\csname v@fk/granite-2b/eng_Latn/before\endcsname{4.7}
\expandafter\def\csname v@fk/granite-2b/fra_Latn/after\endcsname{16.3}
\expandafter\def\csname v@fk/granite-2b/fra_Latn/before\endcsname{7.8}
\expandafter\def\csname v@fk/granite-2b/loss\endcsname{2.6}
\expandafter\def\csname v@fk/granite-2b/loss-ci\endcsname{1.9 to 3.4}
\expandafter\def\csname v@fk/granite-2b/spa_Latn/after\endcsname{6.6}
\expandafter\def\csname v@fk/granite-2b/spa_Latn/before\endcsname{6.0}
\expandafter\def\csname v@fk/least-worse/loss\endcsname{0.4}
\expandafter\def\csname v@fk/least-worse/loss-ci\endcsname{-0.1 to 1.0}
\expandafter\def\csname v@fk/least-worse/name\endcsname{Nemotron 3.5 Transcribe 30B}
\expandafter\def\csname v@fk/least/loss\endcsname{0.4}
\expandafter\def\csname v@fk/least/name\endcsname{Nemotron 3.5 Transcribe 30B}
\expandafter\def\csname v@fk/lfm3-audio/after\endcsname{4.0}
\expandafter\def\csname v@fk/lfm3-audio/before\endcsname{2.0}
\expandafter\def\csname v@fk/lfm3-audio/deu_Latn/after\endcsname{4.8}
\expandafter\def\csname v@fk/lfm3-audio/deu_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/lfm3-audio/eng_Latn/after\endcsname{3.4}
\expandafter\def\csname v@fk/lfm3-audio/eng_Latn/before\endcsname{2.3}
\expandafter\def\csname v@fk/lfm3-audio/fra_Latn/after\endcsname{5.6}
\expandafter\def\csname v@fk/lfm3-audio/fra_Latn/before\endcsname{2.6}
\expandafter\def\csname v@fk/lfm3-audio/loss\endcsname{2.0}
\expandafter\def\csname v@fk/lfm3-audio/loss-ci\endcsname{1.8 to 2.3}
\expandafter\def\csname v@fk/lfm3-audio/spa_Latn/after\endcsname{2.2}
\expandafter\def\csname v@fk/lfm3-audio/spa_Latn/before\endcsname{1.3}
\expandafter\def\csname v@fk/lora/less-n\endcsname{2}
\expandafter\def\csname v@fk/lora/more-names\endcsname{Whisper large-v3}
\expandafter\def\csname v@fk/lora/n\endcsname{3}
\expandafter\def\csname v@fk/lora/names\endcsname{Whisper large-v3, Qwen3-ASR 0.6B and MMS 1B}
\expandafter\def\csname v@fk/loss-max\endcsname{46.4}
\expandafter\def\csname v@fk/loss-median\endcsname{5.7}
\expandafter\def\csname v@fk/mms-1b/after\endcsname{5.7}
\expandafter\def\csname v@fk/mms-1b/before\endcsname{3.2}
\expandafter\def\csname v@fk/mms-1b/deu_Latn/after\endcsname{5.1}
\expandafter\def\csname v@fk/mms-1b/deu_Latn/before\endcsname{2.5}
\expandafter\def\csname v@fk/mms-1b/eng_Latn/after\endcsname{4.7}
\expandafter\def\csname v@fk/mms-1b/eng_Latn/before\endcsname{4.5}
\expandafter\def\csname v@fk/mms-1b/fra_Latn/after\endcsname{7.5}
\expandafter\def\csname v@fk/mms-1b/fra_Latn/before\endcsname{4.0}
\expandafter\def\csname v@fk/mms-1b/lora/after\endcsname{5.0}
\expandafter\def\csname v@fk/mms-1b/lora/before\endcsname{3.2}
\expandafter\def\csname v@fk/mms-1b/lora/deu_Latn/after\endcsname{4.7}
\expandafter\def\csname v@fk/mms-1b/lora/deu_Latn/before\endcsname{2.5}
\expandafter\def\csname v@fk/mms-1b/lora/eng_Latn/after\endcsname{4.4}
\expandafter\def\csname v@fk/mms-1b/lora/eng_Latn/before\endcsname{4.5}
\expandafter\def\csname v@fk/mms-1b/lora/fra_Latn/after\endcsname{6.8}
\expandafter\def\csname v@fk/mms-1b/lora/fra_Latn/before\endcsname{4.0}
\expandafter\def\csname v@fk/mms-1b/lora/loss\endcsname{1.8}
\expandafter\def\csname v@fk/mms-1b/lora/loss-ci\endcsname{1.6 to 2.0}
\expandafter\def\csname v@fk/mms-1b/lora/spa_Latn/after\endcsname{4.0}
\expandafter\def\csname v@fk/mms-1b/lora/spa_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/mms-1b/loss\endcsname{2.5}
\expandafter\def\csname v@fk/mms-1b/loss-ci\endcsname{2.3 to 2.7}
\expandafter\def\csname v@fk/mms-1b/mms/after\endcsname{3.8}
\expandafter\def\csname v@fk/mms-1b/mms/before\endcsname{3.2}
\expandafter\def\csname v@fk/mms-1b/mms/deu_Latn/after\endcsname{3.3}
\expandafter\def\csname v@fk/mms-1b/mms/deu_Latn/before\endcsname{2.5}
\expandafter\def\csname v@fk/mms-1b/mms/eng_Latn/after\endcsname{4.1}
\expandafter\def\csname v@fk/mms-1b/mms/eng_Latn/before\endcsname{4.5}
\expandafter\def\csname v@fk/mms-1b/mms/fra_Latn/after\endcsname{5.4}
\expandafter\def\csname v@fk/mms-1b/mms/fra_Latn/before\endcsname{4.0}
\expandafter\def\csname v@fk/mms-1b/mms/loss\endcsname{0.6}
\expandafter\def\csname v@fk/mms-1b/mms/loss-ci\endcsname{0.4 to 0.7}
\expandafter\def\csname v@fk/mms-1b/mms/spa_Latn/after\endcsname{2.2}
\expandafter\def\csname v@fk/mms-1b/mms/spa_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/mms-1b/spa_Latn/after\endcsname{5.7}
\expandafter\def\csname v@fk/mms-1b/spa_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/n\endcsname{20}
\expandafter\def\csname v@fk/nemotron-30b-first/after\endcsname{1.8}
\expandafter\def\csname v@fk/nemotron-30b-first/before\endcsname{3.7}
\expandafter\def\csname v@fk/nemotron-30b-first/loss-ci\endcsname{-2.5 to -1.4}
\expandafter\def\csname v@fk/nemotron-30b/after\endcsname{4.2}
\expandafter\def\csname v@fk/nemotron-30b/before\endcsname{3.7}
\expandafter\def\csname v@fk/nemotron-30b/deu_Latn/after\endcsname{4.3}
\expandafter\def\csname v@fk/nemotron-30b/deu_Latn/before\endcsname{3.8}
\expandafter\def\csname v@fk/nemotron-30b/eng_Latn/after\endcsname{2.9}
\expandafter\def\csname v@fk/nemotron-30b/eng_Latn/before\endcsname{4.2}
\expandafter\def\csname v@fk/nemotron-30b/fra_Latn/after\endcsname{6.2}
\expandafter\def\csname v@fk/nemotron-30b/fra_Latn/before\endcsname{4.3}
\expandafter\def\csname v@fk/nemotron-30b/loss\endcsname{0.4}
\expandafter\def\csname v@fk/nemotron-30b/loss-ci\endcsname{-0.1 to 1.0}
\expandafter\def\csname v@fk/nemotron-30b/spa_Latn/after\endcsname{3.2}
\expandafter\def\csname v@fk/nemotron-30b/spa_Latn/before\endcsname{2.7}
\expandafter\def\csname v@fk/nemotron-stream/after\endcsname{51.4}
\expandafter\def\csname v@fk/nemotron-stream/before\endcsname{5.1}
\expandafter\def\csname v@fk/nemotron-stream/deu_Latn/after\endcsname{46.8}
\expandafter\def\csname v@fk/nemotron-stream/deu_Latn/before\endcsname{5.3}
\expandafter\def\csname v@fk/nemotron-stream/eng_Latn/after\endcsname{52.3}
\expandafter\def\csname v@fk/nemotron-stream/eng_Latn/before\endcsname{5.9}
\expandafter\def\csname v@fk/nemotron-stream/fra_Latn/after\endcsname{59.8}
\expandafter\def\csname v@fk/nemotron-stream/fra_Latn/before\endcsname{6.0}
\expandafter\def\csname v@fk/nemotron-stream/loss\endcsname{46.4}
\expandafter\def\csname v@fk/nemotron-stream/loss-ci\endcsname{45.5 to 47.2}
\expandafter\def\csname v@fk/nemotron-stream/spa_Latn/after\endcsname{46.8}
\expandafter\def\csname v@fk/nemotron-stream/spa_Latn/before\endcsname{3.2}
\expandafter\def\csname v@fk/omni-ctc-1b/after\endcsname{11.9}
\expandafter\def\csname v@fk/omni-ctc-1b/before\endcsname{3.4}
\expandafter\def\csname v@fk/omni-ctc-1b/deu_Latn/after\endcsname{6.3}
\expandafter\def\csname v@fk/omni-ctc-1b/deu_Latn/before\endcsname{2.6}
\expandafter\def\csname v@fk/omni-ctc-1b/eng_Latn/after\endcsname{10.4}
\expandafter\def\csname v@fk/omni-ctc-1b/eng_Latn/before\endcsname{4.6}
\expandafter\def\csname v@fk/omni-ctc-1b/fra_Latn/after\endcsname{20.7}
\expandafter\def\csname v@fk/omni-ctc-1b/fra_Latn/before\endcsname{4.1}
\expandafter\def\csname v@fk/omni-ctc-1b/loss\endcsname{8.6}
\expandafter\def\csname v@fk/omni-ctc-1b/loss-ci\endcsname{8.2 to 8.9}
\expandafter\def\csname v@fk/omni-ctc-1b/spa_Latn/after\endcsname{10.4}
\expandafter\def\csname v@fk/omni-ctc-1b/spa_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/parakeet-tdt-v3/after\endcsname{13.2}
\expandafter\def\csname v@fk/parakeet-tdt-v3/before\endcsname{1.9}
\expandafter\def\csname v@fk/parakeet-tdt-v3/deu_Latn/after\endcsname{8.6}
\expandafter\def\csname v@fk/parakeet-tdt-v3/deu_Latn/before\endcsname{1.5}
\expandafter\def\csname v@fk/parakeet-tdt-v3/eng_Latn/after\endcsname{9.7}
\expandafter\def\csname v@fk/parakeet-tdt-v3/eng_Latn/before\endcsname{2.4}
\expandafter\def\csname v@fk/parakeet-tdt-v3/fra_Latn/after\endcsname{26.8}
\expandafter\def\csname v@fk/parakeet-tdt-v3/fra_Latn/before\endcsname{2.2}
\expandafter\def\csname v@fk/parakeet-tdt-v3/loss\endcsname{11.3}
\expandafter\def\csname v@fk/parakeet-tdt-v3/loss-ci\endcsname{10.8 to 11.9}
\expandafter\def\csname v@fk/parakeet-tdt-v3/spa_Latn/after\endcsname{7.6}
\expandafter\def\csname v@fk/parakeet-tdt-v3/spa_Latn/before\endcsname{1.3}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/after\endcsname{12.2}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/before\endcsname{2.8}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/deu_Latn/after\endcsname{11.3}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/deu_Latn/before\endcsname{2.8}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/eng_Latn/after\endcsname{7.1}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/eng_Latn/before\endcsname{2.4}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/fra_Latn/after\endcsname{20.2}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/fra_Latn/before\endcsname{4.2}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/after\endcsname{7.1}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/before\endcsname{2.8}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/deu_Latn/after\endcsname{6.5}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/deu_Latn/before\endcsname{2.8}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/eng_Latn/after\endcsname{3.5}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/eng_Latn/before\endcsname{2.4}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/fra_Latn/after\endcsname{12.6}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/fra_Latn/before\endcsname{4.2}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/loss\endcsname{4.3}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/loss-ci\endcsname{4.0 to 4.7}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/spa_Latn/after\endcsname{5.8}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/lora/spa_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/loss\endcsname{9.4}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/loss-ci\endcsname{8.8 to 10.1}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/spa_Latn/after\endcsname{10.1}
\expandafter\def\csname v@fk/qwen3-asr-0.6b/spa_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/after\endcsname{5.2}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/before\endcsname{1.5}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/deu_Latn/after\endcsname{4.8}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/deu_Latn/before\endcsname{1.2}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/eng_Latn/after\endcsname{3.7}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/eng_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/fra_Latn/after\endcsname{8.6}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/fra_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/loss\endcsname{3.7}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/loss-ci\endcsname{3.3 to 4.2}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/spa_Latn/after\endcsname{3.8}
\expandafter\def\csname v@fk/qwen3-asr-1.7b/spa_Latn/before\endcsname{1.0}
\expandafter\def\csname v@fk/voxtral-mini/after\endcsname{6.3}
\expandafter\def\csname v@fk/voxtral-mini/before\endcsname{1.6}
\expandafter\def\csname v@fk/voxtral-mini/deu_Latn/after\endcsname{7.0}
\expandafter\def\csname v@fk/voxtral-mini/deu_Latn/before\endcsname{1.3}
\expandafter\def\csname v@fk/voxtral-mini/eng_Latn/after\endcsname{4.6}
\expandafter\def\csname v@fk/voxtral-mini/eng_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/voxtral-mini/fra_Latn/after\endcsname{7.6}
\expandafter\def\csname v@fk/voxtral-mini/fra_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/voxtral-mini/loss\endcsname{4.7}
\expandafter\def\csname v@fk/voxtral-mini/loss-ci\endcsname{4.2 to 5.3}
\expandafter\def\csname v@fk/voxtral-mini/spa_Latn/after\endcsname{5.9}
\expandafter\def\csname v@fk/voxtral-mini/spa_Latn/before\endcsname{1.1}
\expandafter\def\csname v@fk/whisper-large-v2/after\endcsname{3.4}
\expandafter\def\csname v@fk/whisper-large-v2/before\endcsname{1.8}
\expandafter\def\csname v@fk/whisper-large-v2/deu_Latn/after\endcsname{3.0}
\expandafter\def\csname v@fk/whisper-large-v2/deu_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/whisper-large-v2/eng_Latn/after\endcsname{2.8}
\expandafter\def\csname v@fk/whisper-large-v2/eng_Latn/before\endcsname{2.2}
\expandafter\def\csname v@fk/whisper-large-v2/fra_Latn/after\endcsname{5.9}
\expandafter\def\csname v@fk/whisper-large-v2/fra_Latn/before\endcsname{2.4}
\expandafter\def\csname v@fk/whisper-large-v2/loss\endcsname{1.7}
\expandafter\def\csname v@fk/whisper-large-v2/loss-ci\endcsname{1.5 to 1.9}
\expandafter\def\csname v@fk/whisper-large-v2/spa_Latn/after\endcsname{2.1}
\expandafter\def\csname v@fk/whisper-large-v2/spa_Latn/before\endcsname{1.0}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/after\endcsname{9.4}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/before\endcsname{1.8}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/deu_Latn/after\endcsname{6.3}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/deu_Latn/before\endcsname{1.8}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/eng_Latn/after\endcsname{8.3}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/eng_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/fra_Latn/after\endcsname{18.3}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/fra_Latn/before\endcsname{2.1}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/loss\endcsname{7.6}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/loss-ci\endcsname{7.2 to 8.0}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/spa_Latn/after\endcsname{4.7}
\expandafter\def\csname v@fk/whisper-large-v3-turbo/spa_Latn/before\endcsname{1.1}
\expandafter\def\csname v@fk/whisper-large-v3/after\endcsname{5.1}
\expandafter\def\csname v@fk/whisper-large-v3/before\endcsname{1.7}
\expandafter\def\csname v@fk/whisper-large-v3/deu_Latn/after\endcsname{3.5}
\expandafter\def\csname v@fk/whisper-large-v3/deu_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/whisper-large-v3/eng_Latn/after\endcsname{7.1}
\expandafter\def\csname v@fk/whisper-large-v3/eng_Latn/before\endcsname{2.2}
\expandafter\def\csname v@fk/whisper-large-v3/fra_Latn/after\endcsname{6.6}
\expandafter\def\csname v@fk/whisper-large-v3/fra_Latn/before\endcsname{2.0}
\expandafter\def\csname v@fk/whisper-large-v3/lora/after\endcsname{6.0}
\expandafter\def\csname v@fk/whisper-large-v3/lora/before\endcsname{1.7}
\expandafter\def\csname v@fk/whisper-large-v3/lora/deu_Latn/after\endcsname{5.8}
\expandafter\def\csname v@fk/whisper-large-v3/lora/deu_Latn/before\endcsname{1.4}
\expandafter\def\csname v@fk/whisper-large-v3/lora/eng_Latn/after\endcsname{3.9}
\expandafter\def\csname v@fk/whisper-large-v3/lora/eng_Latn/before\endcsname{2.2}
\expandafter\def\csname v@fk/whisper-large-v3/lora/fra_Latn/after\endcsname{11.1}
\expandafter\def\csname v@fk/whisper-large-v3/lora/fra_Latn/before\endcsname{2.0}
\expandafter\def\csname v@fk/whisper-large-v3/lora/loss\endcsname{4.3}
\expandafter\def\csname v@fk/whisper-large-v3/lora/loss-ci\endcsname{3.9 to 4.6}
\expandafter\def\csname v@fk/whisper-large-v3/lora/spa_Latn/after\endcsname{3.0}
\expandafter\def\csname v@fk/whisper-large-v3/lora/spa_Latn/before\endcsname{1.1}
\expandafter\def\csname v@fk/whisper-large-v3/loss\endcsname{3.4}
\expandafter\def\csname v@fk/whisper-large-v3/loss-ci\endcsname{2.9 to 3.9}
\expandafter\def\csname v@fk/whisper-large-v3/spa_Latn/after\endcsname{3.0}
\expandafter\def\csname v@fk/whisper-large-v3/spa_Latn/before\endcsname{1.1}
\expandafter\def\csname v@fk/whisper-medium/after\endcsname{10.4}
\expandafter\def\csname v@fk/whisper-medium/before\endcsname{2.2}
\expandafter\def\csname v@fk/whisper-medium/deu_Latn/after\endcsname{7.2}
\expandafter\def\csname v@fk/whisper-medium/deu_Latn/before\endcsname{1.9}
\expandafter\def\csname v@fk/whisper-medium/eng_Latn/after\endcsname{13.0}
\expandafter\def\csname v@fk/whisper-medium/eng_Latn/before\endcsname{2.3}
\expandafter\def\csname v@fk/whisper-medium/fra_Latn/after\endcsname{14.6}
\expandafter\def\csname v@fk/whisper-medium/fra_Latn/before\endcsname{3.4}
\expandafter\def\csname v@fk/whisper-medium/loss\endcsname{8.2}
\expandafter\def\csname v@fk/whisper-medium/loss-ci\endcsname{7.4 to 9.2}
\expandafter\def\csname v@fk/whisper-medium/spa_Latn/after\endcsname{6.9}
\expandafter\def\csname v@fk/whisper-medium/spa_Latn/before\endcsname{1.1}
\expandafter\def\csname v@fk/whisper-small/after\endcsname{18.8}
\expandafter\def\csname v@fk/whisper-small/before\endcsname{3.2}
\expandafter\def\csname v@fk/whisper-small/deu_Latn/after\endcsname{14.9}
\expandafter\def\csname v@fk/whisper-small/deu_Latn/before\endcsname{3.0}
\expandafter\def\csname v@fk/whisper-small/eng_Latn/after\endcsname{21.2}
\expandafter\def\csname v@fk/whisper-small/eng_Latn/before\endcsname{2.9}
\expandafter\def\csname v@fk/whisper-small/fra_Latn/after\endcsname{27.5}
\expandafter\def\csname v@fk/whisper-small/fra_Latn/before\endcsname{5.3}
\expandafter\def\csname v@fk/whisper-small/loss\endcsname{15.6}
\expandafter\def\csname v@fk/whisper-small/loss-ci\endcsname{14.9 to 16.3}
\expandafter\def\csname v@fk/whisper-small/spa_Latn/after\endcsname{11.8}
\expandafter\def\csname v@fk/whisper-small/spa_Latn/before\endcsname{1.7}
\expandafter\def\csname v@fk/whisper-tiny/after\endcsname{50.5}
\expandafter\def\csname v@fk/whisper-tiny/before\endcsname{10.4}
\expandafter\def\csname v@fk/whisper-tiny/deu_Latn/after\endcsname{45.9}
\expandafter\def\csname v@fk/whisper-tiny/deu_Latn/before\endcsname{9.6}
\expandafter\def\csname v@fk/whisper-tiny/eng_Latn/after\endcsname{57.5}
\expandafter\def\csname v@fk/whisper-tiny/eng_Latn/before\endcsname{6.6}
\expandafter\def\csname v@fk/whisper-tiny/fra_Latn/after\endcsname{60.4}
\expandafter\def\csname v@fk/whisper-tiny/fra_Latn/before\endcsname{19.7}
\expandafter\def\csname v@fk/whisper-tiny/loss\endcsname{40.1}
\expandafter\def\csname v@fk/whisper-tiny/loss-ci\endcsname{39.2 to 40.9}
\expandafter\def\csname v@fk/whisper-tiny/spa_Latn/after\endcsname{38.0}
\expandafter\def\csname v@fk/whisper-tiny/spa_Latn/before\endcsname{5.7}
\expandafter\def\csname v@fk/worse-n\endcsname{20}
\expandafter\def\csname v@fk/worst/name\endcsname{Nemotron 3.5 streaming 0.6B}
\expandafter\def\csname v@ft/below20\endcsname{17}
\expandafter\def\csname v@ft/best-wer/cer\endcsname{11.0}
\expandafter\def\csname v@ft/best-wer/name\endcsname{MMS 1B}
\expandafter\def\csname v@ft/best-wer/wer\endcsname{39.3}
\expandafter\def\csname v@ft/best/cer\endcsname{11.0}
\expandafter\def\csname v@ft/best/median\endcsname{8.7}
\expandafter\def\csname v@ft/best/name\endcsname{MMS 1B}
\expandafter\def\csname v@ft/best/right\endcsname{89}
\expandafter\def\csname v@ft/best/wer\endcsname{39.3}
\expandafter\def\csname v@ft/best/worst-lang\endcsname{38.5}
\expandafter\def\csname v@ft/cohere-transcribe/before\endcsname{68.0}
\expandafter\def\csname v@ft/cohere-transcribe/cer\endcsname{15.6}
\expandafter\def\csname v@ft/cohere-transcribe/ci\endcsname{15.0--16.3}
\expandafter\def\csname v@ft/cohere-transcribe/clips-s\endcsname{35}
\expandafter\def\csname v@ft/cohere-transcribe/dev\endcsname{22.4}
\expandafter\def\csname v@ft/cohere-transcribe/epoch\endcsname{10}
\expandafter\def\csname v@ft/cohere-transcribe/gain\endcsname{52.4}
\expandafter\def\csname v@ft/cohere-transcribe/gain-ci\endcsname{51.3--53.6}
\expandafter\def\csname v@ft/cohere-transcribe/h-epoch\endcsname{0.34}
\expandafter\def\csname v@ft/cohere-transcribe/loop\endcsname{0}
\expandafter\def\csname v@ft/cohere-transcribe/lr\endcsname{3e-5}
\expandafter\def\csname v@ft/cohere-transcribe/median\endcsname{11.7}
\expandafter\def\csname v@ft/cohere-transcribe/raw\endcsname{15.6}
\expandafter\def\csname v@ft/cohere-transcribe/run\endcsname{fthi}
\expandafter\def\csname v@ft/cohere-transcribe/wer\endcsname{45.8}
\expandafter\def\csname v@ft/count\endcsname{21}
\expandafter\def\csname v@ft/gain-max\endcsname{53.1}
\expandafter\def\csname v@ft/gain-mean\endcsname{38.8}
\expandafter\def\csname v@ft/gain-min\endcsname{16.6}
\expandafter\def\csname v@ft/gemma4-12b/before\endcsname{72.9}
\expandafter\def\csname v@ft/gemma4-12b/cer\endcsname{19.8}
\expandafter\def\csname v@ft/gemma4-12b/ci\endcsname{19.1--20.6}
\expandafter\def\csname v@ft/gemma4-12b/clips-s\endcsname{3}
\expandafter\def\csname v@ft/gemma4-12b/dev\endcsname{28.1}
\expandafter\def\csname v@ft/gemma4-12b/epoch\endcsname{2}
\expandafter\def\csname v@ft/gemma4-12b/gain\endcsname{53.1}
\expandafter\def\csname v@ft/gemma4-12b/gain-ci\endcsname{51.8--54.1}
\expandafter\def\csname v@ft/gemma4-12b/h-epoch\endcsname{4.03}
\expandafter\def\csname v@ft/gemma4-12b/loop\endcsname{11}
\expandafter\def\csname v@ft/gemma4-12b/lr\endcsname{3e-6}
\expandafter\def\csname v@ft/gemma4-12b/median\endcsname{17.8}
\expandafter\def\csname v@ft/gemma4-12b/raw\endcsname{23.2}
\expandafter\def\csname v@ft/gemma4-12b/run\endcsname{ft}
\expandafter\def\csname v@ft/gemma4-12b/wer\endcsname{51.8}
\expandafter\def\csname v@ft/gemma4-e2b/before\endcsname{43.5}
\expandafter\def\csname v@ft/gemma4-e2b/cer\endcsname{18.5}
\expandafter\def\csname v@ft/gemma4-e2b/ci\endcsname{17.8--19.4}
\expandafter\def\csname v@ft/gemma4-e2b/clips-s\endcsname{15}
\expandafter\def\csname v@ft/gemma4-e2b/dev\endcsname{25.7}
\expandafter\def\csname v@ft/gemma4-e2b/epoch\endcsname{5}
\expandafter\def\csname v@ft/gemma4-e2b/gain\endcsname{24.9}
\expandafter\def\csname v@ft/gemma4-e2b/gain-ci\endcsname{24.0--25.9}
\expandafter\def\csname v@ft/gemma4-e2b/h-epoch\endcsname{0.81}
\expandafter\def\csname v@ft/gemma4-e2b/loop\endcsname{1}
\expandafter\def\csname v@ft/gemma4-e2b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/gemma4-e2b/median\endcsname{16.7}
\expandafter\def\csname v@ft/gemma4-e2b/raw\endcsname{19.8}
\expandafter\def\csname v@ft/gemma4-e2b/run\endcsname{ft}
\expandafter\def\csname v@ft/gemma4-e2b/wer\endcsname{49.2}
\expandafter\def\csname v@ft/gemma4-e4b/before\endcsname{39.8}
\expandafter\def\csname v@ft/gemma4-e4b/cer\endcsname{16.6}
\expandafter\def\csname v@ft/gemma4-e4b/ci\endcsname{16.0--17.3}
\expandafter\def\csname v@ft/gemma4-e4b/clips-s\endcsname{6}
\expandafter\def\csname v@ft/gemma4-e4b/dev\endcsname{24.7}
\expandafter\def\csname v@ft/gemma4-e4b/epoch\endcsname{2}
\expandafter\def\csname v@ft/gemma4-e4b/gain\endcsname{23.2}
\expandafter\def\csname v@ft/gemma4-e4b/gain-ci\endcsname{22.4--24.1}
\expandafter\def\csname v@ft/gemma4-e4b/h-epoch\endcsname{1.90}
\expandafter\def\csname v@ft/gemma4-e4b/loop\endcsname{5}
\expandafter\def\csname v@ft/gemma4-e4b/lr\endcsname{3e-6}
\expandafter\def\csname v@ft/gemma4-e4b/median\endcsname{14.2}
\expandafter\def\csname v@ft/gemma4-e4b/raw\endcsname{17.7}
\expandafter\def\csname v@ft/gemma4-e4b/run\endcsname{ft}
\expandafter\def\csname v@ft/gemma4-e4b/wer\endcsname{47.1}
\expandafter\def\csname v@ft/granite-2b/before\endcsname{62.1}
\expandafter\def\csname v@ft/granite-2b/cer\endcsname{22.5}
\expandafter\def\csname v@ft/granite-2b/ci\endcsname{21.8--23.4}
\expandafter\def\csname v@ft/granite-2b/clips-s\endcsname{18}
\expandafter\def\csname v@ft/granite-2b/dev\endcsname{29.0}
\expandafter\def\csname v@ft/granite-2b/epoch\endcsname{7}
\expandafter\def\csname v@ft/granite-2b/gain\endcsname{39.6}
\expandafter\def\csname v@ft/granite-2b/gain-ci\endcsname{38.7--40.6}
\expandafter\def\csname v@ft/granite-2b/h-epoch\endcsname{0.68}
\expandafter\def\csname v@ft/granite-2b/loop\endcsname{1}
\expandafter\def\csname v@ft/granite-2b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/granite-2b/median\endcsname{21.9}
\expandafter\def\csname v@ft/granite-2b/raw\endcsname{22.6}
\expandafter\def\csname v@ft/granite-2b/run\endcsname{ft}
\expandafter\def\csname v@ft/granite-2b/wer\endcsname{58.1}
\expandafter\def\csname v@ft/lfm3-audio/before\endcsname{64.3}
\expandafter\def\csname v@ft/lfm3-audio/cer\endcsname{17.8}
\expandafter\def\csname v@ft/lfm3-audio/ci\endcsname{17.2--18.6}
\expandafter\def\csname v@ft/lfm3-audio/clips-s\endcsname{27}
\expandafter\def\csname v@ft/lfm3-audio/dev\endcsname{24.9}
\expandafter\def\csname v@ft/lfm3-audio/epoch\endcsname{3}
\expandafter\def\csname v@ft/lfm3-audio/gain\endcsname{46.5}
\expandafter\def\csname v@ft/lfm3-audio/gain-ci\endcsname{45.6--47.5}
\expandafter\def\csname v@ft/lfm3-audio/h-epoch\endcsname{0.44}
\expandafter\def\csname v@ft/lfm3-audio/loop\endcsname{6}
\expandafter\def\csname v@ft/lfm3-audio/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/lfm3-audio/median\endcsname{15.1}
\expandafter\def\csname v@ft/lfm3-audio/raw\endcsname{21.8}
\expandafter\def\csname v@ft/lfm3-audio/run\endcsname{ft}
\expandafter\def\csname v@ft/lfm3-audio/wer\endcsname{48.7}
\expandafter\def\csname v@ft/mms-1b/before\endcsname{30.6}
\expandafter\def\csname v@ft/mms-1b/cer\endcsname{11.0}
\expandafter\def\csname v@ft/mms-1b/ci\endcsname{10.6--11.6}
\expandafter\def\csname v@ft/mms-1b/clips-s\endcsname{23}
\expandafter\def\csname v@ft/mms-1b/dev\endcsname{18.7}
\expandafter\def\csname v@ft/mms-1b/epoch\endcsname{10}
\expandafter\def\csname v@ft/mms-1b/gain\endcsname{19.6}
\expandafter\def\csname v@ft/mms-1b/gain-ci\endcsname{19.1--20.0}
\expandafter\def\csname v@ft/mms-1b/h-epoch\endcsname{0.52}
\expandafter\def\csname v@ft/mms-1b/loop\endcsname{1}
\expandafter\def\csname v@ft/mms-1b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/mms-1b/median\endcsname{8.7}
\expandafter\def\csname v@ft/mms-1b/raw\endcsname{11.0}
\expandafter\def\csname v@ft/mms-1b/run\endcsname{ftlow}
\expandafter\def\csname v@ft/mms-1b/wer\endcsname{39.3}
\expandafter\def\csname v@ft/n\endcsname{21}
\expandafter\def\csname v@ft/nemotron-30b/before\endcsname{58.1}
\expandafter\def\csname v@ft/nemotron-30b/cer\endcsname{15.8}
\expandafter\def\csname v@ft/nemotron-30b/ci\endcsname{15.2--16.5}
\expandafter\def\csname v@ft/nemotron-30b/dev\endcsname{22.7}
\expandafter\def\csname v@ft/nemotron-30b/epoch\endcsname{2}
\expandafter\def\csname v@ft/nemotron-30b/gain\endcsname{42.3}
\expandafter\def\csname v@ft/nemotron-30b/gain-ci\endcsname{41.2--43.5}
\expandafter\def\csname v@ft/nemotron-30b/loop\endcsname{2}
\expandafter\def\csname v@ft/nemotron-30b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/nemotron-30b/median\endcsname{13.2}
\expandafter\def\csname v@ft/nemotron-30b/raw\endcsname{15.8}
\expandafter\def\csname v@ft/nemotron-30b/run\endcsname{ftall}
\expandafter\def\csname v@ft/nemotron-30b/wer\endcsname{45.3}
\expandafter\def\csname v@ft/nemotron-stream/before\endcsname{68.7}
\expandafter\def\csname v@ft/nemotron-stream/cer\endcsname{35.9}
\expandafter\def\csname v@ft/nemotron-stream/ci\endcsname{35.3--36.5}
\expandafter\def\csname v@ft/nemotron-stream/clips-s\endcsname{34}
\expandafter\def\csname v@ft/nemotron-stream/dev\endcsname{41.4}
\expandafter\def\csname v@ft/nemotron-stream/epoch\endcsname{10}
\expandafter\def\csname v@ft/nemotron-stream/gain\endcsname{32.8}
\expandafter\def\csname v@ft/nemotron-stream/gain-ci\endcsname{32.0--33.8}
\expandafter\def\csname v@ft/nemotron-stream/h-epoch\endcsname{0.35}
\expandafter\def\csname v@ft/nemotron-stream/loop\endcsname{5}
\expandafter\def\csname v@ft/nemotron-stream/lr\endcsname{1e-4}
\expandafter\def\csname v@ft/nemotron-stream/median\endcsname{32.2}
\expandafter\def\csname v@ft/nemotron-stream/raw\endcsname{36.4}
\expandafter\def\csname v@ft/nemotron-stream/run\endcsname{flawed}
\expandafter\def\csname v@ft/nemotron-stream/start\endcsname{the first start}
\expandafter\def\csname v@ft/nemotron-stream/wer\endcsname{78.2}
\expandafter\def\csname v@ft/omni-ctc-1b/before\endcsname{28.5}
\expandafter\def\csname v@ft/omni-ctc-1b/cer\endcsname{12.0}
\expandafter\def\csname v@ft/omni-ctc-1b/ci\endcsname{11.5--12.6}
\expandafter\def\csname v@ft/omni-ctc-1b/clips-s\endcsname{23}
\expandafter\def\csname v@ft/omni-ctc-1b/dev\endcsname{19.4}
\expandafter\def\csname v@ft/omni-ctc-1b/epoch\endcsname{7}
\expandafter\def\csname v@ft/omni-ctc-1b/gain\endcsname{16.6}
\expandafter\def\csname v@ft/omni-ctc-1b/gain-ci\endcsname{15.8--17.4}
\expandafter\def\csname v@ft/omni-ctc-1b/h-epoch\endcsname{0.51}
\expandafter\def\csname v@ft/omni-ctc-1b/loop\endcsname{1}
\expandafter\def\csname v@ft/omni-ctc-1b/lr\endcsname{3e-5}
\expandafter\def\csname v@ft/omni-ctc-1b/median\endcsname{10.2}
\expandafter\def\csname v@ft/omni-ctc-1b/raw\endcsname{12.1}
\expandafter\def\csname v@ft/omni-ctc-1b/run\endcsname{ft}
\expandafter\def\csname v@ft/omni-ctc-1b/wer\endcsname{43.1}
\expandafter\def\csname v@ft/parakeet-tdt-v3/before\endcsname{55.7}
\expandafter\def\csname v@ft/parakeet-tdt-v3/cer\endcsname{21.0}
\expandafter\def\csname v@ft/parakeet-tdt-v3/ci\endcsname{20.2--21.9}
\expandafter\def\csname v@ft/parakeet-tdt-v3/clips-s\endcsname{15}
\expandafter\def\csname v@ft/parakeet-tdt-v3/dev\endcsname{27.6}
\expandafter\def\csname v@ft/parakeet-tdt-v3/epoch\endcsname{9}
\expandafter\def\csname v@ft/parakeet-tdt-v3/gain\endcsname{34.7}
\expandafter\def\csname v@ft/parakeet-tdt-v3/gain-ci\endcsname{33.8--35.8}
\expandafter\def\csname v@ft/parakeet-tdt-v3/h-epoch\endcsname{0.80}
\expandafter\def\csname v@ft/parakeet-tdt-v3/loop\endcsname{4}
\expandafter\def\csname v@ft/parakeet-tdt-v3/lr\endcsname{3e-4}
\expandafter\def\csname v@ft/parakeet-tdt-v3/median\endcsname{16.4}
\expandafter\def\csname v@ft/parakeet-tdt-v3/raw\endcsname{24.6}
\expandafter\def\csname v@ft/parakeet-tdt-v3/run\endcsname{fthi}
\expandafter\def\csname v@ft/parakeet-tdt-v3/start\endcsname{a copy of the blank's row, ten below it, at 3e-4 rather than 1e-4}
\expandafter\def\csname v@ft/parakeet-tdt-v3/wer\endcsname{52.6}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/before\endcsname{60.9}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/cer\endcsname{18.2}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/ci\endcsname{17.5--18.9}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/clips-s\endcsname{46}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/dev\endcsname{25.3}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/epoch\endcsname{4}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/gain\endcsname{42.8}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/gain-ci\endcsname{41.8--43.8}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/h-epoch\endcsname{0.26}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/loop\endcsname{5}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/median\endcsname{16.1}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/raw\endcsname{18.7}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/run\endcsname{ft}
\expandafter\def\csname v@ft/qwen3-asr-0.6b/wer\endcsname{51.9}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/before\endcsname{59.3}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/cer\endcsname{16.6}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/ci\endcsname{16.0--17.3}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/clips-s\endcsname{25}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/dev\endcsname{23.7}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/epoch\endcsname{4}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/gain\endcsname{42.7}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/gain-ci\endcsname{41.8--43.6}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/h-epoch\endcsname{0.47}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/loop\endcsname{1}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/median\endcsname{13.9}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/raw\endcsname{16.9}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/run\endcsname{ft}
\expandafter\def\csname v@ft/qwen3-asr-1.7b/wer\endcsname{47.9}
\expandafter\def\csname v@ft/top/cer\endcsname{9.5}
\expandafter\def\csname v@ft/top/name\endcsname{omniASR CTC 7B}
\expandafter\def\csname v@ft/voxtral-mini/before\endcsname{61.8}
\expandafter\def\csname v@ft/voxtral-mini/cer\endcsname{16.3}
\expandafter\def\csname v@ft/voxtral-mini/ci\endcsname{15.7--17.1}
\expandafter\def\csname v@ft/voxtral-mini/clips-s\endcsname{4}
\expandafter\def\csname v@ft/voxtral-mini/dev\endcsname{24.3}
\expandafter\def\csname v@ft/voxtral-mini/epoch\endcsname{3}
\expandafter\def\csname v@ft/voxtral-mini/gain\endcsname{45.5}
\expandafter\def\csname v@ft/voxtral-mini/gain-ci\endcsname{44.3--46.6}
\expandafter\def\csname v@ft/voxtral-mini/h-epoch\endcsname{2.93}
\expandafter\def\csname v@ft/voxtral-mini/loop\endcsname{5}
\expandafter\def\csname v@ft/voxtral-mini/lr\endcsname{3e-6}
\expandafter\def\csname v@ft/voxtral-mini/median\endcsname{14.2}
\expandafter\def\csname v@ft/voxtral-mini/raw\endcsname{17.2}
\expandafter\def\csname v@ft/voxtral-mini/run\endcsname{ftlow}
\expandafter\def\csname v@ft/voxtral-mini/wer\endcsname{45.7}
\expandafter\def\csname v@ft/w2v-bert/cer\endcsname{12.7}
\expandafter\def\csname v@ft/w2v-bert/ci\endcsname{12.3--13.3}
\expandafter\def\csname v@ft/w2v-bert/clips-s\endcsname{40}
\expandafter\def\csname v@ft/w2v-bert/dev\endcsname{19.9}
\expandafter\def\csname v@ft/w2v-bert/epoch\endcsname{9}
\expandafter\def\csname v@ft/w2v-bert/h-epoch\endcsname{0.30}
\expandafter\def\csname v@ft/w2v-bert/loop\endcsname{1}
\expandafter\def\csname v@ft/w2v-bert/lr\endcsname{3e-5}
\expandafter\def\csname v@ft/w2v-bert/median\endcsname{10.4}
\expandafter\def\csname v@ft/w2v-bert/raw\endcsname{12.7}
\expandafter\def\csname v@ft/w2v-bert/run\endcsname{ft}
\expandafter\def\csname v@ft/w2v-bert/wer\endcsname{44.9}
\expandafter\def\csname v@ft/whisper-large-v2/before\endcsname{57.8}
\expandafter\def\csname v@ft/whisper-large-v2/cer\endcsname{14.2}
\expandafter\def\csname v@ft/whisper-large-v2/ci\endcsname{13.7--14.9}
\expandafter\def\csname v@ft/whisper-large-v2/clips-s\endcsname{11}
\expandafter\def\csname v@ft/whisper-large-v2/dev\endcsname{21.7}
\expandafter\def\csname v@ft/whisper-large-v2/epoch\endcsname{4}
\expandafter\def\csname v@ft/whisper-large-v2/gain\endcsname{43.5}
\expandafter\def\csname v@ft/whisper-large-v2/gain-ci\endcsname{42.4--44.6}
\expandafter\def\csname v@ft/whisper-large-v2/h-epoch\endcsname{1.09}
\expandafter\def\csname v@ft/whisper-large-v2/loop\endcsname{2}
\expandafter\def\csname v@ft/whisper-large-v2/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/whisper-large-v2/median\endcsname{11.4}
\expandafter\def\csname v@ft/whisper-large-v2/raw\endcsname{14.4}
\expandafter\def\csname v@ft/whisper-large-v2/run\endcsname{ft}
\expandafter\def\csname v@ft/whisper-large-v2/wer\endcsname{43.2}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/before\endcsname{54.6}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/cer\endcsname{14.3}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/ci\endcsname{13.6--15.1}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/clips-s\endcsname{14}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/dev\endcsname{21.5}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/epoch\endcsname{9}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/gain\endcsname{40.2}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/gain-ci\endcsname{39.2--41.4}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/h-epoch\endcsname{0.82}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/loop\endcsname{7}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/median\endcsname{10.8}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/raw\endcsname{15.1}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/run\endcsname{ft}
\expandafter\def\csname v@ft/whisper-large-v3-turbo/wer\endcsname{43.0}
\expandafter\def\csname v@ft/whisper-large-v3/before\endcsname{50.3}
\expandafter\def\csname v@ft/whisper-large-v3/cer\endcsname{13.5}
\expandafter\def\csname v@ft/whisper-large-v3/ci\endcsname{13.0--14.2}
\expandafter\def\csname v@ft/whisper-large-v3/clips-s\endcsname{11}
\expandafter\def\csname v@ft/whisper-large-v3/dev\endcsname{20.6}
\expandafter\def\csname v@ft/whisper-large-v3/epoch\endcsname{8}
\expandafter\def\csname v@ft/whisper-large-v3/gain\endcsname{36.8}
\expandafter\def\csname v@ft/whisper-large-v3/gain-ci\endcsname{35.9--37.7}
\expandafter\def\csname v@ft/whisper-large-v3/h-epoch\endcsname{1.11}
\expandafter\def\csname v@ft/whisper-large-v3/loop\endcsname{1}
\expandafter\def\csname v@ft/whisper-large-v3/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/whisper-large-v3/median\endcsname{10.3}
\expandafter\def\csname v@ft/whisper-large-v3/raw\endcsname{13.7}
\expandafter\def\csname v@ft/whisper-large-v3/run\endcsname{ft}
\expandafter\def\csname v@ft/whisper-large-v3/wer\endcsname{41.5}
\expandafter\def\csname v@ft/whisper-medium/before\endcsname{63.7}
\expandafter\def\csname v@ft/whisper-medium/cer\endcsname{14.8}
\expandafter\def\csname v@ft/whisper-medium/ci\endcsname{14.2--15.5}
\expandafter\def\csname v@ft/whisper-medium/clips-s\endcsname{20}
\expandafter\def\csname v@ft/whisper-medium/dev\endcsname{22.3}
\expandafter\def\csname v@ft/whisper-medium/epoch\endcsname{10}
\expandafter\def\csname v@ft/whisper-medium/gain\endcsname{48.9}
\expandafter\def\csname v@ft/whisper-medium/gain-ci\endcsname{47.8--50.0}
\expandafter\def\csname v@ft/whisper-medium/h-epoch\endcsname{0.59}
\expandafter\def\csname v@ft/whisper-medium/loop\endcsname{2}
\expandafter\def\csname v@ft/whisper-medium/lr\endcsname{1e-5}
\expandafter\def\csname v@ft/whisper-medium/median\endcsname{11.9}
\expandafter\def\csname v@ft/whisper-medium/raw\endcsname{15.0}
\expandafter\def\csname v@ft/whisper-medium/run\endcsname{ftlow}
\expandafter\def\csname v@ft/whisper-medium/wer\endcsname{45.0}
\expandafter\def\csname v@ft/whisper-small/before\endcsname{65.7}
\expandafter\def\csname v@ft/whisper-small/cer\endcsname{16.9}
\expandafter\def\csname v@ft/whisper-small/ci\endcsname{16.4--17.6}
\expandafter\def\csname v@ft/whisper-small/clips-s\endcsname{59}
\expandafter\def\csname v@ft/whisper-small/dev\endcsname{24.5}
\expandafter\def\csname v@ft/whisper-small/epoch\endcsname{9}
\expandafter\def\csname v@ft/whisper-small/gain\endcsname{48.8}
\expandafter\def\csname v@ft/whisper-small/gain-ci\endcsname{47.7--49.9}
\expandafter\def\csname v@ft/whisper-small/h-epoch\endcsname{0.20}
\expandafter\def\csname v@ft/whisper-small/loop\endcsname{0}
\expandafter\def\csname v@ft/whisper-small/lr\endcsname{3e-5}
\expandafter\def\csname v@ft/whisper-small/median\endcsname{12.8}
\expandafter\def\csname v@ft/whisper-small/raw\endcsname{17.1}
\expandafter\def\csname v@ft/whisper-small/run\endcsname{ft}
\expandafter\def\csname v@ft/whisper-small/wer\endcsname{49.2}
\expandafter\def\csname v@ft/whisper-tiny/before\endcsname{66.6}
\expandafter\def\csname v@ft/whisper-tiny/cer\endcsname{25.7}
\expandafter\def\csname v@ft/whisper-tiny/ci\endcsname{24.9--26.5}
\expandafter\def\csname v@ft/whisper-tiny/clips-s\endcsname{312}
\expandafter\def\csname v@ft/whisper-tiny/dev\endcsname{34.0}
\expandafter\def\csname v@ft/whisper-tiny/epoch\endcsname{5}
\expandafter\def\csname v@ft/whisper-tiny/gain\endcsname{40.9}
\expandafter\def\csname v@ft/whisper-tiny/gain-ci\endcsname{39.7--42.0}
\expandafter\def\csname v@ft/whisper-tiny/h-epoch\endcsname{0.04}
\expandafter\def\csname v@ft/whisper-tiny/loop\endcsname{16}
\expandafter\def\csname v@ft/whisper-tiny/lr\endcsname{1e-4}
\expandafter\def\csname v@ft/whisper-tiny/median\endcsname{23.5}
\expandafter\def\csname v@ft/whisper-tiny/raw\endcsname{30.2}
\expandafter\def\csname v@ft/whisper-tiny/run\endcsname{ft}
\expandafter\def\csname v@ft/whisper-tiny/wer\endcsname{63.9}
\expandafter\def\csname v@ft/worst-wer/name\endcsname{Nemotron 3.5 streaming 0.6B}
\expandafter\def\csname v@ft/worst-wer/wer\endcsname{78.2}
\expandafter\def\csname v@ft/worst/cer\endcsname{35.9}
\expandafter\def\csname v@ft/worst/name\endcsname{Nemotron 3.5 streaming 0.6B}
\expandafter\def\csname v@fz/parakeet-tdt-v3/all\endcsname{24.2}
\expandafter\def\csname v@fz/parakeet-tdt-v3/fzd\endcsname{31.2}
\expandafter\def\csname v@fz/parakeet-tdt-v3/fze\endcsname{53.5}
\expandafter\def\csname v@fz/qwen3-asr-0.6b/all\endcsname{18.2}
\expandafter\def\csname v@fz/qwen3-asr-0.6b/fzd\endcsname{19.6}
\expandafter\def\csname v@fz/qwen3-asr-0.6b/fze\endcsname{21.0}
\expandafter\def\csname v@fz/w2v-bert/all\endcsname{13.7}
\expandafter\def\csname v@fz/w2v-bert/fze\endcsname{77.6}
\expandafter\def\csname v@fz/whisper-small/all\endcsname{16.9}
\expandafter\def\csname v@fz/whisper-small/fzd\endcsname{22.9}
\expandafter\def\csname v@fz/whisper-small/fze\endcsname{20.7}
\expandafter\def\csname v@fzd/parakeet-tdt-v3/cer\endcsname{31.2}
\expandafter\def\csname v@fzd/parakeet-tdt-v3/dev\endcsname{36.2}
\expandafter\def\csname v@fzd/parakeet-tdt-v3/epoch\endcsname{6}
\expandafter\def\csname v@fzd/qwen3-asr-0.6b/cer\endcsname{19.6}
\expandafter\def\csname v@fzd/qwen3-asr-0.6b/dev\endcsname{27.2}
\expandafter\def\csname v@fzd/qwen3-asr-0.6b/epoch\endcsname{6}
\expandafter\def\csname v@fzd/whisper-small/cer\endcsname{22.9}
\expandafter\def\csname v@fzd/whisper-small/dev\endcsname{31.0}
\expandafter\def\csname v@fzd/whisper-small/epoch\endcsname{6}
\expandafter\def\csname v@fze/parakeet-tdt-v3/cer\endcsname{53.5}
\expandafter\def\csname v@fze/parakeet-tdt-v3/dev\endcsname{56.7}
\expandafter\def\csname v@fze/parakeet-tdt-v3/epoch\endcsname{6}
\expandafter\def\csname v@fze/qwen3-asr-0.6b/cer\endcsname{21.0}
\expandafter\def\csname v@fze/qwen3-asr-0.6b/dev\endcsname{28.1}
\expandafter\def\csname v@fze/qwen3-asr-0.6b/epoch\endcsname{5}
\expandafter\def\csname v@fze/w2v-bert/cer\endcsname{77.6}
\expandafter\def\csname v@fze/w2v-bert/dev\endcsname{79.7}
\expandafter\def\csname v@fze/w2v-bert/epoch\endcsname{3}
\expandafter\def\csname v@fze/whisper-small/cer\endcsname{20.7}
\expandafter\def\csname v@fze/whisper-small/dev\endcsname{28.3}
\expandafter\def\csname v@fze/whisper-small/epoch\endcsname{5}
\expandafter\def\csname v@gr/full/best\endcsname{6}
\expandafter\def\csname v@gr/full/d3-last\endcsname{0.7}
\expandafter\def\csname v@gr/full/e1\endcsname{23.2}
\expandafter\def\csname v@gr/full/e3\endcsname{18.2}
\expandafter\def\csname v@gr/full/last\endcsname{17.5}
\expandafter\def\csname v@gr/full/n\endcsname{16}
\expandafter\def\csname v@gr/full/within\endcsname{3}
\expandafter\def\csname v@gr/mid/best\endcsname{17}
\expandafter\def\csname v@gr/mid/d3-last\endcsname{0.3}
\expandafter\def\csname v@gr/mid/e1\endcsname{23.8}
\expandafter\def\csname v@gr/mid/e3\endcsname{18.5}
\expandafter\def\csname v@gr/mid/last\endcsname{18.2}
\expandafter\def\csname v@gr/mid/n\endcsname{27}
\expandafter\def\csname v@gr/mid/within\endcsname{3}
\expandafter\def\csname v@gr/scarce/best\endcsname{6}
\expandafter\def\csname v@gr/scarce/d3-last\endcsname{-1.1}
\expandafter\def\csname v@gr/scarce/e1\endcsname{22.6}
\expandafter\def\csname v@gr/scarce/e3\endcsname{18.7}
\expandafter\def\csname v@gr/scarce/last\endcsname{19.8}
\expandafter\def\csname v@gr/scarce/n\endcsname{7}
\expandafter\def\csname v@gr/scarce/within\endcsname{6}
\expandafter\def\csname v@hard/clips/a\endcsname{15.7}
\expandafter\def\csname v@hard/clips/b\endcsname{18.0}
\expandafter\def\csname v@hard/clips/ci\endcsname{-3.8 to 7.9}
\expandafter\def\csname v@hard/clips/diff\endcsname{2.2}
\expandafter\def\csname v@hard/clips/na\endcsname{43}
\expandafter\def\csname v@hard/clips/nb\endcsname{7}
\expandafter\def\csname v@hard/clips/rho\endcsname{-0.09}
\expandafter\def\csname v@hard/clips/rho-ci\endcsname{-0.31 to 0.21}
\expandafter\def\csname v@hard/length/a\endcsname{12.3}
\expandafter\def\csname v@hard/length/b\endcsname{19.8}
\expandafter\def\csname v@hard/length/ci\endcsname{2.4 to 12.7}
\expandafter\def\csname v@hard/length/diff\endcsname{7.4}
\expandafter\def\csname v@hard/length/na\endcsname{25}
\expandafter\def\csname v@hard/length/nb\endcsname{25}
\expandafter\def\csname v@hard/length/rho\endcsname{-0.41}
\expandafter\def\csname v@hard/length/rho-ci\endcsname{-0.64 to -0.15}
\expandafter\def\csname v@hard/list/a\endcsname{15.5}
\expandafter\def\csname v@hard/list/b\endcsname{17.7}
\expandafter\def\csname v@hard/list/ci\endcsname{-2.9 to 6.9}
\expandafter\def\csname v@hard/list/diff\endcsname{2.2}
\expandafter\def\csname v@hard/list/na\endcsname{38}
\expandafter\def\csname v@hard/list/nb\endcsname{12}
\expandafter\def\csname v@hard/r2\endcsname{36}
\expandafter\def\csname v@hard/script/a\endcsname{14.8}
\expandafter\def\csname v@hard/script/b\endcsname{19.3}
\expandafter\def\csname v@hard/script/ci\endcsname{-2.2 to 12.1}
\expandafter\def\csname v@hard/script/diff\endcsname{4.5}
\expandafter\def\csname v@hard/script/na\endcsname{36}
\expandafter\def\csname v@hard/script/nb\endcsname{14}
\expandafter\def\csname v@hard/shared/a\endcsname{10.2}
\expandafter\def\csname v@hard/shared/b\endcsname{16.7}
\expandafter\def\csname v@hard/shared/ci\endcsname{2.9 to 10.4}
\expandafter\def\csname v@hard/shared/diff\endcsname{6.5}
\expandafter\def\csname v@hard/shared/na\endcsname{5}
\expandafter\def\csname v@hard/shared/nb\endcsname{45}
\expandafter\def\csname v@hard/speakers/a\endcsname{12.7}
\expandafter\def\csname v@hard/speakers/b\endcsname{19.4}
\expandafter\def\csname v@hard/speakers/ci\endcsname{1.7 to 12.1}
\expandafter\def\csname v@hard/speakers/diff\endcsname{6.7}
\expandafter\def\csname v@hard/speakers/na\endcsname{25}
\expandafter\def\csname v@hard/speakers/nb\endcsname{25}
\expandafter\def\csname v@hard/speakers/rho\endcsname{0.44}
\expandafter\def\csname v@hard/speakers/rho-ci\endcsname{0.15 to 0.67}
\expandafter\def\csname v@hard/unexplained\endcsname{64}
\expandafter\def\csname v@ho/all/ahead-max\endcsname{1.1}
\expandafter\def\csname v@ho/all/behind-max\endcsname{1.9}
\expandafter\def\csname v@ho/all/behind-n\endcsname{18}
\expandafter\def\csname v@ho/all/k25-behind-max\endcsname{1.7}
\expandafter\def\csname v@ho/all/k25-behind-n\endcsname{7}
\expandafter\def\csname v@ho/all/k25-clause\endcsname{behind in 7 of the 8 pairs at 25 clips, by up to 1.7 points (4 with an interval that leaves out zero), and ahead in Whisper large-v3-turbo's second seed, by 0.2 (-0.6 to 1.0)}
\expandafter\def\csname v@ho/all/more-absmax\endcsname{1.9}
\expandafter\def\csname v@ho/all/more-n\endcsname{16}
\expandafter\def\csname v@ho/all/more-sig-ahead-n\endcsname{1}
\expandafter\def\csname v@ho/all/more-sig-behind-n\endcsname{3}
\expandafter\def\csname v@ho/all/n\endcsname{24}
\expandafter\def\csname v@ho/all/n-25\endcsname{8}
\expandafter\def\csname v@ho/all/sig-25-n\endcsname{4}
\expandafter\def\csname v@ho/all/sig-ahead-n\endcsname{1}
\expandafter\def\csname v@ho/all/sig-n\endcsname{8}
\expandafter\def\csname v@ho/clip-gain-absmax\endcsname{1.5}
\expandafter\def\csname v@ho/clip-gain-n\endcsname{12}
\expandafter\def\csname v@ho/clip-gain-sig\endcsname{Qwen3-ASR 0.6B at 25 clips, by 1.4 points, Whisper large-v3-turbo at 25 clips, by 1.3 points, Whisper large-v3-turbo at 1,000 clips, by 1.2 points and MMS 1B at 25 clips, by 1.5 points}
\expandafter\def\csname v@ho/clip-gain-sig-dir\endcsname{behind}
\expandafter\def\csname v@ho/clip-gain-sig-n\endcsname{4}
\expandafter\def\csname v@ho/mms-1b/from40/0\endcsname{32.9}
\expandafter\def\csname v@ho/mms-1b/from40/100\endcsname{14.4}
\expandafter\def\csname v@ho/mms-1b/from40/1000\endcsname{12.0}
\expandafter\def\csname v@ho/mms-1b/from40/25\endcsname{17.0}
\expandafter\def\csname v@ho/mms-1b/gain/0\endcsname{67.1}
\expandafter\def\csname v@ho/mms-1b/gain/100\endcsname{0.3}
\expandafter\def\csname v@ho/mms-1b/gain/100-ci\endcsname{-0.4 to 1.1}
\expandafter\def\csname v@ho/mms-1b/gain/1000\endcsname{0.2}
\expandafter\def\csname v@ho/mms-1b/gain/1000-ci\endcsname{-0.6 to 0.9}
\expandafter\def\csname v@ho/mms-1b/gain/25\endcsname{-1.5}
\expandafter\def\csname v@ho/mms-1b/gain/25-ci\endcsname{-2.2 to -1.0}
\expandafter\def\csname v@ho/mms-1b/main\endcsname{12.2}
\expandafter\def\csname v@ho/mms-1b/pre/0\endcsname{100.0}
\expandafter\def\csname v@ho/mms-1b/pre/100\endcsname{14.7}
\expandafter\def\csname v@ho/mms-1b/pre/1000\endcsname{12.3}
\expandafter\def\csname v@ho/mms-1b/pre/25\endcsname{15.5}
\expandafter\def\csname v@ho/mms-1b/stage1\endcsname{10.8}
\expandafter\def\csname v@ho/n-held\endcsname{10}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/from40/0\endcsname{50.4}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/from40/100\endcsname{28.0}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/from40/1000\endcsname{17.8}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/from40/25\endcsname{34.9}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/0\endcsname{-0.4}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/100\endcsname{-0.7}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/100-ci\endcsname{-2.3 to 0.5}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/1000\endcsname{-0.5}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/1000-ci\endcsname{-1.2 to 0.3}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/25\endcsname{-1.4}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/gain/25-ci\endcsname{-2.5 to -0.4}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/main\endcsname{18.2}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/pre/0\endcsname{50.1}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/pre/100\endcsname{27.3}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/pre/1000\endcsname{17.3}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/pre/25\endcsname{33.4}
\expandafter\def\csname v@ho/qwen3-asr-0.6b/stage1\endcsname{18.3}
\expandafter\def\csname v@ho/s1/ahead-n\endcsname{3}
\expandafter\def\csname v@ho/s1/behind-max\endcsname{1.9}
\expandafter\def\csname v@ho/s1/mms-1b/gain/100\endcsname{0.0}
\expandafter\def\csname v@ho/s1/mms-1b/gain/100-ci\endcsname{-1.2 to 1.1}
\expandafter\def\csname v@ho/s1/mms-1b/gain/1000\endcsname{1.1}
\expandafter\def\csname v@ho/s1/mms-1b/gain/1000-ci\endcsname{0.8 to 1.4}
\expandafter\def\csname v@ho/s1/mms-1b/gain/25\endcsname{-1.7}
\expandafter\def\csname v@ho/s1/mms-1b/gain/25-ci\endcsname{-2.5 to -1.1}
\expandafter\def\csname v@ho/s1/models\endcsname{MMS 1B, Qwen3-ASR 0.6B, Whisper large-v3-turbo and Whisper small}
\expandafter\def\csname v@ho/s1/n\endcsname{12}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/100\endcsname{-0.3}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/100-ci\endcsname{-1.2 to 0.6}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/1000\endcsname{-0.9}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/1000-ci\endcsname{-1.6 to 0.0}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/25\endcsname{-0.8}
\expandafter\def\csname v@ho/s1/qwen3-asr-0.6b/gain/25-ci\endcsname{-2.1 to 0.5}
\expandafter\def\csname v@ho/s1/sig-n\endcsname{4}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/100\endcsname{-1.9}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/100-ci\endcsname{-2.9 to -1.1}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/1000\endcsname{-0.6}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/1000-ci\endcsname{-1.3 to 0.1}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/25\endcsname{0.2}
\expandafter\def\csname v@ho/s1/whisper-large-v3-turbo/gain/25-ci\endcsname{-0.6 to 1.0}
\expandafter\def\csname v@ho/s1/whisper-small/gain/100\endcsname{-0.1}
\expandafter\def\csname v@ho/s1/whisper-small/gain/100-ci\endcsname{-0.9 to 0.7}
\expandafter\def\csname v@ho/s1/whisper-small/gain/1000\endcsname{0.1}
\expandafter\def\csname v@ho/s1/whisper-small/gain/1000-ci\endcsname{-0.8 to 0.9}
\expandafter\def\csname v@ho/s1/whisper-small/gain/25\endcsname{-0.7}
\expandafter\def\csname v@ho/s1/whisper-small/gain/25-ci\endcsname{-1.7 to 0.6}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/from40/0\endcsname{43.7}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/from40/100\endcsname{21.1}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/from40/1000\endcsname{14.3}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/from40/25\endcsname{26.6}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/0\endcsname{1.9}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/100\endcsname{-0.6}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/100-ci\endcsname{-1.9 to 0.8}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/1000\endcsname{-1.2}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/1000-ci\endcsname{-1.8 to -0.6}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/25\endcsname{-1.3}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/gain/25-ci\endcsname{-2.7 to -0.3}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/main\endcsname{15.4}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/pre/0\endcsname{45.7}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/pre/100\endcsname{20.5}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/pre/1000\endcsname{13.1}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/pre/25\endcsname{25.3}
\expandafter\def\csname v@ho/whisper-large-v3-turbo/stage1\endcsname{13.6}
\expandafter\def\csname v@ho/whisper-small/from40/0\endcsname{50.8}
\expandafter\def\csname v@ho/whisper-small/from40/100\endcsname{25.1}
\expandafter\def\csname v@ho/whisper-small/from40/1000\endcsname{17.0}
\expandafter\def\csname v@ho/whisper-small/from40/25\endcsname{31.0}
\expandafter\def\csname v@ho/whisper-small/gain/0\endcsname{11.0}
\expandafter\def\csname v@ho/whisper-small/gain/100\endcsname{-0.5}
\expandafter\def\csname v@ho/whisper-small/gain/100-ci\endcsname{-1.3 to 0.3}
\expandafter\def\csname v@ho/whisper-small/gain/1000\endcsname{0.3}
\expandafter\def\csname v@ho/whisper-small/gain/1000-ci\endcsname{-1.0 to 1.6}
\expandafter\def\csname v@ho/whisper-small/gain/25\endcsname{-0.2}
\expandafter\def\csname v@ho/whisper-small/gain/25-ci\endcsname{-1.7 to 1.2}
\expandafter\def\csname v@ho/whisper-small/main\endcsname{17.9}
\expandafter\def\csname v@ho/whisper-small/pre/0\endcsname{61.7}
\expandafter\def\csname v@ho/whisper-small/pre/100\endcsname{24.6}
\expandafter\def\csname v@ho/whisper-small/pre/1000\endcsname{17.3}
\expandafter\def\csname v@ho/whisper-small/pre/25\endcsname{30.8}
\expandafter\def\csname v@ho/whisper-small/stage1\endcsname{16.7}
\expandafter\def\csname v@kin/nemotron-30b/gap\endcsname{1.7}
\expandafter\def\csname v@kin/nemotron-30b/listed/n\endcsname{4}
\expandafter\def\csname v@kin/nemotron-30b/listed/tuned\endcsname{4.0}
\expandafter\def\csname v@kin/nemotron-30b/listed/untouched\endcsname{3.7}
\expandafter\def\csname v@kin/nemotron-30b/none/n\endcsname{12}
\expandafter\def\csname v@kin/nemotron-30b/none/tuned\endcsname{16.7}
\expandafter\def\csname v@kin/nemotron-30b/none/untouched\endcsname{61.2}
\expandafter\def\csname v@kin/nemotron-30b/relative/n\endcsname{20}
\expandafter\def\csname v@kin/nemotron-30b/relative/tuned\endcsname{15.0}
\expandafter\def\csname v@kin/nemotron-30b/relative/untouched\endcsname{50.7}
\expandafter\def\csname v@kin/nemotron-stream/gap\endcsname{-1.1}
\expandafter\def\csname v@kin/nemotron-stream/listed/n\endcsname{4}
\expandafter\def\csname v@kin/nemotron-stream/listed/tuned\endcsname{20.8}
\expandafter\def\csname v@kin/nemotron-stream/listed/untouched\endcsname{9.7}
\expandafter\def\csname v@kin/nemotron-stream/none/n\endcsname{14}
\expandafter\def\csname v@kin/nemotron-stream/none/tuned\endcsname{33.8}
\expandafter\def\csname v@kin/nemotron-stream/none/untouched\endcsname{76.2}
\expandafter\def\csname v@kin/nemotron-stream/relative/n\endcsname{18}
\expandafter\def\csname v@kin/nemotron-stream/relative/tuned\endcsname{35.0}
\expandafter\def\csname v@kin/nemotron-stream/relative/untouched\endcsname{65.3}
\expandafter\def\csname v@kin/parakeet-tdt-v3/gap\endcsname{2.1}
\expandafter\def\csname v@kin/parakeet-tdt-v3/listed/n\endcsname{4}
\expandafter\def\csname v@kin/parakeet-tdt-v3/listed/tuned\endcsname{5.4}
\expandafter\def\csname v@kin/parakeet-tdt-v3/listed/untouched\endcsname{5.3}
\expandafter\def\csname v@kin/parakeet-tdt-v3/none/n\endcsname{22}
\expandafter\def\csname v@kin/parakeet-tdt-v3/none/tuned\endcsname{18.3}
\expandafter\def\csname v@kin/parakeet-tdt-v3/none/untouched\endcsname{53.2}
\expandafter\def\csname v@kin/parakeet-tdt-v3/relative/n\endcsname{10}
\expandafter\def\csname v@kin/parakeet-tdt-v3/relative/tuned\endcsname{16.2}
\expandafter\def\csname v@kin/parakeet-tdt-v3/relative/untouched\endcsname{36.0}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/gap\endcsname{1.4}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/listed/n\endcsname{1}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/listed/tuned\endcsname{18.4}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/listed/untouched\endcsname{13.0}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/none/n\endcsname{12}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/none/tuned\endcsname{18.2}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/none/untouched\endcsname{59.2}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/relative/n\endcsname{23}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/relative/tuned\endcsname{16.8}
\expandafter\def\csname v@kin/qwen3-asr-0.6b/relative/untouched\endcsname{51.5}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/gap\endcsname{1.4}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/listed/n\endcsname{1}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/listed/tuned\endcsname{15.1}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/listed/untouched\endcsname{8.6}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/none/n\endcsname{12}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/none/tuned\endcsname{16.7}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/none/untouched\endcsname{51.9}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/relative/n\endcsname{23}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/relative/tuned\endcsname{15.3}
\expandafter\def\csname v@kin/qwen3-asr-1.7b/relative/untouched\endcsname{52.0}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/gap\endcsname{-4.4}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/listed/n\endcsname{11}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/listed/tuned\endcsname{10.8}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/listed/untouched\endcsname{20.3}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/none/n\endcsname{4}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/none/names\endcsname{Karamojong, Southern Pastaza Quechua, Teso, Wayuu}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/none/tuned\endcsname{10.2}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/none/untouched\endcsname{61.7}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/relative/n\endcsname{21}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/relative/tuned\endcsname{14.6}
\expandafter\def\csname v@kin/whisper-large-v3-turbo/relative/untouched\endcsname{58.3}
\expandafter\def\csname v@kin/whisper-large-v3/gap\endcsname{-4.4}
\expandafter\def\csname v@kin/whisper-large-v3/listed/n\endcsname{11}
\expandafter\def\csname v@kin/whisper-large-v3/listed/tuned\endcsname{8.5}
\expandafter\def\csname v@kin/whisper-large-v3/listed/untouched\endcsname{18.1}
\expandafter\def\csname v@kin/whisper-large-v3/none/n\endcsname{4}
\expandafter\def\csname v@kin/whisper-large-v3/none/names\endcsname{Karamojong, Southern Pastaza Quechua, Teso, Wayuu}
\expandafter\def\csname v@kin/whisper-large-v3/none/tuned\endcsname{10.2}
\expandafter\def\csname v@kin/whisper-large-v3/none/untouched\endcsname{55.2}
\expandafter\def\csname v@kin/whisper-large-v3/relative/n\endcsname{21}
\expandafter\def\csname v@kin/whisper-large-v3/relative/tuned\endcsname{14.6}
\expandafter\def\csname v@kin/whisper-large-v3/relative/untouched\endcsname{56.5}
\expandafter\def\csname v@kin/whisper-medium/gap\endcsname{-4.8}
\expandafter\def\csname v@kin/whisper-medium/listed/n\endcsname{11}
\expandafter\def\csname v@kin/whisper-medium/listed/tuned\endcsname{10.5}
\expandafter\def\csname v@kin/whisper-medium/listed/untouched\endcsname{35.0}
\expandafter\def\csname v@kin/whisper-medium/none/n\endcsname{4}
\expandafter\def\csname v@kin/whisper-medium/none/names\endcsname{Karamojong, Southern Pastaza Quechua, Teso, Wayuu}
\expandafter\def\csname v@kin/whisper-medium/none/tuned\endcsname{10.9}
\expandafter\def\csname v@kin/whisper-medium/none/untouched\endcsname{74.0}
\expandafter\def\csname v@kin/whisper-medium/relative/n\endcsname{21}
\expandafter\def\csname v@kin/whisper-medium/relative/tuned\endcsname{15.6}
\expandafter\def\csname v@kin/whisper-medium/relative/untouched\endcsname{66.9}
\expandafter\def\csname v@kin/whisper-small/gap\endcsname{-6.1}
\expandafter\def\csname v@kin/whisper-small/listed/n\endcsname{11}
\expandafter\def\csname v@kin/whisper-small/listed/tuned\endcsname{13.4}
\expandafter\def\csname v@kin/whisper-small/listed/untouched\endcsname{35.0}
\expandafter\def\csname v@kin/whisper-small/none/n\endcsname{4}
\expandafter\def\csname v@kin/whisper-small/none/names\endcsname{Karamojong, Southern Pastaza Quechua, Teso, Wayuu}
\expandafter\def\csname v@kin/whisper-small/none/tuned\endcsname{11.4}
\expandafter\def\csname v@kin/whisper-small/none/untouched\endcsname{68.5}
\expandafter\def\csname v@kin/whisper-small/relative/n\endcsname{21}
\expandafter\def\csname v@kin/whisper-small/relative/tuned\endcsname{17.5}
\expandafter\def\csname v@kin/whisper-small/relative/untouched\endcsname{70.2}
\expandafter\def\csname v@kin/whisper-tiny/gap\endcsname{-9.4}
\expandafter\def\csname v@kin/whisper-tiny/listed/n\endcsname{11}
\expandafter\def\csname v@kin/whisper-tiny/listed/tuned\endcsname{22.9}
\expandafter\def\csname v@kin/whisper-tiny/listed/untouched\endcsname{41.3}
\expandafter\def\csname v@kin/whisper-tiny/none/n\endcsname{4}
\expandafter\def\csname v@kin/whisper-tiny/none/names\endcsname{Karamojong, Southern Pastaza Quechua, Teso, Wayuu}
\expandafter\def\csname v@kin/whisper-tiny/none/tuned\endcsname{17.1}
\expandafter\def\csname v@kin/whisper-tiny/none/untouched\endcsname{68.1}
\expandafter\def\csname v@kin/whisper-tiny/relative/n\endcsname{21}
\expandafter\def\csname v@kin/whisper-tiny/relative/tuned\endcsname{26.5}
\expandafter\def\csname v@kin/whisper-tiny/relative/untouched\endcsname{65.8}
\expandafter\def\csname v@late/none-pending\endcsname{1}
\expandafter\def\csname v@ld/e0-max\endcsname{29}
\expandafter\def\csname v@ld/e0-min\endcsname{15}
\expandafter\def\csname v@ld/kept-max\endcsname{5.1}
\expandafter\def\csname v@ld/kept-min\endcsname{2.6}
\expandafter\def\csname v@ld/lfm3/all/best\endcsname{4.3}
\expandafter\def\csname v@ld/lfm3/all/best-ci\endcsname{0.0 to 5.3}
\expandafter\def\csname v@ld/lfm3/all/e0\endcsname{29.9}
\expandafter\def\csname v@ld/lfm3/all/e0-ci\endcsname{0.0 to 34.7}
\expandafter\def\csname v@ld/lfm3/all/e1\endcsname{5.2}
\expandafter\def\csname v@ld/lfm3/all/e1-ci\endcsname{0.0 to 7.1}
\expandafter\def\csname v@ld/lfm3/all/e10\endcsname{4.1}
\expandafter\def\csname v@ld/lfm3/all/e10-ci\endcsname{0.0 to 5.0}
\expandafter\def\csname v@ld/lfm3/all/e2\endcsname{2.9}
\expandafter\def\csname v@ld/lfm3/all/e2-ci\endcsname{0.0 to 3.8}
\expandafter\def\csname v@ld/lfm3/all/e3\endcsname{3.4}
\expandafter\def\csname v@ld/lfm3/all/e3-ci\endcsname{0.0 to 4.6}
\expandafter\def\csname v@ld/lfm3/all/e5\endcsname{5.1}
\expandafter\def\csname v@ld/lfm3/all/e5-ci\endcsname{0.0 to 6.2}
\expandafter\def\csname v@ld/lfm3/all/n\endcsname{1}
\expandafter\def\csname v@ld/lfm3/latin/best\endcsname{4.2}
\expandafter\def\csname v@ld/lfm3/latin/best-ci\endcsname{0.0 to 5.2}
\expandafter\def\csname v@ld/lfm3/latin/e0\endcsname{31.0}
\expandafter\def\csname v@ld/lfm3/latin/e0-ci\endcsname{0.0 to 36.5}
\expandafter\def\csname v@ld/lfm3/latin/e1\endcsname{4.9}
\expandafter\def\csname v@ld/lfm3/latin/e1-ci\endcsname{0.0 to 6.5}
\expandafter\def\csname v@ld/lfm3/latin/e10\endcsname{4.0}
\expandafter\def\csname v@ld/lfm3/latin/e10-ci\endcsname{0.0 to 4.9}
\expandafter\def\csname v@ld/lfm3/latin/e2\endcsname{2.9}
\expandafter\def\csname v@ld/lfm3/latin/e2-ci\endcsname{0.0 to 3.8}
\expandafter\def\csname v@ld/lfm3/latin/e3\endcsname{3.3}
\expandafter\def\csname v@ld/lfm3/latin/e3-ci\endcsname{0.0 to 4.5}
\expandafter\def\csname v@ld/lfm3/latin/e5\endcsname{4.9}
\expandafter\def\csname v@ld/lfm3/latin/e5-ci\endcsname{0.0 to 6.0}
\expandafter\def\csname v@ld/lfm3/latin/n\endcsname{1}
\expandafter\def\csname v@ld/mms/all/best\endcsname{3.1}
\expandafter\def\csname v@ld/mms/all/best-ci\endcsname{1.4 to 4.9}
\expandafter\def\csname v@ld/mms/all/e0\endcsname{32.3}
\expandafter\def\csname v@ld/mms/all/e0-ci\endcsname{19.1 to 44.1}
\expandafter\def\csname v@ld/mms/all/e1\endcsname{6.5}
\expandafter\def\csname v@ld/mms/all/e1-ci\endcsname{2.5 to 10.4}
\expandafter\def\csname v@ld/mms/all/e10\endcsname{3.2}
\expandafter\def\csname v@ld/mms/all/e10-ci\endcsname{1.5 to 4.9}
\expandafter\def\csname v@ld/mms/all/e2\endcsname{5.4}
\expandafter\def\csname v@ld/mms/all/e2-ci\endcsname{3.1 to 8.0}
\expandafter\def\csname v@ld/mms/all/e3\endcsname{3.6}
\expandafter\def\csname v@ld/mms/all/e3-ci\endcsname{-0.2 to 6.7}
\expandafter\def\csname v@ld/mms/all/e5\endcsname{3.9}
\expandafter\def\csname v@ld/mms/all/e5-ci\endcsname{2.1 to 5.9}
\expandafter\def\csname v@ld/mms/all/n\endcsname{26}
\expandafter\def\csname v@ld/mms/latin/best\endcsname{2.6}
\expandafter\def\csname v@ld/mms/latin/best-ci\endcsname{0.9 to 4.2}
\expandafter\def\csname v@ld/mms/latin/e0\endcsname{14.5}
\expandafter\def\csname v@ld/mms/latin/e0-ci\endcsname{3.2 to 24.9}
\expandafter\def\csname v@ld/mms/latin/e1\endcsname{5.4}
\expandafter\def\csname v@ld/mms/latin/e1-ci\endcsname{1.7 to 8.8}
\expandafter\def\csname v@ld/mms/latin/e10\endcsname{2.7}
\expandafter\def\csname v@ld/mms/latin/e10-ci\endcsname{1.0 to 4.4}
\expandafter\def\csname v@ld/mms/latin/e2\endcsname{5.3}
\expandafter\def\csname v@ld/mms/latin/e2-ci\endcsname{2.9 to 7.8}
\expandafter\def\csname v@ld/mms/latin/e3\endcsname{3.4}
\expandafter\def\csname v@ld/mms/latin/e3-ci\endcsname{-1.4 to 7.1}
\expandafter\def\csname v@ld/mms/latin/e5\endcsname{3.6}
\expandafter\def\csname v@ld/mms/latin/e5-ci\endcsname{1.8 to 5.5}
\expandafter\def\csname v@ld/mms/latin/n\endcsname{18}
\expandafter\def\csname v@ld/n-latin\endcsname{36}
\expandafter\def\csname v@ld/n-models\endcsname{24}
\expandafter\def\csname v@ld/omni/all/best\endcsname{2.4}
\expandafter\def\csname v@ld/omni/all/best-ci\endcsname{-0.3 to 5.4}
\expandafter\def\csname v@ld/omni/all/e0\endcsname{31.3}
\expandafter\def\csname v@ld/omni/all/e0-ci\endcsname{23.2 to 39.8}
\expandafter\def\csname v@ld/omni/all/e1\endcsname{9.8}
\expandafter\def\csname v@ld/omni/all/e1-ci\endcsname{2.0 to 21.5}
\expandafter\def\csname v@ld/omni/all/e10\endcsname{2.3}
\expandafter\def\csname v@ld/omni/all/e10-ci\endcsname{-0.4 to 5.5}
\expandafter\def\csname v@ld/omni/all/e2\endcsname{8.3}
\expandafter\def\csname v@ld/omni/all/e2-ci\endcsname{1.5 to 19.8}
\expandafter\def\csname v@ld/omni/all/e3\endcsname{6.9}
\expandafter\def\csname v@ld/omni/all/e3-ci\endcsname{0.0 to 18.9}
\expandafter\def\csname v@ld/omni/all/e5\endcsname{6.9}
\expandafter\def\csname v@ld/omni/all/e5-ci\endcsname{0.0 to 18.8}
\expandafter\def\csname v@ld/omni/all/n\endcsname{34}
\expandafter\def\csname v@ld/omni/latin/best\endcsname{-0.2}
\expandafter\def\csname v@ld/omni/latin/best-ci\endcsname{-1.8 to 1.4}
\expandafter\def\csname v@ld/omni/latin/e0\endcsname{27.4}
\expandafter\def\csname v@ld/omni/latin/e0-ci\endcsname{19.7 to 35.7}
\expandafter\def\csname v@ld/omni/latin/e1\endcsname{3.3}
\expandafter\def\csname v@ld/omni/latin/e1-ci\endcsname{0.6 to 5.5}
\expandafter\def\csname v@ld/omni/latin/e10\endcsname{-0.4}
\expandafter\def\csname v@ld/omni/latin/e10-ci\endcsname{-2.1 to 1.3}
\expandafter\def\csname v@ld/omni/latin/e2\endcsname{2.3}
\expandafter\def\csname v@ld/omni/latin/e2-ci\endcsname{0.6 to 3.8}
\expandafter\def\csname v@ld/omni/latin/e3\endcsname{0.3}
\expandafter\def\csname v@ld/omni/latin/e3-ci\endcsname{-1.7 to 2.3}
\expandafter\def\csname v@ld/omni/latin/e5\endcsname{-0.1}
\expandafter\def\csname v@ld/omni/latin/e5-ci\endcsname{-1.7 to 1.4}
\expandafter\def\csname v@ld/omni/latin/gone-epoch\endcsname{three epochs}
\expandafter\def\csname v@ld/omni/latin/n\endcsname{25}
\expandafter\def\csname v@ld/qwen/all/best\endcsname{-7.2}
\expandafter\def\csname v@ld/qwen/all/best-ci\endcsname{-7.9 to 0.0}
\expandafter\def\csname v@ld/qwen/all/e0\endcsname{19.0}
\expandafter\def\csname v@ld/qwen/all/e0-ci\endcsname{0.0 to 23.7}
\expandafter\def\csname v@ld/qwen/all/e1\endcsname{-7.2}
\expandafter\def\csname v@ld/qwen/all/e1-ci\endcsname{-8.5 to 0.0}
\expandafter\def\csname v@ld/qwen/all/e10\endcsname{-6.0}
\expandafter\def\csname v@ld/qwen/all/e10-ci\endcsname{-6.5 to 0.0}
\expandafter\def\csname v@ld/qwen/all/e2\endcsname{-5.9}
\expandafter\def\csname v@ld/qwen/all/e2-ci\endcsname{-6.7 to 0.0}
\expandafter\def\csname v@ld/qwen/all/e3\endcsname{-9.0}
\expandafter\def\csname v@ld/qwen/all/e3-ci\endcsname{-9.9 to 0.0}
\expandafter\def\csname v@ld/qwen/all/e5\endcsname{-7.0}
\expandafter\def\csname v@ld/qwen/all/e5-ci\endcsname{-7.6 to 0.0}
\expandafter\def\csname v@ld/qwen/all/n\endcsname{1}
\expandafter\def\csname v@ld/qwen/latin/best\endcsname{-7.3}
\expandafter\def\csname v@ld/qwen/latin/best-ci\endcsname{-8.0 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/e0\endcsname{20.1}
\expandafter\def\csname v@ld/qwen/latin/e0-ci\endcsname{0.0 to 25.6}
\expandafter\def\csname v@ld/qwen/latin/e1\endcsname{-7.5}
\expandafter\def\csname v@ld/qwen/latin/e1-ci\endcsname{-8.2 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/e10\endcsname{-6.0}
\expandafter\def\csname v@ld/qwen/latin/e10-ci\endcsname{-6.5 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/e2\endcsname{-5.8}
\expandafter\def\csname v@ld/qwen/latin/e2-ci\endcsname{-6.6 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/e3\endcsname{-9.2}
\expandafter\def\csname v@ld/qwen/latin/e3-ci\endcsname{-10.1 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/e5\endcsname{-7.2}
\expandafter\def\csname v@ld/qwen/latin/e5-ci\endcsname{-7.7 to 0.0}
\expandafter\def\csname v@ld/qwen/latin/n\endcsname{1}
\expandafter\def\csname v@ld/short/all/best\endcsname{5.1}
\expandafter\def\csname v@ld/short/all/best-ci\endcsname{3.3 to 6.7}
\expandafter\def\csname v@ld/short/all/e0\endcsname{27.8}
\expandafter\def\csname v@ld/short/all/e0-ci\endcsname{23.2 to 31.9}
\expandafter\def\csname v@ld/short/all/e1\endcsname{9.3}
\expandafter\def\csname v@ld/short/all/e1-ci\endcsname{6.3 to 12.2}
\expandafter\def\csname v@ld/short/all/e10\endcsname{5.4}
\expandafter\def\csname v@ld/short/all/e10-ci\endcsname{3.3 to 7.3}
\expandafter\def\csname v@ld/short/all/e2\endcsname{8.1}
\expandafter\def\csname v@ld/short/all/e2-ci\endcsname{5.5 to 10.3}
\expandafter\def\csname v@ld/short/all/e3\endcsname{9.0}
\expandafter\def\csname v@ld/short/all/e3-ci\endcsname{5.1 to 12.6}
\expandafter\def\csname v@ld/short/all/e5\endcsname{6.2}
\expandafter\def\csname v@ld/short/all/e5-ci\endcsname{4.0 to 8.7}
\expandafter\def\csname v@ld/short/all/n\endcsname{4}
\expandafter\def\csname v@ld/short/latin/best\endcsname{5.1}
\expandafter\def\csname v@ld/short/latin/best-ci\endcsname{2.9 to 6.6}
\expandafter\def\csname v@ld/short/latin/e0\endcsname{29.3}
\expandafter\def\csname v@ld/short/latin/e0-ci\endcsname{23.9 to 33.9}
\expandafter\def\csname v@ld/short/latin/e1\endcsname{9.0}
\expandafter\def\csname v@ld/short/latin/e1-ci\endcsname{5.8 to 11.6}
\expandafter\def\csname v@ld/short/latin/e10\endcsname{5.3}
\expandafter\def\csname v@ld/short/latin/e10-ci\endcsname{3.0 to 7.2}
\expandafter\def\csname v@ld/short/latin/e2\endcsname{8.2}
\expandafter\def\csname v@ld/short/latin/e2-ci\endcsname{5.4 to 10.5}
\expandafter\def\csname v@ld/short/latin/e3\endcsname{8.8}
\expandafter\def\csname v@ld/short/latin/e3-ci\endcsname{4.6 to 12.1}
\expandafter\def\csname v@ld/short/latin/e5\endcsname{6.0}
\expandafter\def\csname v@ld/short/latin/e5-ci\endcsname{3.9 to 8.6}
\expandafter\def\csname v@ld/short/latin/n\endcsname{4}
\expandafter\def\csname v@ld/w2v/all/best\endcsname{2.7}
\expandafter\def\csname v@ld/w2v/all/best-ci\endcsname{0.7 to 4.7}
\expandafter\def\csname v@ld/w2v/all/e1\endcsname{7.1}
\expandafter\def\csname v@ld/w2v/all/e1-ci\endcsname{1.7 to 12.0}
\expandafter\def\csname v@ld/w2v/all/e10\endcsname{2.8}
\expandafter\def\csname v@ld/w2v/all/e10-ci\endcsname{0.5 to 4.9}
\expandafter\def\csname v@ld/w2v/all/e2\endcsname{4.7}
\expandafter\def\csname v@ld/w2v/all/e2-ci\endcsname{2.3 to 7.2}
\expandafter\def\csname v@ld/w2v/all/e3\endcsname{4.1}
\expandafter\def\csname v@ld/w2v/all/e3-ci\endcsname{1.9 to 6.3}
\expandafter\def\csname v@ld/w2v/all/e5\endcsname{3.7}
\expandafter\def\csname v@ld/w2v/all/e5-ci\endcsname{1.4 to 6.1}
\expandafter\def\csname v@ld/w2v/all/n\endcsname{11}
\expandafter\def\csname v@ld/w2v/latin/best\endcsname{3.4}
\expandafter\def\csname v@ld/w2v/latin/best-ci\endcsname{1.5 to 5.3}
\expandafter\def\csname v@ld/w2v/latin/e1\endcsname{9.9}
\expandafter\def\csname v@ld/w2v/latin/e1-ci\endcsname{6.9 to 12.9}
\expandafter\def\csname v@ld/w2v/latin/e10\endcsname{2.9}
\expandafter\def\csname v@ld/w2v/latin/e10-ci\endcsname{1.1 to 4.5}
\expandafter\def\csname v@ld/w2v/latin/e2\endcsname{6.8}
\expandafter\def\csname v@ld/w2v/latin/e2-ci\endcsname{4.0 to 9.4}
\expandafter\def\csname v@ld/w2v/latin/e3\endcsname{5.7}
\expandafter\def\csname v@ld/w2v/latin/e3-ci\endcsname{3.1 to 7.9}
\expandafter\def\csname v@ld/w2v/latin/e5\endcsname{5.3}
\expandafter\def\csname v@ld/w2v/latin/e5-ci\endcsname{3.0 to 7.5}
\expandafter\def\csname v@ld/w2v/latin/n\endcsname{7}
\expandafter\def\csname v@ld/whisper/all/best\endcsname{-1.1}
\expandafter\def\csname v@ld/whisper/all/best-ci\endcsname{-2.3 to 0.0}
\expandafter\def\csname v@ld/whisper/all/e0\endcsname{10.7}
\expandafter\def\csname v@ld/whisper/all/e0-ci\endcsname{2.7 to 18.7}
\expandafter\def\csname v@ld/whisper/all/e1\endcsname{-0.9}
\expandafter\def\csname v@ld/whisper/all/e1-ci\endcsname{-5.1 to 2.8}
\expandafter\def\csname v@ld/whisper/all/e10\endcsname{-1.0}
\expandafter\def\csname v@ld/whisper/all/e10-ci\endcsname{-2.0 to 0.1}
\expandafter\def\csname v@ld/whisper/all/e2\endcsname{-1.7}
\expandafter\def\csname v@ld/whisper/all/e2-ci\endcsname{-4.2 to 0.2}
\expandafter\def\csname v@ld/whisper/all/e3\endcsname{-1.6}
\expandafter\def\csname v@ld/whisper/all/e3-ci\endcsname{-3.5 to 0.1}
\expandafter\def\csname v@ld/whisper/all/e5\endcsname{-1.0}
\expandafter\def\csname v@ld/whisper/all/e5-ci\endcsname{-2.3 to 0.4}
\expandafter\def\csname v@ld/whisper/all/n\endcsname{17}
\expandafter\def\csname v@ld/whisper/latin/best\endcsname{-0.9}
\expandafter\def\csname v@ld/whisper/latin/best-ci\endcsname{-1.9 to 0.1}
\expandafter\def\csname v@ld/whisper/latin/e0\endcsname{16.8}
\expandafter\def\csname v@ld/whisper/latin/e0-ci\endcsname{7.5 to 25.5}
\expandafter\def\csname v@ld/whisper/latin/e1\endcsname{-1.1}
\expandafter\def\csname v@ld/whisper/latin/e1-ci\endcsname{-2.4 to 0.4}
\expandafter\def\csname v@ld/whisper/latin/e10\endcsname{-0.7}
\expandafter\def\csname v@ld/whisper/latin/e10-ci\endcsname{-1.8 to 0.5}
\expandafter\def\csname v@ld/whisper/latin/e2\endcsname{-0.7}
\expandafter\def\csname v@ld/whisper/latin/e2-ci\endcsname{-1.7 to 0.4}
\expandafter\def\csname v@ld/whisper/latin/e3\endcsname{-1.1}
\expandafter\def\csname v@ld/whisper/latin/e3-ci\endcsname{-2.6 to 0.3}
\expandafter\def\csname v@ld/whisper/latin/e5\endcsname{-0.5}
\expandafter\def\csname v@ld/whisper/latin/e5-ci\endcsname{-1.5 to 0.6}
\expandafter\def\csname v@ld/whisper/latin/gone-epoch\endcsname{one epoch}
\expandafter\def\csname v@ld/whisper/latin/n\endcsname{11}
\expandafter\def\csname v@lh/behind/max\endcsname{15.6}
\expandafter\def\csname v@lh/behind/min\endcsname{7.3}
\expandafter\def\csname v@lh/behind/n\endcsname{3}
\expandafter\def\csname v@lh/behind/names\endcsname{Burmese, Tibetan and Lao}
\expandafter\def\csname v@lh/behind/redecode-max\endcsname{4.0}
\expandafter\def\csname v@lh/ref-names\endcsname{MMS 1B, omniASR CTC 1B and w2v-BERT 2.0}
\expandafter\def\csname v@lm/best/cer\endcsname{9.8}
\expandafter\def\csname v@lm/best/name\endcsname{MMS 1B}
\expandafter\def\csname v@lm/best/wer\endcsname{34.4}
\expandafter\def\csname v@lm/cer-gain-max\endcsname{1.4}
\expandafter\def\csname v@lm/cer-gain-min\endcsname{1.2}
\expandafter\def\csname v@lm/mms-1b/alpha\endcsname{0.25}
\expandafter\def\csname v@lm/mms-1b/beta\endcsname{2}
\expandafter\def\csname v@lm/mms-1b/cer-gain\endcsname{1.3}
\expandafter\def\csname v@lm/mms-1b/greedy-cer\endcsname{11.1}
\expandafter\def\csname v@lm/mms-1b/greedy-wer\endcsname{40.1}
\expandafter\def\csname v@lm/mms-1b/lm-cer\endcsname{9.8}
\expandafter\def\csname v@lm/mms-1b/lm-wer\endcsname{34.4}
\expandafter\def\csname v@lm/mms-1b/wer-gain\endcsname{5.7}
\expandafter\def\csname v@lm/mms-1b/wer-gain-ci\endcsname{4.8 to 6.4}
\expandafter\def\csname v@lm/n\endcsname{3}
\expandafter\def\csname v@lm/omni-ctc-1b/alpha\endcsname{0.25}
\expandafter\def\csname v@lm/omni-ctc-1b/beta\endcsname{1}
\expandafter\def\csname v@lm/omni-ctc-1b/cer-gain\endcsname{1.2}
\expandafter\def\csname v@lm/omni-ctc-1b/greedy-cer\endcsname{12.0}
\expandafter\def\csname v@lm/omni-ctc-1b/greedy-wer\endcsname{43.1}
\expandafter\def\csname v@lm/omni-ctc-1b/lm-cer\endcsname{10.8}
\expandafter\def\csname v@lm/omni-ctc-1b/lm-wer\endcsname{38.3}
\expandafter\def\csname v@lm/omni-ctc-1b/wer-gain\endcsname{4.8}
\expandafter\def\csname v@lm/omni-ctc-1b/wer-gain-ci\endcsname{4.1 to 5.4}
\expandafter\def\csname v@lm/oov-max\endcsname{68.8}
\expandafter\def\csname v@lm/oov-median\endcsname{20.7}
\expandafter\def\csname v@lm/oov-min\endcsname{0.0}
\expandafter\def\csname v@lm/sentences-median\endcsname{3,213}
\expandafter\def\csname v@lm/sentences-min\endcsname{96}
\expandafter\def\csname v@lm/w2v-bert/alpha\endcsname{0.25}
\expandafter\def\csname v@lm/w2v-bert/beta\endcsname{2}
\expandafter\def\csname v@lm/w2v-bert/cer-gain\endcsname{1.4}
\expandafter\def\csname v@lm/w2v-bert/greedy-cer\endcsname{12.7}
\expandafter\def\csname v@lm/w2v-bert/greedy-wer\endcsname{44.8}
\expandafter\def\csname v@lm/w2v-bert/lm-cer\endcsname{11.3}
\expandafter\def\csname v@lm/w2v-bert/lm-wer\endcsname{38.8}
\expandafter\def\csname v@lm/w2v-bert/wer-gain\endcsname{6.0}
\expandafter\def\csname v@lm/w2v-bert/wer-gain-ci\endcsname{5.0 to 6.7}
\expandafter\def\csname v@lm/wer-gain-max\endcsname{6.0}
\expandafter\def\csname v@lm/wer-gain-min\endcsname{4.8}
\expandafter\def\csname v@lm/words-median\endcsname{30,102}
\expandafter\def\csname v@loss/ep20_mms-1b/1\endcsname{1.64}
\expandafter\def\csname v@loss/ep20_mms-1b/10\endcsname{0.47}
\expandafter\def\csname v@loss/ep20_mms-1b/20\endcsname{0.31}
\expandafter\def\csname v@loss/ep20_mms-1b/3\endcsname{0.65}
\expandafter\def\csname v@loss/ep20_mms-1b/5\endcsname{0.55}
\expandafter\def\csname v@loss/ep20_omni-ctc-1b/1\endcsname{2.06}
\expandafter\def\csname v@loss/ep20_omni-ctc-1b/10\endcsname{0.35}
\expandafter\def\csname v@loss/ep20_omni-ctc-1b/20\endcsname{0.19}
\expandafter\def\csname v@loss/ep20_omni-ctc-1b/3\endcsname{0.65}
\expandafter\def\csname v@loss/ep20_omni-ctc-1b/5\endcsname{0.55}
\expandafter\def\csname v@loss/ep20_parakeet-tdt-v3/1\endcsname{21.56}
\expandafter\def\csname v@loss/ep20_parakeet-tdt-v3/10\endcsname{1.21}
\expandafter\def\csname v@loss/ep20_parakeet-tdt-v3/20\endcsname{0.98}
\expandafter\def\csname v@loss/ep20_parakeet-tdt-v3/3\endcsname{2.48}
\expandafter\def\csname v@loss/ep20_parakeet-tdt-v3/5\endcsname{1.95}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/1\endcsname{1.04}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/10\endcsname{0.04}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/20\endcsname{0.02}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/3\endcsname{0.34}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/30\endcsname{0.01}
\expandafter\def\csname v@loss/ep30_qwen3-asr-0.6b/5\endcsname{0.15}
\expandafter\def\csname v@loss/ep30_w2v-bert/1\endcsname{4.55}
\expandafter\def\csname v@loss/ep30_w2v-bert/10\endcsname{0.49}
\expandafter\def\csname v@loss/ep30_w2v-bert/20\endcsname{0.31}
\expandafter\def\csname v@loss/ep30_w2v-bert/3\endcsname{0.89}
\expandafter\def\csname v@loss/ep30_w2v-bert/30\endcsname{0.19}
\expandafter\def\csname v@loss/ep30_w2v-bert/5\endcsname{0.68}
\expandafter\def\csname v@loss/ep30_whisper-small/1\endcsname{1.13}
\expandafter\def\csname v@loss/ep30_whisper-small/10\endcsname{0.03}
\expandafter\def\csname v@loss/ep30_whisper-small/20\endcsname{0.01}
\expandafter\def\csname v@loss/ep30_whisper-small/3\endcsname{0.27}
\expandafter\def\csname v@loss/ep30_whisper-small/30\endcsname{0.01}
\expandafter\def\csname v@loss/ep30_whisper-small/5\endcsname{0.11}
\expandafter\def\csname v@lr/cohere-transcribe\endcsname{3e-5}
\expandafter\def\csname v@lr/cohere-transcribe/best-dev\endcsname{37.0}
\expandafter\def\csname v@lr/cohere-transcribe/used\endcsname{3e-5}
\expandafter\def\csname v@lr/gemma4-12b\endcsname{3e-6}
\expandafter\def\csname v@lr/gemma4-12b/best-dev\endcsname{35.2}
\expandafter\def\csname v@lr/gemma4-12b/used\endcsname{3e-6}
\expandafter\def\csname v@lr/gemma4-e2b\endcsname{1e-5}
\expandafter\def\csname v@lr/gemma4-e2b/best-dev\endcsname{31.5}
\expandafter\def\csname v@lr/gemma4-e2b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/gemma4-e4b\endcsname{3e-6}
\expandafter\def\csname v@lr/gemma4-e4b/best-dev\endcsname{30.2}
\expandafter\def\csname v@lr/gemma4-e4b/used\endcsname{3e-6}
\expandafter\def\csname v@lr/granite-2b\endcsname{1e-5}
\expandafter\def\csname v@lr/granite-2b/best-dev\endcsname{40.4}
\expandafter\def\csname v@lr/granite-2b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/lfm3-audio\endcsname{1e-5}
\expandafter\def\csname v@lr/lfm3-audio/best-dev\endcsname{32.0}
\expandafter\def\csname v@lr/lfm3-audio/used\endcsname{1e-5}
\expandafter\def\csname v@lr/mms-1b\endcsname{1e-5}
\expandafter\def\csname v@lr/mms-1b/best-dev\endcsname{23.5}
\expandafter\def\csname v@lr/mms-1b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/nemotron-stream\endcsname{1e-4}
\expandafter\def\csname v@lr/nemotron-stream/best-dev\endcsname{69.0}
\expandafter\def\csname v@lr/nemotron-stream/used\endcsname{1e-4}
\expandafter\def\csname v@lr/omni-ctc-1b\endcsname{3e-5}
\expandafter\def\csname v@lr/omni-ctc-1b/best-dev\endcsname{24.4}
\expandafter\def\csname v@lr/omni-ctc-1b/used\endcsname{3e-5}
\expandafter\def\csname v@lr/omni-ctc-300m\endcsname{3e-5}
\expandafter\def\csname v@lr/omni-ctc-300m/best-dev\endcsname{28.1}
\expandafter\def\csname v@lr/omni-ctc-300m/used\endcsname{3e-5}
\expandafter\def\csname v@lr/omni-ctc-7b\endcsname{1e-5}
\expandafter\def\csname v@lr/omni-ctc-7b/best-dev\endcsname{20.8}
\expandafter\def\csname v@lr/omni-ctc-7b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/parakeet-tdt-v3\endcsname{3e-4}
\expandafter\def\csname v@lr/parakeet-tdt-v3/best-dev\endcsname{43.6}
\expandafter\def\csname v@lr/parakeet-tdt-v3/used\endcsname{3e-4}
\expandafter\def\csname v@lr/qwen3-asr-0.6b\endcsname{3e-6}
\expandafter\def\csname v@lr/qwen3-asr-0.6b/best-dev\endcsname{34.8}
\expandafter\def\csname v@lr/qwen3-asr-0.6b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/qwen3-asr-1.7b\endcsname{3e-6}
\expandafter\def\csname v@lr/qwen3-asr-1.7b/best-dev\endcsname{30.3}
\expandafter\def\csname v@lr/qwen3-asr-1.7b/used\endcsname{1e-5}
\expandafter\def\csname v@lr/voxtral-mini\endcsname{3e-6}
\expandafter\def\csname v@lr/voxtral-mini/best-dev\endcsname{29.5}
\expandafter\def\csname v@lr/voxtral-mini/used\endcsname{3e-6}
\expandafter\def\csname v@lr/w2v-bert\endcsname{3e-5}
\expandafter\def\csname v@lr/w2v-bert/best-dev\endcsname{40.8}
\expandafter\def\csname v@lr/w2v-bert/used\endcsname{3e-5}
\expandafter\def\csname v@lr/whisper-base\endcsname{1e-4}
\expandafter\def\csname v@lr/whisper-base/best-dev\endcsname{39.3}
\expandafter\def\csname v@lr/whisper-base/used\endcsname{1e-4}
\expandafter\def\csname v@lr/whisper-large-v3\endcsname{1e-5}
\expandafter\def\csname v@lr/whisper-large-v3-turbo\endcsname{1e-5}
\expandafter\def\csname v@lr/whisper-large-v3-turbo/best-dev\endcsname{32.1}
\expandafter\def\csname v@lr/whisper-large-v3-turbo/used\endcsname{1e-5}
\expandafter\def\csname v@lr/whisper-large-v3/best-dev\endcsname{29.3}
\expandafter\def\csname v@lr/whisper-large-v3/used\endcsname{1e-5}
\expandafter\def\csname v@lr/whisper-medium\endcsname{3e-5}
\expandafter\def\csname v@lr/whisper-medium/best-dev\endcsname{32.7}
\expandafter\def\csname v@lr/whisper-medium/used\endcsname{1e-5}
\expandafter\def\csname v@lr/whisper-small\endcsname{3e-5}
\expandafter\def\csname v@lr/whisper-small/best-dev\endcsname{35.0}
\expandafter\def\csname v@lr/whisper-small/used\endcsname{3e-5}
\expandafter\def\csname v@lr/whisper-tiny\endcsname{1e-4}
\expandafter\def\csname v@lr/whisper-tiny/best-dev\endcsname{47.1}
\expandafter\def\csname v@lr/whisper-tiny/used\endcsname{1e-4}
\expandafter\def\csname v@lrlow/gemma/both\endcsname{1}
\expandafter\def\csname v@lrlow/gemma4-12b/chosen\endcsname{3e-6}
\expandafter\def\csname v@lrlow/gemma4-12b/dev-chosen\endcsname{28.1}
\expandafter\def\csname v@lrlow/gemma4-12b/dev-other\endcsname{28.4}
\expandafter\def\csname v@lrlow/gemma4-12b/other\endcsname{1e-6}
\expandafter\def\csname v@lrlow/gemma4-12b/test-chosen\endcsname{19.8}
\expandafter\def\csname v@lrlow/gemma4-12b/test-other\endcsname{20.8}
\expandafter\def\csname v@lrlow/gemma4-e4b/chosen\endcsname{3e-6}
\expandafter\def\csname v@lrlow/gemma4-e4b/dev-chosen\endcsname{24.7}
\expandafter\def\csname v@lrlow/gemma4-e4b/dev-other\endcsname{26.5}
\expandafter\def\csname v@lrlow/gemma4-e4b/other\endcsname{1e-6}
\expandafter\def\csname v@lrlow/gemma4-e4b/test-chosen\endcsname{16.6}
\expandafter\def\csname v@lrlow/gemma4-e4b/test-other\endcsname{18.5}
\expandafter\def\csname v@lrr/spread-max\endcsname{3.6}
\expandafter\def\csname v@lrr/spread-median\endcsname{0.9}
\expandafter\def\csname v@lrrep/parakeet-tdt-v3/1e-4\endcsname{47.0}
\expandafter\def\csname v@lrrep/w2v-bert/1e-4\endcsname{100.0}
\expandafter\def\csname v@my/bench-cats\endcsname{12}
\expandafter\def\csname v@my/bench-clips\endcsname{820}
\expandafter\def\csname v@my/bench-hours\endcsname{2.1}
\expandafter\def\csname v@my/best-untouched/cer\endcsname{8.4}
\expandafter\def\csname v@my/best-untouched/how\endcsname{told Malay}
\expandafter\def\csname v@my/best-untouched/name\endcsname{Gemma 4 E4B}
\expandafter\def\csname v@my/best-untouched/wer\endcsname{17.1}
\expandafter\def\csname v@my/best/after\endcsname{6.0}
\expandafter\def\csname v@my/best/base\endcsname{8.9}
\expandafter\def\csname v@my/best/base-wer\endcsname{14.9}
\expandafter\def\csname v@my/best/key\endcsname{whisper-large-v3}
\expandafter\def\csname v@my/best/name\endcsname{Whisper large-v3}
\expandafter\def\csname v@my/best/wer\endcsname{13.3}
\expandafter\def\csname v@my/canary-1b-v2/base\endcsname{49.3}
\expandafter\def\csname v@my/canary-1b-v2/base-wer\endcsname{81.9}
\expandafter\def\csname v@my/canary-1b-v2/base/animation\endcsname{55.9}
\expandafter\def\csname v@my/canary-1b-v2/base/commonvoice\endcsname{41.7}
\expandafter\def\csname v@my/canary-1b-v2/base/drama\endcsname{61.0}
\expandafter\def\csname v@my/canary-1b-v2/base/fleurs\endcsname{35.8}
\expandafter\def\csname v@my/canary-1b-v2/base/news\endcsname{32.2}
\expandafter\def\csname v@my/canary-1b-v2/base/parliament\endcsname{49.1}
\expandafter\def\csname v@my/canary-1b-v2/base/podcast\endcsname{59.3}
\expandafter\def\csname v@my/canary-1b-v2/base/read-speech\endcsname{50.2}
\expandafter\def\csname v@my/canary-1b-v2/base/short-inputs\endcsname{36.1}
\expandafter\def\csname v@my/canary-1b-v2/base/singing\endcsname{79.7}
\expandafter\def\csname v@my/canary-1b-v2/base/street interview\endcsname{70.8}
\expandafter\def\csname v@my/canary-1b-v2/base/telephony\endcsname{19.9}
\expandafter\def\csname v@my/canary-1b-v2/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/canary-1b-v2/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/canary-1b-v2/left\endcsname{49.3}
\expandafter\def\csname v@my/canary-1b-v2/left-wer\endcsname{81.9}
\expandafter\def\csname v@my/canary-1b-v2/left/animation\endcsname{55.9}
\expandafter\def\csname v@my/canary-1b-v2/left/commonvoice\endcsname{41.7}
\expandafter\def\csname v@my/canary-1b-v2/left/drama\endcsname{61.0}
\expandafter\def\csname v@my/canary-1b-v2/left/fleurs\endcsname{35.8}
\expandafter\def\csname v@my/canary-1b-v2/left/news\endcsname{32.2}
\expandafter\def\csname v@my/canary-1b-v2/left/parliament\endcsname{49.1}
\expandafter\def\csname v@my/canary-1b-v2/left/podcast\endcsname{59.3}
\expandafter\def\csname v@my/canary-1b-v2/left/read-speech\endcsname{50.2}
\expandafter\def\csname v@my/canary-1b-v2/left/short-inputs\endcsname{36.1}
\expandafter\def\csname v@my/canary-1b-v2/left/singing\endcsname{79.7}
\expandafter\def\csname v@my/canary-1b-v2/left/street interview\endcsname{70.8}
\expandafter\def\csname v@my/canary-1b-v2/left/telephony\endcsname{19.9}
\expandafter\def\csname v@my/cohere-transcribe/after\endcsname{12.1}
\expandafter\def\csname v@my/cohere-transcribe/after-wer\endcsname{29.6}
\expandafter\def\csname v@my/cohere-transcribe/animation\endcsname{11.4}
\expandafter\def\csname v@my/cohere-transcribe/base\endcsname{58.5}
\expandafter\def\csname v@my/cohere-transcribe/base-wer\endcsname{82.2}
\expandafter\def\csname v@my/cohere-transcribe/base/animation\endcsname{67.9}
\expandafter\def\csname v@my/cohere-transcribe/base/commonvoice\endcsname{53.5}
\expandafter\def\csname v@my/cohere-transcribe/base/drama\endcsname{70.0}
\expandafter\def\csname v@my/cohere-transcribe/base/fleurs\endcsname{58.4}
\expandafter\def\csname v@my/cohere-transcribe/base/news\endcsname{52.8}
\expandafter\def\csname v@my/cohere-transcribe/base/parliament\endcsname{88.8}
\expandafter\def\csname v@my/cohere-transcribe/base/podcast\endcsname{70.8}
\expandafter\def\csname v@my/cohere-transcribe/base/read-speech\endcsname{47.5}
\expandafter\def\csname v@my/cohere-transcribe/base/short-inputs\endcsname{30.6}
\expandafter\def\csname v@my/cohere-transcribe/base/singing\endcsname{69.8}
\expandafter\def\csname v@my/cohere-transcribe/base/street interview\endcsname{68.4}
\expandafter\def\csname v@my/cohere-transcribe/base/telephony\endcsname{23.1}
\expandafter\def\csname v@my/cohere-transcribe/commonvoice\endcsname{8.3}
\expandafter\def\csname v@my/cohere-transcribe/curve-dev-first\endcsname{20.3}
\expandafter\def\csname v@my/cohere-transcribe/curve-dev-last\endcsname{20.9}
\expandafter\def\csname v@my/cohere-transcribe/curve-first\endcsname{12.6}
\expandafter\def\csname v@my/cohere-transcribe/curve-last\endcsname{14.0}
\expandafter\def\csname v@my/cohere-transcribe/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/cohere-transcribe/curve-low\endcsname{12.1}
\expandafter\def\csname v@my/cohere-transcribe/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/cohere-transcribe/curve-pick\endcsname{12.1}
\expandafter\def\csname v@my/cohere-transcribe/drama\endcsname{11.6}
\expandafter\def\csname v@my/cohere-transcribe/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/cohere-transcribe/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/cohere-transcribe/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/cohere-transcribe/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/cohere-transcribe/epoch\endcsname{3}
\expandafter\def\csname v@my/cohere-transcribe/fleurs\endcsname{9.2}
\expandafter\def\csname v@my/cohere-transcribe/gain\endcsname{46.4}
\expandafter\def\csname v@my/cohere-transcribe/gain-ci\endcsname{43.9 to 48.6}
\expandafter\def\csname v@my/cohere-transcribe/left\endcsname{58.5}
\expandafter\def\csname v@my/cohere-transcribe/left-wer\endcsname{82.2}
\expandafter\def\csname v@my/cohere-transcribe/left/animation\endcsname{67.9}
\expandafter\def\csname v@my/cohere-transcribe/left/commonvoice\endcsname{53.5}
\expandafter\def\csname v@my/cohere-transcribe/left/drama\endcsname{70.0}
\expandafter\def\csname v@my/cohere-transcribe/left/fleurs\endcsname{58.4}
\expandafter\def\csname v@my/cohere-transcribe/left/news\endcsname{52.8}
\expandafter\def\csname v@my/cohere-transcribe/left/parliament\endcsname{88.8}
\expandafter\def\csname v@my/cohere-transcribe/left/podcast\endcsname{70.8}
\expandafter\def\csname v@my/cohere-transcribe/left/read-speech\endcsname{47.5}
\expandafter\def\csname v@my/cohere-transcribe/left/short-inputs\endcsname{30.6}
\expandafter\def\csname v@my/cohere-transcribe/left/singing\endcsname{69.8}
\expandafter\def\csname v@my/cohere-transcribe/left/street interview\endcsname{68.4}
\expandafter\def\csname v@my/cohere-transcribe/left/telephony\endcsname{23.1}
\expandafter\def\csname v@my/cohere-transcribe/news\endcsname{8.1}
\expandafter\def\csname v@my/cohere-transcribe/parliament\endcsname{10.4}
\expandafter\def\csname v@my/cohere-transcribe/podcast\endcsname{6.5}
\expandafter\def\csname v@my/cohere-transcribe/rank\endcsname{12}
\expandafter\def\csname v@my/cohere-transcribe/rank-word\endcsname{twelfth best}
\expandafter\def\csname v@my/cohere-transcribe/read-speech\endcsname{8.3}
\expandafter\def\csname v@my/cohere-transcribe/short-inputs\endcsname{6.4}
\expandafter\def\csname v@my/cohere-transcribe/singing\endcsname{36.1}
\expandafter\def\csname v@my/cohere-transcribe/street interview\endcsname{16.3}
\expandafter\def\csname v@my/cohere-transcribe/telephony\endcsname{12.7}
\expandafter\def\csname v@my/curve-early\endcsname{16}
\expandafter\def\csname v@my/curve-n\endcsname{24}
\expandafter\def\csname v@my/dev-clips\endcsname{454}
\expandafter\def\csname v@my/down-by\endcsname{by up to}
\expandafter\def\csname v@my/down-n\endcsname{2}
\expandafter\def\csname v@my/down-names\endcsname{Gemma 4 E2B and Qwen3-ASR 0.6B}
\expandafter\def\csname v@my/down-points\endcsname{2.8}
\expandafter\def\csname v@my/down-verb\endcsname{end}
\expandafter\def\csname v@my/en-clips\endcsname{91}
\expandafter\def\csname v@my/flat-n\endcsname{3}
\expandafter\def\csname v@my/flat-names\endcsname{Whisper large-v3-turbo, Whisper base and Qwen3-ASR 1.7B}
\expandafter\def\csname v@my/flat-verb\endcsname{end}
\expandafter\def\csname v@my/fun-asr-nano/base\endcsname{52.9}
\expandafter\def\csname v@my/fun-asr-nano/base-wer\endcsname{81.6}
\expandafter\def\csname v@my/fun-asr-nano/base/animation\endcsname{70.8}
\expandafter\def\csname v@my/fun-asr-nano/base/commonvoice\endcsname{49.4}
\expandafter\def\csname v@my/fun-asr-nano/base/drama\endcsname{70.4}
\expandafter\def\csname v@my/fun-asr-nano/base/fleurs\endcsname{44.6}
\expandafter\def\csname v@my/fun-asr-nano/base/news\endcsname{33.5}
\expandafter\def\csname v@my/fun-asr-nano/base/parliament\endcsname{42.7}
\expandafter\def\csname v@my/fun-asr-nano/base/podcast\endcsname{51.0}
\expandafter\def\csname v@my/fun-asr-nano/base/read-speech\endcsname{53.0}
\expandafter\def\csname v@my/fun-asr-nano/base/short-inputs\endcsname{38.0}
\expandafter\def\csname v@my/fun-asr-nano/base/singing\endcsname{84.4}
\expandafter\def\csname v@my/fun-asr-nano/base/street interview\endcsname{70.7}
\expandafter\def\csname v@my/fun-asr-nano/base/telephony\endcsname{26.2}
\expandafter\def\csname v@my/fun-asr-nano/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/fun-asr-nano/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/fun-asr-nano/left\endcsname{52.9}
\expandafter\def\csname v@my/fun-asr-nano/left-wer\endcsname{81.6}
\expandafter\def\csname v@my/fun-asr-nano/left/animation\endcsname{70.8}
\expandafter\def\csname v@my/fun-asr-nano/left/commonvoice\endcsname{49.4}
\expandafter\def\csname v@my/fun-asr-nano/left/drama\endcsname{70.4}
\expandafter\def\csname v@my/fun-asr-nano/left/fleurs\endcsname{44.6}
\expandafter\def\csname v@my/fun-asr-nano/left/news\endcsname{33.5}
\expandafter\def\csname v@my/fun-asr-nano/left/parliament\endcsname{42.7}
\expandafter\def\csname v@my/fun-asr-nano/left/podcast\endcsname{51.0}
\expandafter\def\csname v@my/fun-asr-nano/left/read-speech\endcsname{53.0}
\expandafter\def\csname v@my/fun-asr-nano/left/short-inputs\endcsname{38.0}
\expandafter\def\csname v@my/fun-asr-nano/left/singing\endcsname{84.4}
\expandafter\def\csname v@my/fun-asr-nano/left/street interview\endcsname{70.7}
\expandafter\def\csname v@my/fun-asr-nano/left/telephony\endcsname{26.2}
\expandafter\def\csname v@my/gain-max\endcsname{46.4}
\expandafter\def\csname v@my/gain-min\endcsname{-2.8}
\expandafter\def\csname v@my/gemma4-12b/after\endcsname{21.4}
\expandafter\def\csname v@my/gemma4-12b/after-wer\endcsname{39.5}
\expandafter\def\csname v@my/gemma4-12b/animation\endcsname{21.7}
\expandafter\def\csname v@my/gemma4-12b/base\endcsname{57.9}
\expandafter\def\csname v@my/gemma4-12b/base-wer\endcsname{73.6}
\expandafter\def\csname v@my/gemma4-12b/base/animation\endcsname{74.8}
\expandafter\def\csname v@my/gemma4-12b/base/commonvoice\endcsname{39.0}
\expandafter\def\csname v@my/gemma4-12b/base/drama\endcsname{74.9}
\expandafter\def\csname v@my/gemma4-12b/base/fleurs\endcsname{29.7}
\expandafter\def\csname v@my/gemma4-12b/base/news\endcsname{39.3}
\expandafter\def\csname v@my/gemma4-12b/base/parliament\endcsname{42.8}
\expandafter\def\csname v@my/gemma4-12b/base/podcast\endcsname{51.7}
\expandafter\def\csname v@my/gemma4-12b/base/read-speech\endcsname{63.4}
\expandafter\def\csname v@my/gemma4-12b/base/short-inputs\endcsname{71.1}
\expandafter\def\csname v@my/gemma4-12b/base/singing\endcsname{90.2}
\expandafter\def\csname v@my/gemma4-12b/base/street interview\endcsname{78.1}
\expandafter\def\csname v@my/gemma4-12b/base/telephony\endcsname{40.1}
\expandafter\def\csname v@my/gemma4-12b/commonvoice\endcsname{12.9}
\expandafter\def\csname v@my/gemma4-12b/curve-dev-first\endcsname{26.8}
\expandafter\def\csname v@my/gemma4-12b/curve-dev-last\endcsname{24.4}
\expandafter\def\csname v@my/gemma4-12b/curve-first\endcsname{25.6}
\expandafter\def\csname v@my/gemma4-12b/curve-last\endcsname{21.5}
\expandafter\def\csname v@my/gemma4-12b/curve-last-epoch\endcsname{3}
\expandafter\def\csname v@my/gemma4-12b/curve-low\endcsname{21.4}
\expandafter\def\csname v@my/gemma4-12b/curve-low-epoch\endcsname{2}
\expandafter\def\csname v@my/gemma4-12b/curve-pick\endcsname{21.4}
\expandafter\def\csname v@my/gemma4-12b/detect\endcsname{61.0}
\expandafter\def\csname v@my/gemma4-12b/detect-en-as-ms\endcsname{0}
\expandafter\def\csname v@my/gemma4-12b/detect-ms-as-en\endcsname{117}
\expandafter\def\csname v@my/gemma4-12b/detect-wer\endcsname{76.8}
\expandafter\def\csname v@my/gemma4-12b/detect/telephony\endcsname{44.7}
\expandafter\def\csname v@my/gemma4-12b/drama\endcsname{23.1}
\expandafter\def\csname v@my/gemma4-12b/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/gemma4-12b/en-as-ms-after\endcsname{1}
\expandafter\def\csname v@my/gemma4-12b/en-as-ms-after-word\endcsname{1}
\expandafter\def\csname v@my/gemma4-12b/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/gemma4-12b/epoch\endcsname{2}
\expandafter\def\csname v@my/gemma4-12b/fleurs\endcsname{21.7}
\expandafter\def\csname v@my/gemma4-12b/gain\endcsname{36.5}
\expandafter\def\csname v@my/gemma4-12b/gain-ci\endcsname{33.5 to 39.4}
\expandafter\def\csname v@my/gemma4-12b/left\endcsname{61.0}
\expandafter\def\csname v@my/gemma4-12b/left-wer\endcsname{76.8}
\expandafter\def\csname v@my/gemma4-12b/left/animation\endcsname{73.3}
\expandafter\def\csname v@my/gemma4-12b/left/commonvoice\endcsname{40.9}
\expandafter\def\csname v@my/gemma4-12b/left/drama\endcsname{75.0}
\expandafter\def\csname v@my/gemma4-12b/left/fleurs\endcsname{35.7}
\expandafter\def\csname v@my/gemma4-12b/left/news\endcsname{39.4}
\expandafter\def\csname v@my/gemma4-12b/left/parliament\endcsname{46.2}
\expandafter\def\csname v@my/gemma4-12b/left/podcast\endcsname{57.7}
\expandafter\def\csname v@my/gemma4-12b/left/read-speech\endcsname{69.4}
\expandafter\def\csname v@my/gemma4-12b/left/short-inputs\endcsname{76.7}
\expandafter\def\csname v@my/gemma4-12b/left/singing\endcsname{93.5}
\expandafter\def\csname v@my/gemma4-12b/left/street interview\endcsname{79.0}
\expandafter\def\csname v@my/gemma4-12b/left/telephony\endcsname{44.7}
\expandafter\def\csname v@my/gemma4-12b/news\endcsname{18.7}
\expandafter\def\csname v@my/gemma4-12b/parliament\endcsname{17.8}
\expandafter\def\csname v@my/gemma4-12b/podcast\endcsname{13.1}
\expandafter\def\csname v@my/gemma4-12b/rank\endcsname{20}
\expandafter\def\csname v@my/gemma4-12b/read-speech\endcsname{12.5}
\expandafter\def\csname v@my/gemma4-12b/short-inputs\endcsname{5.4}
\expandafter\def\csname v@my/gemma4-12b/singing\endcsname{65.0}
\expandafter\def\csname v@my/gemma4-12b/street interview\endcsname{25.7}
\expandafter\def\csname v@my/gemma4-12b/telephony\endcsname{19.3}
\expandafter\def\csname v@my/gemma4-12b/told\endcsname{57.9}
\expandafter\def\csname v@my/gemma4-12b/told-gain\endcsname{36.5}
\expandafter\def\csname v@my/gemma4-12b/told-wer\endcsname{73.6}
\expandafter\def\csname v@my/gemma4-12b/told/animation\endcsname{74.8}
\expandafter\def\csname v@my/gemma4-12b/told/commonvoice\endcsname{39.0}
\expandafter\def\csname v@my/gemma4-12b/told/drama\endcsname{74.9}
\expandafter\def\csname v@my/gemma4-12b/told/fleurs\endcsname{29.7}
\expandafter\def\csname v@my/gemma4-12b/told/news\endcsname{39.3}
\expandafter\def\csname v@my/gemma4-12b/told/parliament\endcsname{42.8}
\expandafter\def\csname v@my/gemma4-12b/told/podcast\endcsname{51.7}
\expandafter\def\csname v@my/gemma4-12b/told/read-speech\endcsname{63.4}
\expandafter\def\csname v@my/gemma4-12b/told/short-inputs\endcsname{71.1}
\expandafter\def\csname v@my/gemma4-12b/told/singing\endcsname{90.2}
\expandafter\def\csname v@my/gemma4-12b/told/street interview\endcsname{78.1}
\expandafter\def\csname v@my/gemma4-12b/told/telephony\endcsname{40.1}
\expandafter\def\csname v@my/gemma4-e2b/after\endcsname{12.1}
\expandafter\def\csname v@my/gemma4-e2b/after-wer\endcsname{24.3}
\expandafter\def\csname v@my/gemma4-e2b/animation\endcsname{11.7}
\expandafter\def\csname v@my/gemma4-e2b/base\endcsname{9.3}
\expandafter\def\csname v@my/gemma4-e2b/base-wer\endcsname{20.0}
\expandafter\def\csname v@my/gemma4-e2b/base/animation\endcsname{6.6}
\expandafter\def\csname v@my/gemma4-e2b/base/commonvoice\endcsname{3.5}
\expandafter\def\csname v@my/gemma4-e2b/base/drama\endcsname{10.1}
\expandafter\def\csname v@my/gemma4-e2b/base/fleurs\endcsname{2.9}
\expandafter\def\csname v@my/gemma4-e2b/base/news\endcsname{3.3}
\expandafter\def\csname v@my/gemma4-e2b/base/parliament\endcsname{4.9}
\expandafter\def\csname v@my/gemma4-e2b/base/podcast\endcsname{7.4}
\expandafter\def\csname v@my/gemma4-e2b/base/read-speech\endcsname{5.5}
\expandafter\def\csname v@my/gemma4-e2b/base/short-inputs\endcsname{11.6}
\expandafter\def\csname v@my/gemma4-e2b/base/singing\endcsname{18.7}
\expandafter\def\csname v@my/gemma4-e2b/base/street interview\endcsname{15.6}
\expandafter\def\csname v@my/gemma4-e2b/base/telephony\endcsname{21.4}
\expandafter\def\csname v@my/gemma4-e2b/commonvoice\endcsname{6.0}
\expandafter\def\csname v@my/gemma4-e2b/curve-dev-first\endcsname{23.1}
\expandafter\def\csname v@my/gemma4-e2b/curve-dev-last\endcsname{22.9}
\expandafter\def\csname v@my/gemma4-e2b/curve-first\endcsname{13.1}
\expandafter\def\csname v@my/gemma4-e2b/curve-last\endcsname{13.4}
\expandafter\def\csname v@my/gemma4-e2b/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/gemma4-e2b/curve-low\endcsname{11.8}
\expandafter\def\csname v@my/gemma4-e2b/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/gemma4-e2b/curve-pick\endcsname{12.1}
\expandafter\def\csname v@my/gemma4-e2b/detect\endcsname{11.0}
\expandafter\def\csname v@my/gemma4-e2b/detect-en-as-ms\endcsname{1}
\expandafter\def\csname v@my/gemma4-e2b/detect-ms-as-en\endcsname{4}
\expandafter\def\csname v@my/gemma4-e2b/detect-wer\endcsname{21.9}
\expandafter\def\csname v@my/gemma4-e2b/detect/telephony\endcsname{23.2}
\expandafter\def\csname v@my/gemma4-e2b/drama\endcsname{13.6}
\expandafter\def\csname v@my/gemma4-e2b/en-as-ms\endcsname{4}
\expandafter\def\csname v@my/gemma4-e2b/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/gemma4-e2b/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/gemma4-e2b/en-as-ms-share\endcsname{2}
\expandafter\def\csname v@my/gemma4-e2b/epoch\endcsname{2}
\expandafter\def\csname v@my/gemma4-e2b/fleurs\endcsname{9.3}
\expandafter\def\csname v@my/gemma4-e2b/gain\endcsname{-2.8}
\expandafter\def\csname v@my/gemma4-e2b/gain-ci\endcsname{-3.9 to -1.9}
\expandafter\def\csname v@my/gemma4-e2b/left\endcsname{11.0}
\expandafter\def\csname v@my/gemma4-e2b/left-wer\endcsname{21.9}
\expandafter\def\csname v@my/gemma4-e2b/left/animation\endcsname{7.4}
\expandafter\def\csname v@my/gemma4-e2b/left/commonvoice\endcsname{3.4}
\expandafter\def\csname v@my/gemma4-e2b/left/drama\endcsname{10.9}
\expandafter\def\csname v@my/gemma4-e2b/left/fleurs\endcsname{3.0}
\expandafter\def\csname v@my/gemma4-e2b/left/news\endcsname{3.3}
\expandafter\def\csname v@my/gemma4-e2b/left/parliament\endcsname{6.7}
\expandafter\def\csname v@my/gemma4-e2b/left/podcast\endcsname{7.2}
\expandafter\def\csname v@my/gemma4-e2b/left/read-speech\endcsname{7.9}
\expandafter\def\csname v@my/gemma4-e2b/left/short-inputs\endcsname{20.2}
\expandafter\def\csname v@my/gemma4-e2b/left/singing\endcsname{23.8}
\expandafter\def\csname v@my/gemma4-e2b/left/street interview\endcsname{15.3}
\expandafter\def\csname v@my/gemma4-e2b/left/telephony\endcsname{23.2}
\expandafter\def\csname v@my/gemma4-e2b/news\endcsname{7.0}
\expandafter\def\csname v@my/gemma4-e2b/parliament\endcsname{8.4}
\expandafter\def\csname v@my/gemma4-e2b/podcast\endcsname{9.7}
\expandafter\def\csname v@my/gemma4-e2b/rank\endcsname{13}
\expandafter\def\csname v@my/gemma4-e2b/read-speech\endcsname{6.2}
\expandafter\def\csname v@my/gemma4-e2b/short-inputs\endcsname{2.6}
\expandafter\def\csname v@my/gemma4-e2b/singing\endcsname{37.7}
\expandafter\def\csname v@my/gemma4-e2b/street interview\endcsname{16.7}
\expandafter\def\csname v@my/gemma4-e2b/telephony\endcsname{16.5}
\expandafter\def\csname v@my/gemma4-e2b/told\endcsname{9.3}
\expandafter\def\csname v@my/gemma4-e2b/told-gain\endcsname{-2.8}
\expandafter\def\csname v@my/gemma4-e2b/told-wer\endcsname{20.0}
\expandafter\def\csname v@my/gemma4-e2b/told/animation\endcsname{6.6}
\expandafter\def\csname v@my/gemma4-e2b/told/commonvoice\endcsname{3.5}
\expandafter\def\csname v@my/gemma4-e2b/told/drama\endcsname{10.1}
\expandafter\def\csname v@my/gemma4-e2b/told/fleurs\endcsname{2.9}
\expandafter\def\csname v@my/gemma4-e2b/told/news\endcsname{3.3}
\expandafter\def\csname v@my/gemma4-e2b/told/parliament\endcsname{4.9}
\expandafter\def\csname v@my/gemma4-e2b/told/podcast\endcsname{7.4}
\expandafter\def\csname v@my/gemma4-e2b/told/read-speech\endcsname{5.5}
\expandafter\def\csname v@my/gemma4-e2b/told/short-inputs\endcsname{11.6}
\expandafter\def\csname v@my/gemma4-e2b/told/singing\endcsname{18.7}
\expandafter\def\csname v@my/gemma4-e2b/told/street interview\endcsname{15.6}
\expandafter\def\csname v@my/gemma4-e2b/told/telephony\endcsname{21.4}
\expandafter\def\csname v@my/gemma4-e4b/after\endcsname{7.6}
\expandafter\def\csname v@my/gemma4-e4b/after-wer\endcsname{16.2}
\expandafter\def\csname v@my/gemma4-e4b/animation\endcsname{6.2}
\expandafter\def\csname v@my/gemma4-e4b/base\endcsname{8.4}
\expandafter\def\csname v@my/gemma4-e4b/base-wer\endcsname{17.1}
\expandafter\def\csname v@my/gemma4-e4b/base/animation\endcsname{5.6}
\expandafter\def\csname v@my/gemma4-e4b/base/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/gemma4-e4b/base/drama\endcsname{9.0}
\expandafter\def\csname v@my/gemma4-e4b/base/fleurs\endcsname{2.0}
\expandafter\def\csname v@my/gemma4-e4b/base/news\endcsname{2.7}
\expandafter\def\csname v@my/gemma4-e4b/base/parliament\endcsname{4.2}
\expandafter\def\csname v@my/gemma4-e4b/base/podcast\endcsname{5.5}
\expandafter\def\csname v@my/gemma4-e4b/base/read-speech\endcsname{3.7}
\expandafter\def\csname v@my/gemma4-e4b/base/short-inputs\endcsname{14.3}
\expandafter\def\csname v@my/gemma4-e4b/base/singing\endcsname{15.3}
\expandafter\def\csname v@my/gemma4-e4b/base/street interview\endcsname{14.2}
\expandafter\def\csname v@my/gemma4-e4b/base/telephony\endcsname{20.9}
\expandafter\def\csname v@my/gemma4-e4b/commonvoice\endcsname{3.2}
\expandafter\def\csname v@my/gemma4-e4b/curve-dev-first\endcsname{22.5}
\expandafter\def\csname v@my/gemma4-e4b/curve-dev-last\endcsname{21.6}
\expandafter\def\csname v@my/gemma4-e4b/curve-first\endcsname{7.5}
\expandafter\def\csname v@my/gemma4-e4b/curve-last\endcsname{8.5}
\expandafter\def\csname v@my/gemma4-e4b/curve-last-epoch\endcsname{3}
\expandafter\def\csname v@my/gemma4-e4b/curve-low\endcsname{7.5}
\expandafter\def\csname v@my/gemma4-e4b/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/gemma4-e4b/curve-pick\endcsname{7.6}
\expandafter\def\csname v@my/gemma4-e4b/detect\endcsname{10.2}
\expandafter\def\csname v@my/gemma4-e4b/detect-en-as-ms\endcsname{3}
\expandafter\def\csname v@my/gemma4-e4b/detect-ms-as-en\endcsname{7}
\expandafter\def\csname v@my/gemma4-e4b/detect-wer\endcsname{19.4}
\expandafter\def\csname v@my/gemma4-e4b/detect/telephony\endcsname{23.0}
\expandafter\def\csname v@my/gemma4-e4b/drama\endcsname{7.9}
\expandafter\def\csname v@my/gemma4-e4b/en-as-ms\endcsname{6}
\expandafter\def\csname v@my/gemma4-e4b/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/gemma4-e4b/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/gemma4-e4b/en-as-ms-share\endcsname{3}
\expandafter\def\csname v@my/gemma4-e4b/epoch\endcsname{2}
\expandafter\def\csname v@my/gemma4-e4b/fleurs\endcsname{3.9}
\expandafter\def\csname v@my/gemma4-e4b/gain\endcsname{0.8}
\expandafter\def\csname v@my/gemma4-e4b/gain-ci\endcsname{-0.1 to 1.7}
\expandafter\def\csname v@my/gemma4-e4b/left\endcsname{10.2}
\expandafter\def\csname v@my/gemma4-e4b/left-wer\endcsname{19.4}
\expandafter\def\csname v@my/gemma4-e4b/left/animation\endcsname{6.1}
\expandafter\def\csname v@my/gemma4-e4b/left/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/gemma4-e4b/left/drama\endcsname{9.0}
\expandafter\def\csname v@my/gemma4-e4b/left/fleurs\endcsname{2.1}
\expandafter\def\csname v@my/gemma4-e4b/left/news\endcsname{2.6}
\expandafter\def\csname v@my/gemma4-e4b/left/parliament\endcsname{4.5}
\expandafter\def\csname v@my/gemma4-e4b/left/podcast\endcsname{5.9}
\expandafter\def\csname v@my/gemma4-e4b/left/read-speech\endcsname{8.2}
\expandafter\def\csname v@my/gemma4-e4b/left/short-inputs\endcsname{26.9}
\expandafter\def\csname v@my/gemma4-e4b/left/singing\endcsname{16.5}
\expandafter\def\csname v@my/gemma4-e4b/left/street interview\endcsname{14.2}
\expandafter\def\csname v@my/gemma4-e4b/left/telephony\endcsname{23.0}
\expandafter\def\csname v@my/gemma4-e4b/news\endcsname{3.1}
\expandafter\def\csname v@my/gemma4-e4b/parliament\endcsname{5.5}
\expandafter\def\csname v@my/gemma4-e4b/podcast\endcsname{6.9}
\expandafter\def\csname v@my/gemma4-e4b/rank\endcsname{4}
\expandafter\def\csname v@my/gemma4-e4b/rank-word\endcsname{fourth best}
\expandafter\def\csname v@my/gemma4-e4b/read-speech\endcsname{2.6}
\expandafter\def\csname v@my/gemma4-e4b/short-inputs\endcsname{2.4}
\expandafter\def\csname v@my/gemma4-e4b/singing\endcsname{21.5}
\expandafter\def\csname v@my/gemma4-e4b/street interview\endcsname{13.6}
\expandafter\def\csname v@my/gemma4-e4b/telephony\endcsname{13.8}
\expandafter\def\csname v@my/gemma4-e4b/told\endcsname{8.4}
\expandafter\def\csname v@my/gemma4-e4b/told-gain\endcsname{0.8}
\expandafter\def\csname v@my/gemma4-e4b/told-wer\endcsname{17.1}
\expandafter\def\csname v@my/gemma4-e4b/told/animation\endcsname{5.6}
\expandafter\def\csname v@my/gemma4-e4b/told/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/gemma4-e4b/told/drama\endcsname{9.0}
\expandafter\def\csname v@my/gemma4-e4b/told/fleurs\endcsname{2.0}
\expandafter\def\csname v@my/gemma4-e4b/told/news\endcsname{2.7}
\expandafter\def\csname v@my/gemma4-e4b/told/parliament\endcsname{4.2}
\expandafter\def\csname v@my/gemma4-e4b/told/podcast\endcsname{5.5}
\expandafter\def\csname v@my/gemma4-e4b/told/read-speech\endcsname{3.7}
\expandafter\def\csname v@my/gemma4-e4b/told/short-inputs\endcsname{14.3}
\expandafter\def\csname v@my/gemma4-e4b/told/singing\endcsname{15.3}
\expandafter\def\csname v@my/gemma4-e4b/told/street interview\endcsname{14.2}
\expandafter\def\csname v@my/gemma4-e4b/told/telephony\endcsname{20.9}
\expandafter\def\csname v@my/granite-2b/after\endcsname{25.3}
\expandafter\def\csname v@my/granite-2b/after-wer\endcsname{49.2}
\expandafter\def\csname v@my/granite-2b/animation\endcsname{25.7}
\expandafter\def\csname v@my/granite-2b/base\endcsname{43.5}
\expandafter\def\csname v@my/granite-2b/base-wer\endcsname{79.6}
\expandafter\def\csname v@my/granite-2b/base/animation\endcsname{44.0}
\expandafter\def\csname v@my/granite-2b/base/commonvoice\endcsname{36.4}
\expandafter\def\csname v@my/granite-2b/base/drama\endcsname{43.1}
\expandafter\def\csname v@my/granite-2b/base/fleurs\endcsname{34.6}
\expandafter\def\csname v@my/granite-2b/base/news\endcsname{39.7}
\expandafter\def\csname v@my/granite-2b/base/parliament\endcsname{67.2}
\expandafter\def\csname v@my/granite-2b/base/podcast\endcsname{39.0}
\expandafter\def\csname v@my/granite-2b/base/read-speech\endcsname{46.4}
\expandafter\def\csname v@my/granite-2b/base/short-inputs\endcsname{37.1}
\expandafter\def\csname v@my/granite-2b/base/singing\endcsname{56.1}
\expandafter\def\csname v@my/granite-2b/base/street interview\endcsname{56.8}
\expandafter\def\csname v@my/granite-2b/base/telephony\endcsname{21.5}
\expandafter\def\csname v@my/granite-2b/commonvoice\endcsname{20.7}
\expandafter\def\csname v@my/granite-2b/curve-dev-first\endcsname{28.6}
\expandafter\def\csname v@my/granite-2b/curve-dev-last\endcsname{25.7}
\expandafter\def\csname v@my/granite-2b/curve-first\endcsname{25.8}
\expandafter\def\csname v@my/granite-2b/curve-last\endcsname{26.0}
\expandafter\def\csname v@my/granite-2b/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/granite-2b/curve-low\endcsname{24.5}
\expandafter\def\csname v@my/granite-2b/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/granite-2b/curve-pick\endcsname{25.3}
\expandafter\def\csname v@my/granite-2b/drama\endcsname{23.5}
\expandafter\def\csname v@my/granite-2b/en-as-ms\endcsname{3}
\expandafter\def\csname v@my/granite-2b/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/granite-2b/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/granite-2b/en-as-ms-share\endcsname{1}
\expandafter\def\csname v@my/granite-2b/epoch\endcsname{4}
\expandafter\def\csname v@my/granite-2b/fleurs\endcsname{25.9}
\expandafter\def\csname v@my/granite-2b/gain\endcsname{18.2}
\expandafter\def\csname v@my/granite-2b/gain-ci\endcsname{16.2 to 20.3}
\expandafter\def\csname v@my/granite-2b/left\endcsname{43.5}
\expandafter\def\csname v@my/granite-2b/left-wer\endcsname{79.6}
\expandafter\def\csname v@my/granite-2b/left/animation\endcsname{44.0}
\expandafter\def\csname v@my/granite-2b/left/commonvoice\endcsname{36.4}
\expandafter\def\csname v@my/granite-2b/left/drama\endcsname{43.1}
\expandafter\def\csname v@my/granite-2b/left/fleurs\endcsname{34.6}
\expandafter\def\csname v@my/granite-2b/left/news\endcsname{39.7}
\expandafter\def\csname v@my/granite-2b/left/parliament\endcsname{67.2}
\expandafter\def\csname v@my/granite-2b/left/podcast\endcsname{39.0}
\expandafter\def\csname v@my/granite-2b/left/read-speech\endcsname{46.4}
\expandafter\def\csname v@my/granite-2b/left/short-inputs\endcsname{37.1}
\expandafter\def\csname v@my/granite-2b/left/singing\endcsname{56.1}
\expandafter\def\csname v@my/granite-2b/left/street interview\endcsname{56.8}
\expandafter\def\csname v@my/granite-2b/left/telephony\endcsname{21.5}
\expandafter\def\csname v@my/granite-2b/news\endcsname{21.1}
\expandafter\def\csname v@my/granite-2b/parliament\endcsname{23.9}
\expandafter\def\csname v@my/granite-2b/podcast\endcsname{15.3}
\expandafter\def\csname v@my/granite-2b/rank\endcsname{22}
\expandafter\def\csname v@my/granite-2b/read-speech\endcsname{19.3}
\expandafter\def\csname v@my/granite-2b/short-inputs\endcsname{15.8}
\expandafter\def\csname v@my/granite-2b/singing\endcsname{66.8}
\expandafter\def\csname v@my/granite-2b/street interview\endcsname{30.1}
\expandafter\def\csname v@my/granite-2b/telephony\endcsname{15.4}
\expandafter\def\csname v@my/granite-ctc/base\endcsname{55.9}
\expandafter\def\csname v@my/granite-ctc/base-wer\endcsname{81.0}
\expandafter\def\csname v@my/granite-ctc/base/animation\endcsname{56.8}
\expandafter\def\csname v@my/granite-ctc/base/commonvoice\endcsname{55.6}
\expandafter\def\csname v@my/granite-ctc/base/drama\endcsname{52.4}
\expandafter\def\csname v@my/granite-ctc/base/fleurs\endcsname{51.6}
\expandafter\def\csname v@my/granite-ctc/base/news\endcsname{60.5}
\expandafter\def\csname v@my/granite-ctc/base/parliament\endcsname{76.8}
\expandafter\def\csname v@my/granite-ctc/base/podcast\endcsname{50.6}
\expandafter\def\csname v@my/granite-ctc/base/read-speech\endcsname{47.6}
\expandafter\def\csname v@my/granite-ctc/base/short-inputs\endcsname{38.2}
\expandafter\def\csname v@my/granite-ctc/base/singing\endcsname{82.7}
\expandafter\def\csname v@my/granite-ctc/base/street interview\endcsname{74.2}
\expandafter\def\csname v@my/granite-ctc/base/telephony\endcsname{23.6}
\expandafter\def\csname v@my/granite-ctc/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/granite-ctc/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/granite-ctc/left\endcsname{55.9}
\expandafter\def\csname v@my/granite-ctc/left-wer\endcsname{81.0}
\expandafter\def\csname v@my/granite-ctc/left/animation\endcsname{56.8}
\expandafter\def\csname v@my/granite-ctc/left/commonvoice\endcsname{55.6}
\expandafter\def\csname v@my/granite-ctc/left/drama\endcsname{52.4}
\expandafter\def\csname v@my/granite-ctc/left/fleurs\endcsname{51.6}
\expandafter\def\csname v@my/granite-ctc/left/news\endcsname{60.5}
\expandafter\def\csname v@my/granite-ctc/left/parliament\endcsname{76.8}
\expandafter\def\csname v@my/granite-ctc/left/podcast\endcsname{50.6}
\expandafter\def\csname v@my/granite-ctc/left/read-speech\endcsname{47.6}
\expandafter\def\csname v@my/granite-ctc/left/short-inputs\endcsname{38.2}
\expandafter\def\csname v@my/granite-ctc/left/singing\endcsname{82.7}
\expandafter\def\csname v@my/granite-ctc/left/street interview\endcsname{74.2}
\expandafter\def\csname v@my/granite-ctc/left/telephony\endcsname{23.6}
\expandafter\def\csname v@my/lfm3-audio/after\endcsname{18.1}
\expandafter\def\csname v@my/lfm3-audio/after-wer\endcsname{37.9}
\expandafter\def\csname v@my/lfm3-audio/animation\endcsname{20.0}
\expandafter\def\csname v@my/lfm3-audio/base\endcsname{60.5}
\expandafter\def\csname v@my/lfm3-audio/base-wer\endcsname{82.0}
\expandafter\def\csname v@my/lfm3-audio/base/animation\endcsname{69.2}
\expandafter\def\csname v@my/lfm3-audio/base/commonvoice\endcsname{61.6}
\expandafter\def\csname v@my/lfm3-audio/base/drama\endcsname{80.2}
\expandafter\def\csname v@my/lfm3-audio/base/fleurs\endcsname{58.6}
\expandafter\def\csname v@my/lfm3-audio/base/news\endcsname{51.0}
\expandafter\def\csname v@my/lfm3-audio/base/parliament\endcsname{70.5}
\expandafter\def\csname v@my/lfm3-audio/base/podcast\endcsname{65.1}
\expandafter\def\csname v@my/lfm3-audio/base/read-speech\endcsname{65.2}
\expandafter\def\csname v@my/lfm3-audio/base/short-inputs\endcsname{34.9}
\expandafter\def\csname v@my/lfm3-audio/base/singing\endcsname{71.6}
\expandafter\def\csname v@my/lfm3-audio/base/street interview\endcsname{73.9}
\expandafter\def\csname v@my/lfm3-audio/base/telephony\endcsname{24.6}
\expandafter\def\csname v@my/lfm3-audio/commonvoice\endcsname{14.1}
\expandafter\def\csname v@my/lfm3-audio/curve-dev-first\endcsname{23.1}
\expandafter\def\csname v@my/lfm3-audio/curve-dev-last\endcsname{23.5}
\expandafter\def\csname v@my/lfm3-audio/curve-first\endcsname{17.0}
\expandafter\def\csname v@my/lfm3-audio/curve-last\endcsname{17.1}
\expandafter\def\csname v@my/lfm3-audio/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/lfm3-audio/curve-low\endcsname{17.0}
\expandafter\def\csname v@my/lfm3-audio/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/lfm3-audio/curve-pick\endcsname{18.1}
\expandafter\def\csname v@my/lfm3-audio/drama\endcsname{17.2}
\expandafter\def\csname v@my/lfm3-audio/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/lfm3-audio/en-as-ms-after\endcsname{3}
\expandafter\def\csname v@my/lfm3-audio/en-as-ms-after-word\endcsname{3}
\expandafter\def\csname v@my/lfm3-audio/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/lfm3-audio/epoch\endcsname{3}
\expandafter\def\csname v@my/lfm3-audio/fleurs\endcsname{17.0}
\expandafter\def\csname v@my/lfm3-audio/gain\endcsname{42.4}
\expandafter\def\csname v@my/lfm3-audio/gain-ci\endcsname{39.9 to 44.8}
\expandafter\def\csname v@my/lfm3-audio/left\endcsname{60.5}
\expandafter\def\csname v@my/lfm3-audio/left-wer\endcsname{82.0}
\expandafter\def\csname v@my/lfm3-audio/left/animation\endcsname{69.2}
\expandafter\def\csname v@my/lfm3-audio/left/commonvoice\endcsname{61.6}
\expandafter\def\csname v@my/lfm3-audio/left/drama\endcsname{80.2}
\expandafter\def\csname v@my/lfm3-audio/left/fleurs\endcsname{58.6}
\expandafter\def\csname v@my/lfm3-audio/left/news\endcsname{51.0}
\expandafter\def\csname v@my/lfm3-audio/left/parliament\endcsname{70.5}
\expandafter\def\csname v@my/lfm3-audio/left/podcast\endcsname{65.1}
\expandafter\def\csname v@my/lfm3-audio/left/read-speech\endcsname{65.2}
\expandafter\def\csname v@my/lfm3-audio/left/short-inputs\endcsname{34.9}
\expandafter\def\csname v@my/lfm3-audio/left/singing\endcsname{71.6}
\expandafter\def\csname v@my/lfm3-audio/left/street interview\endcsname{73.9}
\expandafter\def\csname v@my/lfm3-audio/left/telephony\endcsname{24.6}
\expandafter\def\csname v@my/lfm3-audio/news\endcsname{13.4}
\expandafter\def\csname v@my/lfm3-audio/parliament\endcsname{20.0}
\expandafter\def\csname v@my/lfm3-audio/podcast\endcsname{13.4}
\expandafter\def\csname v@my/lfm3-audio/rank\endcsname{18}
\expandafter\def\csname v@my/lfm3-audio/read-speech\endcsname{10.9}
\expandafter\def\csname v@my/lfm3-audio/short-inputs\endcsname{7.1}
\expandafter\def\csname v@my/lfm3-audio/singing\endcsname{44.6}
\expandafter\def\csname v@my/lfm3-audio/street interview\endcsname{23.4}
\expandafter\def\csname v@my/lfm3-audio/telephony\endcsname{16.6}
\expandafter\def\csname v@my/mms-1b-all/after\endcsname{12.2}
\expandafter\def\csname v@my/mms-1b-all/after-wer\endcsname{32.3}
\expandafter\def\csname v@my/mms-1b-all/animation\endcsname{10.4}
\expandafter\def\csname v@my/mms-1b-all/base\endcsname{15.3}
\expandafter\def\csname v@my/mms-1b-all/base-wer\endcsname{40.2}
\expandafter\def\csname v@my/mms-1b-all/base/animation\endcsname{9.7}
\expandafter\def\csname v@my/mms-1b-all/base/commonvoice\endcsname{4.4}
\expandafter\def\csname v@my/mms-1b-all/base/drama\endcsname{17.6}
\expandafter\def\csname v@my/mms-1b-all/base/fleurs\endcsname{1.5}
\expandafter\def\csname v@my/mms-1b-all/base/news\endcsname{5.4}
\expandafter\def\csname v@my/mms-1b-all/base/parliament\endcsname{7.1}
\expandafter\def\csname v@my/mms-1b-all/base/podcast\endcsname{15.3}
\expandafter\def\csname v@my/mms-1b-all/base/read-speech\endcsname{3.4}
\expandafter\def\csname v@my/mms-1b-all/base/short-inputs\endcsname{29.9}
\expandafter\def\csname v@my/mms-1b-all/base/singing\endcsname{24.0}
\expandafter\def\csname v@my/mms-1b-all/base/street interview\endcsname{28.4}
\expandafter\def\csname v@my/mms-1b-all/base/telephony\endcsname{36.7}
\expandafter\def\csname v@my/mms-1b-all/commonvoice\endcsname{5.3}
\expandafter\def\csname v@my/mms-1b-all/drama\endcsname{10.9}
\expandafter\def\csname v@my/mms-1b-all/en-as-ms\endcsname{9}
\expandafter\def\csname v@my/mms-1b-all/en-as-ms-after\endcsname{5}
\expandafter\def\csname v@my/mms-1b-all/en-as-ms-after-word\endcsname{5}
\expandafter\def\csname v@my/mms-1b-all/en-as-ms-share\endcsname{3}
\expandafter\def\csname v@my/mms-1b-all/epoch\endcsname{10}
\expandafter\def\csname v@my/mms-1b-all/fleurs\endcsname{4.6}
\expandafter\def\csname v@my/mms-1b-all/gain\endcsname{3.1}
\expandafter\def\csname v@my/mms-1b-all/gain-ci\endcsname{2.2 to 4.0}
\expandafter\def\csname v@my/mms-1b-all/news\endcsname{5.9}
\expandafter\def\csname v@my/mms-1b-all/parliament\endcsname{7.0}
\expandafter\def\csname v@my/mms-1b-all/podcast\endcsname{6.8}
\expandafter\def\csname v@my/mms-1b-all/rank\endcsname{14}
\expandafter\def\csname v@my/mms-1b-all/read-speech\endcsname{5.5}
\expandafter\def\csname v@my/mms-1b-all/short-inputs\endcsname{14.3}
\expandafter\def\csname v@my/mms-1b-all/singing\endcsname{37.9}
\expandafter\def\csname v@my/mms-1b-all/street interview\endcsname{17.1}
\expandafter\def\csname v@my/mms-1b-all/telephony\endcsname{20.1}
\expandafter\def\csname v@my/mms-1b-all/told\endcsname{15.3}
\expandafter\def\csname v@my/mms-1b-all/told-gain\endcsname{3.1}
\expandafter\def\csname v@my/mms-1b-all/told-wer\endcsname{40.2}
\expandafter\def\csname v@my/mms-1b-all/told/animation\endcsname{9.7}
\expandafter\def\csname v@my/mms-1b-all/told/commonvoice\endcsname{4.4}
\expandafter\def\csname v@my/mms-1b-all/told/drama\endcsname{17.6}
\expandafter\def\csname v@my/mms-1b-all/told/fleurs\endcsname{1.5}
\expandafter\def\csname v@my/mms-1b-all/told/news\endcsname{5.4}
\expandafter\def\csname v@my/mms-1b-all/told/parliament\endcsname{7.1}
\expandafter\def\csname v@my/mms-1b-all/told/podcast\endcsname{15.3}
\expandafter\def\csname v@my/mms-1b-all/told/read-speech\endcsname{3.4}
\expandafter\def\csname v@my/mms-1b-all/told/short-inputs\endcsname{29.9}
\expandafter\def\csname v@my/mms-1b-all/told/singing\endcsname{24.0}
\expandafter\def\csname v@my/mms-1b-all/told/street interview\endcsname{28.4}
\expandafter\def\csname v@my/mms-1b-all/told/telephony\endcsname{36.7}
\expandafter\def\csname v@my/mms-1b/curve-dev-first\endcsname{24.1}
\expandafter\def\csname v@my/mms-1b/curve-dev-last\endcsname{19.6}
\expandafter\def\csname v@my/mms-1b/curve-first\endcsname{12.8}
\expandafter\def\csname v@my/mms-1b/curve-last\endcsname{12.2}
\expandafter\def\csname v@my/mms-1b/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/mms-1b/curve-low\endcsname{11.7}
\expandafter\def\csname v@my/mms-1b/curve-low-epoch\endcsname{4}
\expandafter\def\csname v@my/mms-1b/curve-pick\endcsname{12.2}
\expandafter\def\csname v@my/n\endcsname{24}
\expandafter\def\csname v@my/nemotron-30b/after\endcsname{11.5}
\expandafter\def\csname v@my/nemotron-30b/after-wer\endcsname{26.7}
\expandafter\def\csname v@my/nemotron-30b/animation\endcsname{12.4}
\expandafter\def\csname v@my/nemotron-30b/base\endcsname{28.0}
\expandafter\def\csname v@my/nemotron-30b/base-wer\endcsname{48.7}
\expandafter\def\csname v@my/nemotron-30b/base/animation\endcsname{41.8}
\expandafter\def\csname v@my/nemotron-30b/base/commonvoice\endcsname{10.0}
\expandafter\def\csname v@my/nemotron-30b/base/drama\endcsname{44.9}
\expandafter\def\csname v@my/nemotron-30b/base/fleurs\endcsname{8.3}
\expandafter\def\csname v@my/nemotron-30b/base/news\endcsname{11.9}
\expandafter\def\csname v@my/nemotron-30b/base/parliament\endcsname{20.7}
\expandafter\def\csname v@my/nemotron-30b/base/podcast\endcsname{22.3}
\expandafter\def\csname v@my/nemotron-30b/base/read-speech\endcsname{24.9}
\expandafter\def\csname v@my/nemotron-30b/base/short-inputs\endcsname{30.4}
\expandafter\def\csname v@my/nemotron-30b/base/singing\endcsname{53.0}
\expandafter\def\csname v@my/nemotron-30b/base/street interview\endcsname{50.5}
\expandafter\def\csname v@my/nemotron-30b/base/telephony\endcsname{17.1}
\expandafter\def\csname v@my/nemotron-30b/commonvoice\endcsname{6.8}
\expandafter\def\csname v@my/nemotron-30b/curve-dev-first\endcsname{20.4}
\expandafter\def\csname v@my/nemotron-30b/curve-dev-last\endcsname{20.2}
\expandafter\def\csname v@my/nemotron-30b/curve-first\endcsname{12.1}
\expandafter\def\csname v@my/nemotron-30b/curve-last\endcsname{11.7}
\expandafter\def\csname v@my/nemotron-30b/curve-last-epoch\endcsname{3}
\expandafter\def\csname v@my/nemotron-30b/curve-low\endcsname{11.5}
\expandafter\def\csname v@my/nemotron-30b/curve-low-epoch\endcsname{2}
\expandafter\def\csname v@my/nemotron-30b/curve-pick\endcsname{11.5}
\expandafter\def\csname v@my/nemotron-30b/drama\endcsname{12.4}
\expandafter\def\csname v@my/nemotron-30b/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/nemotron-30b/en-as-ms-after\endcsname{6}
\expandafter\def\csname v@my/nemotron-30b/en-as-ms-after-word\endcsname{6}
\expandafter\def\csname v@my/nemotron-30b/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/nemotron-30b/epoch\endcsname{2}
\expandafter\def\csname v@my/nemotron-30b/fleurs\endcsname{7.6}
\expandafter\def\csname v@my/nemotron-30b/gain\endcsname{16.5}
\expandafter\def\csname v@my/nemotron-30b/gain-ci\endcsname{14.3 to 18.3}
\expandafter\def\csname v@my/nemotron-30b/left\endcsname{28.0}
\expandafter\def\csname v@my/nemotron-30b/left-wer\endcsname{48.7}
\expandafter\def\csname v@my/nemotron-30b/left/animation\endcsname{41.8}
\expandafter\def\csname v@my/nemotron-30b/left/commonvoice\endcsname{10.0}
\expandafter\def\csname v@my/nemotron-30b/left/drama\endcsname{44.9}
\expandafter\def\csname v@my/nemotron-30b/left/fleurs\endcsname{8.3}
\expandafter\def\csname v@my/nemotron-30b/left/news\endcsname{11.9}
\expandafter\def\csname v@my/nemotron-30b/left/parliament\endcsname{20.7}
\expandafter\def\csname v@my/nemotron-30b/left/podcast\endcsname{22.3}
\expandafter\def\csname v@my/nemotron-30b/left/read-speech\endcsname{24.9}
\expandafter\def\csname v@my/nemotron-30b/left/short-inputs\endcsname{30.4}
\expandafter\def\csname v@my/nemotron-30b/left/singing\endcsname{53.0}
\expandafter\def\csname v@my/nemotron-30b/left/street interview\endcsname{50.5}
\expandafter\def\csname v@my/nemotron-30b/left/telephony\endcsname{17.1}
\expandafter\def\csname v@my/nemotron-30b/news\endcsname{7.7}
\expandafter\def\csname v@my/nemotron-30b/parliament\endcsname{10.2}
\expandafter\def\csname v@my/nemotron-30b/podcast\endcsname{6.0}
\expandafter\def\csname v@my/nemotron-30b/rank\endcsname{10}
\expandafter\def\csname v@my/nemotron-30b/rank-word\endcsname{tenth best}
\expandafter\def\csname v@my/nemotron-30b/read-speech\endcsname{7.2}
\expandafter\def\csname v@my/nemotron-30b/short-inputs\endcsname{5.0}
\expandafter\def\csname v@my/nemotron-30b/singing\endcsname{31.9}
\expandafter\def\csname v@my/nemotron-30b/street interview\endcsname{18.2}
\expandafter\def\csname v@my/nemotron-30b/telephony\endcsname{12.8}
\expandafter\def\csname v@my/nemotron-stream/after\endcsname{48.8}
\expandafter\def\csname v@my/nemotron-stream/after-wer\endcsname{77.3}
\expandafter\def\csname v@my/nemotron-stream/animation\endcsname{49.6}
\expandafter\def\csname v@my/nemotron-stream/base\endcsname{73.3}
\expandafter\def\csname v@my/nemotron-stream/base-wer\endcsname{88.4}
\expandafter\def\csname v@my/nemotron-stream/base/animation\endcsname{87.7}
\expandafter\def\csname v@my/nemotron-stream/base/commonvoice\endcsname{76.9}
\expandafter\def\csname v@my/nemotron-stream/base/drama\endcsname{82.6}
\expandafter\def\csname v@my/nemotron-stream/base/fleurs\endcsname{68.4}
\expandafter\def\csname v@my/nemotron-stream/base/news\endcsname{62.7}
\expandafter\def\csname v@my/nemotron-stream/base/parliament\endcsname{80.6}
\expandafter\def\csname v@my/nemotron-stream/base/podcast\endcsname{71.5}
\expandafter\def\csname v@my/nemotron-stream/base/read-speech\endcsname{73.1}
\expandafter\def\csname v@my/nemotron-stream/base/short-inputs\endcsname{68.1}
\expandafter\def\csname v@my/nemotron-stream/base/singing\endcsname{92.9}
\expandafter\def\csname v@my/nemotron-stream/base/street interview\endcsname{81.4}
\expandafter\def\csname v@my/nemotron-stream/base/telephony\endcsname{33.5}
\expandafter\def\csname v@my/nemotron-stream/commonvoice\endcsname{45.3}
\expandafter\def\csname v@my/nemotron-stream/curve-dev-first\endcsname{70.7}
\expandafter\def\csname v@my/nemotron-stream/curve-dev-last\endcsname{46.4}
\expandafter\def\csname v@my/nemotron-stream/curve-first\endcsname{67.5}
\expandafter\def\csname v@my/nemotron-stream/curve-last\endcsname{48.8}
\expandafter\def\csname v@my/nemotron-stream/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/nemotron-stream/curve-low\endcsname{48.8}
\expandafter\def\csname v@my/nemotron-stream/curve-low-epoch\endcsname{10}
\expandafter\def\csname v@my/nemotron-stream/curve-pick\endcsname{48.8}
\expandafter\def\csname v@my/nemotron-stream/drama\endcsname{49.9}
\expandafter\def\csname v@my/nemotron-stream/en-as-ms\endcsname{0}
\expandafter\def\csname v@my/nemotron-stream/en-as-ms-after\endcsname{12}
\expandafter\def\csname v@my/nemotron-stream/en-as-ms-after-word\endcsname{12}
\expandafter\def\csname v@my/nemotron-stream/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/nemotron-stream/epoch\endcsname{10}
\expandafter\def\csname v@my/nemotron-stream/fleurs\endcsname{51.1}
\expandafter\def\csname v@my/nemotron-stream/gain\endcsname{24.4}
\expandafter\def\csname v@my/nemotron-stream/gain-ci\endcsname{22.3 to 26.5}
\expandafter\def\csname v@my/nemotron-stream/left\endcsname{73.3}
\expandafter\def\csname v@my/nemotron-stream/left-wer\endcsname{88.4}
\expandafter\def\csname v@my/nemotron-stream/left/animation\endcsname{87.7}
\expandafter\def\csname v@my/nemotron-stream/left/commonvoice\endcsname{76.9}
\expandafter\def\csname v@my/nemotron-stream/left/drama\endcsname{82.6}
\expandafter\def\csname v@my/nemotron-stream/left/fleurs\endcsname{68.4}
\expandafter\def\csname v@my/nemotron-stream/left/news\endcsname{62.7}
\expandafter\def\csname v@my/nemotron-stream/left/parliament\endcsname{80.6}
\expandafter\def\csname v@my/nemotron-stream/left/podcast\endcsname{71.5}
\expandafter\def\csname v@my/nemotron-stream/left/read-speech\endcsname{73.1}
\expandafter\def\csname v@my/nemotron-stream/left/short-inputs\endcsname{68.1}
\expandafter\def\csname v@my/nemotron-stream/left/singing\endcsname{92.9}
\expandafter\def\csname v@my/nemotron-stream/left/street interview\endcsname{81.4}
\expandafter\def\csname v@my/nemotron-stream/left/telephony\endcsname{33.5}
\expandafter\def\csname v@my/nemotron-stream/news\endcsname{49.8}
\expandafter\def\csname v@my/nemotron-stream/parliament\endcsname{51.4}
\expandafter\def\csname v@my/nemotron-stream/podcast\endcsname{43.8}
\expandafter\def\csname v@my/nemotron-stream/rank\endcsname{24}
\expandafter\def\csname v@my/nemotron-stream/read-speech\endcsname{44.7}
\expandafter\def\csname v@my/nemotron-stream/short-inputs\endcsname{36.8}
\expandafter\def\csname v@my/nemotron-stream/singing\endcsname{68.4}
\expandafter\def\csname v@my/nemotron-stream/street interview\endcsname{52.2}
\expandafter\def\csname v@my/nemotron-stream/telephony\endcsname{42.9}
\expandafter\def\csname v@my/omni-ctc-1b/after\endcsname{12.5}
\expandafter\def\csname v@my/omni-ctc-1b/after-wer\endcsname{34.2}
\expandafter\def\csname v@my/omni-ctc-1b/animation\endcsname{10.9}
\expandafter\def\csname v@my/omni-ctc-1b/base\endcsname{21.5}
\expandafter\def\csname v@my/omni-ctc-1b/base-wer\endcsname{39.9}
\expandafter\def\csname v@my/omni-ctc-1b/base/animation\endcsname{11.3}
\expandafter\def\csname v@my/omni-ctc-1b/base/commonvoice\endcsname{3.3}
\expandafter\def\csname v@my/omni-ctc-1b/base/drama\endcsname{14.9}
\expandafter\def\csname v@my/omni-ctc-1b/base/fleurs\endcsname{3.2}
\expandafter\def\csname v@my/omni-ctc-1b/base/news\endcsname{9.5}
\expandafter\def\csname v@my/omni-ctc-1b/base/parliament\endcsname{6.7}
\expandafter\def\csname v@my/omni-ctc-1b/base/podcast\endcsname{10.3}
\expandafter\def\csname v@my/omni-ctc-1b/base/read-speech\endcsname{6.1}
\expandafter\def\csname v@my/omni-ctc-1b/base/short-inputs\endcsname{40.5}
\expandafter\def\csname v@my/omni-ctc-1b/base/singing\endcsname{74.0}
\expandafter\def\csname v@my/omni-ctc-1b/base/street interview\endcsname{41.6}
\expandafter\def\csname v@my/omni-ctc-1b/base/telephony\endcsname{36.5}
\expandafter\def\csname v@my/omni-ctc-1b/commonvoice\endcsname{6.3}
\expandafter\def\csname v@my/omni-ctc-1b/curve-dev-first\endcsname{22.8}
\expandafter\def\csname v@my/omni-ctc-1b/curve-dev-last\endcsname{19.0}
\expandafter\def\csname v@my/omni-ctc-1b/curve-first\endcsname{13.8}
\expandafter\def\csname v@my/omni-ctc-1b/curve-last\endcsname{13.6}
\expandafter\def\csname v@my/omni-ctc-1b/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/omni-ctc-1b/curve-low\endcsname{12.5}
\expandafter\def\csname v@my/omni-ctc-1b/curve-low-epoch\endcsname{8}
\expandafter\def\csname v@my/omni-ctc-1b/curve-pick\endcsname{12.5}
\expandafter\def\csname v@my/omni-ctc-1b/drama\endcsname{10.8}
\expandafter\def\csname v@my/omni-ctc-1b/en-as-ms\endcsname{3}
\expandafter\def\csname v@my/omni-ctc-1b/en-as-ms-after\endcsname{6}
\expandafter\def\csname v@my/omni-ctc-1b/en-as-ms-after-word\endcsname{6}
\expandafter\def\csname v@my/omni-ctc-1b/en-as-ms-share\endcsname{1}
\expandafter\def\csname v@my/omni-ctc-1b/epoch\endcsname{8}
\expandafter\def\csname v@my/omni-ctc-1b/fleurs\endcsname{6.4}
\expandafter\def\csname v@my/omni-ctc-1b/gain\endcsname{8.9}
\expandafter\def\csname v@my/omni-ctc-1b/gain-ci\endcsname{7.0 to 10.8}
\expandafter\def\csname v@my/omni-ctc-1b/left\endcsname{21.5}
\expandafter\def\csname v@my/omni-ctc-1b/left-wer\endcsname{39.9}
\expandafter\def\csname v@my/omni-ctc-1b/left/animation\endcsname{11.3}
\expandafter\def\csname v@my/omni-ctc-1b/left/commonvoice\endcsname{3.3}
\expandafter\def\csname v@my/omni-ctc-1b/left/drama\endcsname{14.9}
\expandafter\def\csname v@my/omni-ctc-1b/left/fleurs\endcsname{3.2}
\expandafter\def\csname v@my/omni-ctc-1b/left/news\endcsname{9.5}
\expandafter\def\csname v@my/omni-ctc-1b/left/parliament\endcsname{6.7}
\expandafter\def\csname v@my/omni-ctc-1b/left/podcast\endcsname{10.3}
\expandafter\def\csname v@my/omni-ctc-1b/left/read-speech\endcsname{6.1}
\expandafter\def\csname v@my/omni-ctc-1b/left/short-inputs\endcsname{40.5}
\expandafter\def\csname v@my/omni-ctc-1b/left/singing\endcsname{74.0}
\expandafter\def\csname v@my/omni-ctc-1b/left/street interview\endcsname{41.6}
\expandafter\def\csname v@my/omni-ctc-1b/left/telephony\endcsname{36.5}
\expandafter\def\csname v@my/omni-ctc-1b/news\endcsname{6.9}
\expandafter\def\csname v@my/omni-ctc-1b/parliament\endcsname{8.0}
\expandafter\def\csname v@my/omni-ctc-1b/podcast\endcsname{6.9}
\expandafter\def\csname v@my/omni-ctc-1b/rank\endcsname{15}
\expandafter\def\csname v@my/omni-ctc-1b/read-speech\endcsname{7.2}
\expandafter\def\csname v@my/omni-ctc-1b/short-inputs\endcsname{10.4}
\expandafter\def\csname v@my/omni-ctc-1b/singing\endcsname{40.4}
\expandafter\def\csname v@my/omni-ctc-1b/street interview\endcsname{16.5}
\expandafter\def\csname v@my/omni-ctc-1b/telephony\endcsname{19.9}
\expandafter\def\csname v@my/omni-ctc-300m/after\endcsname{16.1}
\expandafter\def\csname v@my/omni-ctc-300m/after-wer\endcsname{43.6}
\expandafter\def\csname v@my/omni-ctc-300m/animation\endcsname{14.7}
\expandafter\def\csname v@my/omni-ctc-300m/base\endcsname{28.8}
\expandafter\def\csname v@my/omni-ctc-300m/base-wer\endcsname{53.5}
\expandafter\def\csname v@my/omni-ctc-300m/base/animation\endcsname{22.4}
\expandafter\def\csname v@my/omni-ctc-300m/base/commonvoice\endcsname{5.5}
\expandafter\def\csname v@my/omni-ctc-300m/base/drama\endcsname{20.3}
\expandafter\def\csname v@my/omni-ctc-300m/base/fleurs\endcsname{5.3}
\expandafter\def\csname v@my/omni-ctc-300m/base/news\endcsname{9.7}
\expandafter\def\csname v@my/omni-ctc-300m/base/parliament\endcsname{11.5}
\expandafter\def\csname v@my/omni-ctc-300m/base/podcast\endcsname{18.0}
\expandafter\def\csname v@my/omni-ctc-300m/base/read-speech\endcsname{11.2}
\expandafter\def\csname v@my/omni-ctc-300m/base/short-inputs\endcsname{55.2}
\expandafter\def\csname v@my/omni-ctc-300m/base/singing\endcsname{91.1}
\expandafter\def\csname v@my/omni-ctc-300m/base/street interview\endcsname{49.0}
\expandafter\def\csname v@my/omni-ctc-300m/base/telephony\endcsname{46.6}
\expandafter\def\csname v@my/omni-ctc-300m/commonvoice\endcsname{8.6}
\expandafter\def\csname v@my/omni-ctc-300m/curve-dev-first\endcsname{26.3}
\expandafter\def\csname v@my/omni-ctc-300m/curve-dev-last\endcsname{20.5}
\expandafter\def\csname v@my/omni-ctc-300m/curve-first\endcsname{17.7}
\expandafter\def\csname v@my/omni-ctc-300m/curve-last\endcsname{16.1}
\expandafter\def\csname v@my/omni-ctc-300m/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/omni-ctc-300m/curve-low\endcsname{15.7}
\expandafter\def\csname v@my/omni-ctc-300m/curve-low-epoch\endcsname{4}
\expandafter\def\csname v@my/omni-ctc-300m/curve-pick\endcsname{16.1}
\expandafter\def\csname v@my/omni-ctc-300m/drama\endcsname{13.8}
\expandafter\def\csname v@my/omni-ctc-300m/en-as-ms\endcsname{2}
\expandafter\def\csname v@my/omni-ctc-300m/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/omni-ctc-300m/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/omni-ctc-300m/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/omni-ctc-300m/epoch\endcsname{10}
\expandafter\def\csname v@my/omni-ctc-300m/fleurs\endcsname{9.3}
\expandafter\def\csname v@my/omni-ctc-300m/gain\endcsname{12.7}
\expandafter\def\csname v@my/omni-ctc-300m/gain-ci\endcsname{11.1 to 14.5}
\expandafter\def\csname v@my/omni-ctc-300m/left\endcsname{28.8}
\expandafter\def\csname v@my/omni-ctc-300m/left-wer\endcsname{53.5}
\expandafter\def\csname v@my/omni-ctc-300m/left/animation\endcsname{22.4}
\expandafter\def\csname v@my/omni-ctc-300m/left/commonvoice\endcsname{5.5}
\expandafter\def\csname v@my/omni-ctc-300m/left/drama\endcsname{20.3}
\expandafter\def\csname v@my/omni-ctc-300m/left/fleurs\endcsname{5.3}
\expandafter\def\csname v@my/omni-ctc-300m/left/news\endcsname{9.7}
\expandafter\def\csname v@my/omni-ctc-300m/left/parliament\endcsname{11.5}
\expandafter\def\csname v@my/omni-ctc-300m/left/podcast\endcsname{18.0}
\expandafter\def\csname v@my/omni-ctc-300m/left/read-speech\endcsname{11.2}
\expandafter\def\csname v@my/omni-ctc-300m/left/short-inputs\endcsname{55.2}
\expandafter\def\csname v@my/omni-ctc-300m/left/singing\endcsname{91.1}
\expandafter\def\csname v@my/omni-ctc-300m/left/street interview\endcsname{49.0}
\expandafter\def\csname v@my/omni-ctc-300m/left/telephony\endcsname{46.6}
\expandafter\def\csname v@my/omni-ctc-300m/news\endcsname{10.5}
\expandafter\def\csname v@my/omni-ctc-300m/parliament\endcsname{10.6}
\expandafter\def\csname v@my/omni-ctc-300m/podcast\endcsname{10.2}
\expandafter\def\csname v@my/omni-ctc-300m/rank\endcsname{17}
\expandafter\def\csname v@my/omni-ctc-300m/read-speech\endcsname{10.1}
\expandafter\def\csname v@my/omni-ctc-300m/short-inputs\endcsname{17.6}
\expandafter\def\csname v@my/omni-ctc-300m/singing\endcsname{43.0}
\expandafter\def\csname v@my/omni-ctc-300m/street interview\endcsname{20.3}
\expandafter\def\csname v@my/omni-ctc-300m/telephony\endcsname{24.2}
\expandafter\def\csname v@my/omni-ctc-7b/after\endcsname{8.3}
\expandafter\def\csname v@my/omni-ctc-7b/after-wer\endcsname{24.8}
\expandafter\def\csname v@my/omni-ctc-7b/animation\endcsname{8.2}
\expandafter\def\csname v@my/omni-ctc-7b/base\endcsname{26.7}
\expandafter\def\csname v@my/omni-ctc-7b/base-wer\endcsname{43.1}
\expandafter\def\csname v@my/omni-ctc-7b/base/animation\endcsname{20.3}
\expandafter\def\csname v@my/omni-ctc-7b/base/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/omni-ctc-7b/base/drama\endcsname{17.6}
\expandafter\def\csname v@my/omni-ctc-7b/base/fleurs\endcsname{1.5}
\expandafter\def\csname v@my/omni-ctc-7b/base/news\endcsname{6.3}
\expandafter\def\csname v@my/omni-ctc-7b/base/parliament\endcsname{7.1}
\expandafter\def\csname v@my/omni-ctc-7b/base/podcast\endcsname{17.2}
\expandafter\def\csname v@my/omni-ctc-7b/base/read-speech\endcsname{5.0}
\expandafter\def\csname v@my/omni-ctc-7b/base/short-inputs\endcsname{32.6}
\expandafter\def\csname v@my/omni-ctc-7b/base/singing\endcsname{84.5}
\expandafter\def\csname v@my/omni-ctc-7b/base/street interview\endcsname{76.3}
\expandafter\def\csname v@my/omni-ctc-7b/base/telephony\endcsname{48.5}
\expandafter\def\csname v@my/omni-ctc-7b/commonvoice\endcsname{3.6}
\expandafter\def\csname v@my/omni-ctc-7b/curve-dev-first\endcsname{19.7}
\expandafter\def\csname v@my/omni-ctc-7b/curve-dev-last\endcsname{18.2}
\expandafter\def\csname v@my/omni-ctc-7b/curve-first\endcsname{8.9}
\expandafter\def\csname v@my/omni-ctc-7b/curve-last\endcsname{9.0}
\expandafter\def\csname v@my/omni-ctc-7b/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/omni-ctc-7b/curve-low\endcsname{8.3}
\expandafter\def\csname v@my/omni-ctc-7b/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/omni-ctc-7b/curve-pick\endcsname{8.3}
\expandafter\def\csname v@my/omni-ctc-7b/drama\endcsname{7.6}
\expandafter\def\csname v@my/omni-ctc-7b/en-as-ms\endcsname{2}
\expandafter\def\csname v@my/omni-ctc-7b/en-as-ms-after\endcsname{0}
\expandafter\def\csname v@my/omni-ctc-7b/en-as-ms-after-word\endcsname{none}
\expandafter\def\csname v@my/omni-ctc-7b/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/omni-ctc-7b/epoch\endcsname{3}
\expandafter\def\csname v@my/omni-ctc-7b/fleurs\endcsname{3.5}
\expandafter\def\csname v@my/omni-ctc-7b/gain\endcsname{18.3}
\expandafter\def\csname v@my/omni-ctc-7b/gain-ci\endcsname{16.1 to 20.4}
\expandafter\def\csname v@my/omni-ctc-7b/left\endcsname{26.7}
\expandafter\def\csname v@my/omni-ctc-7b/left-wer\endcsname{43.1}
\expandafter\def\csname v@my/omni-ctc-7b/left/animation\endcsname{20.3}
\expandafter\def\csname v@my/omni-ctc-7b/left/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/omni-ctc-7b/left/drama\endcsname{17.6}
\expandafter\def\csname v@my/omni-ctc-7b/left/fleurs\endcsname{1.5}
\expandafter\def\csname v@my/omni-ctc-7b/left/news\endcsname{6.3}
\expandafter\def\csname v@my/omni-ctc-7b/left/parliament\endcsname{7.1}
\expandafter\def\csname v@my/omni-ctc-7b/left/podcast\endcsname{17.2}
\expandafter\def\csname v@my/omni-ctc-7b/left/read-speech\endcsname{5.0}
\expandafter\def\csname v@my/omni-ctc-7b/left/short-inputs\endcsname{32.6}
\expandafter\def\csname v@my/omni-ctc-7b/left/singing\endcsname{84.5}
\expandafter\def\csname v@my/omni-ctc-7b/left/street interview\endcsname{76.3}
\expandafter\def\csname v@my/omni-ctc-7b/left/telephony\endcsname{48.5}
\expandafter\def\csname v@my/omni-ctc-7b/news\endcsname{4.0}
\expandafter\def\csname v@my/omni-ctc-7b/parliament\endcsname{5.4}
\expandafter\def\csname v@my/omni-ctc-7b/podcast\endcsname{4.6}
\expandafter\def\csname v@my/omni-ctc-7b/rank\endcsname{5}
\expandafter\def\csname v@my/omni-ctc-7b/rank-word\endcsname{fifth best}
\expandafter\def\csname v@my/omni-ctc-7b/read-speech\endcsname{2.8}
\expandafter\def\csname v@my/omni-ctc-7b/short-inputs\endcsname{9.8}
\expandafter\def\csname v@my/omni-ctc-7b/singing\endcsname{22.0}
\expandafter\def\csname v@my/omni-ctc-7b/street interview\endcsname{13.0}
\expandafter\def\csname v@my/omni-ctc-7b/telephony\endcsname{15.5}
\expandafter\def\csname v@my/omni-llm-1b/base\endcsname{16.9}
\expandafter\def\csname v@my/omni-llm-1b/base-wer\endcsname{32.5}
\expandafter\def\csname v@my/omni-llm-1b/base/animation\endcsname{16.2}
\expandafter\def\csname v@my/omni-llm-1b/base/commonvoice\endcsname{2.6}
\expandafter\def\csname v@my/omni-llm-1b/base/drama\endcsname{15.7}
\expandafter\def\csname v@my/omni-llm-1b/base/fleurs\endcsname{1.8}
\expandafter\def\csname v@my/omni-llm-1b/base/news\endcsname{4.6}
\expandafter\def\csname v@my/omni-llm-1b/base/parliament\endcsname{6.4}
\expandafter\def\csname v@my/omni-llm-1b/base/podcast\endcsname{11.4}
\expandafter\def\csname v@my/omni-llm-1b/base/read-speech\endcsname{3.8}
\expandafter\def\csname v@my/omni-llm-1b/base/short-inputs\endcsname{41.9}
\expandafter\def\csname v@my/omni-llm-1b/base/singing\endcsname{43.4}
\expandafter\def\csname v@my/omni-llm-1b/base/street interview\endcsname{25.4}
\expandafter\def\csname v@my/omni-llm-1b/base/telephony\endcsname{29.2}
\expandafter\def\csname v@my/omni-llm-1b/en-as-ms\endcsname{3}
\expandafter\def\csname v@my/omni-llm-1b/en-as-ms-share\endcsname{1}
\expandafter\def\csname v@my/omni-llm-1b/left\endcsname{16.9}
\expandafter\def\csname v@my/omni-llm-1b/left-wer\endcsname{32.5}
\expandafter\def\csname v@my/omni-llm-1b/left/animation\endcsname{16.2}
\expandafter\def\csname v@my/omni-llm-1b/left/commonvoice\endcsname{2.6}
\expandafter\def\csname v@my/omni-llm-1b/left/drama\endcsname{15.7}
\expandafter\def\csname v@my/omni-llm-1b/left/fleurs\endcsname{1.8}
\expandafter\def\csname v@my/omni-llm-1b/left/news\endcsname{4.6}
\expandafter\def\csname v@my/omni-llm-1b/left/parliament\endcsname{6.4}
\expandafter\def\csname v@my/omni-llm-1b/left/podcast\endcsname{11.4}
\expandafter\def\csname v@my/omni-llm-1b/left/read-speech\endcsname{3.8}
\expandafter\def\csname v@my/omni-llm-1b/left/short-inputs\endcsname{41.9}
\expandafter\def\csname v@my/omni-llm-1b/left/singing\endcsname{43.4}
\expandafter\def\csname v@my/omni-llm-1b/left/street interview\endcsname{25.4}
\expandafter\def\csname v@my/omni-llm-1b/left/telephony\endcsname{29.2}
\expandafter\def\csname v@my/parakeet-tdt-v3/after\endcsname{18.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/after-wer\endcsname{41.2}
\expandafter\def\csname v@my/parakeet-tdt-v3/animation\endcsname{19.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/base\endcsname{41.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/base-wer\endcsname{77.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/animation\endcsname{62.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/commonvoice\endcsname{30.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/drama\endcsname{50.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/fleurs\endcsname{34.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/news\endcsname{23.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/parliament\endcsname{36.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/podcast\endcsname{39.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/read-speech\endcsname{41.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/short-inputs\endcsname{32.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/singing\endcsname{63.5}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/street interview\endcsname{68.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/base/telephony\endcsname{15.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/commonvoice\endcsname{13.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-dev-first\endcsname{25.7}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-dev-last\endcsname{22.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-first\endcsname{20.5}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-last\endcsname{20.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-low\endcsname{18.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-low-epoch\endcsname{6}
\expandafter\def\csname v@my/parakeet-tdt-v3/curve-pick\endcsname{18.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/drama\endcsname{18.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/en-as-ms\endcsname{1}
\expandafter\def\csname v@my/parakeet-tdt-v3/en-as-ms-after\endcsname{4}
\expandafter\def\csname v@my/parakeet-tdt-v3/en-as-ms-after-word\endcsname{4}
\expandafter\def\csname v@my/parakeet-tdt-v3/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/parakeet-tdt-v3/epoch\endcsname{6}
\expandafter\def\csname v@my/parakeet-tdt-v3/fleurs\endcsname{15.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/gain\endcsname{22.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/gain-ci\endcsname{20.4 to 24.7}
\expandafter\def\csname v@my/parakeet-tdt-v3/left\endcsname{41.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/left-wer\endcsname{77.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/animation\endcsname{62.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/commonvoice\endcsname{30.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/drama\endcsname{50.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/fleurs\endcsname{34.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/news\endcsname{23.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/parliament\endcsname{36.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/podcast\endcsname{39.8}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/read-speech\endcsname{41.9}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/short-inputs\endcsname{32.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/singing\endcsname{63.5}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/street interview\endcsname{68.6}
\expandafter\def\csname v@my/parakeet-tdt-v3/left/telephony\endcsname{15.1}
\expandafter\def\csname v@my/parakeet-tdt-v3/news\endcsname{13.4}
\expandafter\def\csname v@my/parakeet-tdt-v3/parliament\endcsname{16.5}
\expandafter\def\csname v@my/parakeet-tdt-v3/podcast\endcsname{12.0}
\expandafter\def\csname v@my/parakeet-tdt-v3/rank\endcsname{19}
\expandafter\def\csname v@my/parakeet-tdt-v3/read-speech\endcsname{10.5}
\expandafter\def\csname v@my/parakeet-tdt-v3/short-inputs\endcsname{4.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/singing\endcsname{64.3}
\expandafter\def\csname v@my/parakeet-tdt-v3/street interview\endcsname{23.7}
\expandafter\def\csname v@my/parakeet-tdt-v3/telephony\endcsname{16.3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/after\endcsname{14.2}
\expandafter\def\csname v@my/qwen3-asr-0.6b/after-wer\endcsname{31.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/animation\endcsname{16.1}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base\endcsname{11.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base-wer\endcsname{25.2}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/animation\endcsname{10.3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/commonvoice\endcsname{5.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/drama\endcsname{17.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/fleurs\endcsname{4.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/news\endcsname{9.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/parliament\endcsname{7.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/podcast\endcsname{11.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/read-speech\endcsname{4.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/short-inputs\endcsname{14.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/singing\endcsname{13.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/street interview\endcsname{25.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/base/telephony\endcsname{13.1}
\expandafter\def\csname v@my/qwen3-asr-0.6b/commonvoice\endcsname{9.1}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-dev-first\endcsname{22.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-dev-last\endcsname{22.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-first\endcsname{13.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-last\endcsname{14.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-low\endcsname{13.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/qwen3-asr-0.6b/curve-pick\endcsname{14.2}
\expandafter\def\csname v@my/qwen3-asr-0.6b/detect\endcsname{15.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/detect-en-as-ms\endcsname{5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/detect-ms-as-en\endcsname{9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/detect-wer\endcsname{28.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/detect/telephony\endcsname{14.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/drama\endcsname{14.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/en-as-ms\endcsname{7}
\expandafter\def\csname v@my/qwen3-asr-0.6b/en-as-ms-after\endcsname{3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/en-as-ms-after-word\endcsname{3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/en-as-ms-share\endcsname{8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/epoch\endcsname{4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/fleurs\endcsname{11.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/gain\endcsname{-2.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/gain-ci\endcsname{-4.1 to -1.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left\endcsname{15.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left-wer\endcsname{28.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/animation\endcsname{11.3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/commonvoice\endcsname{5.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/drama\endcsname{22.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/fleurs\endcsname{4.7}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/news\endcsname{5.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/parliament\endcsname{8.1}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/podcast\endcsname{11.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/read-speech\endcsname{7.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/short-inputs\endcsname{28.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/singing\endcsname{33.3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/street interview\endcsname{25.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/left/telephony\endcsname{14.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/news\endcsname{10.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/parliament\endcsname{13.2}
\expandafter\def\csname v@my/qwen3-asr-0.6b/podcast\endcsname{9.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/rank\endcsname{16}
\expandafter\def\csname v@my/qwen3-asr-0.6b/read-speech\endcsname{8.9}
\expandafter\def\csname v@my/qwen3-asr-0.6b/short-inputs\endcsname{6.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/singing\endcsname{31.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/street interview\endcsname{22.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/telephony\endcsname{17.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told\endcsname{11.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told-gain\endcsname{-2.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told-wer\endcsname{25.2}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/animation\endcsname{10.3}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/commonvoice\endcsname{5.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/drama\endcsname{17.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/fleurs\endcsname{4.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/news\endcsname{9.8}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/parliament\endcsname{7.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/podcast\endcsname{11.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/read-speech\endcsname{4.5}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/short-inputs\endcsname{14.0}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/singing\endcsname{13.4}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/street interview\endcsname{25.6}
\expandafter\def\csname v@my/qwen3-asr-0.6b/told/telephony\endcsname{13.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/after\endcsname{8.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/after-wer\endcsname{20.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/animation\endcsname{8.4}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base\endcsname{8.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base-wer\endcsname{17.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/animation\endcsname{7.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/commonvoice\endcsname{3.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/drama\endcsname{12.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/fleurs\endcsname{2.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/news\endcsname{4.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/parliament\endcsname{5.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/podcast\endcsname{8.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/read-speech\endcsname{4.2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/short-inputs\endcsname{15.2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/singing\endcsname{9.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/street interview\endcsname{23.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/base/telephony\endcsname{7.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/commonvoice\endcsname{5.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-dev-first\endcsname{20.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-dev-last\endcsname{20.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-first\endcsname{8.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-last\endcsname{11.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-low\endcsname{8.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/curve-pick\endcsname{8.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/detect\endcsname{8.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/detect-en-as-ms\endcsname{2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/detect-ms-as-en\endcsname{3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/detect-wer\endcsname{17.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/detect/telephony\endcsname{7.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/drama\endcsname{9.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/en-as-ms\endcsname{11}
\expandafter\def\csname v@my/qwen3-asr-1.7b/en-as-ms-after\endcsname{1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/en-as-ms-after-word\endcsname{1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/en-as-ms-share\endcsname{19}
\expandafter\def\csname v@my/qwen3-asr-1.7b/epoch\endcsname{1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/fleurs\endcsname{5.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/gain\endcsname{-0.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/gain-ci\endcsname{-1.1 to 1.0}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left\endcsname{8.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left-wer\endcsname{17.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/animation\endcsname{7.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/commonvoice\endcsname{3.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/drama\endcsname{12.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/fleurs\endcsname{2.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/news\endcsname{4.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/parliament\endcsname{5.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/podcast\endcsname{8.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/read-speech\endcsname{4.2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/short-inputs\endcsname{15.2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/singing\endcsname{9.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/street interview\endcsname{23.1}
\expandafter\def\csname v@my/qwen3-asr-1.7b/left/telephony\endcsname{7.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/news\endcsname{5.4}
\expandafter\def\csname v@my/qwen3-asr-1.7b/parliament\endcsname{9.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/podcast\endcsname{6.0}
\expandafter\def\csname v@my/qwen3-asr-1.7b/rank\endcsname{7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/rank-word\endcsname{seventh best}
\expandafter\def\csname v@my/qwen3-asr-1.7b/read-speech\endcsname{3.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/short-inputs\endcsname{2.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/singing\endcsname{20.4}
\expandafter\def\csname v@my/qwen3-asr-1.7b/street interview\endcsname{16.0}
\expandafter\def\csname v@my/qwen3-asr-1.7b/telephony\endcsname{11.5}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told\endcsname{10.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told-gain\endcsname{1.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told-wer\endcsname{20.2}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/animation\endcsname{6.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/commonvoice\endcsname{3.7}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/drama\endcsname{12.4}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/fleurs\endcsname{2.6}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/news\endcsname{16.0}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/parliament\endcsname{5.8}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/podcast\endcsname{8.5}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/read-speech\endcsname{2.9}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/short-inputs\endcsname{29.8}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/singing\endcsname{7.3}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/street interview\endcsname{21.4}
\expandafter\def\csname v@my/qwen3-asr-1.7b/told/telephony\endcsname{10.6}
\expandafter\def\csname v@my/rise-max\endcsname{8.2}
\expandafter\def\csname v@my/rise-median\endcsname{0.7}
\expandafter\def\csname v@my/scored\endcsname{28}
\expandafter\def\csname v@my/size/1000/hours\endcsname{2.0}
\expandafter\def\csname v@my/size/16000/hours\endcsname{30.5}
\expandafter\def\csname v@my/size/4000/hours\endcsname{8.0}
\expandafter\def\csname v@my/size/all/hours\endcsname{60.1}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/1000\endcsname{13.8}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/1000/dev\endcsname{28.0}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/16000\endcsname{13.8}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/16000/dev\endcsname{22.1}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/4000\endcsname{14.6}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/4000/dev\endcsname{25.5}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/all\endcsname{14.2}
\expandafter\def\csname v@my/size/qwen3-asr-0.6b/all/dev\endcsname{21.0}
\expandafter\def\csname v@my/size/whisper-small/1000\endcsname{11.0}
\expandafter\def\csname v@my/size/whisper-small/1000/dev\endcsname{26.3}
\expandafter\def\csname v@my/size/whisper-small/16000\endcsname{10.8}
\expandafter\def\csname v@my/size/whisper-small/16000/dev\endcsname{21.4}
\expandafter\def\csname v@my/size/whisper-small/4000\endcsname{12.5}
\expandafter\def\csname v@my/size/whisper-small/4000/dev\endcsname{23.7}
\expandafter\def\csname v@my/size/whisper-small/all\endcsname{11.7}
\expandafter\def\csname v@my/size/whisper-small/all/dev\endcsname{20.5}
\expandafter\def\csname v@my/tel/tuned\endcsname{11.2}
\expandafter\def\csname v@my/tel/tuned-name\endcsname{Voxtral Mini 3B}
\expandafter\def\csname v@my/tel/untouched\endcsname{7.3}
\expandafter\def\csname v@my/tel/untouched-name\endcsname{Qwen3-ASR 1.7B}
\expandafter\def\csname v@my/train-clips\endcsname{31,622}
\expandafter\def\csname v@my/train-hours\endcsname{60}
\expandafter\def\csname v@my/train-median\endcsname{4.3}
\expandafter\def\csname v@my/up-first\endcsname{Cohere Transcribe 2B}
\expandafter\def\csname v@my/up-n\endcsname{18}
\expandafter\def\csname v@my/up-names\endcsname{Cohere Transcribe 2B, LFM3-Audio 2B, Gemma 4 12B, Nemotron 3.5 streaming 0.6B, Voxtral Mini 3B, Parakeet TDT 0.6B v3, omniASR CTC 7B, Granite Speech 5.0 2B, Nemotron 3.5 Transcribe 30B, omniASR CTC 300M, omniASR CTC 1B, Whisper tiny, Whisper small, Whisper medium, Whisper large-v2, MMS 1B, Whisper large-v3 and Gemma 4 E4B}
\expandafter\def\csname v@my/vibevoice/base\endcsname{64.2}
\expandafter\def\csname v@my/vibevoice/base-wer\endcsname{76.7}
\expandafter\def\csname v@my/vibevoice/base/animation\endcsname{81.3}
\expandafter\def\csname v@my/vibevoice/base/commonvoice\endcsname{41.0}
\expandafter\def\csname v@my/vibevoice/base/drama\endcsname{83.2}
\expandafter\def\csname v@my/vibevoice/base/fleurs\endcsname{38.4}
\expandafter\def\csname v@my/vibevoice/base/news\endcsname{41.1}
\expandafter\def\csname v@my/vibevoice/base/parliament\endcsname{46.0}
\expandafter\def\csname v@my/vibevoice/base/podcast\endcsname{66.5}
\expandafter\def\csname v@my/vibevoice/base/read-speech\endcsname{70.7}
\expandafter\def\csname v@my/vibevoice/base/short-inputs\endcsname{72.5}
\expandafter\def\csname v@my/vibevoice/base/singing\endcsname{89.2}
\expandafter\def\csname v@my/vibevoice/base/street interview\endcsname{86.8}
\expandafter\def\csname v@my/vibevoice/base/telephony\endcsname{54.0}
\expandafter\def\csname v@my/vibevoice/en-as-ms\endcsname{1}
\expandafter\def\csname v@my/vibevoice/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/vibevoice/left\endcsname{64.2}
\expandafter\def\csname v@my/vibevoice/left-wer\endcsname{76.7}
\expandafter\def\csname v@my/vibevoice/left/animation\endcsname{81.3}
\expandafter\def\csname v@my/vibevoice/left/commonvoice\endcsname{41.0}
\expandafter\def\csname v@my/vibevoice/left/drama\endcsname{83.2}
\expandafter\def\csname v@my/vibevoice/left/fleurs\endcsname{38.4}
\expandafter\def\csname v@my/vibevoice/left/news\endcsname{41.1}
\expandafter\def\csname v@my/vibevoice/left/parliament\endcsname{46.0}
\expandafter\def\csname v@my/vibevoice/left/podcast\endcsname{66.5}
\expandafter\def\csname v@my/vibevoice/left/read-speech\endcsname{70.7}
\expandafter\def\csname v@my/vibevoice/left/short-inputs\endcsname{72.5}
\expandafter\def\csname v@my/vibevoice/left/singing\endcsname{89.2}
\expandafter\def\csname v@my/vibevoice/left/street interview\endcsname{86.8}
\expandafter\def\csname v@my/vibevoice/left/telephony\endcsname{54.0}
\expandafter\def\csname v@my/voxtral-mini/after\endcsname{9.0}
\expandafter\def\csname v@my/voxtral-mini/after-wer\endcsname{19.6}
\expandafter\def\csname v@my/voxtral-mini/animation\endcsname{7.6}
\expandafter\def\csname v@my/voxtral-mini/base\endcsname{32.5}
\expandafter\def\csname v@my/voxtral-mini/base-wer\endcsname{44.4}
\expandafter\def\csname v@my/voxtral-mini/base/animation\endcsname{42.3}
\expandafter\def\csname v@my/voxtral-mini/base/commonvoice\endcsname{24.5}
\expandafter\def\csname v@my/voxtral-mini/base/drama\endcsname{53.1}
\expandafter\def\csname v@my/voxtral-mini/base/fleurs\endcsname{19.3}
\expandafter\def\csname v@my/voxtral-mini/base/news\endcsname{13.9}
\expandafter\def\csname v@my/voxtral-mini/base/parliament\endcsname{13.8}
\expandafter\def\csname v@my/voxtral-mini/base/podcast\endcsname{40.2}
\expandafter\def\csname v@my/voxtral-mini/base/read-speech\endcsname{38.2}
\expandafter\def\csname v@my/voxtral-mini/base/short-inputs\endcsname{26.3}
\expandafter\def\csname v@my/voxtral-mini/base/singing\endcsname{40.8}
\expandafter\def\csname v@my/voxtral-mini/base/street interview\endcsname{53.1}
\expandafter\def\csname v@my/voxtral-mini/base/telephony\endcsname{25.0}
\expandafter\def\csname v@my/voxtral-mini/commonvoice\endcsname{7.0}
\expandafter\def\csname v@my/voxtral-mini/curve-dev-first\endcsname{21.3}
\expandafter\def\csname v@my/voxtral-mini/curve-dev-last\endcsname{19.8}
\expandafter\def\csname v@my/voxtral-mini/curve-first\endcsname{9.2}
\expandafter\def\csname v@my/voxtral-mini/curve-last\endcsname{8.7}
\expandafter\def\csname v@my/voxtral-mini/curve-last-epoch\endcsname{3}
\expandafter\def\csname v@my/voxtral-mini/curve-low\endcsname{8.7}
\expandafter\def\csname v@my/voxtral-mini/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/voxtral-mini/curve-pick\endcsname{9.0}
\expandafter\def\csname v@my/voxtral-mini/drama\endcsname{10.4}
\expandafter\def\csname v@my/voxtral-mini/en-as-ms\endcsname{2}
\expandafter\def\csname v@my/voxtral-mini/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/voxtral-mini/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/voxtral-mini/en-as-ms-share\endcsname{0}
\expandafter\def\csname v@my/voxtral-mini/epoch\endcsname{2}
\expandafter\def\csname v@my/voxtral-mini/fleurs\endcsname{6.3}
\expandafter\def\csname v@my/voxtral-mini/gain\endcsname{23.5}
\expandafter\def\csname v@my/voxtral-mini/gain-ci\endcsname{20.8 to 26.4}
\expandafter\def\csname v@my/voxtral-mini/left\endcsname{32.5}
\expandafter\def\csname v@my/voxtral-mini/left-wer\endcsname{44.4}
\expandafter\def\csname v@my/voxtral-mini/left/animation\endcsname{42.3}
\expandafter\def\csname v@my/voxtral-mini/left/commonvoice\endcsname{24.5}
\expandafter\def\csname v@my/voxtral-mini/left/drama\endcsname{53.1}
\expandafter\def\csname v@my/voxtral-mini/left/fleurs\endcsname{19.3}
\expandafter\def\csname v@my/voxtral-mini/left/news\endcsname{13.9}
\expandafter\def\csname v@my/voxtral-mini/left/parliament\endcsname{13.8}
\expandafter\def\csname v@my/voxtral-mini/left/podcast\endcsname{40.2}
\expandafter\def\csname v@my/voxtral-mini/left/read-speech\endcsname{38.2}
\expandafter\def\csname v@my/voxtral-mini/left/short-inputs\endcsname{26.3}
\expandafter\def\csname v@my/voxtral-mini/left/singing\endcsname{40.8}
\expandafter\def\csname v@my/voxtral-mini/left/street interview\endcsname{53.1}
\expandafter\def\csname v@my/voxtral-mini/left/telephony\endcsname{25.0}
\expandafter\def\csname v@my/voxtral-mini/news\endcsname{6.0}
\expandafter\def\csname v@my/voxtral-mini/parliament\endcsname{13.6}
\expandafter\def\csname v@my/voxtral-mini/podcast\endcsname{4.6}
\expandafter\def\csname v@my/voxtral-mini/rank\endcsname{8}
\expandafter\def\csname v@my/voxtral-mini/rank-word\endcsname{eighth best}
\expandafter\def\csname v@my/voxtral-mini/read-speech\endcsname{2.5}
\expandafter\def\csname v@my/voxtral-mini/short-inputs\endcsname{5.9}
\expandafter\def\csname v@my/voxtral-mini/singing\endcsname{19.7}
\expandafter\def\csname v@my/voxtral-mini/street interview\endcsname{13.7}
\expandafter\def\csname v@my/voxtral-mini/telephony\endcsname{11.2}
\expandafter\def\csname v@my/w2v-bert/after\endcsname{9.3}
\expandafter\def\csname v@my/w2v-bert/after-wer\endcsname{27.9}
\expandafter\def\csname v@my/w2v-bert/animation\endcsname{7.4}
\expandafter\def\csname v@my/w2v-bert/commonvoice\endcsname{4.4}
\expandafter\def\csname v@my/w2v-bert/curve-dev-first\endcsname{100.0}
\expandafter\def\csname v@my/w2v-bert/curve-dev-last\endcsname{19.2}
\expandafter\def\csname v@my/w2v-bert/curve-first\endcsname{100.0}
\expandafter\def\csname v@my/w2v-bert/curve-last\endcsname{9.8}
\expandafter\def\csname v@my/w2v-bert/curve-last-epoch\endcsname{15}
\expandafter\def\csname v@my/w2v-bert/curve-low\endcsname{9.3}
\expandafter\def\csname v@my/w2v-bert/curve-low-epoch\endcsname{12}
\expandafter\def\csname v@my/w2v-bert/curve-pick\endcsname{9.3}
\expandafter\def\csname v@my/w2v-bert/drama\endcsname{7.9}
\expandafter\def\csname v@my/w2v-bert/epoch\endcsname{12}
\expandafter\def\csname v@my/w2v-bert/fleurs\endcsname{4.9}
\expandafter\def\csname v@my/w2v-bert/news\endcsname{5.3}
\expandafter\def\csname v@my/w2v-bert/parliament\endcsname{6.3}
\expandafter\def\csname v@my/w2v-bert/podcast\endcsname{5.4}
\expandafter\def\csname v@my/w2v-bert/rank\endcsname{9}
\expandafter\def\csname v@my/w2v-bert/rank-word\endcsname{ninth best}
\expandafter\def\csname v@my/w2v-bert/read-speech\endcsname{4.4}
\expandafter\def\csname v@my/w2v-bert/short-inputs\endcsname{13.6}
\expandafter\def\csname v@my/w2v-bert/singing\endcsname{20.8}
\expandafter\def\csname v@my/w2v-bert/street interview\endcsname{14.2}
\expandafter\def\csname v@my/w2v-bert/telephony\endcsname{17.0}
\expandafter\def\csname v@my/whisper-base/after\endcsname{24.8}
\expandafter\def\csname v@my/whisper-base/after-wer\endcsname{48.7}
\expandafter\def\csname v@my/whisper-base/animation\endcsname{25.3}
\expandafter\def\csname v@my/whisper-base/base\endcsname{24.6}
\expandafter\def\csname v@my/whisper-base/base-wer\endcsname{47.8}
\expandafter\def\csname v@my/whisper-base/base/animation\endcsname{24.5}
\expandafter\def\csname v@my/whisper-base/base/commonvoice\endcsname{10.7}
\expandafter\def\csname v@my/whisper-base/base/drama\endcsname{24.4}
\expandafter\def\csname v@my/whisper-base/base/fleurs\endcsname{10.8}
\expandafter\def\csname v@my/whisper-base/base/news\endcsname{16.8}
\expandafter\def\csname v@my/whisper-base/base/parliament\endcsname{16.0}
\expandafter\def\csname v@my/whisper-base/base/podcast\endcsname{27.4}
\expandafter\def\csname v@my/whisper-base/base/read-speech\endcsname{16.4}
\expandafter\def\csname v@my/whisper-base/base/short-inputs\endcsname{32.3}
\expandafter\def\csname v@my/whisper-base/base/singing\endcsname{41.4}
\expandafter\def\csname v@my/whisper-base/base/street interview\endcsname{40.8}
\expandafter\def\csname v@my/whisper-base/base/telephony\endcsname{33.4}
\expandafter\def\csname v@my/whisper-base/commonvoice\endcsname{19.0}
\expandafter\def\csname v@my/whisper-base/curve-dev-first\endcsname{35.3}
\expandafter\def\csname v@my/whisper-base/curve-dev-last\endcsname{26.7}
\expandafter\def\csname v@my/whisper-base/curve-first\endcsname{25.1}
\expandafter\def\csname v@my/whisper-base/curve-last\endcsname{27.5}
\expandafter\def\csname v@my/whisper-base/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/whisper-base/curve-low\endcsname{23.5}
\expandafter\def\csname v@my/whisper-base/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/whisper-base/curve-pick\endcsname{24.8}
\expandafter\def\csname v@my/whisper-base/detect\endcsname{24.6}
\expandafter\def\csname v@my/whisper-base/detect-en-as-ms\endcsname{18}
\expandafter\def\csname v@my/whisper-base/detect-ms-as-en\endcsname{9}
\expandafter\def\csname v@my/whisper-base/detect-wer\endcsname{47.8}
\expandafter\def\csname v@my/whisper-base/detect/telephony\endcsname{33.4}
\expandafter\def\csname v@my/whisper-base/drama\endcsname{20.3}
\expandafter\def\csname v@my/whisper-base/en-as-ms\endcsname{62}
\expandafter\def\csname v@my/whisper-base/en-as-ms-after\endcsname{10}
\expandafter\def\csname v@my/whisper-base/en-as-ms-after-word\endcsname{10}
\expandafter\def\csname v@my/whisper-base/en-as-ms-share\endcsname{22}
\expandafter\def\csname v@my/whisper-base/epoch\endcsname{4}
\expandafter\def\csname v@my/whisper-base/fleurs\endcsname{25.7}
\expandafter\def\csname v@my/whisper-base/gain\endcsname{-0.2}
\expandafter\def\csname v@my/whisper-base/gain-ci\endcsname{-2.0 to 1.7}
\expandafter\def\csname v@my/whisper-base/left\endcsname{24.6}
\expandafter\def\csname v@my/whisper-base/left-wer\endcsname{47.8}
\expandafter\def\csname v@my/whisper-base/left/animation\endcsname{24.5}
\expandafter\def\csname v@my/whisper-base/left/commonvoice\endcsname{10.7}
\expandafter\def\csname v@my/whisper-base/left/drama\endcsname{24.4}
\expandafter\def\csname v@my/whisper-base/left/fleurs\endcsname{10.8}
\expandafter\def\csname v@my/whisper-base/left/news\endcsname{16.8}
\expandafter\def\csname v@my/whisper-base/left/parliament\endcsname{16.0}
\expandafter\def\csname v@my/whisper-base/left/podcast\endcsname{27.4}
\expandafter\def\csname v@my/whisper-base/left/read-speech\endcsname{16.4}
\expandafter\def\csname v@my/whisper-base/left/short-inputs\endcsname{32.3}
\expandafter\def\csname v@my/whisper-base/left/singing\endcsname{41.4}
\expandafter\def\csname v@my/whisper-base/left/street interview\endcsname{40.8}
\expandafter\def\csname v@my/whisper-base/left/telephony\endcsname{33.4}
\expandafter\def\csname v@my/whisper-base/news\endcsname{24.7}
\expandafter\def\csname v@my/whisper-base/parliament\endcsname{22.6}
\expandafter\def\csname v@my/whisper-base/podcast\endcsname{17.1}
\expandafter\def\csname v@my/whisper-base/rank\endcsname{21}
\expandafter\def\csname v@my/whisper-base/read-speech\endcsname{14.7}
\expandafter\def\csname v@my/whisper-base/short-inputs\endcsname{11.6}
\expandafter\def\csname v@my/whisper-base/singing\endcsname{62.3}
\expandafter\def\csname v@my/whisper-base/street interview\endcsname{30.5}
\expandafter\def\csname v@my/whisper-base/telephony\endcsname{23.5}
\expandafter\def\csname v@my/whisper-base/told\endcsname{28.0}
\expandafter\def\csname v@my/whisper-base/told-gain\endcsname{3.2}
\expandafter\def\csname v@my/whisper-base/told-wer\endcsname{51.8}
\expandafter\def\csname v@my/whisper-base/told/animation\endcsname{20.8}
\expandafter\def\csname v@my/whisper-base/told/commonvoice\endcsname{10.4}
\expandafter\def\csname v@my/whisper-base/told/drama\endcsname{24.8}
\expandafter\def\csname v@my/whisper-base/told/fleurs\endcsname{10.6}
\expandafter\def\csname v@my/whisper-base/told/news\endcsname{35.5}
\expandafter\def\csname v@my/whisper-base/told/parliament\endcsname{14.3}
\expandafter\def\csname v@my/whisper-base/told/podcast\endcsname{26.4}
\expandafter\def\csname v@my/whisper-base/told/read-speech\endcsname{11.7}
\expandafter\def\csname v@my/whisper-base/told/short-inputs\endcsname{41.2}
\expandafter\def\csname v@my/whisper-base/told/singing\endcsname{35.9}
\expandafter\def\csname v@my/whisper-base/told/street interview\endcsname{40.8}
\expandafter\def\csname v@my/whisper-base/told/telephony\endcsname{63.7}
\expandafter\def\csname v@my/whisper-large-v2/after\endcsname{6.8}
\expandafter\def\csname v@my/whisper-large-v2/after-wer\endcsname{16.2}
\expandafter\def\csname v@my/whisper-large-v2/animation\endcsname{5.1}
\expandafter\def\csname v@my/whisper-large-v2/base\endcsname{11.6}
\expandafter\def\csname v@my/whisper-large-v2/base-wer\endcsname{18.7}
\expandafter\def\csname v@my/whisper-large-v2/base/animation\endcsname{3.4}
\expandafter\def\csname v@my/whisper-large-v2/base/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/whisper-large-v2/base/drama\endcsname{10.7}
\expandafter\def\csname v@my/whisper-large-v2/base/fleurs\endcsname{2.1}
\expandafter\def\csname v@my/whisper-large-v2/base/news\endcsname{4.5}
\expandafter\def\csname v@my/whisper-large-v2/base/parliament\endcsname{5.5}
\expandafter\def\csname v@my/whisper-large-v2/base/podcast\endcsname{12.1}
\expandafter\def\csname v@my/whisper-large-v2/base/read-speech\endcsname{2.6}
\expandafter\def\csname v@my/whisper-large-v2/base/short-inputs\endcsname{34.9}
\expandafter\def\csname v@my/whisper-large-v2/base/singing\endcsname{14.0}
\expandafter\def\csname v@my/whisper-large-v2/base/street interview\endcsname{19.7}
\expandafter\def\csname v@my/whisper-large-v2/base/telephony\endcsname{26.6}
\expandafter\def\csname v@my/whisper-large-v2/commonvoice\endcsname{3.5}
\expandafter\def\csname v@my/whisper-large-v2/curve-dev-first\endcsname{19.9}
\expandafter\def\csname v@my/whisper-large-v2/curve-dev-last\endcsname{19.2}
\expandafter\def\csname v@my/whisper-large-v2/curve-first\endcsname{6.9}
\expandafter\def\csname v@my/whisper-large-v2/curve-last\endcsname{7.1}
\expandafter\def\csname v@my/whisper-large-v2/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/whisper-large-v2/curve-low\endcsname{6.8}
\expandafter\def\csname v@my/whisper-large-v2/curve-low-epoch\endcsname{4}
\expandafter\def\csname v@my/whisper-large-v2/curve-pick\endcsname{6.8}
\expandafter\def\csname v@my/whisper-large-v2/detect\endcsname{11.6}
\expandafter\def\csname v@my/whisper-large-v2/detect-en-as-ms\endcsname{17}
\expandafter\def\csname v@my/whisper-large-v2/detect-ms-as-en\endcsname{1}
\expandafter\def\csname v@my/whisper-large-v2/detect-wer\endcsname{18.7}
\expandafter\def\csname v@my/whisper-large-v2/detect/telephony\endcsname{26.6}
\expandafter\def\csname v@my/whisper-large-v2/drama\endcsname{6.2}
\expandafter\def\csname v@my/whisper-large-v2/en-as-ms\endcsname{60}
\expandafter\def\csname v@my/whisper-large-v2/en-as-ms-after\endcsname{3}
\expandafter\def\csname v@my/whisper-large-v2/en-as-ms-after-word\endcsname{3}
\expandafter\def\csname v@my/whisper-large-v2/en-as-ms-share\endcsname{44}
\expandafter\def\csname v@my/whisper-large-v2/epoch\endcsname{4}
\expandafter\def\csname v@my/whisper-large-v2/fleurs\endcsname{4.0}
\expandafter\def\csname v@my/whisper-large-v2/gain\endcsname{4.8}
\expandafter\def\csname v@my/whisper-large-v2/gain-ci\endcsname{3.0 to 6.5}
\expandafter\def\csname v@my/whisper-large-v2/left\endcsname{11.6}
\expandafter\def\csname v@my/whisper-large-v2/left-wer\endcsname{18.7}
\expandafter\def\csname v@my/whisper-large-v2/left/animation\endcsname{3.4}
\expandafter\def\csname v@my/whisper-large-v2/left/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/whisper-large-v2/left/drama\endcsname{10.7}
\expandafter\def\csname v@my/whisper-large-v2/left/fleurs\endcsname{2.1}
\expandafter\def\csname v@my/whisper-large-v2/left/news\endcsname{4.5}
\expandafter\def\csname v@my/whisper-large-v2/left/parliament\endcsname{5.5}
\expandafter\def\csname v@my/whisper-large-v2/left/podcast\endcsname{12.1}
\expandafter\def\csname v@my/whisper-large-v2/left/read-speech\endcsname{2.6}
\expandafter\def\csname v@my/whisper-large-v2/left/short-inputs\endcsname{34.9}
\expandafter\def\csname v@my/whisper-large-v2/left/singing\endcsname{14.0}
\expandafter\def\csname v@my/whisper-large-v2/left/street interview\endcsname{19.7}
\expandafter\def\csname v@my/whisper-large-v2/left/telephony\endcsname{26.6}
\expandafter\def\csname v@my/whisper-large-v2/news\endcsname{4.1}
\expandafter\def\csname v@my/whisper-large-v2/parliament\endcsname{5.9}
\expandafter\def\csname v@my/whisper-large-v2/podcast\endcsname{4.8}
\expandafter\def\csname v@my/whisper-large-v2/rank\endcsname{2}
\expandafter\def\csname v@my/whisper-large-v2/rank-word\endcsname{second best}
\expandafter\def\csname v@my/whisper-large-v2/read-speech\endcsname{2.1}
\expandafter\def\csname v@my/whisper-large-v2/short-inputs\endcsname{4.0}
\expandafter\def\csname v@my/whisper-large-v2/singing\endcsname{17.6}
\expandafter\def\csname v@my/whisper-large-v2/street interview\endcsname{12.1}
\expandafter\def\csname v@my/whisper-large-v2/telephony\endcsname{12.8}
\expandafter\def\csname v@my/whisper-large-v2/told\endcsname{16.5}
\expandafter\def\csname v@my/whisper-large-v2/told-gain\endcsname{9.7}
\expandafter\def\csname v@my/whisper-large-v2/told-wer\endcsname{24.2}
\expandafter\def\csname v@my/whisper-large-v2/told/animation\endcsname{4.3}
\expandafter\def\csname v@my/whisper-large-v2/told/commonvoice\endcsname{3.0}
\expandafter\def\csname v@my/whisper-large-v2/told/drama\endcsname{10.7}
\expandafter\def\csname v@my/whisper-large-v2/told/fleurs\endcsname{2.1}
\expandafter\def\csname v@my/whisper-large-v2/told/news\endcsname{24.5}
\expandafter\def\csname v@my/whisper-large-v2/told/parliament\endcsname{5.5}
\expandafter\def\csname v@my/whisper-large-v2/told/podcast\endcsname{12.0}
\expandafter\def\csname v@my/whisper-large-v2/told/read-speech\endcsname{1.3}
\expandafter\def\csname v@my/whisper-large-v2/told/short-inputs\endcsname{45.7}
\expandafter\def\csname v@my/whisper-large-v2/told/singing\endcsname{13.8}
\expandafter\def\csname v@my/whisper-large-v2/told/street interview\endcsname{19.8}
\expandafter\def\csname v@my/whisper-large-v2/told/telephony\endcsname{55.7}
\expandafter\def\csname v@my/whisper-large-v3-turbo/after\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/after-wer\endcsname{19.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/animation\endcsname{7.1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/animation\endcsname{3.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/commonvoice\endcsname{2.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/drama\endcsname{9.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/fleurs\endcsname{1.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/news\endcsname{2.5}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/parliament\endcsname{8.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/podcast\endcsname{8.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/read-speech\endcsname{1.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/short-inputs\endcsname{16.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/singing\endcsname{13.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/street interview\endcsname{15.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/base/telephony\endcsname{17.3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/commonvoice\endcsname{4.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-dev-first\endcsname{19.7}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-dev-last\endcsname{19.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-first\endcsname{8.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-last\endcsname{8.3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-low\endcsname{8.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/curve-pick\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/detect\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/detect-en-as-ms\endcsname{4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/detect-ms-as-en\endcsname{3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/detect-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/detect/telephony\endcsname{17.3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/drama\endcsname{8.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/en-as-ms\endcsname{20}
\expandafter\def\csname v@my/whisper-large-v3-turbo/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/en-as-ms-share\endcsname{26}
\expandafter\def\csname v@my/whisper-large-v3-turbo/epoch\endcsname{3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/fleurs\endcsname{4.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/gain\endcsname{0.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/gain-ci\endcsname{-1.4 to 1.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/animation\endcsname{3.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/commonvoice\endcsname{2.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/drama\endcsname{9.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/fleurs\endcsname{1.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/news\endcsname{2.5}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/parliament\endcsname{8.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/podcast\endcsname{8.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/read-speech\endcsname{1.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/short-inputs\endcsname{16.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/singing\endcsname{13.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/street interview\endcsname{15.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/left/telephony\endcsname{17.3}
\expandafter\def\csname v@my/whisper-large-v3-turbo/news\endcsname{4.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/parliament\endcsname{8.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/podcast\endcsname{4.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/rank\endcsname{6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/rank-word\endcsname{sixth best}
\expandafter\def\csname v@my/whisper-large-v3-turbo/read-speech\endcsname{2.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/short-inputs\endcsname{6.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/singing\endcsname{22.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/street interview\endcsname{14.1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/telephony\endcsname{14.1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told\endcsname{10.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told-gain\endcsname{1.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told-wer\endcsname{17.1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/animation\endcsname{4.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/commonvoice\endcsname{2.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/drama\endcsname{9.1}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/fleurs\endcsname{1.9}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/news\endcsname{11.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/parliament\endcsname{8.6}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/podcast\endcsname{9.4}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/read-speech\endcsname{0.8}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/short-inputs\endcsname{19.0}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/singing\endcsname{13.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/street interview\endcsname{15.2}
\expandafter\def\csname v@my/whisper-large-v3-turbo/told/telephony\endcsname{26.4}
\expandafter\def\csname v@my/whisper-large-v3/after\endcsname{6.0}
\expandafter\def\csname v@my/whisper-large-v3/after-wer\endcsname{13.3}
\expandafter\def\csname v@my/whisper-large-v3/animation\endcsname{3.8}
\expandafter\def\csname v@my/whisper-large-v3/base\endcsname{8.9}
\expandafter\def\csname v@my/whisper-large-v3/base-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3/base/animation\endcsname{3.8}
\expandafter\def\csname v@my/whisper-large-v3/base/commonvoice\endcsname{2.7}
\expandafter\def\csname v@my/whisper-large-v3/base/drama\endcsname{8.5}
\expandafter\def\csname v@my/whisper-large-v3/base/fleurs\endcsname{1.8}
\expandafter\def\csname v@my/whisper-large-v3/base/news\endcsname{3.0}
\expandafter\def\csname v@my/whisper-large-v3/base/parliament\endcsname{12.2}
\expandafter\def\csname v@my/whisper-large-v3/base/podcast\endcsname{6.0}
\expandafter\def\csname v@my/whisper-large-v3/base/read-speech\endcsname{2.2}
\expandafter\def\csname v@my/whisper-large-v3/base/short-inputs\endcsname{19.9}
\expandafter\def\csname v@my/whisper-large-v3/base/singing\endcsname{14.0}
\expandafter\def\csname v@my/whisper-large-v3/base/street interview\endcsname{15.1}
\expandafter\def\csname v@my/whisper-large-v3/base/telephony\endcsname{17.8}
\expandafter\def\csname v@my/whisper-large-v3/commonvoice\endcsname{2.8}
\expandafter\def\csname v@my/whisper-large-v3/curve-dev-first\endcsname{17.6}
\expandafter\def\csname v@my/whisper-large-v3/curve-dev-last\endcsname{18.0}
\expandafter\def\csname v@my/whisper-large-v3/curve-first\endcsname{5.5}
\expandafter\def\csname v@my/whisper-large-v3/curve-last\endcsname{5.8}
\expandafter\def\csname v@my/whisper-large-v3/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/whisper-large-v3/curve-low\endcsname{5.5}
\expandafter\def\csname v@my/whisper-large-v3/curve-low-epoch\endcsname{1}
\expandafter\def\csname v@my/whisper-large-v3/curve-pick\endcsname{6.0}
\expandafter\def\csname v@my/whisper-large-v3/detect\endcsname{8.9}
\expandafter\def\csname v@my/whisper-large-v3/detect-en-as-ms\endcsname{9}
\expandafter\def\csname v@my/whisper-large-v3/detect-ms-as-en\endcsname{2}
\expandafter\def\csname v@my/whisper-large-v3/detect-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3/detect/telephony\endcsname{17.8}
\expandafter\def\csname v@my/whisper-large-v3/drama\endcsname{4.6}
\expandafter\def\csname v@my/whisper-large-v3/en-as-ms\endcsname{57}
\expandafter\def\csname v@my/whisper-large-v3/en-as-ms-after\endcsname{0}
\expandafter\def\csname v@my/whisper-large-v3/en-as-ms-after-word\endcsname{none}
\expandafter\def\csname v@my/whisper-large-v3/en-as-ms-share\endcsname{46}
\expandafter\def\csname v@my/whisper-large-v3/epoch\endcsname{2}
\expandafter\def\csname v@my/whisper-large-v3/fleurs\endcsname{2.7}
\expandafter\def\csname v@my/whisper-large-v3/gain\endcsname{2.9}
\expandafter\def\csname v@my/whisper-large-v3/gain-ci\endcsname{1.6 to 4.4}
\expandafter\def\csname v@my/whisper-large-v3/left\endcsname{8.9}
\expandafter\def\csname v@my/whisper-large-v3/left-wer\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3/left/animation\endcsname{3.8}
\expandafter\def\csname v@my/whisper-large-v3/left/commonvoice\endcsname{2.7}
\expandafter\def\csname v@my/whisper-large-v3/left/drama\endcsname{8.5}
\expandafter\def\csname v@my/whisper-large-v3/left/fleurs\endcsname{1.8}
\expandafter\def\csname v@my/whisper-large-v3/left/news\endcsname{3.0}
\expandafter\def\csname v@my/whisper-large-v3/left/parliament\endcsname{12.2}
\expandafter\def\csname v@my/whisper-large-v3/left/podcast\endcsname{6.0}
\expandafter\def\csname v@my/whisper-large-v3/left/read-speech\endcsname{2.2}
\expandafter\def\csname v@my/whisper-large-v3/left/short-inputs\endcsname{19.9}
\expandafter\def\csname v@my/whisper-large-v3/left/singing\endcsname{14.0}
\expandafter\def\csname v@my/whisper-large-v3/left/street interview\endcsname{15.1}
\expandafter\def\csname v@my/whisper-large-v3/left/telephony\endcsname{17.8}
\expandafter\def\csname v@my/whisper-large-v3/news\endcsname{4.7}
\expandafter\def\csname v@my/whisper-large-v3/parliament\endcsname{3.9}
\expandafter\def\csname v@my/whisper-large-v3/podcast\endcsname{2.9}
\expandafter\def\csname v@my/whisper-large-v3/rank\endcsname{1}
\expandafter\def\csname v@my/whisper-large-v3/rank-word\endcsname{best}
\expandafter\def\csname v@my/whisper-large-v3/read-speech\endcsname{0.9}
\expandafter\def\csname v@my/whisper-large-v3/short-inputs\endcsname{7.0}
\expandafter\def\csname v@my/whisper-large-v3/singing\endcsname{17.1}
\expandafter\def\csname v@my/whisper-large-v3/street interview\endcsname{9.9}
\expandafter\def\csname v@my/whisper-large-v3/telephony\endcsname{11.7}
\expandafter\def\csname v@my/whisper-large-v3/told\endcsname{14.9}
\expandafter\def\csname v@my/whisper-large-v3/told-gain\endcsname{8.9}
\expandafter\def\csname v@my/whisper-large-v3/told-wer\endcsname{22.0}
\expandafter\def\csname v@my/whisper-large-v3/told/animation\endcsname{4.6}
\expandafter\def\csname v@my/whisper-large-v3/told/commonvoice\endcsname{2.7}
\expandafter\def\csname v@my/whisper-large-v3/told/drama\endcsname{8.5}
\expandafter\def\csname v@my/whisper-large-v3/told/fleurs\endcsname{1.8}
\expandafter\def\csname v@my/whisper-large-v3/told/news\endcsname{22.6}
\expandafter\def\csname v@my/whisper-large-v3/told/parliament\endcsname{12.2}
\expandafter\def\csname v@my/whisper-large-v3/told/podcast\endcsname{6.0}
\expandafter\def\csname v@my/whisper-large-v3/told/read-speech\endcsname{1.0}
\expandafter\def\csname v@my/whisper-large-v3/told/short-inputs\endcsname{31.6}
\expandafter\def\csname v@my/whisper-large-v3/told/singing\endcsname{13.3}
\expandafter\def\csname v@my/whisper-large-v3/told/street interview\endcsname{15.2}
\expandafter\def\csname v@my/whisper-large-v3/told/telephony\endcsname{58.8}
\expandafter\def\csname v@my/whisper-medium/after\endcsname{6.9}
\expandafter\def\csname v@my/whisper-medium/after-wer\endcsname{16.1}
\expandafter\def\csname v@my/whisper-medium/animation\endcsname{5.9}
\expandafter\def\csname v@my/whisper-medium/base\endcsname{12.4}
\expandafter\def\csname v@my/whisper-medium/base-wer\endcsname{22.0}
\expandafter\def\csname v@my/whisper-medium/base/animation\endcsname{4.6}
\expandafter\def\csname v@my/whisper-medium/base/commonvoice\endcsname{3.6}
\expandafter\def\csname v@my/whisper-medium/base/drama\endcsname{13.2}
\expandafter\def\csname v@my/whisper-medium/base/fleurs\endcsname{3.1}
\expandafter\def\csname v@my/whisper-medium/base/news\endcsname{4.9}
\expandafter\def\csname v@my/whisper-medium/base/parliament\endcsname{6.6}
\expandafter\def\csname v@my/whisper-medium/base/podcast\endcsname{15.8}
\expandafter\def\csname v@my/whisper-medium/base/read-speech\endcsname{5.4}
\expandafter\def\csname v@my/whisper-medium/base/short-inputs\endcsname{28.0}
\expandafter\def\csname v@my/whisper-medium/base/singing\endcsname{8.0}
\expandafter\def\csname v@my/whisper-medium/base/street interview\endcsname{25.5}
\expandafter\def\csname v@my/whisper-medium/base/telephony\endcsname{30.4}
\expandafter\def\csname v@my/whisper-medium/commonvoice\endcsname{4.1}
\expandafter\def\csname v@my/whisper-medium/curve-dev-first\endcsname{20.1}
\expandafter\def\csname v@my/whisper-medium/curve-dev-last\endcsname{19.0}
\expandafter\def\csname v@my/whisper-medium/curve-first\endcsname{7.0}
\expandafter\def\csname v@my/whisper-medium/curve-last\endcsname{8.1}
\expandafter\def\csname v@my/whisper-medium/curve-last-epoch\endcsname{5}
\expandafter\def\csname v@my/whisper-medium/curve-low\endcsname{6.6}
\expandafter\def\csname v@my/whisper-medium/curve-low-epoch\endcsname{3}
\expandafter\def\csname v@my/whisper-medium/curve-pick\endcsname{6.9}
\expandafter\def\csname v@my/whisper-medium/detect\endcsname{12.4}
\expandafter\def\csname v@my/whisper-medium/detect-en-as-ms\endcsname{25}
\expandafter\def\csname v@my/whisper-medium/detect-ms-as-en\endcsname{1}
\expandafter\def\csname v@my/whisper-medium/detect-wer\endcsname{22.0}
\expandafter\def\csname v@my/whisper-medium/detect/telephony\endcsname{30.4}
\expandafter\def\csname v@my/whisper-medium/drama\endcsname{5.2}
\expandafter\def\csname v@my/whisper-medium/en-as-ms\endcsname{69}
\expandafter\def\csname v@my/whisper-medium/en-as-ms-after\endcsname{2}
\expandafter\def\csname v@my/whisper-medium/en-as-ms-after-word\endcsname{2}
\expandafter\def\csname v@my/whisper-medium/en-as-ms-share\endcsname{44}
\expandafter\def\csname v@my/whisper-medium/epoch\endcsname{2}
\expandafter\def\csname v@my/whisper-medium/fleurs\endcsname{4.2}
\expandafter\def\csname v@my/whisper-medium/gain\endcsname{5.6}
\expandafter\def\csname v@my/whisper-medium/gain-ci\endcsname{3.8 to 7.3}
\expandafter\def\csname v@my/whisper-medium/left\endcsname{12.4}
\expandafter\def\csname v@my/whisper-medium/left-wer\endcsname{22.0}
\expandafter\def\csname v@my/whisper-medium/left/animation\endcsname{4.6}
\expandafter\def\csname v@my/whisper-medium/left/commonvoice\endcsname{3.6}
\expandafter\def\csname v@my/whisper-medium/left/drama\endcsname{13.2}
\expandafter\def\csname v@my/whisper-medium/left/fleurs\endcsname{3.1}
\expandafter\def\csname v@my/whisper-medium/left/news\endcsname{4.9}
\expandafter\def\csname v@my/whisper-medium/left/parliament\endcsname{6.6}
\expandafter\def\csname v@my/whisper-medium/left/podcast\endcsname{15.8}
\expandafter\def\csname v@my/whisper-medium/left/read-speech\endcsname{5.4}
\expandafter\def\csname v@my/whisper-medium/left/short-inputs\endcsname{28.0}
\expandafter\def\csname v@my/whisper-medium/left/singing\endcsname{8.0}
\expandafter\def\csname v@my/whisper-medium/left/street interview\endcsname{25.5}
\expandafter\def\csname v@my/whisper-medium/left/telephony\endcsname{30.4}
\expandafter\def\csname v@my/whisper-medium/news\endcsname{3.6}
\expandafter\def\csname v@my/whisper-medium/parliament\endcsname{6.0}
\expandafter\def\csname v@my/whisper-medium/podcast\endcsname{4.2}
\expandafter\def\csname v@my/whisper-medium/rank\endcsname{3}
\expandafter\def\csname v@my/whisper-medium/rank-word\endcsname{third best}
\expandafter\def\csname v@my/whisper-medium/read-speech\endcsname{2.7}
\expandafter\def\csname v@my/whisper-medium/short-inputs\endcsname{4.4}
\expandafter\def\csname v@my/whisper-medium/singing\endcsname{18.4}
\expandafter\def\csname v@my/whisper-medium/street interview\endcsname{11.5}
\expandafter\def\csname v@my/whisper-medium/telephony\endcsname{12.1}
\expandafter\def\csname v@my/whisper-medium/told\endcsname{17.7}
\expandafter\def\csname v@my/whisper-medium/told-gain\endcsname{10.8}
\expandafter\def\csname v@my/whisper-medium/told-wer\endcsname{27.8}
\expandafter\def\csname v@my/whisper-medium/told/animation\endcsname{5.4}
\expandafter\def\csname v@my/whisper-medium/told/commonvoice\endcsname{3.6}
\expandafter\def\csname v@my/whisper-medium/told/drama\endcsname{13.2}
\expandafter\def\csname v@my/whisper-medium/told/fleurs\endcsname{3.1}
\expandafter\def\csname v@my/whisper-medium/told/news\endcsname{25.9}
\expandafter\def\csname v@my/whisper-medium/told/parliament\endcsname{6.1}
\expandafter\def\csname v@my/whisper-medium/told/podcast\endcsname{15.8}
\expandafter\def\csname v@my/whisper-medium/told/read-speech\endcsname{3.7}
\expandafter\def\csname v@my/whisper-medium/told/short-inputs\endcsname{38.3}
\expandafter\def\csname v@my/whisper-medium/told/singing\endcsname{8.6}
\expandafter\def\csname v@my/whisper-medium/told/street interview\endcsname{25.4}
\expandafter\def\csname v@my/whisper-medium/told/telephony\endcsname{63.0}
\expandafter\def\csname v@my/whisper-small/after\endcsname{11.7}
\expandafter\def\csname v@my/whisper-small/after-wer\endcsname{27.1}
\expandafter\def\csname v@my/whisper-small/animation\endcsname{9.2}
\expandafter\def\csname v@my/whisper-small/base\endcsname{17.3}
\expandafter\def\csname v@my/whisper-small/base-wer\endcsname{30.8}
\expandafter\def\csname v@my/whisper-small/base/animation\endcsname{10.9}
\expandafter\def\csname v@my/whisper-small/base/commonvoice\endcsname{5.9}
\expandafter\def\csname v@my/whisper-small/base/drama\endcsname{15.3}
\expandafter\def\csname v@my/whisper-small/base/fleurs\endcsname{5.2}
\expandafter\def\csname v@my/whisper-small/base/news\endcsname{6.5}
\expandafter\def\csname v@my/whisper-small/base/parliament\endcsname{9.3}
\expandafter\def\csname v@my/whisper-small/base/podcast\endcsname{20.7}
\expandafter\def\csname v@my/whisper-small/base/read-speech\endcsname{7.7}
\expandafter\def\csname v@my/whisper-small/base/short-inputs\endcsname{39.4}
\expandafter\def\csname v@my/whisper-small/base/singing\endcsname{30.9}
\expandafter\def\csname v@my/whisper-small/base/street interview\endcsname{27.6}
\expandafter\def\csname v@my/whisper-small/base/telephony\endcsname{28.0}
\expandafter\def\csname v@my/whisper-small/commonvoice\endcsname{7.3}
\expandafter\def\csname v@my/whisper-small/curve-dev-first\endcsname{22.6}
\expandafter\def\csname v@my/whisper-small/curve-dev-last\endcsname{21.0}
\expandafter\def\csname v@my/whisper-small/curve-first\endcsname{11.8}
\expandafter\def\csname v@my/whisper-small/curve-last\endcsname{14.0}
\expandafter\def\csname v@my/whisper-small/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/whisper-small/curve-low\endcsname{11.3}
\expandafter\def\csname v@my/whisper-small/curve-low-epoch\endcsname{4}
\expandafter\def\csname v@my/whisper-small/curve-pick\endcsname{11.7}
\expandafter\def\csname v@my/whisper-small/detect\endcsname{17.3}
\expandafter\def\csname v@my/whisper-small/detect-en-as-ms\endcsname{20}
\expandafter\def\csname v@my/whisper-small/detect-ms-as-en\endcsname{5}
\expandafter\def\csname v@my/whisper-small/detect-wer\endcsname{30.8}
\expandafter\def\csname v@my/whisper-small/detect/telephony\endcsname{28.0}
\expandafter\def\csname v@my/whisper-small/drama\endcsname{15.0}
\expandafter\def\csname v@my/whisper-small/en-as-ms\endcsname{64}
\expandafter\def\csname v@my/whisper-small/en-as-ms-after\endcsname{4}
\expandafter\def\csname v@my/whisper-small/en-as-ms-after-word\endcsname{4}
\expandafter\def\csname v@my/whisper-small/en-as-ms-share\endcsname{30}
\expandafter\def\csname v@my/whisper-small/epoch\endcsname{3}
\expandafter\def\csname v@my/whisper-small/fleurs\endcsname{8.4}
\expandafter\def\csname v@my/whisper-small/gain\endcsname{5.6}
\expandafter\def\csname v@my/whisper-small/gain-ci\endcsname{3.9 to 7.4}
\expandafter\def\csname v@my/whisper-small/left\endcsname{17.3}
\expandafter\def\csname v@my/whisper-small/left-wer\endcsname{30.8}
\expandafter\def\csname v@my/whisper-small/left/animation\endcsname{10.9}
\expandafter\def\csname v@my/whisper-small/left/commonvoice\endcsname{5.9}
\expandafter\def\csname v@my/whisper-small/left/drama\endcsname{15.3}
\expandafter\def\csname v@my/whisper-small/left/fleurs\endcsname{5.2}
\expandafter\def\csname v@my/whisper-small/left/news\endcsname{6.5}
\expandafter\def\csname v@my/whisper-small/left/parliament\endcsname{9.3}
\expandafter\def\csname v@my/whisper-small/left/podcast\endcsname{20.7}
\expandafter\def\csname v@my/whisper-small/left/read-speech\endcsname{7.7}
\expandafter\def\csname v@my/whisper-small/left/short-inputs\endcsname{39.4}
\expandafter\def\csname v@my/whisper-small/left/singing\endcsname{30.9}
\expandafter\def\csname v@my/whisper-small/left/street interview\endcsname{27.6}
\expandafter\def\csname v@my/whisper-small/left/telephony\endcsname{28.0}
\expandafter\def\csname v@my/whisper-small/news\endcsname{7.4}
\expandafter\def\csname v@my/whisper-small/parliament\endcsname{10.4}
\expandafter\def\csname v@my/whisper-small/podcast\endcsname{7.6}
\expandafter\def\csname v@my/whisper-small/rank\endcsname{11}
\expandafter\def\csname v@my/whisper-small/rank-word\endcsname{eleventh best}
\expandafter\def\csname v@my/whisper-small/read-speech\endcsname{6.2}
\expandafter\def\csname v@my/whisper-small/short-inputs\endcsname{5.8}
\expandafter\def\csname v@my/whisper-small/singing\endcsname{31.1}
\expandafter\def\csname v@my/whisper-small/street interview\endcsname{16.8}
\expandafter\def\csname v@my/whisper-small/telephony\endcsname{15.4}
\expandafter\def\csname v@my/whisper-small/told\endcsname{21.0}
\expandafter\def\csname v@my/whisper-small/told-gain\endcsname{9.3}
\expandafter\def\csname v@my/whisper-small/told-wer\endcsname{35.5}
\expandafter\def\csname v@my/whisper-small/told/animation\endcsname{11.4}
\expandafter\def\csname v@my/whisper-small/told/commonvoice\endcsname{5.8}
\expandafter\def\csname v@my/whisper-small/told/drama\endcsname{15.1}
\expandafter\def\csname v@my/whisper-small/told/fleurs\endcsname{4.7}
\expandafter\def\csname v@my/whisper-small/told/news\endcsname{29.1}
\expandafter\def\csname v@my/whisper-small/told/parliament\endcsname{8.2}
\expandafter\def\csname v@my/whisper-small/told/podcast\endcsname{20.6}
\expandafter\def\csname v@my/whisper-small/told/read-speech\endcsname{3.9}
\expandafter\def\csname v@my/whisper-small/told/short-inputs\endcsname{40.7}
\expandafter\def\csname v@my/whisper-small/told/singing\endcsname{22.1}
\expandafter\def\csname v@my/whisper-small/told/street interview\endcsname{27.2}
\expandafter\def\csname v@my/whisper-small/told/telephony\endcsname{63.7}
\expandafter\def\csname v@my/whisper-tiny/after\endcsname{30.6}
\expandafter\def\csname v@my/whisper-tiny/after-wer\endcsname{56.8}
\expandafter\def\csname v@my/whisper-tiny/animation\endcsname{32.9}
\expandafter\def\csname v@my/whisper-tiny/base\endcsname{37.7}
\expandafter\def\csname v@my/whisper-tiny/base-wer\endcsname{65.8}
\expandafter\def\csname v@my/whisper-tiny/base/animation\endcsname{29.8}
\expandafter\def\csname v@my/whisper-tiny/base/commonvoice\endcsname{19.5}
\expandafter\def\csname v@my/whisper-tiny/base/drama\endcsname{36.7}
\expandafter\def\csname v@my/whisper-tiny/base/fleurs\endcsname{19.8}
\expandafter\def\csname v@my/whisper-tiny/base/news\endcsname{42.0}
\expandafter\def\csname v@my/whisper-tiny/base/parliament\endcsname{24.6}
\expandafter\def\csname v@my/whisper-tiny/base/podcast\endcsname{44.7}
\expandafter\def\csname v@my/whisper-tiny/base/read-speech\endcsname{18.4}
\expandafter\def\csname v@my/whisper-tiny/base/short-inputs\endcsname{39.0}
\expandafter\def\csname v@my/whisper-tiny/base/singing\endcsname{51.3}
\expandafter\def\csname v@my/whisper-tiny/base/street interview\endcsname{57.3}
\expandafter\def\csname v@my/whisper-tiny/base/telephony\endcsname{69.5}
\expandafter\def\csname v@my/whisper-tiny/commonvoice\endcsname{23.9}
\expandafter\def\csname v@my/whisper-tiny/curve-dev-first\endcsname{39.7}
\expandafter\def\csname v@my/whisper-tiny/curve-dev-last\endcsname{30.9}
\expandafter\def\csname v@my/whisper-tiny/curve-first\endcsname{30.9}
\expandafter\def\csname v@my/whisper-tiny/curve-last\endcsname{36.6}
\expandafter\def\csname v@my/whisper-tiny/curve-last-epoch\endcsname{10}
\expandafter\def\csname v@my/whisper-tiny/curve-low\endcsname{28.4}
\expandafter\def\csname v@my/whisper-tiny/curve-low-epoch\endcsname{2}
\expandafter\def\csname v@my/whisper-tiny/curve-pick\endcsname{30.6}
\expandafter\def\csname v@my/whisper-tiny/detect\endcsname{38.5}
\expandafter\def\csname v@my/whisper-tiny/detect-en-as-ms\endcsname{21}
\expandafter\def\csname v@my/whisper-tiny/detect-ms-as-en\endcsname{34}
\expandafter\def\csname v@my/whisper-tiny/detect-wer\endcsname{64.9}
\expandafter\def\csname v@my/whisper-tiny/detect/telephony\endcsname{41.5}
\expandafter\def\csname v@my/whisper-tiny/drama\endcsname{25.6}
\expandafter\def\csname v@my/whisper-tiny/en-as-ms\endcsname{62}
\expandafter\def\csname v@my/whisper-tiny/en-as-ms-after\endcsname{7}
\expandafter\def\csname v@my/whisper-tiny/en-as-ms-after-word\endcsname{7}
\expandafter\def\csname v@my/whisper-tiny/en-as-ms-share\endcsname{17}
\expandafter\def\csname v@my/whisper-tiny/epoch\endcsname{4}
\expandafter\def\csname v@my/whisper-tiny/fleurs\endcsname{29.8}
\expandafter\def\csname v@my/whisper-tiny/gain\endcsname{7.1}
\expandafter\def\csname v@my/whisper-tiny/gain-ci\endcsname{4.8 to 9.3}
\expandafter\def\csname v@my/whisper-tiny/left\endcsname{38.5}
\expandafter\def\csname v@my/whisper-tiny/left-wer\endcsname{64.9}
\expandafter\def\csname v@my/whisper-tiny/left/animation\endcsname{38.2}
\expandafter\def\csname v@my/whisper-tiny/left/commonvoice\endcsname{20.9}
\expandafter\def\csname v@my/whisper-tiny/left/drama\endcsname{37.9}
\expandafter\def\csname v@my/whisper-tiny/left/fleurs\endcsname{22.7}
\expandafter\def\csname v@my/whisper-tiny/left/news\endcsname{24.1}
\expandafter\def\csname v@my/whisper-tiny/left/parliament\endcsname{27.1}
\expandafter\def\csname v@my/whisper-tiny/left/podcast\endcsname{44.0}
\expandafter\def\csname v@my/whisper-tiny/left/read-speech\endcsname{28.2}
\expandafter\def\csname v@my/whisper-tiny/left/short-inputs\endcsname{46.9}
\expandafter\def\csname v@my/whisper-tiny/left/singing\endcsname{71.9}
\expandafter\def\csname v@my/whisper-tiny/left/street interview\endcsname{58.8}
\expandafter\def\csname v@my/whisper-tiny/left/telephony\endcsname{41.5}
\expandafter\def\csname v@my/whisper-tiny/news\endcsname{30.6}
\expandafter\def\csname v@my/whisper-tiny/parliament\endcsname{29.1}
\expandafter\def\csname v@my/whisper-tiny/podcast\endcsname{23.4}
\expandafter\def\csname v@my/whisper-tiny/rank\endcsname{23}
\expandafter\def\csname v@my/whisper-tiny/read-speech\endcsname{21.7}
\expandafter\def\csname v@my/whisper-tiny/short-inputs\endcsname{20.6}
\expandafter\def\csname v@my/whisper-tiny/singing\endcsname{67.5}
\expandafter\def\csname v@my/whisper-tiny/street interview\endcsname{36.1}
\expandafter\def\csname v@my/whisper-tiny/telephony\endcsname{26.1}
\expandafter\def\csname v@my/whisper-tiny/told\endcsname{37.7}
\expandafter\def\csname v@my/whisper-tiny/told-gain\endcsname{7.1}
\expandafter\def\csname v@my/whisper-tiny/told-wer\endcsname{65.8}
\expandafter\def\csname v@my/whisper-tiny/told/animation\endcsname{29.8}
\expandafter\def\csname v@my/whisper-tiny/told/commonvoice\endcsname{19.5}
\expandafter\def\csname v@my/whisper-tiny/told/drama\endcsname{36.7}
\expandafter\def\csname v@my/whisper-tiny/told/fleurs\endcsname{19.8}
\expandafter\def\csname v@my/whisper-tiny/told/news\endcsname{42.0}
\expandafter\def\csname v@my/whisper-tiny/told/parliament\endcsname{24.6}
\expandafter\def\csname v@my/whisper-tiny/told/podcast\endcsname{44.7}
\expandafter\def\csname v@my/whisper-tiny/told/read-speech\endcsname{18.4}
\expandafter\def\csname v@my/whisper-tiny/told/short-inputs\endcsname{39.0}
\expandafter\def\csname v@my/whisper-tiny/told/singing\endcsname{51.3}
\expandafter\def\csname v@my/whisper-tiny/told/street interview\endcsname{57.3}
\expandafter\def\csname v@my/whisper-tiny/told/telephony\endcsname{69.5}
\expandafter\def\csname v@mycs/after-gap-median\endcsname{1.7}
\expandafter\def\csname v@mycs/before-gap-median\endcsname{7.5}
\expandafter\def\csname v@mycs/cohere-transcribe/after-mixed\endcsname{9.8}
\expandafter\def\csname v@mycs/cohere-transcribe/after-plain\endcsname{10.5}
\expandafter\def\csname v@mycs/cohere-transcribe/before-mixed\endcsname{52.4}
\expandafter\def\csname v@mycs/cohere-transcribe/before-plain\endcsname{62.3}
\expandafter\def\csname v@mycs/cohere-transcribe/strat-extra\endcsname{-24.0}
\expandafter\def\csname v@mycs/en-share\endcsname{9.4}
\expandafter\def\csname v@mycs/gain-mixed-median\endcsname{10.9}
\expandafter\def\csname v@mycs/gain-plain-median\endcsname{-0.3}
\expandafter\def\csname v@mycs/gemma4-12b/after-mixed\endcsname{17.4}
\expandafter\def\csname v@mycs/gemma4-12b/after-plain\endcsname{19.8}
\expandafter\def\csname v@mycs/gemma4-12b/before-mixed\endcsname{43.9}
\expandafter\def\csname v@mycs/gemma4-12b/before-plain\endcsname{47.0}
\expandafter\def\csname v@mycs/gemma4-12b/strat-extra\endcsname{-25.3}
\expandafter\def\csname v@mycs/gemma4-e2b/after-mixed\endcsname{11.6}
\expandafter\def\csname v@mycs/gemma4-e2b/after-plain\endcsname{9.1}
\expandafter\def\csname v@mycs/gemma4-e2b/before-mixed\endcsname{10.1}
\expandafter\def\csname v@mycs/gemma4-e2b/before-plain\endcsname{4.6}
\expandafter\def\csname v@mycs/gemma4-e2b/strat-extra\endcsname{-0.4}
\expandafter\def\csname v@mycs/gemma4-e4b/after-mixed\endcsname{8.5}
\expandafter\def\csname v@mycs/gemma4-e4b/after-plain\endcsname{4.8}
\expandafter\def\csname v@mycs/gemma4-e4b/before-mixed\endcsname{9.0}
\expandafter\def\csname v@mycs/gemma4-e4b/before-plain\endcsname{3.8}
\expandafter\def\csname v@mycs/gemma4-e4b/strat-extra\endcsname{0.7}
\expandafter\def\csname v@mycs/granite-2b/after-mixed\endcsname{19.0}
\expandafter\def\csname v@mycs/granite-2b/after-plain\endcsname{25.6}
\expandafter\def\csname v@mycs/granite-2b/before-mixed\endcsname{36.4}
\expandafter\def\csname v@mycs/granite-2b/before-plain\endcsname{42.5}
\expandafter\def\csname v@mycs/granite-2b/strat-extra\endcsname{-15.4}
\expandafter\def\csname v@mycs/lfm3-audio/after-mixed\endcsname{15.1}
\expandafter\def\csname v@mycs/lfm3-audio/after-plain\endcsname{17.5}
\expandafter\def\csname v@mycs/lfm3-audio/before-mixed\endcsname{52.0}
\expandafter\def\csname v@mycs/lfm3-audio/before-plain\endcsname{65.5}
\expandafter\def\csname v@mycs/lfm3-audio/strat-extra\endcsname{-18.1}
\expandafter\def\csname v@mycs/mixed\endcsname{171}
\expandafter\def\csname v@mycs/mixed-worse-after-n\endcsname{16}
\expandafter\def\csname v@mycs/mms-1b/after-mixed\endcsname{11.3}
\expandafter\def\csname v@mycs/mms-1b/after-plain\endcsname{7.1}
\expandafter\def\csname v@mycs/mms-1b/before-mixed\endcsname{18.8}
\expandafter\def\csname v@mycs/mms-1b/before-plain\endcsname{5.7}
\expandafter\def\csname v@mycs/mms-1b/strat-extra\endcsname{-0.7}
\expandafter\def\csname v@mycs/models\endcsname{23}
\expandafter\def\csname v@mycs/n\endcsname{820}
\expandafter\def\csname v@mycs/nemotron-30b/after-mixed\endcsname{9.7}
\expandafter\def\csname v@mycs/nemotron-30b/after-plain\endcsname{9.3}
\expandafter\def\csname v@mycs/nemotron-30b/before-mixed\endcsname{22.0}
\expandafter\def\csname v@mycs/nemotron-30b/before-plain\endcsname{18.0}
\expandafter\def\csname v@mycs/nemotron-30b/strat-extra\endcsname{-10.5}
\expandafter\def\csname v@mycs/nemotron-stream/after-mixed\endcsname{48.0}
\expandafter\def\csname v@mycs/nemotron-stream/after-plain\endcsname{49.2}
\expandafter\def\csname v@mycs/nemotron-stream/before-mixed\endcsname{58.9}
\expandafter\def\csname v@mycs/nemotron-stream/before-plain\endcsname{77.3}
\expandafter\def\csname v@mycs/nemotron-stream/strat-extra\endcsname{-22.9}
\expandafter\def\csname v@mycs/omni-ctc-1b/after-mixed\endcsname{12.2}
\expandafter\def\csname v@mycs/omni-ctc-1b/after-plain\endcsname{8.2}
\expandafter\def\csname v@mycs/omni-ctc-1b/before-mixed\endcsname{23.8}
\expandafter\def\csname v@mycs/omni-ctc-1b/before-plain\endcsname{7.6}
\expandafter\def\csname v@mycs/omni-ctc-1b/strat-extra\endcsname{2.8}
\expandafter\def\csname v@mycs/omni-ctc-300m/after-mixed\endcsname{15.8}
\expandafter\def\csname v@mycs/omni-ctc-300m/after-plain\endcsname{10.9}
\expandafter\def\csname v@mycs/omni-ctc-300m/before-mixed\endcsname{28.8}
\expandafter\def\csname v@mycs/omni-ctc-300m/before-plain\endcsname{11.6}
\expandafter\def\csname v@mycs/omni-ctc-300m/strat-extra\endcsname{3.8}
\expandafter\def\csname v@mycs/omni-ctc-7b/after-mixed\endcsname{8.1}
\expandafter\def\csname v@mycs/omni-ctc-7b/after-plain\endcsname{4.9}
\expandafter\def\csname v@mycs/omni-ctc-7b/before-mixed\endcsname{31.2}
\expandafter\def\csname v@mycs/omni-ctc-7b/before-plain\endcsname{9.2}
\expandafter\def\csname v@mycs/omni-ctc-7b/strat-extra\endcsname{6.6}
\expandafter\def\csname v@mycs/parakeet-tdt-v3/after-mixed\endcsname{15.4}
\expandafter\def\csname v@mycs/parakeet-tdt-v3/after-plain\endcsname{17.0}
\expandafter\def\csname v@mycs/parakeet-tdt-v3/before-mixed\endcsname{32.9}
\expandafter\def\csname v@mycs/parakeet-tdt-v3/before-plain\endcsname{38.1}
\expandafter\def\csname v@mycs/parakeet-tdt-v3/strat-extra\endcsname{-22.7}
\expandafter\def\csname v@mycs/plain\endcsname{564}
\expandafter\def\csname v@mycs/qwen3-asr-0.6b/after-mixed\endcsname{13.4}
\expandafter\def\csname v@mycs/qwen3-asr-0.6b/after-plain\endcsname{12.1}
\expandafter\def\csname v@mycs/qwen3-asr-0.6b/before-mixed\endcsname{14.9}
\expandafter\def\csname v@mycs/qwen3-asr-0.6b/before-plain\endcsname{6.9}
\expandafter\def\csname v@mycs/qwen3-asr-0.6b/strat-extra\endcsname{-2.2}
\expandafter\def\csname v@mycs/qwen3-asr-1.7b/after-mixed\endcsname{8.6}
\expandafter\def\csname v@mycs/qwen3-asr-1.7b/after-plain\endcsname{7.1}
\expandafter\def\csname v@mycs/qwen3-asr-1.7b/before-mixed\endcsname{10.5}
\expandafter\def\csname v@mycs/qwen3-asr-1.7b/before-plain\endcsname{4.7}
\expandafter\def\csname v@mycs/qwen3-asr-1.7b/strat-extra\endcsname{-4.1}
\expandafter\def\csname v@mycs/strat-cats\endcsname{9}
\expandafter\def\csname v@mycs/strat-extra-median\endcsname{-0.7}
\expandafter\def\csname v@mycs/strat-extra-pos\endcsname{10}
\expandafter\def\csname v@mycs/strat-mixed\endcsname{168}
\expandafter\def\csname v@mycs/strat-n\endcsname{23}
\expandafter\def\csname v@mycs/top-cat\endcsname{telephony}
\expandafter\def\csname v@mycs/top-cat-n\endcsname{45}
\expandafter\def\csname v@mycs/top-cat-of\endcsname{66}
\expandafter\def\csname v@mycs/train-en-share\endcsname{26}
\expandafter\def\csname v@mycs/train-mixed-share\endcsname{38}
\expandafter\def\csname v@mycs/voxtral-mini/after-mixed\endcsname{7.3}
\expandafter\def\csname v@mycs/voxtral-mini/after-plain\endcsname{8.3}
\expandafter\def\csname v@mycs/voxtral-mini/before-mixed\endcsname{32.1}
\expandafter\def\csname v@mycs/voxtral-mini/before-plain\endcsname{25.8}
\expandafter\def\csname v@mycs/voxtral-mini/strat-extra\endcsname{-9.5}
\expandafter\def\csname v@mycs/whisper-base/after-mixed\endcsname{25.1}
\expandafter\def\csname v@mycs/whisper-base/after-plain\endcsname{23.4}
\expandafter\def\csname v@mycs/whisper-base/before-mixed\endcsname{29.8}
\expandafter\def\csname v@mycs/whisper-base/before-plain\endcsname{14.5}
\expandafter\def\csname v@mycs/whisper-base/strat-extra\endcsname{0.2}
\expandafter\def\csname v@mycs/whisper-large-v2/after-mixed\endcsname{7.1}
\expandafter\def\csname v@mycs/whisper-large-v2/after-plain\endcsname{4.7}
\expandafter\def\csname v@mycs/whisper-large-v2/before-mixed\endcsname{15.4}
\expandafter\def\csname v@mycs/whisper-large-v2/before-plain\endcsname{3.6}
\expandafter\def\csname v@mycs/whisper-large-v2/strat-extra\endcsname{0.1}
\expandafter\def\csname v@mycs/whisper-large-v3-turbo/after-mixed\endcsname{8.5}
\expandafter\def\csname v@mycs/whisper-large-v3-turbo/after-plain\endcsname{5.7}
\expandafter\def\csname v@mycs/whisper-large-v3-turbo/before-mixed\endcsname{10.7}
\expandafter\def\csname v@mycs/whisper-large-v3-turbo/before-plain\endcsname{3.3}
\expandafter\def\csname v@mycs/whisper-large-v3-turbo/strat-extra\endcsname{-3.2}
\expandafter\def\csname v@mycs/whisper-large-v3/after-mixed\endcsname{6.4}
\expandafter\def\csname v@mycs/whisper-large-v3/after-plain\endcsname{3.2}
\expandafter\def\csname v@mycs/whisper-large-v3/before-mixed\endcsname{12.3}
\expandafter\def\csname v@mycs/whisper-large-v3/before-plain\endcsname{3.1}
\expandafter\def\csname v@mycs/whisper-large-v3/strat-extra\endcsname{0.6}
\expandafter\def\csname v@mycs/whisper-medium/after-mixed\endcsname{7.4}
\expandafter\def\csname v@mycs/whisper-medium/after-plain\endcsname{4.8}
\expandafter\def\csname v@mycs/whisper-medium/before-mixed\endcsname{18.0}
\expandafter\def\csname v@mycs/whisper-medium/before-plain\endcsname{4.6}
\expandafter\def\csname v@mycs/whisper-medium/strat-extra\endcsname{5.1}
\expandafter\def\csname v@mycs/whisper-small/after-mixed\endcsname{13.1}
\expandafter\def\csname v@mycs/whisper-small/after-plain\endcsname{8.8}
\expandafter\def\csname v@mycs/whisper-small/before-mixed\endcsname{20.9}
\expandafter\def\csname v@mycs/whisper-small/before-plain\endcsname{7.9}
\expandafter\def\csname v@mycs/whisper-small/strat-extra\endcsname{0.0}
\expandafter\def\csname v@mycs/whisper-tiny/after-mixed\endcsname{30.2}
\expandafter\def\csname v@mycs/whisper-tiny/after-plain\endcsname{28.6}
\expandafter\def\csname v@mycs/whisper-tiny/before-mixed\endcsname{54.1}
\expandafter\def\csname v@mycs/whisper-tiny/before-plain\endcsname{23.4}
\expandafter\def\csname v@mycs/whisper-tiny/strat-extra\endcsname{19.1}
\expandafter\def\csname v@mytry/my2_w2v-bert/bench\endcsname{99.1}
\expandafter\def\csname v@mytry/my2_w2v-bert/bench-wer\endcsname{100.0}
\expandafter\def\csname v@mytry/my2_w2v-bert/dev\endcsname{99.4}
\expandafter\def\csname v@mytry/my2_w2v-bert/epochs\endcsname{7}
\expandafter\def\csname v@mytry/my2_w2v-bert/out\endcsname{never}
\expandafter\def\csname v@mytry/my2_w2v-bert/stuck\endcsname{7}
\expandafter\def\csname v@mytry/my3_w2v-bert/bench\endcsname{14.4}
\expandafter\def\csname v@mytry/my3_w2v-bert/bench-wer\endcsname{36.7}
\expandafter\def\csname v@mytry/my3_w2v-bert/dev\endcsname{20.4}
\expandafter\def\csname v@mytry/my3_w2v-bert/epochs\endcsname{15}
\expandafter\def\csname v@mytry/my3_w2v-bert/out\endcsname{7}
\expandafter\def\csname v@mytry/my3_w2v-bert/stuck\endcsname{6}
\expandafter\def\csname v@mytry/my_w2v-bert/bench\endcsname{73.8}
\expandafter\def\csname v@mytry/my_w2v-bert/bench-wer\endcsname{99.8}
\expandafter\def\csname v@mytry/my_w2v-bert/dev\endcsname{69.6}
\expandafter\def\csname v@mytry/my_w2v-bert/epochs\endcsname{15}
\expandafter\def\csname v@mytry/my_w2v-bert/out\endcsname{8}
\expandafter\def\csname v@mytry/my_w2v-bert/stuck\endcsname{7}
\expandafter\def\csname v@mytry/mylow_w2v-bert/bench\endcsname{9.3}
\expandafter\def\csname v@mytry/mylow_w2v-bert/bench-wer\endcsname{27.9}
\expandafter\def\csname v@mytry/mylow_w2v-bert/dev\endcsname{18.4}
\expandafter\def\csname v@mytry/mylow_w2v-bert/epochs\endcsname{15}
\expandafter\def\csname v@mytry/mylow_w2v-bert/out\endcsname{3}
\expandafter\def\csname v@mytry/mylow_w2v-bert/stuck\endcsname{2}
\expandafter\def\csname v@n/parakeet-tdt-v3/100\endcsname{34.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/100/epoch\endcsname{24}
\expandafter\def\csname v@n/parakeet-tdt-v3/1000\endcsname{21.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/1000/epoch\endcsname{10}
\expandafter\def\csname v@n/parakeet-tdt-v3/200\endcsname{32.8}
\expandafter\def\csname v@n/parakeet-tdt-v3/200/epoch\endcsname{15}
\expandafter\def\csname v@n/parakeet-tdt-v3/2000\endcsname{21.4}
\expandafter\def\csname v@n/parakeet-tdt-v3/2000/epoch\endcsname{5}
\expandafter\def\csname v@n/parakeet-tdt-v3/25\endcsname{45.6}
\expandafter\def\csname v@n/parakeet-tdt-v3/25/epoch\endcsname{50}
\expandafter\def\csname v@n/parakeet-tdt-v3/4000\endcsname{20.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/4000/epoch\endcsname{3}
\expandafter\def\csname v@n/parakeet-tdt-v3/50\endcsname{43.2}
\expandafter\def\csname v@n/parakeet-tdt-v3/50/epoch\endcsname{40}
\expandafter\def\csname v@n/parakeet-tdt-v3/500\endcsname{27.3}
\expandafter\def\csname v@n/parakeet-tdt-v3/500/epoch\endcsname{10}
\expandafter\def\csname v@n/parakeet-tdt-v3/large-presented\endcsname{128,448}
\expandafter\def\csname v@n/parakeet-tdt-v3/large-same\endcsname{31.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/large-same-epoch\endcsname{3}
\expandafter\def\csname v@n/parakeet-tdt-v3/same-gain\endcsname{2.9}
\expandafter\def\csname v@n/parakeet-tdt-v3/small-best\endcsname{34.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/small-epochs\endcsname{24}
\expandafter\def\csname v@n/parakeet-tdt-v3/small-presented\endcsname{115,680}
\expandafter\def\csname v@n/parakeet-tdt-v3/top-gain\endcsname{1.0}
\expandafter\def\csname v@n/parakeet-tdt-v3/top-gain-ci\endcsname{0.4 to 1.7}
\expandafter\def\csname v@n/parakeet-tdt-v3/top-loss\endcsname{-1.0}
\expandafter\def\csname v@n/parakeet-tdt-v3/top-loss-ci\endcsname{-1.7 to -0.4}
\expandafter\def\csname v@n/presented/100\endcsname{115,680}
\expandafter\def\csname v@n/presented/1000\endcsname{428,160}
\expandafter\def\csname v@n/presented/200\endcsname{143,130}
\expandafter\def\csname v@n/presented/2000\endcsname{386,390}
\expandafter\def\csname v@n/presented/25\endcsname{72,540}
\expandafter\def\csname v@n/presented/4000\endcsname{387,708}
\expandafter\def\csname v@n/presented/50\endcsname{96,760}
\expandafter\def\csname v@n/presented/500\endcsname{228,960}
\expandafter\def\csname v@n/qwen3-asr-0.6b/100\endcsname{28.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/100/epoch\endcsname{8}
\expandafter\def\csname v@n/qwen3-asr-0.6b/1000\endcsname{18.2}
\expandafter\def\csname v@n/qwen3-asr-0.6b/1000/epoch\endcsname{4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/200\endcsname{24.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/200/epoch\endcsname{15}
\expandafter\def\csname v@n/qwen3-asr-0.6b/2000\endcsname{16.1}
\expandafter\def\csname v@n/qwen3-asr-0.6b/2000/epoch\endcsname{3}
\expandafter\def\csname v@n/qwen3-asr-0.6b/25\endcsname{39.3}
\expandafter\def\csname v@n/qwen3-asr-0.6b/25/epoch\endcsname{40}
\expandafter\def\csname v@n/qwen3-asr-0.6b/4000\endcsname{15.3}
\expandafter\def\csname v@n/qwen3-asr-0.6b/4000/epoch\endcsname{3}
\expandafter\def\csname v@n/qwen3-asr-0.6b/50\endcsname{33.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/50/epoch\endcsname{24}
\expandafter\def\csname v@n/qwen3-asr-0.6b/500\endcsname{20.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/500/epoch\endcsname{4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/large-presented\endcsname{128,448}
\expandafter\def\csname v@n/qwen3-asr-0.6b/large-same\endcsname{18.7}
\expandafter\def\csname v@n/qwen3-asr-0.6b/large-same-epoch\endcsname{3}
\expandafter\def\csname v@n/qwen3-asr-0.6b/same-gain\endcsname{9.7}
\expandafter\def\csname v@n/qwen3-asr-0.6b/small-best\endcsname{28.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/small-epochs\endcsname{24}
\expandafter\def\csname v@n/qwen3-asr-0.6b/small-presented\endcsname{115,680}
\expandafter\def\csname v@n/qwen3-asr-0.6b/top-gain\endcsname{2.9}
\expandafter\def\csname v@n/qwen3-asr-0.6b/top-gain-ci\endcsname{2.4 to 3.4}
\expandafter\def\csname v@n/qwen3-asr-0.6b/top-loss\endcsname{-2.9}
\expandafter\def\csname v@n/qwen3-asr-0.6b/top-loss-ci\endcsname{-3.4 to -2.4}
\expandafter\def\csname v@n/whisper-large-v3-turbo/100\endcsname{22.4}
\expandafter\def\csname v@n/whisper-large-v3-turbo/100/epoch\endcsname{24}
\expandafter\def\csname v@n/whisper-large-v3-turbo/1000\endcsname{14.3}
\expandafter\def\csname v@n/whisper-large-v3-turbo/1000/epoch\endcsname{9}
\expandafter\def\csname v@n/whisper-large-v3-turbo/200\endcsname{19.1}
\expandafter\def\csname v@n/whisper-large-v3-turbo/200/epoch\endcsname{12}
\expandafter\def\csname v@n/whisper-large-v3-turbo/2000\endcsname{12.7}
\expandafter\def\csname v@n/whisper-large-v3-turbo/2000/epoch\endcsname{5}
\expandafter\def\csname v@n/whisper-large-v3-turbo/25\endcsname{32.3}
\expandafter\def\csname v@n/whisper-large-v3-turbo/25/epoch\endcsname{50}
\expandafter\def\csname v@n/whisper-large-v3-turbo/4000\endcsname{12.8}
\expandafter\def\csname v@n/whisper-large-v3-turbo/4000/epoch\endcsname{3}
\expandafter\def\csname v@n/whisper-large-v3-turbo/50\endcsname{26.7}
\expandafter\def\csname v@n/whisper-large-v3-turbo/50/epoch\endcsname{16}
\expandafter\def\csname v@n/whisper-large-v3-turbo/500\endcsname{15.9}
\expandafter\def\csname v@n/whisper-large-v3-turbo/500/epoch\endcsname{8}
\expandafter\def\csname v@n/whisper-large-v3-turbo/large-presented\endcsname{128,448}
\expandafter\def\csname v@n/whisper-large-v3-turbo/large-same\endcsname{15.1}
\expandafter\def\csname v@n/whisper-large-v3-turbo/large-same-epoch\endcsname{3}
\expandafter\def\csname v@n/whisper-large-v3-turbo/same-gain\endcsname{7.3}
\expandafter\def\csname v@n/whisper-large-v3-turbo/small-best\endcsname{22.4}
\expandafter\def\csname v@n/whisper-large-v3-turbo/small-epochs\endcsname{24}
\expandafter\def\csname v@n/whisper-large-v3-turbo/small-presented\endcsname{115,680}
\expandafter\def\csname v@n/whisper-large-v3-turbo/top-gain\endcsname{1.5}
\expandafter\def\csname v@n/whisper-large-v3-turbo/top-gain-ci\endcsname{1.0 to 2.1}
\expandafter\def\csname v@n/whisper-large-v3-turbo/top-loss\endcsname{-1.5}
\expandafter\def\csname v@n/whisper-large-v3-turbo/top-loss-ci\endcsname{-2.1 to -1.0}
\expandafter\def\csname v@n/whisper-small/100\endcsname{26.7}
\expandafter\def\csname v@n/whisper-small/100/epoch\endcsname{24}
\expandafter\def\csname v@n/whisper-small/1000\endcsname{16.9}
\expandafter\def\csname v@n/whisper-small/1000/epoch\endcsname{9}
\expandafter\def\csname v@n/whisper-small/200\endcsname{22.5}
\expandafter\def\csname v@n/whisper-small/200/epoch\endcsname{15}
\expandafter\def\csname v@n/whisper-small/2000\endcsname{15.4}
\expandafter\def\csname v@n/whisper-small/2000/epoch\endcsname{3}
\expandafter\def\csname v@n/whisper-small/25\endcsname{38.4}
\expandafter\def\csname v@n/whisper-small/25/epoch\endcsname{40}
\expandafter\def\csname v@n/whisper-small/4000\endcsname{14.4}
\expandafter\def\csname v@n/whisper-small/4000/epoch\endcsname{3}
\expandafter\def\csname v@n/whisper-small/50\endcsname{31.7}
\expandafter\def\csname v@n/whisper-small/50/epoch\endcsname{16}
\expandafter\def\csname v@n/whisper-small/500\endcsname{18.7}
\expandafter\def\csname v@n/whisper-small/500/epoch\endcsname{10}
\expandafter\def\csname v@n/whisper-small/large-presented\endcsname{128,448}
\expandafter\def\csname v@n/whisper-small/large-same\endcsname{17.6}
\expandafter\def\csname v@n/whisper-small/large-same-epoch\endcsname{3}
\expandafter\def\csname v@n/whisper-small/same-gain\endcsname{9.1}
\expandafter\def\csname v@n/whisper-small/small-best\endcsname{26.7}
\expandafter\def\csname v@n/whisper-small/small-epochs\endcsname{24}
\expandafter\def\csname v@n/whisper-small/small-presented\endcsname{115,680}
\expandafter\def\csname v@n/whisper-small/top-gain\endcsname{2.5}
\expandafter\def\csname v@n/whisper-small/top-gain-ci\endcsname{2.2 to 2.9}
\expandafter\def\csname v@n/whisper-small/top-loss\endcsname{-2.5}
\expandafter\def\csname v@n/whisper-small/top-loss-ci\endcsname{-2.9 to -2.2}
\expandafter\def\csname v@nabl/best-key\endcsname{full-linear}
\expandafter\def\csname v@nabl/best-label\endcsname{everything, rate falling to zero}
\expandafter\def\csname v@nabl/best-test\endcsname{14.0}
\expandafter\def\csname v@nabl/const-best-test\endcsname{15.5}
\expandafter\def\csname v@nabl/cost/enc\endcsname{0.8}
\expandafter\def\csname v@nabl/cost/enc-ci\endcsname{0.3 to 1.2}
\expandafter\def\csname v@nabl/cost/enc-frz\endcsname{1.8}
\expandafter\def\csname v@nabl/cost/enc-frz-ci\endcsname{1.3 to 2.2}
\expandafter\def\csname v@nabl/cost/enc-proj\endcsname{0.9}
\expandafter\def\csname v@nabl/cost/enc-proj-ci\endcsname{0.5 to 1.3}
\expandafter\def\csname v@nabl/cost/experts\endcsname{0.1}
\expandafter\def\csname v@nabl/cost/experts-ci\endcsname{-0.3 to 0.5}
\expandafter\def\csname v@nabl/cost/experts-linear\endcsname{0.8}
\expandafter\def\csname v@nabl/cost/experts-linear-ci\endcsname{0.5 to 1.1}
\expandafter\def\csname v@nabl/cost/first\endcsname{0.4}
\expandafter\def\csname v@nabl/cost/first-ci\endcsname{0.0 to 0.8}
\expandafter\def\csname v@nabl/cost/lm\endcsname{3.1}
\expandafter\def\csname v@nabl/cost/lm-ci\endcsname{2.6 to 3.5}
\expandafter\def\csname v@nabl/cost/proj\endcsname{-0.2}
\expandafter\def\csname v@nabl/cost/proj-ci\endcsname{-0.6 to 0.2}
\expandafter\def\csname v@nabl/cost/proj-frz\endcsname{0.2}
\expandafter\def\csname v@nabl/cost/proj-frz-ci\endcsname{-0.1 to 0.5}
\expandafter\def\csname v@nabl/cost/shared\endcsname{0.4}
\expandafter\def\csname v@nabl/cost/shared-ci\endcsname{0.0 to 0.8}
\expandafter\def\csname v@nabl/e4/behind-two\endcsname{0.4}
\expandafter\def\csname v@nabl/e4/behind-two-ci\endcsname{0.2 to 0.8}
\expandafter\def\csname v@nabl/e4/dev\endcsname{21.2}
\expandafter\def\csname v@nabl/e4/e1\endcsname{14.9}
\expandafter\def\csname v@nabl/e4/e2\endcsname{14.5}
\expandafter\def\csname v@nabl/e4/e3\endcsname{14.6}
\expandafter\def\csname v@nabl/e4/e4\endcsname{14.5}
\expandafter\def\csname v@nabl/e4/epoch\endcsname{4}
\expandafter\def\csname v@nabl/e4/test\endcsname{14.5}
\expandafter\def\csname v@nabl/e4/two-dev\endcsname{20.9}
\expandafter\def\csname v@nabl/e4/vs-main\endcsname{1.3}
\expandafter\def\csname v@nabl/e4/vs-main-ci\endcsname{0.9 to 1.6}
\expandafter\def\csname v@nabl/e4/vs-two\endcsname{-0.4}
\expandafter\def\csname v@nabl/experts-extra\endcsname{29.4}
\expandafter\def\csname v@nabl/first/e1\endcsname{17.5}
\expandafter\def\csname v@nabl/first/e2\endcsname{16.2}
\expandafter\def\csname v@nabl/first/epoch\endcsname{2}
\expandafter\def\csname v@nabl/first/share\endcsname{6.3}
\expandafter\def\csname v@nabl/first/test\endcsname{16.2}
\expandafter\def\csname v@nabl/first/trained\endcsname{2.02}
\expandafter\def\csname v@nabl/first/vs-full\endcsname{0.5}
\expandafter\def\csname v@nabl/first/vs-full-ci\endcsname{0.1 to 0.9}
\expandafter\def\csname v@nabl/frozen-best\endcsname{15.7}
\expandafter\def\csname v@nabl/frozen-worst\endcsname{18.9}
\expandafter\def\csname v@nabl/frz-encoder-projector/e1\endcsname{16.4}
\expandafter\def\csname v@nabl/frz-encoder-projector/e2\endcsname{16.4}
\expandafter\def\csname v@nabl/frz-encoder-projector/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-encoder-projector/share\endcsname{97.6}
\expandafter\def\csname v@nabl/frz-encoder-projector/test\endcsname{16.4}
\expandafter\def\csname v@nabl/frz-encoder-projector/trained\endcsname{31.58}
\expandafter\def\csname v@nabl/frz-encoder-projector/vs-first\endcsname{-0.2}
\expandafter\def\csname v@nabl/frz-encoder-projector/vs-first-ci\endcsname{-0.7 to 0.3}
\expandafter\def\csname v@nabl/frz-encoder-projector/vs-full\endcsname{0.7}
\expandafter\def\csname v@nabl/frz-encoder-projector/vs-full-ci\endcsname{0.2 to 1.1}
\expandafter\def\csname v@nabl/frz-encoder/e1\endcsname{16.5}
\expandafter\def\csname v@nabl/frz-encoder/e2\endcsname{16.7}
\expandafter\def\csname v@nabl/frz-encoder/epoch\endcsname{1}
\expandafter\def\csname v@nabl/frz-encoder/share\endcsname{97.6}
\expandafter\def\csname v@nabl/frz-encoder/test\endcsname{16.5}
\expandafter\def\csname v@nabl/frz-encoder/trained\endcsname{31.58}
\expandafter\def\csname v@nabl/frz-encoder/vs-first\endcsname{-0.3}
\expandafter\def\csname v@nabl/frz-encoder/vs-first-ci\endcsname{-0.7 to 0.1}
\expandafter\def\csname v@nabl/frz-encoder/vs-full\endcsname{0.8}
\expandafter\def\csname v@nabl/frz-encoder/vs-full-ci\endcsname{0.3 to 1.2}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/e1\endcsname{23.6}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/e2\endcsname{23.5}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/test\endcsname{23.5}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-first\endcsname{-7.2}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-first-ci\endcsname{-7.8 to -6.8}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-full\endcsname{7.7}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-full-ci\endcsname{7.2 to 8.2}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-rate\endcsname{7.6}
\expandafter\def\csname v@nabl/frz-experts-enc1e-4/vs-rate-ci\endcsname{7.1 to 8.1}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/e1\endcsname{18.1}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/e2\endcsname{17.1}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/test\endcsname{17.1}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-first\endcsname{-0.8}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-first-ci\endcsname{-1.2 to -0.4}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-full\endcsname{1.3}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-full-ci\endcsname{0.9 to 1.7}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-rate\endcsname{1.2}
\expandafter\def\csname v@nabl/frz-experts-enc3e-5/vs-rate-ci\endcsname{0.9 to 1.5}
\expandafter\def\csname v@nabl/frz-experts-encoder/e1\endcsname{18.5}
\expandafter\def\csname v@nabl/frz-experts-encoder/e2\endcsname{17.6}
\expandafter\def\csname v@nabl/frz-experts-encoder/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-encoder/share\endcsname{6.8}
\expandafter\def\csname v@nabl/frz-experts-encoder/test\endcsname{17.6}
\expandafter\def\csname v@nabl/frz-experts-encoder/trained\endcsname{2.21}
\expandafter\def\csname v@nabl/frz-experts-encoder/vs-first\endcsname{-1.4}
\expandafter\def\csname v@nabl/frz-experts-encoder/vs-first-ci\endcsname{-1.8 to -0.9}
\expandafter\def\csname v@nabl/frz-experts-encoder/vs-full\endcsname{1.8}
\expandafter\def\csname v@nabl/frz-experts-encoder/vs-full-ci\endcsname{1.4 to 2.3}
\expandafter\def\csname v@nabl/frz-experts-linear/ahead\endcsname{1.0}
\expandafter\def\csname v@nabl/frz-experts-linear/ahead-ci\endcsname{0.7 to 1.3}
\expandafter\def\csname v@nabl/frz-experts-linear/e1\endcsname{16.2}
\expandafter\def\csname v@nabl/frz-experts-linear/e2\endcsname{14.9}
\expandafter\def\csname v@nabl/frz-experts-linear/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-linear/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-linear/test\endcsname{14.9}
\expandafter\def\csname v@nabl/frz-experts-linear/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-first\endcsname{1.4}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-first-ci\endcsname{1.1 to 1.7}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-full\endcsname{-0.9}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-full-ci\endcsname{-1.3 to -0.6}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-rate\endcsname{-1.0}
\expandafter\def\csname v@nabl/frz-experts-linear/vs-rate-ci\endcsname{-1.3 to -0.7}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/e1\endcsname{19.6}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/e2\endcsname{19.1}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/test\endcsname{19.1}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-first\endcsname{-2.9}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-first-ci\endcsname{-3.4 to -2.4}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-full\endcsname{3.3}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-full-ci\endcsname{2.9 to 3.8}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-rate\endcsname{3.3}
\expandafter\def\csname v@nabl/frz-experts-lr3e-5/vs-rate-ci\endcsname{2.8 to 3.7}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/e1\endcsname{18.4}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/e2\endcsname{16.2}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/test\endcsname{16.2}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-first\endcsname{0.0}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-first-ci\endcsname{-0.3 to 0.4}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-full\endcsname{0.5}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-full-ci\endcsname{0.1 to 0.8}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-rate\endcsname{0.4}
\expandafter\def\csname v@nabl/frz-experts-lr3e-6/vs-rate-ci\endcsname{0.0 to 0.7}
\expandafter\def\csname v@nabl/frz-experts-projector/e1\endcsname{16.8}
\expandafter\def\csname v@nabl/frz-experts-projector/e2\endcsname{16.1}
\expandafter\def\csname v@nabl/frz-experts-projector/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-projector/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-projector/test\endcsname{16.1}
\expandafter\def\csname v@nabl/frz-experts-projector/trained\endcsname{2.83}
\expandafter\def\csname v@nabl/frz-experts-projector/vs-first\endcsname{0.2}
\expandafter\def\csname v@nabl/frz-experts-projector/vs-first-ci\endcsname{-0.2 to 0.6}
\expandafter\def\csname v@nabl/frz-experts-projector/vs-full\endcsname{0.3}
\expandafter\def\csname v@nabl/frz-experts-projector/vs-full-ci\endcsname{-0.1 to 0.7}
\expandafter\def\csname v@nabl/frz-experts-seed1/e1\endcsname{17.1}
\expandafter\def\csname v@nabl/frz-experts-seed1/e2\endcsname{15.7}
\expandafter\def\csname v@nabl/frz-experts-seed1/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-seed1/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts-seed1/test\endcsname{15.7}
\expandafter\def\csname v@nabl/frz-experts-seed1/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts-seed1/vs-first\endcsname{0.6}
\expandafter\def\csname v@nabl/frz-experts-seed1/vs-first-ci\endcsname{0.2 to 1.0}
\expandafter\def\csname v@nabl/frz-experts-seed1/vs-full\endcsname{-0.1}
\expandafter\def\csname v@nabl/frz-experts-seed1/vs-full-ci\endcsname{-0.6 to 0.3}
\expandafter\def\csname v@nabl/frz-experts-shared/e1\endcsname{17.0}
\expandafter\def\csname v@nabl/frz-experts-shared/e2\endcsname{16.2}
\expandafter\def\csname v@nabl/frz-experts-shared/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts-shared/share\endcsname{7.3}
\expandafter\def\csname v@nabl/frz-experts-shared/test\endcsname{16.2}
\expandafter\def\csname v@nabl/frz-experts-shared/trained\endcsname{2.38}
\expandafter\def\csname v@nabl/frz-experts-shared/vs-first\endcsname{0.0}
\expandafter\def\csname v@nabl/frz-experts-shared/vs-first-ci\endcsname{-0.4 to 0.4}
\expandafter\def\csname v@nabl/frz-experts-shared/vs-full\endcsname{0.5}
\expandafter\def\csname v@nabl/frz-experts-shared/vs-full-ci\endcsname{0.0 to 0.9}
\expandafter\def\csname v@nabl/frz-experts/e1\endcsname{17.0}
\expandafter\def\csname v@nabl/frz-experts/e2\endcsname{15.9}
\expandafter\def\csname v@nabl/frz-experts/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-experts/share\endcsname{8.8}
\expandafter\def\csname v@nabl/frz-experts/test\endcsname{15.9}
\expandafter\def\csname v@nabl/frz-experts/trained\endcsname{2.84}
\expandafter\def\csname v@nabl/frz-experts/vs-first\endcsname{0.4}
\expandafter\def\csname v@nabl/frz-experts/vs-first-ci\endcsname{0.0 to 0.8}
\expandafter\def\csname v@nabl/frz-experts/vs-full\endcsname{0.1}
\expandafter\def\csname v@nabl/frz-experts/vs-full-ci\endcsname{-0.3 to 0.5}
\expandafter\def\csname v@nabl/frz-lm/e1\endcsname{23.2}
\expandafter\def\csname v@nabl/frz-lm/e2\endcsname{18.9}
\expandafter\def\csname v@nabl/frz-lm/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-lm/share\endcsname{2.0}
\expandafter\def\csname v@nabl/frz-lm/test\endcsname{18.9}
\expandafter\def\csname v@nabl/frz-lm/trained\endcsname{0.63}
\expandafter\def\csname v@nabl/frz-lm/vs-first\endcsname{-2.7}
\expandafter\def\csname v@nabl/frz-lm/vs-first-ci\endcsname{-3.1 to -2.2}
\expandafter\def\csname v@nabl/frz-lm/vs-full\endcsname{3.1}
\expandafter\def\csname v@nabl/frz-lm/vs-full-ci\endcsname{2.7 to 3.6}
\expandafter\def\csname v@nabl/frz-projector/e1\endcsname{15.6}
\expandafter\def\csname v@nabl/frz-projector/e2\endcsname{15.6}
\expandafter\def\csname v@nabl/frz-projector/epoch\endcsname{2}
\expandafter\def\csname v@nabl/frz-projector/share\endcsname{99.5}
\expandafter\def\csname v@nabl/frz-projector/test\endcsname{15.6}
\expandafter\def\csname v@nabl/frz-projector/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/frz-projector/vs-first\endcsname{0.7}
\expandafter\def\csname v@nabl/frz-projector/vs-first-ci\endcsname{0.3 to 1.1}
\expandafter\def\csname v@nabl/frz-projector/vs-full\endcsname{-0.2}
\expandafter\def\csname v@nabl/frz-projector/vs-full-ci\endcsname{-0.6 to 0.2}
\expandafter\def\csname v@nabl/full-linear/ahead\endcsname{1.8}
\expandafter\def\csname v@nabl/full-linear/ahead-ci\endcsname{1.4 to 2.1}
\expandafter\def\csname v@nabl/full-linear/e1\endcsname{14.6}
\expandafter\def\csname v@nabl/full-linear/e2\endcsname{14.0}
\expandafter\def\csname v@nabl/full-linear/epoch\endcsname{2}
\expandafter\def\csname v@nabl/full-linear/share\endcsname{99.5}
\expandafter\def\csname v@nabl/full-linear/test\endcsname{14.0}
\expandafter\def\csname v@nabl/full-linear/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/full-linear/vs-first\endcsname{2.2}
\expandafter\def\csname v@nabl/full-linear/vs-first-ci\endcsname{1.8 to 2.6}
\expandafter\def\csname v@nabl/full-linear/vs-full\endcsname{-1.8}
\expandafter\def\csname v@nabl/full-linear/vs-full-ci\endcsname{-2.1 to -1.4}
\expandafter\def\csname v@nabl/full-linear/vs-rate\endcsname{-1.8}
\expandafter\def\csname v@nabl/full-linear/vs-rate-ci\endcsname{-2.1 to -1.4}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/e1\endcsname{16.3}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/e2\endcsname{16.2}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/epoch\endcsname{2}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/share\endcsname{99.5}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/test\endcsname{16.2}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-first\endcsname{0.1}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-first-ci\endcsname{-0.3 to 0.5}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-full\endcsname{0.4}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-full-ci\endcsname{-0.1 to 0.8}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-linear\endcsname{2.1}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-linear-ci\endcsname{1.8 to 2.5}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-rate\endcsname{0.7}
\expandafter\def\csname v@nabl/full-lr3e-6-linear/vs-rate-ci\endcsname{0.3 to 1.0}
\expandafter\def\csname v@nabl/full-lr3e-6/ahead\endcsname{0.3}
\expandafter\def\csname v@nabl/full-lr3e-6/ahead-ci\endcsname{-0.1 to 0.7}
\expandafter\def\csname v@nabl/full-lr3e-6/e1\endcsname{16.2}
\expandafter\def\csname v@nabl/full-lr3e-6/e2\endcsname{15.5}
\expandafter\def\csname v@nabl/full-lr3e-6/epoch\endcsname{2}
\expandafter\def\csname v@nabl/full-lr3e-6/share\endcsname{99.5}
\expandafter\def\csname v@nabl/full-lr3e-6/test\endcsname{15.5}
\expandafter\def\csname v@nabl/full-lr3e-6/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-first\endcsname{0.7}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-first-ci\endcsname{0.4 to 1.1}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-full\endcsname{-0.3}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-full-ci\endcsname{-0.7 to 0.1}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-rate\endcsname{-0.3}
\expandafter\def\csname v@nabl/full-lr3e-6/vs-rate-ci\endcsname{-0.7 to 0.1}
\expandafter\def\csname v@nabl/full-seed1/e1\endcsname{16.9}
\expandafter\def\csname v@nabl/full-seed1/e2\endcsname{15.5}
\expandafter\def\csname v@nabl/full-seed1/epoch\endcsname{2}
\expandafter\def\csname v@nabl/full-seed1/share\endcsname{99.5}
\expandafter\def\csname v@nabl/full-seed1/test\endcsname{15.5}
\expandafter\def\csname v@nabl/full-seed1/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/full-seed1/vs-first\endcsname{0.8}
\expandafter\def\csname v@nabl/full-seed1/vs-first-ci\endcsname{0.3 to 1.2}
\expandafter\def\csname v@nabl/full-seed1/vs-full\endcsname{-0.3}
\expandafter\def\csname v@nabl/full-seed1/vs-full-ci\endcsname{-0.7 to 0.2}
\expandafter\def\csname v@nabl/full/e1\endcsname{16.7}
\expandafter\def\csname v@nabl/full/e2\endcsname{15.8}
\expandafter\def\csname v@nabl/full/epoch\endcsname{2}
\expandafter\def\csname v@nabl/full/share\endcsname{99.5}
\expandafter\def\csname v@nabl/full/test\endcsname{15.8}
\expandafter\def\csname v@nabl/full/trained\endcsname{32.21}
\expandafter\def\csname v@nabl/full/vs-first\endcsname{0.5}
\expandafter\def\csname v@nabl/full/vs-first-ci\endcsname{0.1 to 0.9}
\expandafter\def\csname v@nabl/lowest-key\endcsname{full-linear}
\expandafter\def\csname v@nabl/lowest-label\endcsname{everything, rate falling to zero}
\expandafter\def\csname v@nabl/lowest-test\endcsname{14.0}
\expandafter\def\csname v@nabl/n\endcsname{20}
\expandafter\def\csname v@nabl/n-more\endcsname{18}
\expandafter\def\csname v@nabl/projector-max\endcsname{0.2}
\expandafter\def\csname v@nabl/sched/frz-gain\endcsname{1.0}
\expandafter\def\csname v@nabl/sched/frz-gain-ci\endcsname{0.7 to 1.3}
\expandafter\def\csname v@nabl/sched/full-gain\endcsname{1.8}
\expandafter\def\csname v@nabl/sched/full-gain-ci\endcsname{1.4 to 2.1}
\expandafter\def\csname v@nabl/seed-diff\endcsname{0.3}
\expandafter\def\csname v@nabl/seed-diff-ci\endcsname{-0.2 to 0.7}
\expandafter\def\csname v@nabl/seed-diff-frz\endcsname{0.2}
\expandafter\def\csname v@nabl/seed-diff-frz-ci\endcsname{-0.2 to 0.6}
\expandafter\def\csname v@nabl/trains-best\endcsname{15.5}
\expandafter\def\csname v@nabl/trains-worst\endcsname{16.5}
\expandafter\def\csname v@nabl/upto\endcsname{2}
\expandafter\def\csname v@nl/before-max\endcsname{71}
\expandafter\def\csname v@nl/before-min\endcsname{46}
\expandafter\def\csname v@nl/best/before\endcsname{54.8}
\expandafter\def\csname v@nl/best/cer\endcsname{11.7}
\expandafter\def\csname v@nl/best/ci\endcsname{10.8 to 12.8}
\expandafter\def\csname v@nl/best/name\endcsname{omniASR CTC 7B}
\expandafter\def\csname v@nl/cohere-transcribe/after\endcsname{16.7}
\expandafter\def\csname v@nl/cohere-transcribe/before\endcsname{65.5}
\expandafter\def\csname v@nl/cohere-transcribe/ci\endcsname{15.7 to 17.9}
\expandafter\def\csname v@nl/cohere-transcribe/gain\endcsname{48.7}
\expandafter\def\csname v@nl/cohere-transcribe/rest\endcsname{15.2}
\expandafter\def\csname v@nl/cohere-transcribe/rest-before\endcsname{68.9}
\expandafter\def\csname v@nl/ctc-ahead-n\endcsname{5}
\expandafter\def\csname v@nl/dec-gap\endcsname{0.4}
\expandafter\def\csname v@nl/dec-gap-ci\endcsname{-0.3 to 1.3}
\expandafter\def\csname v@nl/gain-max\endcsname{51.0}
\expandafter\def\csname v@nl/gain-median\endcsname{42.1}
\expandafter\def\csname v@nl/gain-min\endcsname{27.9}
\expandafter\def\csname v@nl/gemma4-12b/after\endcsname{20.2}
\expandafter\def\csname v@nl/gemma4-12b/before\endcsname{71.2}
\expandafter\def\csname v@nl/gemma4-12b/ci\endcsname{18.9 to 21.6}
\expandafter\def\csname v@nl/gemma4-12b/gain\endcsname{51.0}
\expandafter\def\csname v@nl/gemma4-12b/rest\endcsname{19.7}
\expandafter\def\csname v@nl/gemma4-12b/rest-before\endcsname{73.4}
\expandafter\def\csname v@nl/gemma4-e2b/after\endcsname{21.4}
\expandafter\def\csname v@nl/gemma4-e2b/before\endcsname{59.5}
\expandafter\def\csname v@nl/gemma4-e2b/ci\endcsname{20.2 to 22.9}
\expandafter\def\csname v@nl/gemma4-e2b/gain\endcsname{38.0}
\expandafter\def\csname v@nl/gemma4-e2b/rest\endcsname{17.6}
\expandafter\def\csname v@nl/gemma4-e2b/rest-before\endcsname{38.4}
\expandafter\def\csname v@nl/gemma4-e4b/after\endcsname{19.4}
\expandafter\def\csname v@nl/gemma4-e4b/before\endcsname{47.3}
\expandafter\def\csname v@nl/gemma4-e4b/ci\endcsname{18.2 to 20.6}
\expandafter\def\csname v@nl/gemma4-e4b/gain\endcsname{27.9}
\expandafter\def\csname v@nl/gemma4-e4b/rest\endcsname{15.7}
\expandafter\def\csname v@nl/gemma4-e4b/rest-before\endcsname{37.4}
\expandafter\def\csname v@nl/granite-2b/after\endcsname{22.4}
\expandafter\def\csname v@nl/granite-2b/before\endcsname{61.4}
\expandafter\def\csname v@nl/granite-2b/ci\endcsname{21.2 to 23.7}
\expandafter\def\csname v@nl/granite-2b/gain\endcsname{39.0}
\expandafter\def\csname v@nl/granite-2b/rest\endcsname{22.5}
\expandafter\def\csname v@nl/granite-2b/rest-before\endcsname{62.3}
\expandafter\def\csname v@nl/harder-median\endcsname{2.2}
\expandafter\def\csname v@nl/harder-n\endcsname{23}
\expandafter\def\csname v@nl/lfm3-audio/after\endcsname{18.8}
\expandafter\def\csname v@nl/lfm3-audio/before\endcsname{62.6}
\expandafter\def\csname v@nl/lfm3-audio/ci\endcsname{17.7 to 20.0}
\expandafter\def\csname v@nl/lfm3-audio/gain\endcsname{43.8}
\expandafter\def\csname v@nl/lfm3-audio/rest\endcsname{17.5}
\expandafter\def\csname v@nl/lfm3-audio/rest-before\endcsname{64.8}
\expandafter\def\csname v@nl/mms-1b/after\endcsname{14.4}
\expandafter\def\csname v@nl/mms-1b/before\endcsname{53.5}
\expandafter\def\csname v@nl/mms-1b/before-gap\endcsname{30.1}
\expandafter\def\csname v@nl/mms-1b/ci\endcsname{13.5 to 15.3}
\expandafter\def\csname v@nl/mms-1b/gain\endcsname{39.1}
\expandafter\def\csname v@nl/mms-1b/rest\endcsname{10.0}
\expandafter\def\csname v@nl/mms-1b/rest-before\endcsname{23.4}
\expandafter\def\csname v@nl/n\endcsname{12}
\expandafter\def\csname v@nl/n-models\endcsname{24}
\expandafter\def\csname v@nl/names\endcsname{Angami Naga, Ao Naga, Chokri Naga, Gronings, Gurani, Karbi, Ladino, Lule Sami, Moroccan Tamazight, Southern Kurdish, Southern Rengma Naga and Swiss German}
\expandafter\def\csname v@nl/nemotron-30b/after\endcsname{18.3}
\expandafter\def\csname v@nl/nemotron-30b/before\endcsname{60.9}
\expandafter\def\csname v@nl/nemotron-30b/ci\endcsname{16.9 to 19.6}
\expandafter\def\csname v@nl/nemotron-30b/gain\endcsname{42.7}
\expandafter\def\csname v@nl/nemotron-30b/rest\endcsname{15.0}
\expandafter\def\csname v@nl/nemotron-30b/rest-before\endcsname{57.2}
\expandafter\def\csname v@nl/nemotron-stream/after\endcsname{36.6}
\expandafter\def\csname v@nl/nemotron-stream/before\endcsname{70.1}
\expandafter\def\csname v@nl/nemotron-stream/ci\endcsname{35.1 to 37.9}
\expandafter\def\csname v@nl/nemotron-stream/gain\endcsname{33.5}
\expandafter\def\csname v@nl/nemotron-stream/rest\endcsname{35.6}
\expandafter\def\csname v@nl/nemotron-stream/rest-before\endcsname{68.3}
\expandafter\def\csname v@nl/omni-ctc-1b/after\endcsname{14.4}
\expandafter\def\csname v@nl/omni-ctc-1b/before\endcsname{46.5}
\expandafter\def\csname v@nl/omni-ctc-1b/before-gap\endcsname{23.6}
\expandafter\def\csname v@nl/omni-ctc-1b/ci\endcsname{13.5 to 15.5}
\expandafter\def\csname v@nl/omni-ctc-1b/gain\endcsname{32.0}
\expandafter\def\csname v@nl/omni-ctc-1b/rest\endcsname{11.2}
\expandafter\def\csname v@nl/omni-ctc-1b/rest-before\endcsname{22.9}
\expandafter\def\csname v@nl/omni-ctc-300m/after\endcsname{14.8}
\expandafter\def\csname v@nl/omni-ctc-300m/before\endcsname{49.9}
\expandafter\def\csname v@nl/omni-ctc-300m/ci\endcsname{13.9 to 15.8}
\expandafter\def\csname v@nl/omni-ctc-300m/gain\endcsname{35.1}
\expandafter\def\csname v@nl/omni-ctc-300m/rest\endcsname{12.8}
\expandafter\def\csname v@nl/omni-ctc-300m/rest-before\endcsname{25.7}
\expandafter\def\csname v@nl/omni-ctc-7b/after\endcsname{11.7}
\expandafter\def\csname v@nl/omni-ctc-7b/before\endcsname{54.8}
\expandafter\def\csname v@nl/omni-ctc-7b/ci\endcsname{10.8 to 12.8}
\expandafter\def\csname v@nl/omni-ctc-7b/gain\endcsname{43.0}
\expandafter\def\csname v@nl/omni-ctc-7b/rest\endcsname{8.9}
\expandafter\def\csname v@nl/omni-ctc-7b/rest-before\endcsname{21.8}
\expandafter\def\csname v@nl/pair/omni-ctc-1b/mms-1b\endcsname{0.1}
\expandafter\def\csname v@nl/pair/omni-ctc-1b/mms-1b-all\endcsname{1.0}
\expandafter\def\csname v@nl/pair/omni-ctc-1b/mms-1b-ci\endcsname{-0.3 to 0.6}
\expandafter\def\csname v@nl/pair/w2v-bert/omni-ctc-1b\endcsname{0.5}
\expandafter\def\csname v@nl/pair/w2v-bert/omni-ctc-1b-all\endcsname{0.7}
\expandafter\def\csname v@nl/pair/w2v-bert/omni-ctc-1b-ci\endcsname{-0.1 to 0.9}
\expandafter\def\csname v@nl/pair/whisper-large-v3/mms-1b\endcsname{1.0}
\expandafter\def\csname v@nl/pair/whisper-large-v3/mms-1b-all\endcsname{2.5}
\expandafter\def\csname v@nl/pair/whisper-large-v3/mms-1b-ci\endcsname{0.3 to 1.7}
\expandafter\def\csname v@nl/pair/whisper-large-v3/omni-ctc-1b\endcsname{0.9}
\expandafter\def\csname v@nl/pair/whisper-large-v3/omni-ctc-1b-all\endcsname{1.5}
\expandafter\def\csname v@nl/pair/whisper-large-v3/omni-ctc-1b-ci\endcsname{0.3 to 1.6}
\expandafter\def\csname v@nl/pair/whisper-large-v3/w2v-bert\endcsname{0.4}
\expandafter\def\csname v@nl/pair/whisper-large-v3/w2v-bert-all\endcsname{0.8}
\expandafter\def\csname v@nl/pair/whisper-large-v3/w2v-bert-ci\endcsname{-0.3 to 1.3}
\expandafter\def\csname v@nl/parakeet-tdt-v3/after\endcsname{21.8}
\expandafter\def\csname v@nl/parakeet-tdt-v3/before\endcsname{56.4}
\expandafter\def\csname v@nl/parakeet-tdt-v3/ci\endcsname{20.3 to 23.1}
\expandafter\def\csname v@nl/parakeet-tdt-v3/gain\endcsname{34.6}
\expandafter\def\csname v@nl/parakeet-tdt-v3/rest\endcsname{20.8}
\expandafter\def\csname v@nl/parakeet-tdt-v3/rest-before\endcsname{55.5}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/after\endcsname{19.2}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/before\endcsname{58.0}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/ci\endcsname{17.9 to 20.5}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/gain\endcsname{38.9}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/rest\endcsname{17.8}
\expandafter\def\csname v@nl/qwen3-asr-0.6b/rest-before\endcsname{61.8}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/after\endcsname{17.2}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/before\endcsname{54.1}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/ci\endcsname{16.0 to 18.4}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/gain\endcsname{36.9}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/rest\endcsname{16.4}
\expandafter\def\csname v@nl/qwen3-asr-1.7b/rest-before\endcsname{61.0}
\expandafter\def\csname v@nl/rest-n\endcsname{38}
\expandafter\def\csname v@nl/rho\endcsname{0.97}
\expandafter\def\csname v@nl/voxtral-mini/after\endcsname{17.5}
\expandafter\def\csname v@nl/voxtral-mini/before\endcsname{62.8}
\expandafter\def\csname v@nl/voxtral-mini/ci\endcsname{16.5 to 18.8}
\expandafter\def\csname v@nl/voxtral-mini/gain\endcsname{45.3}
\expandafter\def\csname v@nl/voxtral-mini/rest\endcsname{15.9}
\expandafter\def\csname v@nl/voxtral-mini/rest-before\endcsname{61.5}
\expandafter\def\csname v@nl/w2v-bert/after\endcsname{14.9}
\expandafter\def\csname v@nl/w2v-bert/ci\endcsname{14.0 to 15.8}
\expandafter\def\csname v@nl/w2v-bert/rest\endcsname{12.0}
\expandafter\def\csname v@nl/whisper-base/after\endcsname{24.5}
\expandafter\def\csname v@nl/whisper-base/before\endcsname{64.6}
\expandafter\def\csname v@nl/whisper-base/ci\endcsname{23.0 to 26.2}
\expandafter\def\csname v@nl/whisper-base/gain\endcsname{40.1}
\expandafter\def\csname v@nl/whisper-base/rest\endcsname{21.9}
\expandafter\def\csname v@nl/whisper-base/rest-before\endcsname{62.1}
\expandafter\def\csname v@nl/whisper-large-v2/after\endcsname{16.1}
\expandafter\def\csname v@nl/whisper-large-v2/before\endcsname{60.5}
\expandafter\def\csname v@nl/whisper-large-v2/ci\endcsname{15.0 to 17.4}
\expandafter\def\csname v@nl/whisper-large-v2/gain\endcsname{44.4}
\expandafter\def\csname v@nl/whisper-large-v2/rest\endcsname{13.6}
\expandafter\def\csname v@nl/whisper-large-v2/rest-before\endcsname{56.9}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/after\endcsname{15.6}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/before\endcsname{62.5}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/ci\endcsname{14.4 to 16.9}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/gain\endcsname{46.8}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/rest\endcsname{13.9}
\expandafter\def\csname v@nl/whisper-large-v3-turbo/rest-before\endcsname{52.1}
\expandafter\def\csname v@nl/whisper-large-v3/after\endcsname{15.3}
\expandafter\def\csname v@nl/whisper-large-v3/before\endcsname{57.4}
\expandafter\def\csname v@nl/whisper-large-v3/ci\endcsname{14.4 to 16.6}
\expandafter\def\csname v@nl/whisper-large-v3/gain\endcsname{42.1}
\expandafter\def\csname v@nl/whisper-large-v3/rest\endcsname{12.9}
\expandafter\def\csname v@nl/whisper-large-v3/rest-before\endcsname{48.1}
\expandafter\def\csname v@nl/whisper-medium/after\endcsname{16.9}
\expandafter\def\csname v@nl/whisper-medium/before\endcsname{66.0}
\expandafter\def\csname v@nl/whisper-medium/ci\endcsname{15.9 to 18.1}
\expandafter\def\csname v@nl/whisper-medium/gain\endcsname{49.1}
\expandafter\def\csname v@nl/whisper-medium/rest\endcsname{14.1}
\expandafter\def\csname v@nl/whisper-medium/rest-before\endcsname{63.0}
\expandafter\def\csname v@nl/whisper-small/after\endcsname{18.3}
\expandafter\def\csname v@nl/whisper-small/before\endcsname{67.9}
\expandafter\def\csname v@nl/whisper-small/ci\endcsname{17.2 to 19.5}
\expandafter\def\csname v@nl/whisper-small/gain\endcsname{49.6}
\expandafter\def\csname v@nl/whisper-small/rest\endcsname{16.4}
\expandafter\def\csname v@nl/whisper-small/rest-before\endcsname{65.0}
\expandafter\def\csname v@nl/whisper-tiny/after\endcsname{27.7}
\expandafter\def\csname v@nl/whisper-tiny/before\endcsname{70.8}
\expandafter\def\csname v@nl/whisper-tiny/ci\endcsname{26.1 to 29.4}
\expandafter\def\csname v@nl/whisper-tiny/gain\endcsname{43.1}
\expandafter\def\csname v@nl/whisper-tiny/rest\endcsname{25.0}
\expandafter\def\csname v@nl/whisper-tiny/rest-before\endcsname{65.3}
\expandafter\def\csname v@ooc/best-ours/cer\endcsname{5.3}
\expandafter\def\csname v@ooc/best-ours/name\endcsname{w2v-BERT 2.0}
\expandafter\def\csname v@ooc/best/cer\endcsname{6.6}
\expandafter\def\csname v@ooc/best/name\endcsname{MMS 1B}
\expandafter\def\csname v@ooc/clean-names\endcsname{Finnish, Gujarati, Lingala and Shona}
\expandafter\def\csname v@ooc/cohere-transcribe/fl-after\endcsname{16.5}
\expandafter\def\csname v@ooc/cohere-transcribe/fl-before\endcsname{68.5}
\expandafter\def\csname v@ooc/cohere-transcribe/fl-gain\endcsname{52.0}
\expandafter\def\csname v@ooc/cohere-transcribe/fl-gain-ci\endcsname{50.1 to 54.0}
\expandafter\def\csname v@ooc/cohere-transcribe/keep\endcsname{101}
\expandafter\def\csname v@ooc/cohere-transcribe/n\endcsname{4}
\expandafter\def\csname v@ooc/cohere-transcribe/ours-after\endcsname{9.1}
\expandafter\def\csname v@ooc/cohere-transcribe/ours-before\endcsname{60.9}
\expandafter\def\csname v@ooc/cohere-transcribe/ours-gain\endcsname{51.7}
\expandafter\def\csname v@ooc/cohere-transcribe/run\endcsname{fthi_cohere-transcribe}
\expandafter\def\csname v@ooc/fleurs-test-in-train-max\endcsname{181}
\expandafter\def\csname v@ooc/fleurs-test-in-train-max-name\endcsname{Tajik}
\expandafter\def\csname v@ooc/from-fleurs-names\endcsname{Burmese, Estonian, Lao, Latvian, Occitan, Slovenian and Tajik}
\expandafter\def\csname v@ooc/gemma4-12b/fl-after\endcsname{20.3}
\expandafter\def\csname v@ooc/gemma4-12b/fl-before\endcsname{76.2}
\expandafter\def\csname v@ooc/gemma4-12b/fl-gain\endcsname{55.9}
\expandafter\def\csname v@ooc/gemma4-12b/fl-gain-ci\endcsname{53.9 to 57.8}
\expandafter\def\csname v@ooc/gemma4-12b/keep\endcsname{87}
\expandafter\def\csname v@ooc/gemma4-12b/n\endcsname{4}
\expandafter\def\csname v@ooc/gemma4-12b/ours-after\endcsname{13.5}
\expandafter\def\csname v@ooc/gemma4-12b/ours-before\endcsname{77.9}
\expandafter\def\csname v@ooc/gemma4-12b/ours-gain\endcsname{64.4}
\expandafter\def\csname v@ooc/gemma4-12b/run\endcsname{ft_gemma4-12b}
\expandafter\def\csname v@ooc/gemma4-e2b/fl-after\endcsname{16.5}
\expandafter\def\csname v@ooc/gemma4-e2b/fl-before\endcsname{10.3}
\expandafter\def\csname v@ooc/gemma4-e2b/fl-gain\endcsname{-6.1}
\expandafter\def\csname v@ooc/gemma4-e2b/fl-gain-ci\endcsname{-7.2 to -5.3}
\expandafter\def\csname v@ooc/gemma4-e2b/n\endcsname{4}
\expandafter\def\csname v@ooc/gemma4-e2b/ours-after\endcsname{9.7}
\expandafter\def\csname v@ooc/gemma4-e2b/ours-before\endcsname{10.9}
\expandafter\def\csname v@ooc/gemma4-e2b/ours-gain\endcsname{1.3}
\expandafter\def\csname v@ooc/gemma4-e2b/run\endcsname{ft_gemma4-e2b}
\expandafter\def\csname v@ooc/gemma4-e4b/fl-after\endcsname{10.5}
\expandafter\def\csname v@ooc/gemma4-e4b/fl-before\endcsname{8.7}
\expandafter\def\csname v@ooc/gemma4-e4b/fl-gain\endcsname{-1.8}
\expandafter\def\csname v@ooc/gemma4-e4b/fl-gain-ci\endcsname{-2.4 to -1.3}
\expandafter\def\csname v@ooc/gemma4-e4b/n\endcsname{4}
\expandafter\def\csname v@ooc/gemma4-e4b/ours-after\endcsname{7.9}
\expandafter\def\csname v@ooc/gemma4-e4b/ours-before\endcsname{11.0}
\expandafter\def\csname v@ooc/gemma4-e4b/ours-gain\endcsname{3.1}
\expandafter\def\csname v@ooc/gemma4-e4b/run\endcsname{ft_gemma4-e4b}
\expandafter\def\csname v@ooc/granite-2b/fl-after\endcsname{24.1}
\expandafter\def\csname v@ooc/granite-2b/fl-before\endcsname{50.5}
\expandafter\def\csname v@ooc/granite-2b/fl-gain\endcsname{26.4}
\expandafter\def\csname v@ooc/granite-2b/fl-gain-ci\endcsname{25.5 to 27.3}
\expandafter\def\csname v@ooc/granite-2b/keep\endcsname{73}
\expandafter\def\csname v@ooc/granite-2b/n\endcsname{4}
\expandafter\def\csname v@ooc/granite-2b/ours-after\endcsname{16.8}
\expandafter\def\csname v@ooc/granite-2b/ours-before\endcsname{53.0}
\expandafter\def\csname v@ooc/granite-2b/ours-gain\endcsname{36.2}
\expandafter\def\csname v@ooc/granite-2b/run\endcsname{ck_granite-2b}
\expandafter\def\csname v@ooc/keep-max\endcsname{101}
\expandafter\def\csname v@ooc/keep-median\endcsname{79}
\expandafter\def\csname v@ooc/keep-min\endcsname{33}
\expandafter\def\csname v@ooc/keep-min-gain\endcsname{5}
\expandafter\def\csname v@ooc/keep-n\endcsname{16}
\expandafter\def\csname v@ooc/knew-before-max\endcsname{11.0}
\expandafter\def\csname v@ooc/knew-n\endcsname{4}
\expandafter\def\csname v@ooc/knew-names\endcsname{MMS 1B, omniASR CTC 1B, Gemma 4 E4B and Gemma 4 E2B}
\expandafter\def\csname v@ooc/lfm3-audio/fl-after\endcsname{14.9}
\expandafter\def\csname v@ooc/lfm3-audio/fl-before\endcsname{51.1}
\expandafter\def\csname v@ooc/lfm3-audio/fl-gain\endcsname{36.2}
\expandafter\def\csname v@ooc/lfm3-audio/fl-gain-ci\endcsname{34.6 to 37.8}
\expandafter\def\csname v@ooc/lfm3-audio/keep\endcsname{84}
\expandafter\def\csname v@ooc/lfm3-audio/n\endcsname{4}
\expandafter\def\csname v@ooc/lfm3-audio/ours-after\endcsname{10.3}
\expandafter\def\csname v@ooc/lfm3-audio/ours-before\endcsname{53.2}
\expandafter\def\csname v@ooc/lfm3-audio/ours-gain\endcsname{42.9}
\expandafter\def\csname v@ooc/lfm3-audio/run\endcsname{ft_lfm3-audio}
\expandafter\def\csname v@ooc/mms-1b/fl-after\endcsname{6.6}
\expandafter\def\csname v@ooc/mms-1b/fl-before\endcsname{4.2}
\expandafter\def\csname v@ooc/mms-1b/fl-gain\endcsname{-2.4}
\expandafter\def\csname v@ooc/mms-1b/fl-gain-ci\endcsname{-2.7 to -2.2}
\expandafter\def\csname v@ooc/mms-1b/n\endcsname{4}
\expandafter\def\csname v@ooc/mms-1b/ours-after\endcsname{5.4}
\expandafter\def\csname v@ooc/mms-1b/ours-before\endcsname{6.8}
\expandafter\def\csname v@ooc/mms-1b/ours-gain\endcsname{1.4}
\expandafter\def\csname v@ooc/mms-1b/run\endcsname{ck_mms-1b}
\expandafter\def\csname v@ooc/n-from-fleurs\endcsname{7}
\expandafter\def\csname v@ooc/n-langs\endcsname{4}
\expandafter\def\csname v@ooc/n-models\endcsname{21}
\expandafter\def\csname v@ooc/n-shared\endcsname{11}
\expandafter\def\csname v@ooc/nemotron-30b/fl-after\endcsname{11.5}
\expandafter\def\csname v@ooc/nemotron-30b/fl-before\endcsname{22.5}
\expandafter\def\csname v@ooc/nemotron-30b/fl-gain\endcsname{11.0}
\expandafter\def\csname v@ooc/nemotron-30b/fl-gain-ci\endcsname{9.8 to 12.2}
\expandafter\def\csname v@ooc/nemotron-30b/keep\endcsname{61}
\expandafter\def\csname v@ooc/nemotron-30b/n\endcsname{4}
\expandafter\def\csname v@ooc/nemotron-30b/ours-after\endcsname{7.6}
\expandafter\def\csname v@ooc/nemotron-30b/ours-before\endcsname{25.6}
\expandafter\def\csname v@ooc/nemotron-30b/ours-gain\endcsname{18.0}
\expandafter\def\csname v@ooc/nemotron-30b/run\endcsname{ftall_nemotron-30b}
\expandafter\def\csname v@ooc/nemotron-stream/fl-after\endcsname{44.1}
\expandafter\def\csname v@ooc/nemotron-stream/fl-before\endcsname{48.5}
\expandafter\def\csname v@ooc/nemotron-stream/fl-gain\endcsname{4.4}
\expandafter\def\csname v@ooc/nemotron-stream/fl-gain-ci\endcsname{3.1 to 5.5}
\expandafter\def\csname v@ooc/nemotron-stream/keep\endcsname{33}
\expandafter\def\csname v@ooc/nemotron-stream/n\endcsname{4}
\expandafter\def\csname v@ooc/nemotron-stream/ours-after\endcsname{41.3}
\expandafter\def\csname v@ooc/nemotron-stream/ours-before\endcsname{54.4}
\expandafter\def\csname v@ooc/nemotron-stream/ours-gain\endcsname{13.1}
\expandafter\def\csname v@ooc/nemotron-stream/run\endcsname{ft_nemotron-stream}
\expandafter\def\csname v@ooc/omni-ctc-1b/fl-after\endcsname{7.6}
\expandafter\def\csname v@ooc/omni-ctc-1b/fl-before\endcsname{4.6}
\expandafter\def\csname v@ooc/omni-ctc-1b/fl-gain\endcsname{-3.0}
\expandafter\def\csname v@ooc/omni-ctc-1b/fl-gain-ci\endcsname{-3.2 to -2.8}
\expandafter\def\csname v@ooc/omni-ctc-1b/n\endcsname{4}
\expandafter\def\csname v@ooc/omni-ctc-1b/ours-after\endcsname{5.7}
\expandafter\def\csname v@ooc/omni-ctc-1b/ours-before\endcsname{5.2}
\expandafter\def\csname v@ooc/omni-ctc-1b/ours-gain\endcsname{-0.4}
\expandafter\def\csname v@ooc/omni-ctc-1b/run\endcsname{ft_omni-ctc-1b}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/fl-after\endcsname{16.7}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/fl-before\endcsname{43.2}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/fl-gain\endcsname{26.5}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/fl-gain-ci\endcsname{25.3 to 27.7}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/keep\endcsname{95}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/n\endcsname{4}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/ours-after\endcsname{11.8}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/ours-before\endcsname{39.8}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/ours-gain\endcsname{28.0}
\expandafter\def\csname v@ooc/parakeet-tdt-v3/run\endcsname{ck_parakeet-tdt-v3}
\expandafter\def\csname v@ooc/per-lang\endcsname{200}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/fl-after\endcsname{20.1}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/fl-before\endcsname{47.5}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/fl-gain\endcsname{27.4}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/fl-gain-ci\endcsname{26.5 to 28.5}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/keep\endcsname{77}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/n\endcsname{4}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/ours-after\endcsname{13.3}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/ours-before\endcsname{49.1}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/ours-gain\endcsname{35.8}
\expandafter\def\csname v@ooc/qwen3-asr-0.6b/run\endcsname{ft_qwen3-asr-0.6b}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/fl-after\endcsname{16.4}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/fl-before\endcsname{39.7}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/fl-gain\endcsname{23.3}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/fl-gain-ci\endcsname{22.6 to 24.1}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/keep\endcsname{81}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/n\endcsname{4}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/ours-after\endcsname{11.4}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/ours-before\endcsname{40.1}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/ours-gain\endcsname{28.7}
\expandafter\def\csname v@ooc/qwen3-asr-1.7b/run\endcsname{ft_qwen3-asr-1.7b}
\expandafter\def\csname v@ooc/rank-rho\endcsname{0.94}
\expandafter\def\csname v@ooc/voxtral-mini/fl-after\endcsname{11.7}
\expandafter\def\csname v@ooc/voxtral-mini/fl-before\endcsname{45.8}
\expandafter\def\csname v@ooc/voxtral-mini/fl-gain\endcsname{34.1}
\expandafter\def\csname v@ooc/voxtral-mini/fl-gain-ci\endcsname{32.4 to 36.0}
\expandafter\def\csname v@ooc/voxtral-mini/keep\endcsname{91}
\expandafter\def\csname v@ooc/voxtral-mini/n\endcsname{4}
\expandafter\def\csname v@ooc/voxtral-mini/ours-after\endcsname{7.8}
\expandafter\def\csname v@ooc/voxtral-mini/ours-before\endcsname{45.5}
\expandafter\def\csname v@ooc/voxtral-mini/ours-gain\endcsname{37.7}
\expandafter\def\csname v@ooc/voxtral-mini/run\endcsname{ck_voxtral-mini}
\expandafter\def\csname v@ooc/w2v-bert/fl-after\endcsname{7.3}
\expandafter\def\csname v@ooc/w2v-bert/n\endcsname{4}
\expandafter\def\csname v@ooc/w2v-bert/ours-after\endcsname{5.3}
\expandafter\def\csname v@ooc/w2v-bert/run\endcsname{ft_w2v-bert}
\expandafter\def\csname v@ooc/whisper-large-v2/fl-after\endcsname{12.0}
\expandafter\def\csname v@ooc/whisper-large-v2/fl-before\endcsname{36.5}
\expandafter\def\csname v@ooc/whisper-large-v2/fl-gain\endcsname{24.5}
\expandafter\def\csname v@ooc/whisper-large-v2/fl-gain-ci\endcsname{23.4 to 25.8}
\expandafter\def\csname v@ooc/whisper-large-v2/keep\endcsname{74}
\expandafter\def\csname v@ooc/whisper-large-v2/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-large-v2/ours-after\endcsname{7.2}
\expandafter\def\csname v@ooc/whisper-large-v2/ours-before\endcsname{40.5}
\expandafter\def\csname v@ooc/whisper-large-v2/ours-gain\endcsname{33.3}
\expandafter\def\csname v@ooc/whisper-large-v2/run\endcsname{ft_whisper-large-v2}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/fl-after\endcsname{13.0}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/fl-before\endcsname{21.5}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/fl-gain\endcsname{8.4}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/fl-gain-ci\endcsname{7.2 to 9.8}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/keep\endcsname{79}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/ours-after\endcsname{8.9}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/ours-before\endcsname{19.6}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/ours-gain\endcsname{10.7}
\expandafter\def\csname v@ooc/whisper-large-v3-turbo/run\endcsname{ft_whisper-large-v3-turbo}
\expandafter\def\csname v@ooc/whisper-large-v3/fl-after\endcsname{11.3}
\expandafter\def\csname v@ooc/whisper-large-v3/fl-before\endcsname{16.2}
\expandafter\def\csname v@ooc/whisper-large-v3/fl-gain\endcsname{4.9}
\expandafter\def\csname v@ooc/whisper-large-v3/fl-gain-ci\endcsname{4.4 to 5.4}
\expandafter\def\csname v@ooc/whisper-large-v3/keep\endcsname{52}
\expandafter\def\csname v@ooc/whisper-large-v3/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-large-v3/ours-after\endcsname{6.9}
\expandafter\def\csname v@ooc/whisper-large-v3/ours-before\endcsname{16.3}
\expandafter\def\csname v@ooc/whisper-large-v3/ours-gain\endcsname{9.4}
\expandafter\def\csname v@ooc/whisper-large-v3/run\endcsname{ft_whisper-large-v3}
\expandafter\def\csname v@ooc/whisper-medium/fl-after\endcsname{13.1}
\expandafter\def\csname v@ooc/whisper-medium/fl-before\endcsname{58.9}
\expandafter\def\csname v@ooc/whisper-medium/fl-gain\endcsname{45.8}
\expandafter\def\csname v@ooc/whisper-medium/fl-gain-ci\endcsname{44.3 to 47.3}
\expandafter\def\csname v@ooc/whisper-medium/keep\endcsname{90}
\expandafter\def\csname v@ooc/whisper-medium/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-medium/ours-after\endcsname{7.7}
\expandafter\def\csname v@ooc/whisper-medium/ours-before\endcsname{58.4}
\expandafter\def\csname v@ooc/whisper-medium/ours-gain\endcsname{50.7}
\expandafter\def\csname v@ooc/whisper-medium/run\endcsname{ck_whisper-medium}
\expandafter\def\csname v@ooc/whisper-small/fl-after\endcsname{17.5}
\expandafter\def\csname v@ooc/whisper-small/fl-before\endcsname{52.8}
\expandafter\def\csname v@ooc/whisper-small/fl-gain\endcsname{35.3}
\expandafter\def\csname v@ooc/whisper-small/fl-gain-ci\endcsname{33.9 to 36.7}
\expandafter\def\csname v@ooc/whisper-small/keep\endcsname{80}
\expandafter\def\csname v@ooc/whisper-small/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-small/ours-after\endcsname{10.1}
\expandafter\def\csname v@ooc/whisper-small/ours-before\endcsname{54.2}
\expandafter\def\csname v@ooc/whisper-small/ours-gain\endcsname{44.2}
\expandafter\def\csname v@ooc/whisper-small/run\endcsname{ft_whisper-small}
\expandafter\def\csname v@ooc/whisper-tiny/fl-after\endcsname{32.2}
\expandafter\def\csname v@ooc/whisper-tiny/fl-before\endcsname{55.5}
\expandafter\def\csname v@ooc/whisper-tiny/fl-gain\endcsname{23.4}
\expandafter\def\csname v@ooc/whisper-tiny/fl-gain-ci\endcsname{21.9 to 24.9}
\expandafter\def\csname v@ooc/whisper-tiny/keep\endcsname{70}
\expandafter\def\csname v@ooc/whisper-tiny/n\endcsname{4}
\expandafter\def\csname v@ooc/whisper-tiny/ours-after\endcsname{19.1}
\expandafter\def\csname v@ooc/whisper-tiny/ours-before\endcsname{52.4}
\expandafter\def\csname v@ooc/whisper-tiny/ours-gain\endcsname{33.4}
\expandafter\def\csname v@ooc/whisper-tiny/run\endcsname{ck_whisper-tiny}
\expandafter\def\csname v@ooc/worse-n\endcsname{4}
\expandafter\def\csname v@ooc/worse-names\endcsname{MMS 1B, omniASR CTC 1B, Gemma 4 E4B and Gemma 4 E2B}
\expandafter\def\csname v@ooc/worse-word\endcsname{four}
\expandafter\def\csname v@order/both/cohere-transcribe/first\endcsname{0}
\expandafter\def\csname v@order/both/cohere-transcribe/rank\endcsname{7 to 11}
\expandafter\def\csname v@order/both/dec-ci\endcsname{-0.5 to 1.9}
\expandafter\def\csname v@order/both/dec-share\endcsname{91}
\expandafter\def\csname v@order/both/gemma4-12b/first\endcsname{0}
\expandafter\def\csname v@order/both/gemma4-12b/rank\endcsname{16 to 18}
\expandafter\def\csname v@order/both/gemma4-e2b/first\endcsname{0}
\expandafter\def\csname v@order/both/gemma4-e2b/rank\endcsname{14 to 17}
\expandafter\def\csname v@order/both/gemma4-e4b/first\endcsname{0}
\expandafter\def\csname v@order/both/gemma4-e4b/rank\endcsname{8 to 14}
\expandafter\def\csname v@order/both/granite-2b/first\endcsname{0}
\expandafter\def\csname v@order/both/granite-2b/rank\endcsname{18 to 19}
\expandafter\def\csname v@order/both/held\endcsname{183}
\expandafter\def\csname v@order/both/lfm3-audio/first\endcsname{0}
\expandafter\def\csname v@order/both/lfm3-audio/rank\endcsname{13 to 16}
\expandafter\def\csname v@order/both/loose\endcsname{27}
\expandafter\def\csname v@order/both/loose-reach\endcsname{4}
\expandafter\def\csname v@order/both/mms-1b/first\endcsname{99}
\expandafter\def\csname v@order/both/mms-1b/rank\endcsname{1}
\expandafter\def\csname v@order/both/nemotron-30b/first\endcsname{0}
\expandafter\def\csname v@order/both/nemotron-30b/rank\endcsname{8 to 11}
\expandafter\def\csname v@order/both/nemotron-stream/first\endcsname{0}
\expandafter\def\csname v@order/both/nemotron-stream/rank\endcsname{21}
\expandafter\def\csname v@order/both/omni-ctc-1b/first\endcsname{1}
\expandafter\def\csname v@order/both/omni-ctc-1b/rank\endcsname{2 to 3}
\expandafter\def\csname v@order/both/parakeet-tdt-v3/first\endcsname{0}
\expandafter\def\csname v@order/both/parakeet-tdt-v3/rank\endcsname{16 to 19}
\expandafter\def\csname v@order/both/qwen3-asr-0.6b/first\endcsname{0}
\expandafter\def\csname v@order/both/qwen3-asr-0.6b/rank\endcsname{13 to 16}
\expandafter\def\csname v@order/both/qwen3-asr-1.7b/first\endcsname{0}
\expandafter\def\csname v@order/both/qwen3-asr-1.7b/rank\endcsname{9 to 13}
\expandafter\def\csname v@order/both/top-first\endcsname{99}
\expandafter\def\csname v@order/both/voxtral-mini/first\endcsname{0}
\expandafter\def\csname v@order/both/voxtral-mini/rank\endcsname{8 to 13}
\expandafter\def\csname v@order/both/w2v-bert/first\endcsname{0}
\expandafter\def\csname v@order/both/w2v-bert/rank\endcsname{2 to 4}
\expandafter\def\csname v@order/both/whisper-large-v2/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-large-v2/rank\endcsname{5 to 6}
\expandafter\def\csname v@order/both/whisper-large-v3-turbo/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-large-v3-turbo/rank\endcsname{5 to 7}
\expandafter\def\csname v@order/both/whisper-large-v3/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-large-v3/rank\endcsname{3 to 4}
\expandafter\def\csname v@order/both/whisper-medium/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-medium/rank\endcsname{6 to 8}
\expandafter\def\csname v@order/both/whisper-small/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-small/rank\endcsname{10 to 14}
\expandafter\def\csname v@order/both/whisper-tiny/first\endcsname{0}
\expandafter\def\csname v@order/both/whisper-tiny/rank\endcsname{20}
\expandafter\def\csname v@order/draws\endcsname{5,000}
\expandafter\def\csname v@order/n\endcsname{21}
\expandafter\def\csname v@order/pairs\endcsname{210}
\expandafter\def\csname v@order/spk/cohere-transcribe/first\endcsname{0}
\expandafter\def\csname v@order/spk/cohere-transcribe/rank\endcsname{8 to 9}
\expandafter\def\csname v@order/spk/dec-ci\endcsname{0.4 to 1.2}
\expandafter\def\csname v@order/spk/dec-share\endcsname{100}
\expandafter\def\csname v@order/spk/gemma4-12b/first\endcsname{0}
\expandafter\def\csname v@order/spk/gemma4-12b/rank\endcsname{17}
\expandafter\def\csname v@order/spk/gemma4-e2b/first\endcsname{0}
\expandafter\def\csname v@order/spk/gemma4-e2b/rank\endcsname{15 to 16}
\expandafter\def\csname v@order/spk/gemma4-e4b/first\endcsname{0}
\expandafter\def\csname v@order/spk/gemma4-e4b/rank\endcsname{10 to 13}
\expandafter\def\csname v@order/spk/granite-2b/first\endcsname{0}
\expandafter\def\csname v@order/spk/granite-2b/rank\endcsname{19}
\expandafter\def\csname v@order/spk/held\endcsname{201}
\expandafter\def\csname v@order/spk/lfm3-audio/first\endcsname{0}
\expandafter\def\csname v@order/spk/lfm3-audio/rank\endcsname{14 to 15}
\expandafter\def\csname v@order/spk/loose\endcsname{9}
\expandafter\def\csname v@order/spk/mms-1b/first\endcsname{100}
\expandafter\def\csname v@order/spk/mms-1b/rank\endcsname{1}
\expandafter\def\csname v@order/spk/nemotron-30b/first\endcsname{0}
\expandafter\def\csname v@order/spk/nemotron-30b/rank\endcsname{8 to 9}
\expandafter\def\csname v@order/spk/nemotron-stream/first\endcsname{0}
\expandafter\def\csname v@order/spk/nemotron-stream/rank\endcsname{21}
\expandafter\def\csname v@order/spk/omni-ctc-1b/first\endcsname{0}
\expandafter\def\csname v@order/spk/omni-ctc-1b/rank\endcsname{2}
\expandafter\def\csname v@order/spk/parakeet-tdt-v3/first\endcsname{0}
\expandafter\def\csname v@order/spk/parakeet-tdt-v3/rank\endcsname{18}
\expandafter\def\csname v@order/spk/qwen3-asr-0.6b/first\endcsname{0}
\expandafter\def\csname v@order/spk/qwen3-asr-0.6b/rank\endcsname{14 to 16}
\expandafter\def\csname v@order/spk/qwen3-asr-1.7b/first\endcsname{0}
\expandafter\def\csname v@order/spk/qwen3-asr-1.7b/rank\endcsname{10 to 13}
\expandafter\def\csname v@order/spk/top-first\endcsname{100}
\expandafter\def\csname v@order/spk/voxtral-mini/first\endcsname{0}
\expandafter\def\csname v@order/spk/voxtral-mini/rank\endcsname{10 to 12}
\expandafter\def\csname v@order/spk/w2v-bert/first\endcsname{0}
\expandafter\def\csname v@order/spk/w2v-bert/rank\endcsname{3}
\expandafter\def\csname v@order/spk/whisper-large-v2/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-large-v2/rank\endcsname{5 to 6}
\expandafter\def\csname v@order/spk/whisper-large-v3-turbo/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-large-v3-turbo/rank\endcsname{5 to 6}
\expandafter\def\csname v@order/spk/whisper-large-v3/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-large-v3/rank\endcsname{4}
\expandafter\def\csname v@order/spk/whisper-medium/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-medium/rank\endcsname{7}
\expandafter\def\csname v@order/spk/whisper-small/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-small/rank\endcsname{11 to 13}
\expandafter\def\csname v@order/spk/whisper-tiny/first\endcsname{0}
\expandafter\def\csname v@order/spk/whisper-tiny/rank\endcsname{20}
\expandafter\def\csname v@order/top/name\endcsname{MMS 1B}
\expandafter\def\csname v@rd/gain-max\endcsname{0.3}
\expandafter\def\csname v@rd/gain-max-name\endcsname{Whisper large-v3-turbo}
\expandafter\def\csname v@rd/gain-min\endcsname{-0.1}
\expandafter\def\csname v@rd/n\endcsname{7}
\expandafter\def\csname v@rd/qwen3-asr-0.6b/after\endcsname{18.1}
\expandafter\def\csname v@rd/qwen3-asr-0.6b/before\endcsname{18.2}
\expandafter\def\csname v@rd/qwen3-asr-0.6b/gain\endcsname{0.1}
\expandafter\def\csname v@rd/qwen3-asr-1.7b/after\endcsname{16.6}
\expandafter\def\csname v@rd/qwen3-asr-1.7b/before\endcsname{16.6}
\expandafter\def\csname v@rd/qwen3-asr-1.7b/gain\endcsname{-0.1}
\expandafter\def\csname v@rd/whisper-large-v2/after\endcsname{14.1}
\expandafter\def\csname v@rd/whisper-large-v2/before\endcsname{14.2}
\expandafter\def\csname v@rd/whisper-large-v2/gain\endcsname{0.2}
\expandafter\def\csname v@rd/whisper-large-v3-turbo/after\endcsname{14.0}
\expandafter\def\csname v@rd/whisper-large-v3-turbo/before\endcsname{14.3}
\expandafter\def\csname v@rd/whisper-large-v3-turbo/gain\endcsname{0.3}
\expandafter\def\csname v@rd/whisper-large-v3/after\endcsname{13.3}
\expandafter\def\csname v@rd/whisper-large-v3/before\endcsname{13.5}
\expandafter\def\csname v@rd/whisper-large-v3/gain\endcsname{0.2}
\expandafter\def\csname v@rd/whisper-medium/after\endcsname{15.3}
\expandafter\def\csname v@rd/whisper-medium/before\endcsname{15.5}
\expandafter\def\csname v@rd/whisper-medium/gain\endcsname{0.2}
\expandafter\def\csname v@rd/whisper-small/after\endcsname{16.7}
\expandafter\def\csname v@rd/whisper-small/before\endcsname{16.9}
\expandafter\def\csname v@rd/whisper-small/gain\endcsname{0.2}
\expandafter\def\csname v@rec/cohere-transcribe/epochs\endcsname{10}
\expandafter\def\csname v@rec/cohere/dec\endcsname{0.14}
\expandafter\def\csname v@rec/cohere/enc\endcsname{1.90}
\expandafter\def\csname v@rec/cohere/new\endcsname{50}
\expandafter\def\csname v@rec/cohere/spare\endcsname{29}
\expandafter\def\csname v@rec/cohere/tags\endcsname{21}
\expandafter\def\csname v@rec/ctc/chars\endcsname{825}
\expandafter\def\csname v@rec/enc-share/ctc-min\endcsname{97}
\expandafter\def\csname v@rec/enc-share/lm-max\endcsname{24}
\expandafter\def\csname v@rec/enc-share/lm-min\endcsname{0}
\expandafter\def\csname v@rec/fewer-epochs\endcsname{Whisper large-v2 (5), Voxtral (4), Nemotron 30B (4), Gemma 4 E2B (5), Gemma 4 E4B (5) and Gemma 4 12B (4)}
\expandafter\def\csname v@rec/gemma4-12b/epochs\endcsname{4}
\expandafter\def\csname v@rec/gemma4-12b/lookup\endcsname{0.00}
\expandafter\def\csname v@rec/gemma4-12b/lookup-share\endcsname{0}
\expandafter\def\csname v@rec/gemma4-12b/stored\endcsname{11.96}
\expandafter\def\csname v@rec/gemma4-12b/trained\endcsname{11.91}
\expandafter\def\csname v@rec/gemma4-12b/unused\endcsname{0.05}
\expandafter\def\csname v@rec/gemma4-e2b/epochs\endcsname{5}
\expandafter\def\csname v@rec/gemma4-e2b/lookup\endcsname{2.35}
\expandafter\def\csname v@rec/gemma4-e2b/lookup-share\endcsname{46}
\expandafter\def\csname v@rec/gemma4-e2b/stored\endcsname{5.10}
\expandafter\def\csname v@rec/gemma4-e2b/trained\endcsname{2.59}
\expandafter\def\csname v@rec/gemma4-e2b/unused\endcsname{0.17}
\expandafter\def\csname v@rec/gemma4-e4b/epochs\endcsname{5}
\expandafter\def\csname v@rec/gemma4-e4b/lookup\endcsname{2.82}
\expandafter\def\csname v@rec/gemma4-e4b/lookup-share\endcsname{35}
\expandafter\def\csname v@rec/gemma4-e4b/stored\endcsname{7.94}
\expandafter\def\csname v@rec/gemma4-e4b/trained\endcsname{4.95}
\expandafter\def\csname v@rec/gemma4-e4b/unused\endcsname{0.17}
\expandafter\def\csname v@rec/granite-2b/epochs\endcsname{10}
\expandafter\def\csname v@rec/lfm3-audio/epochs\endcsname{10}
\expandafter\def\csname v@rec/lfm3-audio/lookup\endcsname{0.00}
\expandafter\def\csname v@rec/lfm3-audio/lookup-share\endcsname{0}
\expandafter\def\csname v@rec/lfm3-audio/stored\endcsname{1.98}
\expandafter\def\csname v@rec/lfm3-audio/trained\endcsname{1.84}
\expandafter\def\csname v@rec/lfm3-audio/unused\endcsname{0.13}
\expandafter\def\csname v@rec/mms-1b/epochs\endcsname{10}
\expandafter\def\csname v@rec/mms/head-rate\endcsname{1e-3}
\expandafter\def\csname v@rec/mms/mask\endcsname{5}
\expandafter\def\csname v@rec/mms/mask-len\endcsname{10}
\expandafter\def\csname v@rec/n\endcsname{24}
\expandafter\def\csname v@rec/nemo-stream/new\endcsname{660}
\expandafter\def\csname v@rec/nemo-stream/row-rate\endcsname{1e-3}
\expandafter\def\csname v@rec/nemo30/all\endcsname{32.2}
\expandafter\def\csname v@rec/nemo30/all-cer\endcsname{15.8}
\expandafter\def\csname v@rec/nemo30/all-dev\endcsname{22.7}
\expandafter\def\csname v@rec/nemo30/all-epoch\endcsname{2}
\expandafter\def\csname v@rec/nemo30/all-gain\endcsname{0.2}
\expandafter\def\csname v@rec/nemo30/all-gain-ci\endcsname{-0.2 to 0.6}
\expandafter\def\csname v@rec/nemo30/experts\endcsname{29.8}
\expandafter\def\csname v@rec/nemo30/first-cer\endcsname{16.0}
\expandafter\def\csname v@rec/nemo30/first-dev\endcsname{22.9}
\expandafter\def\csname v@rec/nemo30/first-epoch\endcsname{3}
\expandafter\def\csname v@rec/nemo30/main\endcsname{the second}
\expandafter\def\csname v@rec/nemo30/proj\endcsname{3.4}
\expandafter\def\csname v@rec/nemo30/share\endcsname{6}
\expandafter\def\csname v@rec/nemo30/table\endcsname{0.35}
\expandafter\def\csname v@rec/nemo30/total\endcsname{32.4}
\expandafter\def\csname v@rec/nemo30/trained\endcsname{2.02}
\expandafter\def\csname v@rec/nemotron-30b/epochs\endcsname{4}
\expandafter\def\csname v@rec/nemotron-stream/epochs\endcsname{10}
\expandafter\def\csname v@rec/omni-ctc-1b/epochs\endcsname{10}
\expandafter\def\csname v@rec/omni-ctc-300m/epochs\endcsname{10}
\expandafter\def\csname v@rec/omni-ctc-7b/epochs\endcsname{10}
\expandafter\def\csname v@rec/omni/new\endcsname{75}
\expandafter\def\csname v@rec/omni/vocab\endcsname{9,812}
\expandafter\def\csname v@rec/parakeet-tdt-v3/epochs\endcsname{10}
\expandafter\def\csname v@rec/parakeet/new\endcsname{746}
\expandafter\def\csname v@rec/parakeet/row-rate\endcsname{3e-3}
\expandafter\def\csname v@rec/qwen3-asr-0.6b/epochs\endcsname{10}
\expandafter\def\csname v@rec/qwen3-asr-1.7b/epochs\endcsname{10}
\expandafter\def\csname v@rec/voxtral-mini/epochs\endcsname{4}
\expandafter\def\csname v@rec/w2v-bert/epochs\endcsname{10}
\expandafter\def\csname v@rec/w2v-bert/head-rate\endcsname{3e-5}
\expandafter\def\csname v@rec/whisper-base/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper-large-v2/epochs\endcsname{5}
\expandafter\def\csname v@rec/whisper-large-v3-turbo/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper-large-v3/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper-medium/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper-small/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper-tiny/epochs\endcsname{10}
\expandafter\def\csname v@rec/whisper/new\endcsname{33}
\expandafter\def\csname v@rec/whisper/own\endcsname{17}
\expandafter\def\csname v@rerun/mms-1b/changed\endcsname{yes}
\expandafter\def\csname v@rerun/mms-1b/first\endcsname{16.2}
\expandafter\def\csname v@rerun/mms-1b/first-rate\endcsname{1e-4}
\expandafter\def\csname v@rerun/mms-1b/main\endcsname{11.0}
\expandafter\def\csname v@rerun/mms-1b/main-rate\endcsname{1e-5}
\expandafter\def\csname v@rerun/voxtral-mini/changed\endcsname{yes}
\expandafter\def\csname v@rerun/voxtral-mini/first\endcsname{17.2}
\expandafter\def\csname v@rerun/voxtral-mini/first-rate\endcsname{1e-5}
\expandafter\def\csname v@rerun/voxtral-mini/main\endcsname{16.3}
\expandafter\def\csname v@rerun/voxtral-mini/main-rate\endcsname{3e-6}
\expandafter\def\csname v@rerun/whisper-medium/changed\endcsname{yes}
\expandafter\def\csname v@rerun/whisper-medium/first\endcsname{15.5}
\expandafter\def\csname v@rerun/whisper-medium/first-rate\endcsname{3e-5}
\expandafter\def\csname v@rerun/whisper-medium/main\endcsname{14.8}
\expandafter\def\csname v@rerun/whisper-medium/main-rate\endcsname{1e-5}
\expandafter\def\csname v@rerun/whisper-tiny/changed\endcsname{no}
\expandafter\def\csname v@rerun/whisper-tiny/first\endcsname{25.7}
\expandafter\def\csname v@rerun/whisper-tiny/first-rate\endcsname{1e-4}
\expandafter\def\csname v@rerun/whisper-tiny/main\endcsname{25.7}
\expandafter\def\csname v@rerun/whisper-tiny/main-rate\endcsname{1e-4}
\expandafter\def\csname v@rows/nemotron-stream/blank-norm\endcsname{107}
\expandafter\def\csname v@rows/nemotron-stream/low/below\endcsname{10.0}
\expandafter\def\csname v@rows/nemotron-stream/low/cos\endcsname{1.000}
\expandafter\def\csname v@rows/nemotron-stream/low/cos-min\endcsname{1.000}
\expandafter\def\csname v@rows/nemotron-stream/mean-cos\endcsname{0.82}
\expandafter\def\csname v@rows/nemotron-stream/n\endcsname{660}
\expandafter\def\csname v@rows/nemotron-stream/pre-cos\endcsname{0.76}
\expandafter\def\csname v@rows/nemotron-stream/row-norm\endcsname{149}
\expandafter\def\csname v@rows/nemotron-stream/ten/below\endcsname{9.9}
\expandafter\def\csname v@rows/nemotron-stream/ten/cos\endcsname{0.997}
\expandafter\def\csname v@rows/nemotron-stream/ten/cos-min\endcsname{0.988}
\expandafter\def\csname v@rows/parakeet-tdt-v3/blank-norm\endcsname{28}
\expandafter\def\csname v@rows/parakeet-tdt-v3/low/below\endcsname{10.0}
\expandafter\def\csname v@rows/parakeet-tdt-v3/low/cos\endcsname{0.960}
\expandafter\def\csname v@rows/parakeet-tdt-v3/low/cos-min\endcsname{0.865}
\expandafter\def\csname v@rows/parakeet-tdt-v3/mean-cos\endcsname{0.45}
\expandafter\def\csname v@rows/parakeet-tdt-v3/n\endcsname{746}
\expandafter\def\csname v@rows/parakeet-tdt-v3/pre-cos\endcsname{0.32}
\expandafter\def\csname v@rows/parakeet-tdt-v3/row-norm\endcsname{44}
\expandafter\def\csname v@rows/parakeet-tdt-v3/ten/below\endcsname{10.0}
\expandafter\def\csname v@rows/parakeet-tdt-v3/ten/cos\endcsname{0.948}
\expandafter\def\csname v@rows/parakeet-tdt-v3/ten/cos-min\endcsname{0.820}
\expandafter\def\csname v@sc/cohere-transcribe/best/latin\endcsname{100}
\expandafter\def\csname v@sc/cohere-transcribe/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/cohere-transcribe/best/non\endcsname{99}
\expandafter\def\csname v@sc/cohere-transcribe/best/non-wrong\endcsname{1}
\expandafter\def\csname v@sc/cohere-transcribe/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/cohere-transcribe/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/cohere-transcribe/epoch1/non\endcsname{93}
\expandafter\def\csname v@sc/cohere-transcribe/epoch1/non-wrong\endcsname{7}
\expandafter\def\csname v@sc/cohere-transcribe/told/latin\endcsname{56}
\expandafter\def\csname v@sc/cohere-transcribe/told/latin-wrong\endcsname{44}
\expandafter\def\csname v@sc/cohere-transcribe/told/non\endcsname{14}
\expandafter\def\csname v@sc/cohere-transcribe/told/non-wrong\endcsname{86}
\expandafter\def\csname v@sc/cohere-transcribe/untouched/latin\endcsname{100}
\expandafter\def\csname v@sc/cohere-transcribe/untouched/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/cohere-transcribe/untouched/non\endcsname{1}
\expandafter\def\csname v@sc/cohere-transcribe/untouched/non-wrong\endcsname{99}
\expandafter\def\csname v@sc/full-after-one\endcsname{13}
\expandafter\def\csname v@sc/gemma4-12b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/gemma4-12b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-12b/best/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-12b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-12b/epoch1/latin\endcsname{99}
\expandafter\def\csname v@sc/gemma4-12b/epoch1/latin-wrong\endcsname{1}
\expandafter\def\csname v@sc/gemma4-12b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-12b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-12b/told/latin\endcsname{59}
\expandafter\def\csname v@sc/gemma4-12b/told/latin-wrong\endcsname{41}
\expandafter\def\csname v@sc/gemma4-12b/told/non\endcsname{39}
\expandafter\def\csname v@sc/gemma4-12b/told/non-wrong\endcsname{61}
\expandafter\def\csname v@sc/gemma4-12b/untouched/latin\endcsname{59}
\expandafter\def\csname v@sc/gemma4-12b/untouched/latin-wrong\endcsname{41}
\expandafter\def\csname v@sc/gemma4-12b/untouched/non\endcsname{39}
\expandafter\def\csname v@sc/gemma4-12b/untouched/non-wrong\endcsname{61}
\expandafter\def\csname v@sc/gemma4-e2b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e2b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e2b/best/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e2b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e2b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e2b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e2b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e2b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e2b/told/latin\endcsname{83}
\expandafter\def\csname v@sc/gemma4-e2b/told/latin-wrong\endcsname{17}
\expandafter\def\csname v@sc/gemma4-e2b/told/non\endcsname{67}
\expandafter\def\csname v@sc/gemma4-e2b/told/non-wrong\endcsname{33}
\expandafter\def\csname v@sc/gemma4-e2b/untouched/latin\endcsname{83}
\expandafter\def\csname v@sc/gemma4-e2b/untouched/latin-wrong\endcsname{17}
\expandafter\def\csname v@sc/gemma4-e2b/untouched/non\endcsname{67}
\expandafter\def\csname v@sc/gemma4-e2b/untouched/non-wrong\endcsname{33}
\expandafter\def\csname v@sc/gemma4-e4b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e4b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e4b/best/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e4b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e4b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e4b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e4b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/gemma4-e4b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/gemma4-e4b/told/latin\endcsname{92}
\expandafter\def\csname v@sc/gemma4-e4b/told/latin-wrong\endcsname{8}
\expandafter\def\csname v@sc/gemma4-e4b/told/non\endcsname{61}
\expandafter\def\csname v@sc/gemma4-e4b/told/non-wrong\endcsname{39}
\expandafter\def\csname v@sc/gemma4-e4b/untouched/latin\endcsname{92}
\expandafter\def\csname v@sc/gemma4-e4b/untouched/latin-wrong\endcsname{8}
\expandafter\def\csname v@sc/gemma4-e4b/untouched/non\endcsname{61}
\expandafter\def\csname v@sc/gemma4-e4b/untouched/non-wrong\endcsname{39}
\expandafter\def\csname v@sc/granite-2b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/granite-2b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/granite-2b/best/non\endcsname{100}
\expandafter\def\csname v@sc/granite-2b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/granite-2b/epoch1/latin\endcsname{99}
\expandafter\def\csname v@sc/granite-2b/epoch1/latin-wrong\endcsname{1}
\expandafter\def\csname v@sc/granite-2b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/granite-2b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/granite-2b/told/latin\endcsname{95}
\expandafter\def\csname v@sc/granite-2b/told/latin-wrong\endcsname{5}
\expandafter\def\csname v@sc/granite-2b/told/non\endcsname{9}
\expandafter\def\csname v@sc/granite-2b/told/non-wrong\endcsname{91}
\expandafter\def\csname v@sc/granite-2b/untouched/latin\endcsname{97}
\expandafter\def\csname v@sc/granite-2b/untouched/latin-wrong\endcsname{3}
\expandafter\def\csname v@sc/granite-2b/untouched/non\endcsname{0}
\expandafter\def\csname v@sc/granite-2b/untouched/non-wrong\endcsname{100}
\expandafter\def\csname v@sc/lfm3-audio/best/latin\endcsname{100}
\expandafter\def\csname v@sc/lfm3-audio/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/lfm3-audio/best/non\endcsname{100}
\expandafter\def\csname v@sc/lfm3-audio/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/lfm3-audio/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/lfm3-audio/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/lfm3-audio/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/lfm3-audio/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/lfm3-audio/told/latin\endcsname{89}
\expandafter\def\csname v@sc/lfm3-audio/told/latin-wrong\endcsname{11}
\expandafter\def\csname v@sc/lfm3-audio/told/non\endcsname{25}
\expandafter\def\csname v@sc/lfm3-audio/told/non-wrong\endcsname{75}
\expandafter\def\csname v@sc/lfm3-audio/untouched/latin\endcsname{74}
\expandafter\def\csname v@sc/lfm3-audio/untouched/latin-wrong\endcsname{26}
\expandafter\def\csname v@sc/lfm3-audio/untouched/non\endcsname{15}
\expandafter\def\csname v@sc/lfm3-audio/untouched/non-wrong\endcsname{85}
\expandafter\def\csname v@sc/mms-1b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/mms-1b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/mms-1b/best/non\endcsname{100}
\expandafter\def\csname v@sc/mms-1b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/mms-1b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/mms-1b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/mms-1b/epoch1/non\endcsname{99}
\expandafter\def\csname v@sc/mms-1b/epoch1/non-wrong\endcsname{1}
\expandafter\def\csname v@sc/mms-1b/told/latin\endcsname{1}
\expandafter\def\csname v@sc/mms-1b/told/latin-wrong\endcsname{99}
\expandafter\def\csname v@sc/mms-1b/told/non\endcsname{9}
\expandafter\def\csname v@sc/mms-1b/told/non-wrong\endcsname{91}
\expandafter\def\csname v@sc/mms-1b/untouched/latin\endcsname{97}
\expandafter\def\csname v@sc/mms-1b/untouched/latin-wrong\endcsname{3}
\expandafter\def\csname v@sc/mms-1b/untouched/non\endcsname{57}
\expandafter\def\csname v@sc/mms-1b/untouched/non-wrong\endcsname{43}
\expandafter\def\csname v@sc/nemotron-30b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/nemotron-30b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/nemotron-30b/best/non\endcsname{100}
\expandafter\def\csname v@sc/nemotron-30b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/nemotron-30b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/nemotron-30b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/nemotron-30b/epoch1/non\endcsname{97}
\expandafter\def\csname v@sc/nemotron-30b/epoch1/non-wrong\endcsname{3}
\expandafter\def\csname v@sc/nemotron-30b/told/latin\endcsname{91}
\expandafter\def\csname v@sc/nemotron-30b/told/latin-wrong\endcsname{9}
\expandafter\def\csname v@sc/nemotron-30b/told/non\endcsname{33}
\expandafter\def\csname v@sc/nemotron-30b/told/non-wrong\endcsname{67}
\expandafter\def\csname v@sc/nemotron-30b/untouched/latin\endcsname{90}
\expandafter\def\csname v@sc/nemotron-30b/untouched/latin-wrong\endcsname{10}
\expandafter\def\csname v@sc/nemotron-30b/untouched/non\endcsname{24}
\expandafter\def\csname v@sc/nemotron-30b/untouched/non-wrong\endcsname{76}
\expandafter\def\csname v@sc/nemotron-stream/best/latin\endcsname{100}
\expandafter\def\csname v@sc/nemotron-stream/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/nemotron-stream/best/non\endcsname{99}
\expandafter\def\csname v@sc/nemotron-stream/best/non-wrong\endcsname{1}
\expandafter\def\csname v@sc/nemotron-stream/epoch1/latin\endcsname{99}
\expandafter\def\csname v@sc/nemotron-stream/epoch1/latin-wrong\endcsname{1}
\expandafter\def\csname v@sc/nemotron-stream/epoch1/non\endcsname{87}
\expandafter\def\csname v@sc/nemotron-stream/epoch1/non-wrong\endcsname{13}
\expandafter\def\csname v@sc/nemotron-stream/told/latin\endcsname{60}
\expandafter\def\csname v@sc/nemotron-stream/told/latin-wrong\endcsname{40}
\expandafter\def\csname v@sc/nemotron-stream/told/non\endcsname{25}
\expandafter\def\csname v@sc/nemotron-stream/told/non-wrong\endcsname{75}
\expandafter\def\csname v@sc/nemotron-stream/untouched/latin\endcsname{60}
\expandafter\def\csname v@sc/nemotron-stream/untouched/latin-wrong\endcsname{40}
\expandafter\def\csname v@sc/nemotron-stream/untouched/non\endcsname{25}
\expandafter\def\csname v@sc/nemotron-stream/untouched/non-wrong\endcsname{75}
\expandafter\def\csname v@sc/omni-ctc-1b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/omni-ctc-1b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/omni-ctc-1b/best/non\endcsname{100}
\expandafter\def\csname v@sc/omni-ctc-1b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/omni-ctc-1b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/omni-ctc-1b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/omni-ctc-1b/epoch1/non\endcsname{92}
\expandafter\def\csname v@sc/omni-ctc-1b/epoch1/non-wrong\endcsname{8}
\expandafter\def\csname v@sc/omni-ctc-1b/told/latin\endcsname{89}
\expandafter\def\csname v@sc/omni-ctc-1b/told/latin-wrong\endcsname{11}
\expandafter\def\csname v@sc/omni-ctc-1b/told/non\endcsname{78}
\expandafter\def\csname v@sc/omni-ctc-1b/told/non-wrong\endcsname{22}
\expandafter\def\csname v@sc/omni-ctc-1b/untouched/latin\endcsname{89}
\expandafter\def\csname v@sc/omni-ctc-1b/untouched/latin-wrong\endcsname{11}
\expandafter\def\csname v@sc/omni-ctc-1b/untouched/non\endcsname{78}
\expandafter\def\csname v@sc/omni-ctc-1b/untouched/non-wrong\endcsname{22}
\expandafter\def\csname v@sc/parakeet-tdt-v3/best/latin\endcsname{100}
\expandafter\def\csname v@sc/parakeet-tdt-v3/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/parakeet-tdt-v3/best/non\endcsname{92}
\expandafter\def\csname v@sc/parakeet-tdt-v3/best/non-wrong\endcsname{8}
\expandafter\def\csname v@sc/parakeet-tdt-v3/epoch1/latin\endcsname{94}
\expandafter\def\csname v@sc/parakeet-tdt-v3/epoch1/latin-wrong\endcsname{6}
\expandafter\def\csname v@sc/parakeet-tdt-v3/epoch1/non\endcsname{61}
\expandafter\def\csname v@sc/parakeet-tdt-v3/epoch1/non-wrong\endcsname{39}
\expandafter\def\csname v@sc/parakeet-tdt-v3/told/latin\endcsname{91}
\expandafter\def\csname v@sc/parakeet-tdt-v3/told/latin-wrong\endcsname{9}
\expandafter\def\csname v@sc/parakeet-tdt-v3/told/non\endcsname{13}
\expandafter\def\csname v@sc/parakeet-tdt-v3/told/non-wrong\endcsname{87}
\expandafter\def\csname v@sc/parakeet-tdt-v3/untouched/latin\endcsname{91}
\expandafter\def\csname v@sc/parakeet-tdt-v3/untouched/latin-wrong\endcsname{9}
\expandafter\def\csname v@sc/parakeet-tdt-v3/untouched/non\endcsname{13}
\expandafter\def\csname v@sc/parakeet-tdt-v3/untouched/non-wrong\endcsname{87}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/best/non\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/told/latin\endcsname{93}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/told/latin-wrong\endcsname{7}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/told/non\endcsname{31}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/told/non-wrong\endcsname{69}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/untouched/latin\endcsname{82}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/untouched/latin-wrong\endcsname{18}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/untouched/non\endcsname{27}
\expandafter\def\csname v@sc/qwen3-asr-0.6b/untouched/non-wrong\endcsname{73}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/best/latin\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/best/non\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/told/latin\endcsname{90}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/told/latin-wrong\endcsname{10}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/told/non\endcsname{30}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/told/non-wrong\endcsname{70}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/untouched/latin\endcsname{80}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/untouched/latin-wrong\endcsname{20}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/untouched/non\endcsname{23}
\expandafter\def\csname v@sc/qwen3-asr-1.7b/untouched/non-wrong\endcsname{77}
\expandafter\def\csname v@sc/untouched-max\endcsname{78}
\expandafter\def\csname v@sc/untouched-min\endcsname{0}
\expandafter\def\csname v@sc/voxtral-mini/best/latin\endcsname{100}
\expandafter\def\csname v@sc/voxtral-mini/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/voxtral-mini/best/non\endcsname{100}
\expandafter\def\csname v@sc/voxtral-mini/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/voxtral-mini/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/voxtral-mini/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/voxtral-mini/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/voxtral-mini/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/voxtral-mini/told/latin\endcsname{88}
\expandafter\def\csname v@sc/voxtral-mini/told/latin-wrong\endcsname{12}
\expandafter\def\csname v@sc/voxtral-mini/told/non\endcsname{35}
\expandafter\def\csname v@sc/voxtral-mini/told/non-wrong\endcsname{65}
\expandafter\def\csname v@sc/voxtral-mini/untouched/latin\endcsname{86}
\expandafter\def\csname v@sc/voxtral-mini/untouched/latin-wrong\endcsname{14}
\expandafter\def\csname v@sc/voxtral-mini/untouched/non\endcsname{22}
\expandafter\def\csname v@sc/voxtral-mini/untouched/non-wrong\endcsname{78}
\expandafter\def\csname v@sc/w2v-bert/best/latin\endcsname{100}
\expandafter\def\csname v@sc/w2v-bert/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/w2v-bert/best/non\endcsname{100}
\expandafter\def\csname v@sc/w2v-bert/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/w2v-bert/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/w2v-bert/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/w2v-bert/epoch1/non\endcsname{87}
\expandafter\def\csname v@sc/w2v-bert/epoch1/non-wrong\endcsname{13}
\expandafter\def\csname v@sc/w2v-bert/told/latin\endcsname{26}
\expandafter\def\csname v@sc/w2v-bert/told/latin-wrong\endcsname{74}
\expandafter\def\csname v@sc/w2v-bert/told/non\endcsname{6}
\expandafter\def\csname v@sc/w2v-bert/told/non-wrong\endcsname{94}
\expandafter\def\csname v@sc/whisper-large-v2/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v2/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v2/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v2/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v2/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v2/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v2/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v2/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v2/told/latin\endcsname{83}
\expandafter\def\csname v@sc/whisper-large-v2/told/latin-wrong\endcsname{17}
\expandafter\def\csname v@sc/whisper-large-v2/told/non\endcsname{17}
\expandafter\def\csname v@sc/whisper-large-v2/told/non-wrong\endcsname{83}
\expandafter\def\csname v@sc/whisper-large-v2/untouched/latin\endcsname{83}
\expandafter\def\csname v@sc/whisper-large-v2/untouched/latin-wrong\endcsname{17}
\expandafter\def\csname v@sc/whisper-large-v2/untouched/non\endcsname{30}
\expandafter\def\csname v@sc/whisper-large-v2/untouched/non-wrong\endcsname{70}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/told/latin\endcsname{97}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/told/latin-wrong\endcsname{3}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/told/non\endcsname{26}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/told/non-wrong\endcsname{74}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/untouched/latin\endcsname{88}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/untouched/latin-wrong\endcsname{12}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/untouched/non\endcsname{47}
\expandafter\def\csname v@sc/whisper-large-v3-turbo/untouched/non-wrong\endcsname{53}
\expandafter\def\csname v@sc/whisper-large-v3/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-large-v3/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-large-v3/told/latin\endcsname{98}
\expandafter\def\csname v@sc/whisper-large-v3/told/latin-wrong\endcsname{2}
\expandafter\def\csname v@sc/whisper-large-v3/told/non\endcsname{27}
\expandafter\def\csname v@sc/whisper-large-v3/told/non-wrong\endcsname{73}
\expandafter\def\csname v@sc/whisper-large-v3/untouched/latin\endcsname{82}
\expandafter\def\csname v@sc/whisper-large-v3/untouched/latin-wrong\endcsname{18}
\expandafter\def\csname v@sc/whisper-large-v3/untouched/non\endcsname{52}
\expandafter\def\csname v@sc/whisper-large-v3/untouched/non-wrong\endcsname{48}
\expandafter\def\csname v@sc/whisper-medium/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-medium/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-medium/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-medium/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-medium/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-medium/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-medium/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-medium/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-medium/told/latin\endcsname{67}
\expandafter\def\csname v@sc/whisper-medium/told/latin-wrong\endcsname{33}
\expandafter\def\csname v@sc/whisper-medium/told/non\endcsname{11}
\expandafter\def\csname v@sc/whisper-medium/told/non-wrong\endcsname{89}
\expandafter\def\csname v@sc/whisper-medium/untouched/latin\endcsname{75}
\expandafter\def\csname v@sc/whisper-medium/untouched/latin-wrong\endcsname{25}
\expandafter\def\csname v@sc/whisper-medium/untouched/non\endcsname{32}
\expandafter\def\csname v@sc/whisper-medium/untouched/non-wrong\endcsname{68}
\expandafter\def\csname v@sc/whisper-small/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-small/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-small/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-small/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-small/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-small/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-small/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-small/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-small/told/latin\endcsname{83}
\expandafter\def\csname v@sc/whisper-small/told/latin-wrong\endcsname{17}
\expandafter\def\csname v@sc/whisper-small/told/non\endcsname{9}
\expandafter\def\csname v@sc/whisper-small/told/non-wrong\endcsname{91}
\expandafter\def\csname v@sc/whisper-small/untouched/latin\endcsname{68}
\expandafter\def\csname v@sc/whisper-small/untouched/latin-wrong\endcsname{32}
\expandafter\def\csname v@sc/whisper-small/untouched/non\endcsname{27}
\expandafter\def\csname v@sc/whisper-small/untouched/non-wrong\endcsname{73}
\expandafter\def\csname v@sc/whisper-tiny/best/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-tiny/best/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-tiny/best/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-tiny/best/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-tiny/epoch1/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-tiny/epoch1/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-tiny/epoch1/non\endcsname{100}
\expandafter\def\csname v@sc/whisper-tiny/epoch1/non-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-tiny/told/latin\endcsname{100}
\expandafter\def\csname v@sc/whisper-tiny/told/latin-wrong\endcsname{0}
\expandafter\def\csname v@sc/whisper-tiny/told/non\endcsname{6}
\expandafter\def\csname v@sc/whisper-tiny/told/non-wrong\endcsname{94}
\expandafter\def\csname v@sc/whisper-tiny/untouched/latin\endcsname{84}
\expandafter\def\csname v@sc/whisper-tiny/untouched/latin-wrong\endcsname{16}
\expandafter\def\csname v@sc/whisper-tiny/untouched/non\endcsname{19}
\expandafter\def\csname v@sc/whisper-tiny/untouched/non-wrong\endcsname{81}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1\endcsname{43.5}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1/best\endcsname{43.5}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1/best-epoch\endcsname{1}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1/const\endcsname{39.5}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1/cost\endcsname{4.0}
\expandafter\def\csname v@sch/parakeet-tdt-v3/1/gain\endcsname{-4.0}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10\endcsname{23.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10/best\endcsname{23.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10/best-epoch\endcsname{10}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10/const\endcsname{21.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10/cost\endcsname{1.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/10/gain\endcsname{-1.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3\endcsname{34.3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3/best\endcsname{34.3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3/best-epoch\endcsname{3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3/const\endcsname{31.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3/cost\endcsname{2.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/3/gain\endcsname{-2.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5\endcsname{29.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5/best\endcsname{29.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5/best-epoch\endcsname{5}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5/const\endcsname{25.3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5/cost\endcsname{4.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/5/gain\endcsname{-4.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const-best\endcsname{21.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const-best-epoch\endcsname{10}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const1\endcsname{39.5}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const10\endcsname{21.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const3\endcsname{31.7}
\expandafter\def\csname v@sch/parakeet-tdt-v3/const5\endcsname{25.3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain-max3\endcsname{-1.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain-min3\endcsname{-4.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain1\endcsname{-4.0}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain10\endcsname{-1.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain3\endcsname{-2.6}
\expandafter\def\csname v@sch/parakeet-tdt-v3/gain5\endcsname{-4.4}
\expandafter\def\csname v@sch/parakeet-tdt-v3/n3\endcsname{3}
\expandafter\def\csname v@sch/parakeet-tdt-v3/ten-gain\endcsname{6.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1\endcsname{21.0}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1/best\endcsname{21.0}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1/best-epoch\endcsname{1}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1/const\endcsname{22.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1/cost\endcsname{-1.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/1/gain\endcsname{1.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10\endcsname{17.4}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10/best\endcsname{17.5}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10/best-epoch\endcsname{8}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10/const\endcsname{18.2}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10/cost\endcsname{-0.7}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/10/gain\endcsname{0.7}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3\endcsname{17.6}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3/best\endcsname{17.6}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3/best-epoch\endcsname{3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3/const\endcsname{18.7}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3/cost\endcsname{-1.1}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/3/gain\endcsname{1.1}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5\endcsname{17.8}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5/best\endcsname{17.5}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5/best-epoch\endcsname{4}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5/const\endcsname{18.2}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5/cost\endcsname{-0.6}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/5/gain\endcsname{0.6}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const-best\endcsname{18.2}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const-best-epoch\endcsname{4}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const1\endcsname{22.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const10\endcsname{18.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const3\endcsname{18.7}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/const5\endcsname{18.2}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain-max3\endcsname{1.1}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain-min3\endcsname{0.6}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain1\endcsname{1.3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain10\endcsname{0.9}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain3\endcsname{1.1}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/gain5\endcsname{0.4}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/n3\endcsname{3}
\expandafter\def\csname v@sch/qwen3-asr-0.6b/ten-gain\endcsname{0.0}
\expandafter\def\csname v@sch/w2v-bert/1\endcsname{41.6}
\expandafter\def\csname v@sch/w2v-bert/1/best\endcsname{41.6}
\expandafter\def\csname v@sch/w2v-bert/1/best-epoch\endcsname{1}
\expandafter\def\csname v@sch/w2v-bert/1/const\endcsname{26.6}
\expandafter\def\csname v@sch/w2v-bert/1/cost\endcsname{15.0}
\expandafter\def\csname v@sch/w2v-bert/1/gain\endcsname{-15.0}
\expandafter\def\csname v@sch/w2v-bert/10\endcsname{12.6}
\expandafter\def\csname v@sch/w2v-bert/10/best\endcsname{12.6}
\expandafter\def\csname v@sch/w2v-bert/10/best-epoch\endcsname{10}
\expandafter\def\csname v@sch/w2v-bert/10/const\endcsname{12.7}
\expandafter\def\csname v@sch/w2v-bert/10/cost\endcsname{-0.1}
\expandafter\def\csname v@sch/w2v-bert/10/gain\endcsname{0.1}
\expandafter\def\csname v@sch/w2v-bert/3\endcsname{18.3}
\expandafter\def\csname v@sch/w2v-bert/3/best\endcsname{18.3}
\expandafter\def\csname v@sch/w2v-bert/3/best-epoch\endcsname{3}
\expandafter\def\csname v@sch/w2v-bert/3/const\endcsname{16.5}
\expandafter\def\csname v@sch/w2v-bert/3/cost\endcsname{1.9}
\expandafter\def\csname v@sch/w2v-bert/3/gain\endcsname{-1.9}
\expandafter\def\csname v@sch/w2v-bert/5\endcsname{15.5}
\expandafter\def\csname v@sch/w2v-bert/5/best\endcsname{15.5}
\expandafter\def\csname v@sch/w2v-bert/5/best-epoch\endcsname{5}
\expandafter\def\csname v@sch/w2v-bert/5/const\endcsname{14.6}
\expandafter\def\csname v@sch/w2v-bert/5/cost\endcsname{0.9}
\expandafter\def\csname v@sch/w2v-bert/5/gain\endcsname{-0.9}
\expandafter\def\csname v@sch/w2v-bert/const-best\endcsname{12.7}
\expandafter\def\csname v@sch/w2v-bert/const-best-epoch\endcsname{9}
\expandafter\def\csname v@sch/w2v-bert/const1\endcsname{26.6}
\expandafter\def\csname v@sch/w2v-bert/const10\endcsname{12.7}
\expandafter\def\csname v@sch/w2v-bert/const3\endcsname{16.5}
\expandafter\def\csname v@sch/w2v-bert/const5\endcsname{14.6}
\expandafter\def\csname v@sch/w2v-bert/gain-max3\endcsname{0.1}
\expandafter\def\csname v@sch/w2v-bert/gain-min3\endcsname{-1.9}
\expandafter\def\csname v@sch/w2v-bert/gain1\endcsname{-15.0}
\expandafter\def\csname v@sch/w2v-bert/gain10\endcsname{0.1}
\expandafter\def\csname v@sch/w2v-bert/gain3\endcsname{-1.9}
\expandafter\def\csname v@sch/w2v-bert/gain5\endcsname{-0.9}
\expandafter\def\csname v@sch/w2v-bert/n3\endcsname{3}
\expandafter\def\csname v@sch/w2v-bert/ten-gain\endcsname{2.9}
\expandafter\def\csname v@sch/whisper-small/1\endcsname{23.5}
\expandafter\def\csname v@sch/whisper-small/1/best\endcsname{23.5}
\expandafter\def\csname v@sch/whisper-small/1/best-epoch\endcsname{1}
\expandafter\def\csname v@sch/whisper-small/1/const\endcsname{22.2}
\expandafter\def\csname v@sch/whisper-small/1/cost\endcsname{1.3}
\expandafter\def\csname v@sch/whisper-small/1/gain\endcsname{-1.3}
\expandafter\def\csname v@sch/whisper-small/10\endcsname{15.9}
\expandafter\def\csname v@sch/whisper-small/10/best\endcsname{16.0}
\expandafter\def\csname v@sch/whisper-small/10/best-epoch\endcsname{9}
\expandafter\def\csname v@sch/whisper-small/10/const\endcsname{16.9}
\expandafter\def\csname v@sch/whisper-small/10/cost\endcsname{-0.9}
\expandafter\def\csname v@sch/whisper-small/10/gain\endcsname{0.9}
\expandafter\def\csname v@sch/whisper-small/3\endcsname{17.2}
\expandafter\def\csname v@sch/whisper-small/3/best\endcsname{17.2}
\expandafter\def\csname v@sch/whisper-small/3/best-epoch\endcsname{3}
\expandafter\def\csname v@sch/whisper-small/3/const\endcsname{17.6}
\expandafter\def\csname v@sch/whisper-small/3/cost\endcsname{-0.4}
\expandafter\def\csname v@sch/whisper-small/3/gain\endcsname{0.4}
\expandafter\def\csname v@sch/whisper-small/5\endcsname{16.7}
\expandafter\def\csname v@sch/whisper-small/5/best\endcsname{16.7}
\expandafter\def\csname v@sch/whisper-small/5/best-epoch\endcsname{4}
\expandafter\def\csname v@sch/whisper-small/5/const\endcsname{16.9}
\expandafter\def\csname v@sch/whisper-small/5/cost\endcsname{-0.2}
\expandafter\def\csname v@sch/whisper-small/5/gain\endcsname{0.2}
\expandafter\def\csname v@sch/whisper-small/const-best\endcsname{16.9}
\expandafter\def\csname v@sch/whisper-small/const-best-epoch\endcsname{9}
\expandafter\def\csname v@sch/whisper-small/const1\endcsname{22.2}
\expandafter\def\csname v@sch/whisper-small/const10\endcsname{17.4}
\expandafter\def\csname v@sch/whisper-small/const3\endcsname{17.6}
\expandafter\def\csname v@sch/whisper-small/const5\endcsname{16.9}
\expandafter\def\csname v@sch/whisper-small/gain-max3\endcsname{0.9}
\expandafter\def\csname v@sch/whisper-small/gain-min3\endcsname{0.2}
\expandafter\def\csname v@sch/whisper-small/gain1\endcsname{-1.3}
\expandafter\def\csname v@sch/whisper-small/gain10\endcsname{1.5}
\expandafter\def\csname v@sch/whisper-small/gain3\endcsname{0.4}
\expandafter\def\csname v@sch/whisper-small/gain5\endcsname{0.2}
\expandafter\def\csname v@sch/whisper-small/n3\endcsname{3}
\expandafter\def\csname v@sch/whisper-small/ten-gain\endcsname{0.7}
\expandafter\def\csname v@scr/gap-max\endcsname{77}
\expandafter\def\csname v@scr/gap-min\endcsname{60}
\expandafter\def\csname v@scr/parakeet-tdt-v3/cer\endcsname{98.7}
\expandafter\def\csname v@scr/parakeet-tdt-v3/dev\endcsname{98.9}
\expandafter\def\csname v@scr/parakeet-tdt-v3/done\endcsname{8}
\expandafter\def\csname v@scr/parakeet-tdt-v3/epoch\endcsname{8}
\expandafter\def\csname v@scr/parakeet-tdt-v3/gap\endcsname{76.9}
\expandafter\def\csname v@scr/parakeet-tdt-v3/last-cer\endcsname{98.7}
\expandafter\def\csname v@scr/parakeet-tdt-v3/loop\endcsname{1,145}
\expandafter\def\csname v@scr/parakeet-tdt-v3/pre\endcsname{21.7}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/cer\endcsname{78.1}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/dev\endcsname{79.3}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/done\endcsname{20}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/epoch\endcsname{2}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/gap\endcsname{60.0}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/last-cer\endcsname{80.4}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/loop\endcsname{2}
\expandafter\def\csname v@scr/qwen3-asr-0.6b/pre\endcsname{18.2}
\expandafter\def\csname v@scr/w2v-bert/cer\endcsname{88.9}
\expandafter\def\csname v@scr/w2v-bert/dev\endcsname{88.3}
\expandafter\def\csname v@scr/w2v-bert/done\endcsname{20}
\expandafter\def\csname v@scr/w2v-bert/epoch\endcsname{11}
\expandafter\def\csname v@scr/w2v-bert/gap\endcsname{76.2}
\expandafter\def\csname v@scr/w2v-bert/last-cer\endcsname{92.4}
\expandafter\def\csname v@scr/w2v-bert/loop\endcsname{318}
\expandafter\def\csname v@scr/w2v-bert/pre\endcsname{12.7}
\expandafter\def\csname v@scr/whisper-small/cer\endcsname{77.2}
\expandafter\def\csname v@scr/whisper-small/dev\endcsname{78.8}
\expandafter\def\csname v@scr/whisper-small/done\endcsname{20}
\expandafter\def\csname v@scr/whisper-small/epoch\endcsname{5}
\expandafter\def\csname v@scr/whisper-small/gap\endcsname{60.3}
\expandafter\def\csname v@scr/whisper-small/last-cer\endcsname{79.3}
\expandafter\def\csname v@scr/whisper-small/loop\endcsname{0}
\expandafter\def\csname v@scr/whisper-small/pre\endcsname{16.9}
\expandafter\def\csname v@seed/parakeet-tdt-v3/1/diff\endcsname{0.6}
\expandafter\def\csname v@seed/parakeet-tdt-v3/10/diff\endcsname{0.2}
\expandafter\def\csname v@seed/parakeet-tdt-v3/3/diff\endcsname{3.7}
\expandafter\def\csname v@seed/parakeet-tdt-v3/5/diff\endcsname{0.1}
\expandafter\def\csname v@seed/parakeet-tdt-v3/diff\endcsname{0.2}
\expandafter\def\csname v@seed/parakeet-tdt-v3/diff-max3\endcsname{3.7}
\expandafter\def\csname v@seed/parakeet-tdt-v3/one\endcsname{21.7}
\expandafter\def\csname v@seed/parakeet-tdt-v3/one-epoch\endcsname{10}
\expandafter\def\csname v@seed/parakeet-tdt-v3/two\endcsname{21.5}
\expandafter\def\csname v@seed/parakeet-tdt-v3/two-epoch\endcsname{10}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/1/diff\endcsname{1.1}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/10/diff\endcsname{0.1}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/3/diff\endcsname{0.5}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/5/diff\endcsname{0.1}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/diff\endcsname{0.1}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/diff-max3\endcsname{0.5}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/one\endcsname{18.2}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/one-epoch\endcsname{4}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/two\endcsname{18.2}
\expandafter\def\csname v@seed/qwen3-asr-0.6b/two-epoch\endcsname{3}
\expandafter\def\csname v@seed/whisper-small/1/diff\endcsname{0.6}
\expandafter\def\csname v@seed/whisper-small/10/diff\endcsname{0.1}
\expandafter\def\csname v@seed/whisper-small/3/diff\endcsname{0.0}
\expandafter\def\csname v@seed/whisper-small/5/diff\endcsname{0.4}
\expandafter\def\csname v@seed/whisper-small/diff\endcsname{0.1}
\expandafter\def\csname v@seed/whisper-small/diff-max3\endcsname{0.4}
\expandafter\def\csname v@seed/whisper-small/one\endcsname{16.9}
\expandafter\def\csname v@seed/whisper-small/one-epoch\endcsname{9}
\expandafter\def\csname v@seed/whisper-small/two\endcsname{17.0}
\expandafter\def\csname v@seed/whisper-small/two-epoch\endcsname{9}
\expandafter\def\csname v@seed1/mms-1b/cer\endcsname{11.3}
\expandafter\def\csname v@seed1/mms-1b/main\endcsname{11.0}
\expandafter\def\csname v@seed1/omni-ctc-1b/cer\endcsname{11.6}
\expandafter\def\csname v@seed1/omni-ctc-1b/main\endcsname{12.0}
\expandafter\def\csname v@seed1/qwen3-asr-0.6b/cer\endcsname{18.2}
\expandafter\def\csname v@seed1/qwen3-asr-0.6b/main\endcsname{18.2}
\expandafter\def\csname v@seed1/w2v-bert/cer\endcsname{12.8}
\expandafter\def\csname v@seed1/w2v-bert/main\endcsname{12.7}
\expandafter\def\csname v@seed1/whisper-small/cer\endcsname{17.2}
\expandafter\def\csname v@seed1/whisper-small/main\endcsname{16.9}
\expandafter\def\csname v@seed2/mms-1b/cer\endcsname{11.1}
\expandafter\def\csname v@seed2/mms-1b/dev\endcsname{18.6}
\expandafter\def\csname v@seed2/mms-1b/epoch\endcsname{10}
\expandafter\def\csname v@seed2/omni-ctc-1b/cer\endcsname{11.7}
\expandafter\def\csname v@seed2/omni-ctc-1b/dev\endcsname{19.4}
\expandafter\def\csname v@seed2/omni-ctc-1b/epoch\endcsname{10}
\expandafter\def\csname v@seed2/parakeet-tdt-v3/cer\endcsname{21.5}
\expandafter\def\csname v@seed2/parakeet-tdt-v3/dev\endcsname{27.6}
\expandafter\def\csname v@seed2/parakeet-tdt-v3/epoch\endcsname{10}
\expandafter\def\csname v@seed2/qwen3-asr-0.6b/cer\endcsname{18.2}
\expandafter\def\csname v@seed2/qwen3-asr-0.6b/dev\endcsname{25.3}
\expandafter\def\csname v@seed2/qwen3-asr-0.6b/epoch\endcsname{3}
\expandafter\def\csname v@seed2/w2v-bert/cer\endcsname{12.4}
\expandafter\def\csname v@seed2/w2v-bert/dev\endcsname{19.7}
\expandafter\def\csname v@seed2/w2v-bert/epoch\endcsname{10}
\expandafter\def\csname v@seed2/whisper-small/cer\endcsname{17.0}
\expandafter\def\csname v@seed2/whisper-small/dev\endcsname{24.9}
\expandafter\def\csname v@seed2/whisper-small/epoch\endcsname{9}
\expandafter\def\csname v@seedall/max-diff\endcsname{0.4}
\expandafter\def\csname v@seedall/n-draws\endcsname{10}
\expandafter\def\csname v@seedall/n-models\endcsname{5}
\expandafter\def\csname v@seeds/mms-1b/max\endcsname{11.3}
\expandafter\def\csname v@seeds/mms-1b/mean\endcsname{11.2}
\expandafter\def\csname v@seeds/mms-1b/min\endcsname{11.0}
\expandafter\def\csname v@seeds/mms-1b/n\endcsname{3}
\expandafter\def\csname v@seeds/omni-ctc-1b/max\endcsname{12.0}
\expandafter\def\csname v@seeds/omni-ctc-1b/mean\endcsname{11.8}
\expandafter\def\csname v@seeds/omni-ctc-1b/min\endcsname{11.6}
\expandafter\def\csname v@seeds/omni-ctc-1b/n\endcsname{3}
\expandafter\def\csname v@seeds/w2v-bert/max\endcsname{12.8}
\expandafter\def\csname v@seeds/w2v-bert/mean\endcsname{12.6}
\expandafter\def\csname v@seeds/w2v-bert/min\endcsname{12.4}
\expandafter\def\csname v@seeds/w2v-bert/n\endcsname{3}
\expandafter\def\csname v@size/7b-vs-main\endcsname{1.5}
\expandafter\def\csname v@size/7b-vs-main-ci\endcsname{1.2 to 1.7}
\expandafter\def\csname v@size/7b-vs-main-name\endcsname{MMS 1B}
\expandafter\def\csname v@size/dev-gap/omni-1b-7b\endcsname{3.0}
\expandafter\def\csname v@size/dev-gap/omni-300m-1b\endcsname{1.8}
\expandafter\def\csname v@size/gemma/behind\endcsname{3.3}
\expandafter\def\csname v@size/gemma4-12b/after\endcsname{19.8}
\expandafter\def\csname v@size/gemma4-12b/before\endcsname{72.9}
\expandafter\def\csname v@size/gemma4-12b/ci\endcsname{19.1--20.6}
\expandafter\def\csname v@size/gemma4-12b/lr\endcsname{3e-6}
\expandafter\def\csname v@size/gemma4-e2b/after\endcsname{18.5}
\expandafter\def\csname v@size/gemma4-e2b/before\endcsname{43.5}
\expandafter\def\csname v@size/gemma4-e2b/ci\endcsname{17.8--19.4}
\expandafter\def\csname v@size/gemma4-e2b/lr\endcsname{1e-5}
\expandafter\def\csname v@size/gemma4-e4b/after\endcsname{16.6}
\expandafter\def\csname v@size/gemma4-e4b/before\endcsname{39.8}
\expandafter\def\csname v@size/gemma4-e4b/ci\endcsname{16.0--17.3}
\expandafter\def\csname v@size/gemma4-e4b/lr\endcsname{3e-6}
\expandafter\def\csname v@size/omni-7b-done\endcsname{1}
\expandafter\def\csname v@size/omni-ctc-1b/after\endcsname{12.0}
\expandafter\def\csname v@size/omni-ctc-1b/at-e7\endcsname{12.0}
\expandafter\def\csname v@size/omni-ctc-1b/at-e7-epoch\endcsname{7}
\expandafter\def\csname v@size/omni-ctc-1b/before\endcsname{28.5}
\expandafter\def\csname v@size/omni-ctc-1b/ci\endcsname{11.5--12.6}
\expandafter\def\csname v@size/omni-ctc-1b/lr\endcsname{3e-5}
\expandafter\def\csname v@size/omni-ctc-300m/after\endcsname{13.3}
\expandafter\def\csname v@size/omni-ctc-300m/at-e7\endcsname{13.3}
\expandafter\def\csname v@size/omni-ctc-300m/at-e7-epoch\endcsname{8}
\expandafter\def\csname v@size/omni-ctc-300m/before\endcsname{31.5}
\expandafter\def\csname v@size/omni-ctc-300m/ci\endcsname{12.9--13.9}
\expandafter\def\csname v@size/omni-ctc-300m/lr\endcsname{3e-5}
\expandafter\def\csname v@size/omni-ctc-7b/after\endcsname{9.5}
\expandafter\def\csname v@size/omni-ctc-7b/at-e7\endcsname{9.5}
\expandafter\def\csname v@size/omni-ctc-7b/at-e7-epoch\endcsname{10}
\expandafter\def\csname v@size/omni-ctc-7b/before\endcsname{29.7}
\expandafter\def\csname v@size/omni-ctc-7b/ci\endcsname{9.1--10.2}
\expandafter\def\csname v@size/omni-ctc-7b/lr\endcsname{1e-5}
\expandafter\def\csname v@size/omni-ctc-7b/wer\endcsname{35.2}
\expandafter\def\csname v@size/omni-epochs\endcsname{10}
\expandafter\def\csname v@size/omni-epochs-phrase\endcsname{ten epochs}
\expandafter\def\csname v@size/qwen3-asr-0.6b/after\endcsname{18.2}
\expandafter\def\csname v@size/qwen3-asr-0.6b/before\endcsname{60.9}
\expandafter\def\csname v@size/qwen3-asr-0.6b/ci\endcsname{17.5--18.9}
\expandafter\def\csname v@size/qwen3-asr-0.6b/lr\endcsname{1e-5}
\expandafter\def\csname v@size/qwen3-asr-1.7b/after\endcsname{16.6}
\expandafter\def\csname v@size/qwen3-asr-1.7b/before\endcsname{59.3}
\expandafter\def\csname v@size/qwen3-asr-1.7b/ci\endcsname{16.0--17.3}
\expandafter\def\csname v@size/qwen3-asr-1.7b/lr\endcsname{1e-5}
\expandafter\def\csname v@size/step/omni-1b-7b\endcsname{2.4}
\expandafter\def\csname v@size/step/omni-1b-7b-ci\endcsname{2.2 to 2.7}
\expandafter\def\csname v@size/step/omni-300m-1b\endcsname{1.3}
\expandafter\def\csname v@size/step/omni-300m-1b-ci\endcsname{1.1 to 1.5}
\expandafter\def\csname v@size/step/qwen\endcsname{1.6}
\expandafter\def\csname v@size/step/qwen-ci\endcsname{1.1 to 2.1}
\expandafter\def\csname v@size/step/whisper-small-large\endcsname{3.4}
\expandafter\def\csname v@size/step/whisper-small-large-ci\endcsname{3.0 to 3.7}
\expandafter\def\csname v@size/step/whisper-tiny-large\endcsname{12.2}
\expandafter\def\csname v@size/step/whisper-tiny-large-ci\endcsname{11.5 to 12.8}
\expandafter\def\csname v@size/step/whisper-tiny-small\endcsname{8.8}
\expandafter\def\csname v@size/step/whisper-tiny-small-ci\endcsname{8.2 to 9.4}
\expandafter\def\csname v@size/sweep-gap/omni-1b-7b\endcsname{3.7}
\expandafter\def\csname v@size/sweep-gap/omni-300m-1b\endcsname{3.7}
\expandafter\def\csname v@size/whisper-base/after\endcsname{22.5}
\expandafter\def\csname v@size/whisper-base/before\endcsname{62.7}
\expandafter\def\csname v@size/whisper-base/ci\endcsname{21.8--23.5}
\expandafter\def\csname v@size/whisper-base/lr\endcsname{1e-4}
\expandafter\def\csname v@size/whisper-large-v3/after\endcsname{13.5}
\expandafter\def\csname v@size/whisper-large-v3/before\endcsname{50.3}
\expandafter\def\csname v@size/whisper-large-v3/ci\endcsname{13.0--14.2}
\expandafter\def\csname v@size/whisper-large-v3/lr\endcsname{1e-5}
\expandafter\def\csname v@size/whisper-medium/after\endcsname{14.8}
\expandafter\def\csname v@size/whisper-medium/before\endcsname{63.7}
\expandafter\def\csname v@size/whisper-medium/ci\endcsname{14.2--15.5}
\expandafter\def\csname v@size/whisper-medium/lr\endcsname{1e-5}
\expandafter\def\csname v@size/whisper-small/after\endcsname{16.9}
\expandafter\def\csname v@size/whisper-small/before\endcsname{65.7}
\expandafter\def\csname v@size/whisper-small/ci\endcsname{16.4--17.6}
\expandafter\def\csname v@size/whisper-small/lr\endcsname{3e-5}
\expandafter\def\csname v@size/whisper-tiny/after\endcsname{25.7}
\expandafter\def\csname v@size/whisper-tiny/before\endcsname{66.6}
\expandafter\def\csname v@size/whisper-tiny/ci\endcsname{24.9--26.5}
\expandafter\def\csname v@size/whisper-tiny/lr\endcsname{1e-4}
\expandafter\def\csname v@sl/alone\endcsname{15.3}
\expandafter\def\csname v@sl/alone-last\endcsname{15.9}
\expandafter\def\csname v@sl/better-joint\endcsname{8}
\expandafter\def\csname v@sl/better-joint-last\endcsname{8}
\expandafter\def\csname v@sl/diff\endcsname{2.8}
\expandafter\def\csname v@sl/joint\endcsname{18.2}
\expandafter\def\csname v@sl/joint-last\endcsname{18.3}
\expandafter\def\csname v@sl/n\endcsname{50}
\expandafter\def\csname v@sl/n-last\endcsname{50}
\expandafter\def\csname v@sl/scarce-alone\endcsname{15.8}
\expandafter\def\csname v@sl/scarce-better-joint\endcsname{1}
\expandafter\def\csname v@sl/scarce-joint\endcsname{18.5}
\expandafter\def\csname v@sl/scarce-n\endcsname{7}
\expandafter\def\csname v@sr/n\endcsname{1,250}
\expandafter\def\csname v@sr/nemotron-stream/flawed-cer\endcsname{35.9}
\expandafter\def\csname v@sr/nemotron-stream/flawed-e0\endcsname{86.2}
\expandafter\def\csname v@sr/nemotron-stream/flawed-identical\endcsname{35}
\expandafter\def\csname v@sr/nemotron-stream/flawed-wer\endcsname{78.2}
\expandafter\def\csname v@sr/nemotron-stream/gain\endcsname{0.0}
\expandafter\def\csname v@sr/nemotron-stream/identical\endcsname{1,250}
\expandafter\def\csname v@sr/nemotron-stream/stuck\endcsname{1,149}
\expandafter\def\csname v@sr/parakeet-tdt-v3/flawed-cer\endcsname{25.6}
\expandafter\def\csname v@sr/parakeet-tdt-v3/flawed-e0\endcsname{65.2}
\expandafter\def\csname v@sr/parakeet-tdt-v3/flawed-identical\endcsname{794}
\expandafter\def\csname v@sr/parakeet-tdt-v3/flawed-wer\endcsname{56.1}
\expandafter\def\csname v@sr/parakeet-tdt-v3/gain\endcsname{3.8}
\expandafter\def\csname v@sr/parakeet-tdt-v3/identical\endcsname{1,208}
\expandafter\def\csname v@sr/parakeet-tdt-v3/stuck\endcsname{221}
\expandafter\def\csname v@stall/stall_sch10_w2v-bert/cer\endcsname{99.1}
\expandafter\def\csname v@stall/stall_sch10_w2v-bert/epochs\endcsname{3}
\expandafter\def\csname v@stall/stall_sch10_w2v-bert/last\endcsname{99.1}
\expandafter\def\csname v@stall/stall_sch10_w2v-bert/stuck\endcsname{3}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/best\endcsname{12.6}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/best-epoch\endcsname{10}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/cer\endcsname{30.9}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/epochs\endcsname{10}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/last\endcsname{12.6}
\expandafter\def\csname v@stall/stallrep_sch10_w2v-bert/stuck\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/first/cer\endcsname{35.9}
\expandafter\def\csname v@start/nemotron-stream/first/dev\endcsname{41.4}
\expandafter\def\csname v@start/nemotron-stream/first/done\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/first/e0\endcsname{86.2}
\expandafter\def\csname v@start/nemotron-stream/first/e1\endcsname{45.7}
\expandafter\def\csname v@start/nemotron-stream/first/epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/first/last\endcsname{35.9}
\expandafter\def\csname v@start/nemotron-stream/first/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/first/latin-e1\endcsname{39.7}
\expandafter\def\csname v@start/nemotron-stream/first/latin-e2\endcsname{42.5}
\expandafter\def\csname v@start/nemotron-stream/first/len/best/empty\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/first/len/best/latin\endcsname{93}
\expandafter\def\csname v@start/nemotron-stream/first/len/best/other\endcsname{88}
\expandafter\def\csname v@start/nemotron-stream/first/len/e0/empty\endcsname{260}
\expandafter\def\csname v@start/nemotron-stream/first/len/e0/latin\endcsname{37}
\expandafter\def\csname v@start/nemotron-stream/first/len/e0/other\endcsname{50}
\expandafter\def\csname v@start/nemotron-stream/first/len/e1/empty\endcsname{20}
\expandafter\def\csname v@start/nemotron-stream/first/len/e1/latin\endcsname{74}
\expandafter\def\csname v@start/nemotron-stream/first/len/e1/other\endcsname{101}
\expandafter\def\csname v@start/nemotron-stream/first/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/first/len/last/empty\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/first/len/last/latin\endcsname{93}
\expandafter\def\csname v@start/nemotron-stream/first/len/last/other\endcsname{88}
\expandafter\def\csname v@start/nemotron-stream/first/other-e1\endcsname{61.2}
\expandafter\def\csname v@start/nemotron-stream/first/other-e2\endcsname{53.9}
\expandafter\def\csname v@start/nemotron-stream/five/cer\endcsname{54.8}
\expandafter\def\csname v@start/nemotron-stream/five/dev\endcsname{59.2}
\expandafter\def\csname v@start/nemotron-stream/five/done\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/five/e0\endcsname{68.7}
\expandafter\def\csname v@start/nemotron-stream/five/e1\endcsname{68.0}
\expandafter\def\csname v@start/nemotron-stream/five/epoch\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/five/last\endcsname{54.8}
\expandafter\def\csname v@start/nemotron-stream/five/last-epoch\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/five/latin-e1\endcsname{63.6}
\expandafter\def\csname v@start/nemotron-stream/five/latin-e2\endcsname{50.5}
\expandafter\def\csname v@start/nemotron-stream/five/len/best/empty\endcsname{62}
\expandafter\def\csname v@start/nemotron-stream/five/len/best/latin\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/five/len/best/other\endcsname{51}
\expandafter\def\csname v@start/nemotron-stream/five/len/e0/empty\endcsname{120}
\expandafter\def\csname v@start/nemotron-stream/five/len/e0/latin\endcsname{70}
\expandafter\def\csname v@start/nemotron-stream/five/len/e0/other\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/five/len/e1/empty\endcsname{160}
\expandafter\def\csname v@start/nemotron-stream/five/len/e1/latin\endcsname{50}
\expandafter\def\csname v@start/nemotron-stream/five/len/e1/other\endcsname{29}
\expandafter\def\csname v@start/nemotron-stream/five/len/last-epoch\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/five/len/last/empty\endcsname{62}
\expandafter\def\csname v@start/nemotron-stream/five/len/last/latin\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/five/len/last/other\endcsname{51}
\expandafter\def\csname v@start/nemotron-stream/five/other-e1\endcsname{79.3}
\expandafter\def\csname v@start/nemotron-stream/five/other-e2\endcsname{65.7}
\expandafter\def\csname v@start/nemotron-stream/hi/cer\endcsname{99.0}
\expandafter\def\csname v@start/nemotron-stream/hi/dev\endcsname{99.1}
\expandafter\def\csname v@start/nemotron-stream/hi/done\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/hi/e0\endcsname{68.7}
\expandafter\def\csname v@start/nemotron-stream/hi/e1\endcsname{99.0}
\expandafter\def\csname v@start/nemotron-stream/hi/epoch\endcsname{1}
\expandafter\def\csname v@start/nemotron-stream/hi/last\endcsname{99.9}
\expandafter\def\csname v@start/nemotron-stream/hi/last-epoch\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/hi/latin-e1\endcsname{98.7}
\expandafter\def\csname v@start/nemotron-stream/hi/latin-e2\endcsname{99.9}
\expandafter\def\csname v@start/nemotron-stream/hi/len/best/empty\endcsname{710}
\expandafter\def\csname v@start/nemotron-stream/hi/len/best/latin\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/hi/len/best/other\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e0/empty\endcsname{120}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e0/latin\endcsname{70}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e0/other\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e1/empty\endcsname{710}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e1/latin\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/hi/len/e1/other\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/hi/len/last-epoch\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/hi/len/last/empty\endcsname{1,225}
\expandafter\def\csname v@start/nemotron-stream/hi/len/last/latin\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/hi/len/last/other\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/hi/other-e1\endcsname{99.9}
\expandafter\def\csname v@start/nemotron-stream/hi/other-e2\endcsname{100.0}
\expandafter\def\csname v@start/nemotron-stream/mean/cer\endcsname{42.8}
\expandafter\def\csname v@start/nemotron-stream/mean/dev\endcsname{48.5}
\expandafter\def\csname v@start/nemotron-stream/mean/done\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/mean/e0\endcsname{68.7}
\expandafter\def\csname v@start/nemotron-stream/mean/e1\endcsname{66.2}
\expandafter\def\csname v@start/nemotron-stream/mean/epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/mean/last\endcsname{42.8}
\expandafter\def\csname v@start/nemotron-stream/mean/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/mean/latin-e1\endcsname{59.4}
\expandafter\def\csname v@start/nemotron-stream/mean/latin-e2\endcsname{54.9}
\expandafter\def\csname v@start/nemotron-stream/mean/len/best/empty\endcsname{21}
\expandafter\def\csname v@start/nemotron-stream/mean/len/best/latin\endcsname{91}
\expandafter\def\csname v@start/nemotron-stream/mean/len/best/other\endcsname{77}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e0/empty\endcsname{120}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e0/latin\endcsname{70}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e0/other\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e1/empty\endcsname{2}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e1/latin\endcsname{51}
\expandafter\def\csname v@start/nemotron-stream/mean/len/e1/other\endcsname{57}
\expandafter\def\csname v@start/nemotron-stream/mean/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/mean/len/last/empty\endcsname{21}
\expandafter\def\csname v@start/nemotron-stream/mean/len/last/latin\endcsname{91}
\expandafter\def\csname v@start/nemotron-stream/mean/len/last/other\endcsname{77}
\expandafter\def\csname v@start/nemotron-stream/mean/other-e1\endcsname{83.8}
\expandafter\def\csname v@start/nemotron-stream/mean/other-e2\endcsname{71.7}
\expandafter\def\csname v@start/nemotron-stream/ten/cer\endcsname{48.2}
\expandafter\def\csname v@start/nemotron-stream/ten/dev\endcsname{52.5}
\expandafter\def\csname v@start/nemotron-stream/ten/done\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/ten/e0\endcsname{68.7}
\expandafter\def\csname v@start/nemotron-stream/ten/e1\endcsname{66.3}
\expandafter\def\csname v@start/nemotron-stream/ten/epoch\endcsname{6}
\expandafter\def\csname v@start/nemotron-stream/ten/last\endcsname{53.2}
\expandafter\def\csname v@start/nemotron-stream/ten/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/ten/latin-e1\endcsname{61.7}
\expandafter\def\csname v@start/nemotron-stream/ten/latin-e2\endcsname{52.3}
\expandafter\def\csname v@start/nemotron-stream/ten/len/best/empty\endcsname{5}
\expandafter\def\csname v@start/nemotron-stream/ten/len/best/latin\endcsname{80}
\expandafter\def\csname v@start/nemotron-stream/ten/len/best/other\endcsname{62}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e0/empty\endcsname{120}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e0/latin\endcsname{70}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e0/other\endcsname{73}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e1/empty\endcsname{174}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e1/latin\endcsname{50}
\expandafter\def\csname v@start/nemotron-stream/ten/len/e1/other\endcsname{30}
\expandafter\def\csname v@start/nemotron-stream/ten/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/nemotron-stream/ten/len/last/empty\endcsname{0}
\expandafter\def\csname v@start/nemotron-stream/ten/len/last/latin\endcsname{83}
\expandafter\def\csname v@start/nemotron-stream/ten/len/last/other\endcsname{64}
\expandafter\def\csname v@start/nemotron-stream/ten/other-e1\endcsname{78.3}
\expandafter\def\csname v@start/nemotron-stream/ten/other-e2\endcsname{73.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/cer\endcsname{25.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/dev\endcsname{31.1}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/done\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/e0\endcsname{65.2}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/e1\endcsname{43.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/last\endcsname{25.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/latin-e1\endcsname{29.5}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/latin-e2\endcsname{24.2}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/best/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/best/latin\endcsname{96}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/best/other\endcsname{100}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e0/empty\endcsname{144}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e0/latin\endcsname{67}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e0/other\endcsname{85}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e1/empty\endcsname{5}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e1/latin\endcsname{127}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/e1/other\endcsname{628}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/last/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/last/latin\endcsname{96}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/len/last/other\endcsname{100}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/other-e1\endcsname{78.9}
\expandafter\def\csname v@start/parakeet-tdt-v3/first/other-e2\endcsname{76.0}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/cer\endcsname{21.0}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/dev\endcsname{27.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/done\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/e0\endcsname{55.8}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/e1\endcsname{35.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/epoch\endcsname{9}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/last\endcsname{20.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/latin-e1\endcsname{25.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/latin-e2\endcsname{22.1}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/best/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/best/latin\endcsname{97}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/best/other\endcsname{108}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e0/empty\endcsname{73}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e0/latin\endcsname{83}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e0/other\endcsname{91}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e1/empty\endcsname{2}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e1/latin\endcsname{119}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/e1/other\endcsname{199}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/last/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/last/latin\endcsname{96}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/len/last/other\endcsname{101}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/other-e1\endcsname{60.1}
\expandafter\def\csname v@start/parakeet-tdt-v3/hi/other-e2\endcsname{53.4}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/cer\endcsname{30.2}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/dev\endcsname{35.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/done\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/e0\endcsname{55.8}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/e1\endcsname{44.1}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/last\endcsname{30.2}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/latin-e1\endcsname{30.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/latin-e2\endcsname{25.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/best/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/best/latin\endcsname{96}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/best/other\endcsname{196}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e0/empty\endcsname{73}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e0/latin\endcsname{83}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e0/other\endcsname{91}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e1/empty\endcsname{4}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e1/latin\endcsname{117}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/e1/other\endcsname{581}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/last/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/last/latin\endcsname{96}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/len/last/other\endcsname{196}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/other-e1\endcsname{79.4}
\expandafter\def\csname v@start/parakeet-tdt-v3/mean/other-e2\endcsname{75.6}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/cer\endcsname{21.7}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/dev\endcsname{28.0}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/done\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/e0\endcsname{55.8}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/e1\endcsname{39.5}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/last\endcsname{21.7}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/latin-e1\endcsname{29.3}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/latin-e2\endcsname{24.9}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/best/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/best/latin\endcsname{98}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/best/other\endcsname{100}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e0/empty\endcsname{73}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e0/latin\endcsname{83}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e0/other\endcsname{91}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e1/empty\endcsname{62}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e1/latin\endcsname{91}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/e1/other\endcsname{100}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/last-epoch\endcsname{10}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/last/empty\endcsname{0}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/last/latin\endcsname{98}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/len/last/other\endcsname{100}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/other-e1\endcsname{65.9}
\expandafter\def\csname v@start/parakeet-tdt-v3/ten/other-e2\endcsname{56.0}
\expandafter\def\csname v@sv/n\endcsname{29}
\expandafter\def\csname v@sv/pending-n\endcsname{0}
\expandafter\def\csname v@sv/scored\endcsname{28}
\expandafter\def\csname v@sv/top\endcsname{400}
\expandafter\def\csname v@sv/tuned\endcsname{24}
\expandafter\def\csname v@sv/untuned-n\endcsname{5}
\expandafter\def\csname v@sv/untuned-names\endcsname{Canary 1B v2, omniASR LLM 1B, Granite Speech 5.0 470M, Fun-ASR Nano and VibeVoice-ASR}
\expandafter\def\csname v@tok/bci_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/bci_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/bci_Latn/per-char\endcsname{0.8}
\expandafter\def\csname v@tok/bci_Latn/per-sec\endcsname{3.6}
\expandafter\def\csname v@tok/bod_Tibt/clips\endcsname{25}
\expandafter\def\csname v@tok/bod_Tibt/over\endcsname{17}
\expandafter\def\csname v@tok/bod_Tibt/per-char\endcsname{3.3}
\expandafter\def\csname v@tok/bod_Tibt/per-sec\endcsname{42.9}
\expandafter\def\csname v@tok/bre_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/bre_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/bre_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/bre_Latn/per-sec\endcsname{4.2}
\expandafter\def\csname v@tok/chv_Cyrl/clips\endcsname{25}
\expandafter\def\csname v@tok/chv_Cyrl/over\endcsname{0}
\expandafter\def\csname v@tok/chv_Cyrl/per-char\endcsname{0.9}
\expandafter\def\csname v@tok/chv_Cyrl/per-sec\endcsname{9.7}
\expandafter\def\csname v@tok/crh_Cyrl/clips\endcsname{25}
\expandafter\def\csname v@tok/crh_Cyrl/over\endcsname{0}
\expandafter\def\csname v@tok/crh_Cyrl/per-char\endcsname{0.7}
\expandafter\def\csname v@tok/crh_Cyrl/per-sec\endcsname{7.9}
\expandafter\def\csname v@tok/crh_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/crh_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/crh_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/crh_Latn/per-sec\endcsname{4.7}
\expandafter\def\csname v@tok/ekk_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/ekk_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/ekk_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/ekk_Latn/per-sec\endcsname{4.2}
\expandafter\def\csname v@tok/fin_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/fin_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/fin_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/fin_Latn/per-sec\endcsname{6.3}
\expandafter\def\csname v@tok/fon_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/fon_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/fon_Latn/per-char\endcsname{0.9}
\expandafter\def\csname v@tok/fon_Latn/per-sec\endcsname{7.1}
\expandafter\def\csname v@tok/fry_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/fry_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/fry_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/fry_Latn/per-sec\endcsname{4.1}
\expandafter\def\csname v@tok/fuv_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/fuv_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/fuv_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/fuv_Latn/per-sec\endcsname{7.5}
\expandafter\def\csname v@tok/gom_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/gom_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/gom_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/gom_Latn/per-sec\endcsname{5.0}
\expandafter\def\csname v@tok/gos_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/gos_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/gos_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/gos_Latn/per-sec\endcsname{5.5}
\expandafter\def\csname v@tok/gsw_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/gsw_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/gsw_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/gsw_Latn/per-sec\endcsname{7.1}
\expandafter\def\csname v@tok/guc_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/guc_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/guc_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/guc_Latn/per-sec\endcsname{7.3}
\expandafter\def\csname v@tok/guj_Gujr/clips\endcsname{25}
\expandafter\def\csname v@tok/guj_Gujr/over\endcsname{0}
\expandafter\def\csname v@tok/guj_Gujr/per-char\endcsname{3.1}
\expandafter\def\csname v@tok/guj_Gujr/per-sec\endcsname{22.9}
\expandafter\def\csname v@tok/hac_Arab/clips\endcsname{25}
\expandafter\def\csname v@tok/hac_Arab/over\endcsname{0}
\expandafter\def\csname v@tok/hac_Arab/per-char\endcsname{1.1}
\expandafter\def\csname v@tok/hac_Arab/per-sec\endcsname{11.5}
\expandafter\def\csname v@tok/hat_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/hat_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/hat_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/hat_Latn/per-sec\endcsname{4.3}
\expandafter\def\csname v@tok/iba_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/iba_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/iba_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/iba_Latn/per-sec\endcsname{5.0}
\expandafter\def\csname v@tok/kbd_Cyrl/clips\endcsname{25}
\expandafter\def\csname v@tok/kbd_Cyrl/over\endcsname{0}
\expandafter\def\csname v@tok/kbd_Cyrl/per-char\endcsname{0.9}
\expandafter\def\csname v@tok/kbd_Cyrl/per-sec\endcsname{10.0}
\expandafter\def\csname v@tok/kdj_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/kdj_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/kdj_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/kdj_Latn/per-sec\endcsname{5.9}
\expandafter\def\csname v@tok/kha_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/kha_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/kha_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/kha_Latn/per-sec\endcsname{5.5}
\expandafter\def\csname v@tok/lad_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/lad_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/lad_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/lad_Latn/per-sec\endcsname{4.5}
\expandafter\def\csname v@tok/lao_Laoo/clips\endcsname{25}
\expandafter\def\csname v@tok/lao_Laoo/over\endcsname{12}
\expandafter\def\csname v@tok/lao_Laoo/per-char\endcsname{3.0}
\expandafter\def\csname v@tok/lao_Laoo/per-sec\endcsname{33.5}
\expandafter\def\csname v@tok/lat_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/lat_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/lat_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/lat_Latn/per-sec\endcsname{4.0}
\expandafter\def\csname v@tok/latin-median/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/lin_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/lin_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/lin_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/lin_Latn/per-sec\endcsname{3.6}
\expandafter\def\csname v@tok/lvs_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/lvs_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/lvs_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/lvs_Latn/per-sec\endcsname{5.2}
\expandafter\def\csname v@tok/mjw_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/mjw_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/mjw_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/mjw_Latn/per-sec\endcsname{4.8}
\expandafter\def\csname v@tok/mni_Mtei/clips\endcsname{25}
\expandafter\def\csname v@tok/mni_Mtei/over\endcsname{1}
\expandafter\def\csname v@tok/mni_Mtei/per-char\endcsname{2.9}
\expandafter\def\csname v@tok/mni_Mtei/per-sec\endcsname{28.6}
\expandafter\def\csname v@tok/mya_Mymr/clips\endcsname{25}
\expandafter\def\csname v@tok/mya_Mymr/over\endcsname{4}
\expandafter\def\csname v@tok/mya_Mymr/per-char\endcsname{2.9}
\expandafter\def\csname v@tok/mya_Mymr/per-sec\endcsname{25.9}
\expandafter\def\csname v@tok/njm_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/njm_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/njm_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/njm_Latn/per-sec\endcsname{4.8}
\expandafter\def\csname v@tok/njo_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/njo_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/njo_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/njo_Latn/per-sec\endcsname{4.5}
\expandafter\def\csname v@tok/nre_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/nre_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/nre_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/nre_Latn/per-sec\endcsname{5.8}
\expandafter\def\csname v@tok/nri_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/nri_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/nri_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/nri_Latn/per-sec\endcsname{5.3}
\expandafter\def\csname v@tok/oci_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/oci_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/oci_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/oci_Latn/per-sec\endcsname{3.3}
\expandafter\def\csname v@tok/plt_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/plt_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/plt_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/plt_Latn/per-sec\endcsname{6.2}
\expandafter\def\csname v@tok/qup_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/qup_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/qup_Latn/per-char\endcsname{0.4}
\expandafter\def\csname v@tok/qup_Latn/per-sec\endcsname{5.1}
\expandafter\def\csname v@tok/san_Deva/clips\endcsname{25}
\expandafter\def\csname v@tok/san_Deva/over\endcsname{0}
\expandafter\def\csname v@tok/san_Deva/per-char\endcsname{1.3}
\expandafter\def\csname v@tok/san_Deva/per-sec\endcsname{13.5}
\expandafter\def\csname v@tok/sdh_Arab/clips\endcsname{25}
\expandafter\def\csname v@tok/sdh_Arab/over\endcsname{0}
\expandafter\def\csname v@tok/sdh_Arab/per-char\endcsname{1.2}
\expandafter\def\csname v@tok/sdh_Arab/per-sec\endcsname{8.0}
\expandafter\def\csname v@tok/slv_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/slv_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/slv_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/slv_Latn/per-sec\endcsname{5.2}
\expandafter\def\csname v@tok/smj_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/smj_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/smj_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/smj_Latn/per-sec\endcsname{5.9}
\expandafter\def\csname v@tok/sna_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/sna_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/sna_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/sna_Latn/per-sec\endcsname{4.5}
\expandafter\def\csname v@tok/suk_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/suk_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/suk_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/suk_Latn/per-sec\endcsname{6.3}
\expandafter\def\csname v@tok/teo_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/teo_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/teo_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/teo_Latn/per-sec\endcsname{6.4}
\expandafter\def\csname v@tok/tgk_Cyrl/clips\endcsname{25}
\expandafter\def\csname v@tok/tgk_Cyrl/over\endcsname{0}
\expandafter\def\csname v@tok/tgk_Cyrl/per-char\endcsname{0.7}
\expandafter\def\csname v@tok/tgk_Cyrl/per-sec\endcsname{5.8}
\expandafter\def\csname v@tok/tir_Ethi/clips\endcsname{25}
\expandafter\def\csname v@tok/tir_Ethi/over\endcsname{0}
\expandafter\def\csname v@tok/tir_Ethi/per-char\endcsname{2.9}
\expandafter\def\csname v@tok/tir_Ethi/per-sec\endcsname{18.1}
\expandafter\def\csname v@tok/trp_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/trp_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/trp_Latn/per-char\endcsname{0.5}
\expandafter\def\csname v@tok/trp_Latn/per-sec\endcsname{6.2}
\expandafter\def\csname v@tok/vag_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/vag_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/vag_Latn/per-char\endcsname{0.8}
\expandafter\def\csname v@tok/vag_Latn/per-sec\endcsname{8.3}
\expandafter\def\csname v@tok/xsm_Latn/clips\endcsname{25}
\expandafter\def\csname v@tok/xsm_Latn/over\endcsname{0}
\expandafter\def\csname v@tok/xsm_Latn/per-char\endcsname{0.6}
\expandafter\def\csname v@tok/xsm_Latn/per-sec\endcsname{5.6}
\expandafter\def\csname v@tok/zgh_Tfng/clips\endcsname{25}
\expandafter\def\csname v@tok/zgh_Tfng/over\endcsname{1}
\expandafter\def\csname v@tok/zgh_Tfng/per-char\endcsname{2.9}
\expandafter\def\csname v@tok/zgh_Tfng/per-sec\endcsname{36.4}
\expandafter\def\csname v@z/cohere-transcribe\endcsname{79.1}
\expandafter\def\csname v@z/cohere-transcribe/gain\endcsname{-11.1}
\expandafter\def\csname v@z/cohere-transcribe/loss\endcsname{11.1}
\expandafter\def\csname v@z/dagger\endcsname{1}
\expandafter\def\csname v@z/gemma4-12b\endcsname{72.8}
\expandafter\def\csname v@z/gemma4-12b/gain\endcsname{0.1}
\expandafter\def\csname v@z/gemma4-12b/loss\endcsname{-0.1}
\expandafter\def\csname v@z/gemma4-e2b\endcsname{43.5}
\expandafter\def\csname v@z/gemma4-e2b/gain\endcsname{0.0}
\expandafter\def\csname v@z/gemma4-e2b/loss\endcsname{0.0}
\expandafter\def\csname v@z/gemma4-e4b\endcsname{39.8}
\expandafter\def\csname v@z/gemma4-e4b/gain\endcsname{0.0}
\expandafter\def\csname v@z/gemma4-e4b/loss\endcsname{0.0}
\expandafter\def\csname v@z/granite-2b\endcsname{62.6}
\expandafter\def\csname v@z/granite-2b/gain\endcsname{-0.5}
\expandafter\def\csname v@z/granite-2b/loss\endcsname{0.5}
\expandafter\def\csname v@z/lfm3-audio\endcsname{57.5}
\expandafter\def\csname v@z/lfm3-audio/gain\endcsname{6.8}
\expandafter\def\csname v@z/lfm3-audio/loss\endcsname{-6.8}
\expandafter\def\csname v@z/mms-1b\endcsname{100.0}
\expandafter\def\csname v@z/nemotron-30b\endcsname{54.4}
\expandafter\def\csname v@z/nemotron-30b/gain\endcsname{3.7}
\expandafter\def\csname v@z/nemotron-30b/loss\endcsname{-3.7}
\expandafter\def\csname v@z/nemotron-stream\endcsname{68.7}
\expandafter\def\csname v@z/nemotron-stream/gain\endcsname{0.0}
\expandafter\def\csname v@z/nemotron-stream/loss\endcsname{0.0}
\expandafter\def\csname v@z/omni-ctc-1b\endcsname{28.5}
\expandafter\def\csname v@z/omni-ctc-1b/gain\endcsname{0.0}
\expandafter\def\csname v@z/omni-ctc-1b/loss\endcsname{0.0}
\expandafter\def\csname v@z/parakeet-tdt-v3\endcsname{55.8}
\expandafter\def\csname v@z/parakeet-tdt-v3/gain\endcsname{0.0}
\expandafter\def\csname v@z/parakeet-tdt-v3/loss\endcsname{0.0}
\expandafter\def\csname v@z/qwen3-asr-0.6b\endcsname{51.5}
\expandafter\def\csname v@z/qwen3-asr-0.6b/gain\endcsname{9.5}
\expandafter\def\csname v@z/qwen3-asr-0.6b/loss\endcsname{-9.5}
\expandafter\def\csname v@z/qwen3-asr-1.7b\endcsname{50.9}
\expandafter\def\csname v@z/qwen3-asr-1.7b/gain\endcsname{8.4}
\expandafter\def\csname v@z/qwen3-asr-1.7b/loss\endcsname{-8.4}
\expandafter\def\csname v@z/voxtral-mini\endcsname{57.3}
\expandafter\def\csname v@z/voxtral-mini/gain\endcsname{4.6}
\expandafter\def\csname v@z/voxtral-mini/loss\endcsname{-4.6}
\expandafter\def\csname v@z/w2v-bert\endcsname{100.0}
\expandafter\def\csname v@z/whisper-large-v2\endcsname{56.4}
\expandafter\def\csname v@z/whisper-large-v2/gain\endcsname{1.3}
\expandafter\def\csname v@z/whisper-large-v2/loss\endcsname{-1.3}
\expandafter\def\csname v@z/whisper-large-v3\endcsname{45.1}
\expandafter\def\csname v@z/whisper-large-v3-turbo\endcsname{49.1}
\expandafter\def\csname v@z/whisper-large-v3-turbo/gain\endcsname{5.5}
\expandafter\def\csname v@z/whisper-large-v3-turbo/loss\endcsname{-5.5}
\expandafter\def\csname v@z/whisper-large-v3/gain\endcsname{5.3}
\expandafter\def\csname v@z/whisper-large-v3/loss\endcsname{-5.3}
\expandafter\def\csname v@z/whisper-medium\endcsname{76.4}
\expandafter\def\csname v@z/whisper-medium/gain\endcsname{-12.7}
\expandafter\def\csname v@z/whisper-medium/loss\endcsname{12.7}
\expandafter\def\csname v@z/whisper-small\endcsname{61.9}
\expandafter\def\csname v@z/whisper-small/gain\endcsname{3.8}
\expandafter\def\csname v@z/whisper-small/loss\endcsname{-3.8}
\expandafter\def\csname v@z/whisper-tiny\endcsname{60.9}
\expandafter\def\csname v@z/whisper-tiny/gain\endcsname{5.7}
\expandafter\def\csname v@z/whisper-tiny/loss\endcsname{-5.7}
\makeatother

